Visual Jev: Accurate and Efficient Decisions from Shared Visual Context

Applications increasingly ask multiple closed-choice questions about the same image, requiring accurate probabilities and efficient inference. We present Visual Jev, a visual decision model combining LM-head candidate readout, answer-supervised post-training, and independent question branches over a shared visual prefix. On held-out test images from four benchmarks, task SFT raises the 4B model's macro accuracy from 83.4% to 88.5% and error-discrimination AUROC from 0.834 to 0.890. Its macro accuracy exceeds the hosted Jev and OpenAI Decisions APIs by 2.77 and 5.06 percentage points, respectively, with the lowest NLL. We further show that better accuracy and calibration do not ensure reliable decisions. Fixed confidence thresholds exceed target error rates, and simply reordering options changes 17% of the model's accept-or-review decisions on SNLI-VE. At 32 questions per image, shared-prefix inference reduces amortized time per question from 20.5 to 5.6 ms, a 3.7x speedup over batched full sequences on one RTX 5090. Engine-level prefix caching reduces KV memory to 24.3% of that used by our custom shared-prefix path.

==> generated/v3/macros_v3.tex <==
% generated by reports/make_tables_v3.py -- do not edit
\makeatletter
\newcommand{\VJ}[1]{\@ifundefined{VJ@#1}{\textbf{??\detokenize{#1}??}\PackageWarning{VJ}{undefined number \detokenize{#1}}}{\@nameuse{VJ@#1}}}
\@namedef{VJ@A2k.raw.gqa_val.accuracy}{0.921}
\@namedef{VJ@A2k.raw.gqa_val.accuracy.ci}{[0.914, 0.928]}
\@namedef{VJ@A2k.raw.gqa_val.aurc_maxp}{0.012}
\@namedef{VJ@A2k.raw.gqa_val.aurc_maxp.ci}{[0.010, 0.014]}
\@namedef{VJ@A2k.raw.gqa_val.brier}{0.127}
\@namedef{VJ@A2k.raw.gqa_val.brier.ci}{[0.116, 0.138]}
\@namedef{VJ@A2k.raw.gqa_val.cov@0.05}{0.893}
\@namedef{VJ@A2k.raw.gqa_val.cov@0.05.ci}{[0.886, 0.900]}
\@namedef{VJ@A2k.raw.gqa_val.cov@0.05.pct}{89.3\%}
\@namedef{VJ@A2k.raw.gqa_val.cov@0.1}{0.999}
\@namedef{VJ@A2k.raw.gqa_val.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@A2k.raw.gqa_val.cov@0.1.pct}{99.9\%}
\@namedef{VJ@A2k.raw.gqa_val.ece15}{0.045}
\@namedef{VJ@A2k.raw.gqa_val.ece15.ci}{[0.040, 0.051]}
\@namedef{VJ@A2k.raw.gqa_val.nll}{0.242}
\@namedef{VJ@A2k.raw.gqa_val.nll.ci}{[0.219, 0.264]}
\@namedef{VJ@A2k.raw.gqa_val.risk@0.05}{0.041}
\@namedef{VJ@A2k.raw.gqa_val.risk@0.05.ci}{[0.036, 0.046]}
\@namedef{VJ@A2k.raw.gqa_val.risk@0.05.pct}{4.1\%}
\@namedef{VJ@A2k.raw.gqa_val.risk@0.1}{0.079}
\@namedef{VJ@A2k.raw.gqa_val.risk@0.1.ci}{[0.072, 0.085]}
\@namedef{VJ@A2k.raw.gqa_val.risk@0.1.pct}{7.9\%}
\@namedef{VJ@A2k.raw.macro.accuracy}{0.889}
\@namedef{VJ@A2k.raw.macro.accuracy.ci}{[0.882, 0.895]}
\@namedef{VJ@A2k.raw.macro.aurc_maxp}{0.029}
\@namedef{VJ@A2k.raw.macro.aurc_maxp.ci}{[0.026, 0.033]}
\@namedef{VJ@A2k.raw.macro.brier}{0.167}
\@namedef{VJ@A2k.raw.macro.brier.ci}{[0.158, 0.177]}
\@namedef{VJ@A2k.raw.macro.ece15}{0.043}
\@namedef{VJ@A2k.raw.macro.ece15.ci}{[0.040, 0.050]}
\@namedef{VJ@A2k.raw.macro.nll}{0.323}
\@namedef{VJ@A2k.raw.macro.nll.ci}{[0.304, 0.340]}
\@namedef{VJ@A2k.raw.snli_ve.accuracy}{0.812}
\@namedef{VJ@A2k.raw.snli_ve.accuracy.ci}{[0.793, 0.831]}
\@namedef{VJ@A2k.raw.snli_ve.aurc_maxp}{0.072}
\@namedef{VJ@A2k.raw.snli_ve.aurc_maxp.ci}{[0.059, 0.086]}
\@namedef{VJ@A2k.raw.snli_ve.brier}{0.281}
\@namedef{VJ@A2k.raw.snli_ve.brier.ci}{[0.255, 0.309]}
\@namedef{VJ@A2k.raw.snli_ve.cov@0.05}{0.352}
\@namedef{VJ@A2k.raw.snli_ve.cov@0.05.ci}{[0.333, 0.373]}
\@namedef{VJ@A2k.raw.snli_ve.cov@0.05.pct}{35.2\%}
\@namedef{VJ@A2k.raw.snli_ve.cov@0.1}{0.648}
\@namedef{VJ@A2k.raw.snli_ve.cov@0.1.ci}{[0.626, 0.669]}
\@namedef{VJ@A2k.raw.snli_ve.cov@0.1.pct}{64.8\%}
\@namedef{VJ@A2k.raw.snli_ve.ece15}{0.064}
\@namedef{VJ@A2k.raw.snli_ve.ece15.ci}{[0.051, 0.083]}
\@namedef{VJ@A2k.raw.snli_ve.nll}{0.507}
\@namedef{VJ@A2k.raw.snli_ve.nll.ci}{[0.459, 0.558]}
\@namedef{VJ@A2k.raw.snli_ve.risk@0.05}{0.044}
\@namedef{VJ@A2k.raw.snli_ve.risk@0.05.ci}{[0.029, 0.060]}
\@namedef{VJ@A2k.raw.snli_ve.risk@0.05.pct}{4.4\%}
\@namedef{VJ@A2k.raw.snli_ve.risk@0.1}{0.087}
\@namedef{VJ@A2k.raw.snli_ve.risk@0.1.ci}{[0.071, 0.106]}
\@namedef{VJ@A2k.raw.snli_ve.risk@0.1.pct}{8.7\%}
\@namedef{VJ@A2k.raw.tallyqa_l.accuracy}{0.848}
\@namedef{VJ@A2k.raw.tallyqa_l.accuracy.ci}{[0.835, 0.859]}
\@namedef{VJ@A2k.raw.tallyqa_l.aurc_maxp}{0.032}
\@namedef{VJ@A2k.raw.tallyqa_l.aurc_maxp.ci}{[0.028, 0.038]}
\@namedef{VJ@A2k.raw.tallyqa_l.brier}{0.222}
\@namedef{VJ@A2k.raw.tallyqa_l.brier.ci}{[0.205, 0.240]}
\@namedef{VJ@A2k.raw.tallyqa_l.cov@0.05}{0.773}
\@namedef{VJ@A2k.raw.tallyqa_l.cov@0.05.ci}{[0.757, 0.787]}
\@namedef{VJ@A2k.raw.tallyqa_l.cov@0.05.pct}{77.3\%}
\@namedef{VJ@A2k.raw.tallyqa_l.cov@0.1}{0.899}
\@namedef{VJ@A2k.raw.tallyqa_l.cov@0.1.ci}{[0.890, 0.909]}
\@namedef{VJ@A2k.raw.tallyqa_l.cov@0.1.pct}{89.9\%}
\@namedef{VJ@A2k.raw.tallyqa_l.ece15}{0.054}
\@namedef{VJ@A2k.raw.tallyqa_l.ece15.ci}{[0.045, 0.064]}
\@namedef{VJ@A2k.raw.tallyqa_l.nll}{0.438}
\@namedef{VJ@A2k.raw.tallyqa_l.nll.ci}{[0.403, 0.475]}
\@namedef{VJ@A2k.raw.tallyqa_l.risk@0.05}{0.057}
\@namedef{VJ@A2k.raw.tallyqa_l.risk@0.05.ci}{[0.050, 0.065]}
\@namedef{VJ@A2k.raw.tallyqa_l.risk@0.05.pct}{5.7\%}
\@namedef{VJ@A2k.raw.tallyqa_l.risk@0.1}{0.106}
\@namedef{VJ@A2k.raw.tallyqa_l.risk@0.1.ci}{[0.096, 0.117]}
\@namedef{VJ@A2k.raw.tallyqa_l.risk@0.1.pct}{10.6\%}
\@namedef{VJ@A2k.raw.textvqa_k8.accuracy}{0.974}
\@namedef{VJ@A2k.raw.textvqa_k8.accuracy.ci}{[0.967, 0.981]}
\@namedef{VJ@A2k.raw.textvqa_k8.aurc_maxp}{0.001}
\@namedef{VJ@A2k.raw.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@A2k.raw.textvqa_k8.brier}{0.040}
\@namedef{VJ@A2k.raw.textvqa_k8.brier.ci}{[0.029, 0.051]}
\@namedef{VJ@A2k.raw.textvqa_k8.cov@0.05}{0.999}
\@namedef{VJ@A2k.raw.textvqa_k8.cov@0.05.ci}{[0.998, 1.000]}
\@namedef{VJ@A2k.raw.textvqa_k8.cov@0.05.pct}{99.9\%}
\@namedef{VJ@A2k.raw.textvqa_k8.cov@0.1}{0.999}
\@namedef{VJ@A2k.raw.textvqa_k8.cov@0.1.ci}{[0.998, 1.000]}
\@namedef{VJ@A2k.raw.textvqa_k8.cov@0.1.pct}{99.9\%}
\@namedef{VJ@A2k.raw.textvqa_k8.ece15}{0.011}
\@namedef{VJ@A2k.raw.textvqa_k8.ece15.ci}{[0.009, 0.018]}
\@namedef{VJ@A2k.raw.textvqa_k8.nll}{0.103}
\@namedef{VJ@A2k.raw.textvqa_k8.nll.ci}{[0.073, 0.133]}
\@namedef{VJ@A2k.raw.textvqa_k8.risk@0.05}{0.025}
\@namedef{VJ@A2k.raw.textvqa_k8.risk@0.05.ci}{[0.019, 0.032]}
\@namedef{VJ@A2k.raw.textvqa_k8.risk@0.05.pct}{2.5\%}
\@namedef{VJ@A2k.raw.textvqa_k8.risk@0.1}{0.025}
\@namedef{VJ@A2k.raw.textvqa_k8.risk@0.1.ci}{[0.019, 0.032]}
\@namedef{VJ@A2k.raw.textvqa_k8.risk@0.1.pct}{2.5\%}
\@namedef{VJ@A2k.ts_local.gqa_val.accuracy}{0.921}
\@namedef{VJ@A2k.ts_local.gqa_val.accuracy.ci}{[0.914, 0.928]}
\@namedef{VJ@A2k.ts_local.gqa_val.aurc_maxp}{0.012}
\@namedef{VJ@A2k.ts_local.gqa_val.aurc_maxp.ci}{[0.010, 0.014]}
\@namedef{VJ@A2k.ts_local.gqa_val.brier}{0.118}
\@namedef{VJ@A2k.ts_local.gqa_val.brier.ci}{[0.108, 0.127]}
\@namedef{VJ@A2k.ts_local.gqa_val.cov@0.05}{0.893}
\@namedef{VJ@A2k.ts_local.gqa_val.cov@0.05.ci}{[0.885, 0.900]}
\@namedef{VJ@A2k.ts_local.gqa_val.cov@0.05.pct}{89.3\%}
\@namedef{VJ@A2k.ts_local.gqa_val.cov@0.1}{0.999}
\@namedef{VJ@A2k.ts_local.gqa_val.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@A2k.ts_local.gqa_val.cov@0.1.pct}{99.9\%}
\@namedef{VJ@A2k.ts_local.gqa_val.ece15}{0.019}
\@namedef{VJ@A2k.ts_local.gqa_val.ece15.ci}{[0.017, 0.025]}
\@namedef{VJ@A2k.ts_local.gqa_val.nll}{0.209}
\@namedef{VJ@A2k.ts_local.gqa_val.nll.ci}{[0.194, 0.224]}
\@namedef{VJ@A2k.ts_local.gqa_val.risk@0.05}{0.041}
\@namedef{VJ@A2k.ts_local.gqa_val.risk@0.05.ci}{[0.036, 0.046]}
\@namedef{VJ@A2k.ts_local.gqa_val.risk@0.05.pct}{4.1\%}
\@namedef{VJ@A2k.ts_local.gqa_val.risk@0.1}{0.078}
\@namedef{VJ@A2k.ts_local.gqa_val.risk@0.1.ci}{[0.071, 0.085]}
\@namedef{VJ@A2k.ts_local.gqa_val.risk@0.1.pct}{7.8\%}
\@namedef{VJ@A2k.ts_local.macro.accuracy}{0.889}
\@namedef{VJ@A2k.ts_local.macro.accuracy.ci}{[0.882, 0.895]}
\@namedef{VJ@A2k.ts_local.macro.aurc_maxp}{0.029}
\@namedef{VJ@A2k.ts_local.macro.aurc_maxp.ci}{[0.026, 0.033]}
\@namedef{VJ@A2k.ts_local.macro.brier}{0.161}
\@namedef{VJ@A2k.ts_local.macro.brier.ci}{[0.153, 0.169]}
\@namedef{VJ@A2k.ts_local.macro.ece15}{0.025}
\@namedef{VJ@A2k.ts_local.macro.ece15.ci}{[0.025, 0.032]}
\@namedef{VJ@A2k.ts_local.macro.nll}{0.304}
\@namedef{VJ@A2k.ts_local.macro.nll.ci}{[0.289, 0.317]}
\@namedef{VJ@A2k.ts_local.snli_ve.accuracy}{0.812}
\@namedef{VJ@A2k.ts_local.snli_ve.accuracy.ci}{[0.793, 0.831]}
\@namedef{VJ@A2k.ts_local.snli_ve.aurc_maxp}{0.071}
\@namedef{VJ@A2k.ts_local.snli_ve.aurc_maxp.ci}{[0.059, 0.085]}
\@namedef{VJ@A2k.ts_local.snli_ve.brier}{0.273}
\@namedef{VJ@A2k.ts_local.snli_ve.brier.ci}{[0.250, 0.297]}
\@namedef{VJ@A2k.ts_local.snli_ve.cov@0.05}{0.353}
\@namedef{VJ@A2k.ts_local.snli_ve.cov@0.05.ci}{[0.334, 0.374]}
\@namedef{VJ@A2k.ts_local.snli_ve.cov@0.05.pct}{35.3\%}
\@namedef{VJ@A2k.ts_local.snli_ve.cov@0.1}{0.644}
\@namedef{VJ@A2k.ts_local.snli_ve.cov@0.1.ci}{[0.622, 0.666]}
\@namedef{VJ@A2k.ts_local.snli_ve.cov@0.1.pct}{64.4\%}
\@namedef{VJ@A2k.ts_local.snli_ve.ece15}{0.036}
\@namedef{VJ@A2k.ts_local.snli_ve.ece15.ci}{[0.032, 0.054]}
\@namedef{VJ@A2k.ts_local.snli_ve.nll}{0.489}
\@namedef{VJ@A2k.ts_local.snli_ve.nll.ci}{[0.453, 0.527]}
\@namedef{VJ@A2k.ts_local.snli_ve.risk@0.05}{0.042}
\@namedef{VJ@A2k.ts_local.snli_ve.risk@0.05.ci}{[0.028, 0.058]}
\@namedef{VJ@A2k.ts_local.snli_ve.risk@0.05.pct}{4.2\%}
\@namedef{VJ@A2k.ts_local.snli_ve.risk@0.1}{0.085}
\@namedef{VJ@A2k.ts_local.snli_ve.risk@0.1.ci}{[0.069, 0.104]}
\@namedef{VJ@A2k.ts_local.snli_ve.risk@0.1.pct}{8.5\%}
\@namedef{VJ@A2k.ts_local.tallyqa_l.accuracy}{0.848}
\@namedef{VJ@A2k.ts_local.tallyqa_l.accuracy.ci}{[0.835, 0.859]}
\@namedef{VJ@A2k.ts_local.tallyqa_l.aurc_maxp}{0.032}
\@namedef{VJ@A2k.ts_local.tallyqa_l.aurc_maxp.ci}{[0.028, 0.038]}
\@namedef{VJ@A2k.ts_local.tallyqa_l.brier}{0.214}
\@namedef{VJ@A2k.ts_local.tallyqa_l.brier.ci}{[0.199, 0.232]}
\@namedef{VJ@A2k.ts_local.tallyqa_l.cov@0.05}{0.774}
\@namedef{VJ@A2k.ts_local.tallyqa_l.cov@0.05.ci}{[0.759, 0.789]}
\@namedef{VJ@A2k.ts_local.tallyqa_l.cov@0.05.pct}{77.4\%}
\@namedef{VJ@A2k.ts_local.tallyqa_l.cov@0.1}{0.900}
\@namedef{VJ@A2k.ts_local.tallyqa_l.cov@0.1.ci}{[0.891, 0.910]}
\@namedef{VJ@A2k.ts_local.tallyqa_l.cov@0.1.pct}{90.0\%}
\@namedef{VJ@A2k.ts_local.tallyqa_l.ece15}{0.035}
\@namedef{VJ@A2k.ts_local.tallyqa_l.ece15.ci}{[0.030, 0.045]}
\@namedef{VJ@A2k.ts_local.tallyqa_l.nll}{0.420}
\@namedef{VJ@A2k.ts_local.tallyqa_l.nll.ci}{[0.390, 0.452]}
\@namedef{VJ@A2k.ts_local.tallyqa_l.risk@0.05}{0.057}
\@namedef{VJ@A2k.ts_local.tallyqa_l.risk@0.05.ci}{[0.050, 0.066]}
\@namedef{VJ@A2k.ts_local.tallyqa_l.risk@0.05.pct}{5.7\%}
\@namedef{VJ@A2k.ts_local.tallyqa_l.risk@0.1}{0.106}
\@namedef{VJ@A2k.ts_local.tallyqa_l.risk@0.1.ci}{[0.096, 0.117]}
\@namedef{VJ@A2k.ts_local.tallyqa_l.risk@0.1.pct}{10.6\%}
\@namedef{VJ@A2k.ts_local.textvqa_k8.accuracy}{0.974}
\@namedef{VJ@A2k.ts_local.textvqa_k8.accuracy.ci}{[0.967, 0.981]}
\@namedef{VJ@A2k.ts_local.textvqa_k8.aurc_maxp}{0.001}
\@namedef{VJ@A2k.ts_local.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@A2k.ts_local.textvqa_k8.brier}{0.039}
\@namedef{VJ@A2k.ts_local.textvqa_k8.brier.ci}{[0.029, 0.049]}
\@namedef{VJ@A2k.ts_local.textvqa_k8.cov@0.05}{0.999}
\@namedef{VJ@A2k.ts_local.textvqa_k8.cov@0.05.ci}{[0.998, 1.000]}
\@namedef{VJ@A2k.ts_local.textvqa_k8.cov@0.05.pct}{99.9\%}
\@namedef{VJ@A2k.ts_local.textvqa_k8.cov@0.1}{0.999}
\@namedef{VJ@A2k.ts_local.textvqa_k8.cov@0.1.ci}{[0.998, 1.000]}
\@namedef{VJ@A2k.ts_local.textvqa_k8.cov@0.1.pct}{99.9\%}
\@namedef{VJ@A2k.ts_local.textvqa_k8.ece15}{0.008}
\@namedef{VJ@A2k.ts_local.textvqa_k8.ece15.ci}{[0.008, 0.015]}
\@namedef{VJ@A2k.ts_local.textvqa_k8.nll}{0.096}
\@namedef{VJ@A2k.ts_local.textvqa_k8.nll.ci}{[0.071, 0.121]}
\@namedef{VJ@A2k.ts_local.textvqa_k8.risk@0.05}{0.025}
\@namedef{VJ@A2k.ts_local.textvqa_k8.risk@0.05.ci}{[0.019, 0.032]}
\@namedef{VJ@A2k.ts_local.textvqa_k8.risk@0.05.pct}{2.5\%}
\@namedef{VJ@A2k.ts_local.textvqa_k8.risk@0.1}{0.025}
\@namedef{VJ@A2k.ts_local.textvqa_k8.risk@0.1.ci}{[0.019, 0.032]}
\@namedef{VJ@A2k.ts_local.textvqa_k8.risk@0.1.pct}{2.5\%}
\@namedef{VJ@A2k.ts_transfer.gqa_val.accuracy}{0.921}
\@namedef{VJ@A2k.ts_transfer.gqa_val.accuracy.ci}{[0.914, 0.928]}
\@namedef{VJ@A2k.ts_transfer.gqa_val.aurc_maxp}{0.012}
\@namedef{VJ@A2k.ts_transfer.gqa_val.aurc_maxp.ci}{[0.010, 0.014]}
\@namedef{VJ@A2k.ts_transfer.gqa_val.brier}{0.118}
\@namedef{VJ@A2k.ts_transfer.gqa_val.brier.ci}{[0.108, 0.127]}
\@namedef{VJ@A2k.ts_transfer.gqa_val.cov@0.05}{0.890}
\@namedef{VJ@A2k.ts_transfer.gqa_val.cov@0.05.ci}{[0.882, 0.898]}
\@namedef{VJ@A2k.ts_transfer.gqa_val.cov@0.05.pct}{89.0\%}
\@namedef{VJ@A2k.ts_transfer.gqa_val.cov@0.1}{0.999}
\@namedef{VJ@A2k.ts_transfer.gqa_val.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@A2k.ts_transfer.gqa_val.cov@0.1.pct}{99.9\%}
\@namedef{VJ@A2k.ts_transfer.gqa_val.ece15}{0.021}
\@namedef{VJ@A2k.ts_transfer.gqa_val.ece15.ci}{[0.018, 0.026]}
\@namedef{VJ@A2k.ts_transfer.gqa_val.nll}{0.208}
\@namedef{VJ@A2k.ts_transfer.gqa_val.nll.ci}{[0.192, 0.224]}
\@namedef{VJ@A2k.ts_transfer.gqa_val.risk@0.05}{0.040}
\@namedef{VJ@A2k.ts_transfer.gqa_val.risk@0.05.ci}{[0.035, 0.045]}
\@namedef{VJ@A2k.ts_transfer.gqa_val.risk@0.05.pct}{4.0\%}
\@namedef{VJ@A2k.ts_transfer.gqa_val.risk@0.1}{0.079}
\@namedef{VJ@A2k.ts_transfer.gqa_val.risk@0.1.ci}{[0.072, 0.085]}
\@namedef{VJ@A2k.ts_transfer.gqa_val.risk@0.1.pct}{7.9\%}
\@namedef{VJ@A2k.ts_transfer.macro.accuracy}{0.889}
\@namedef{VJ@A2k.ts_transfer.macro.accuracy.ci}{[0.882, 0.895]}
\@namedef{VJ@A2k.ts_transfer.macro.aurc_maxp}{0.029}
\@namedef{VJ@A2k.ts_transfer.macro.aurc_maxp.ci}{[0.026, 0.033]}
\@namedef{VJ@A2k.ts_transfer.macro.brier}{0.162}
\@namedef{VJ@A2k.ts_transfer.macro.brier.ci}{[0.154, 0.169]}
\@namedef{VJ@A2k.ts_transfer.macro.ece15}{0.036}
\@namedef{VJ@A2k.ts_transfer.macro.ece15.ci}{[0.036, 0.043]}
\@namedef{VJ@A2k.ts_transfer.macro.nll}{0.313}
\@namedef{VJ@A2k.ts_transfer.macro.nll.ci}{[0.300, 0.325]}
\@namedef{VJ@A2k.ts_transfer.snli_ve.accuracy}{0.812}
\@namedef{VJ@A2k.ts_transfer.snli_ve.accuracy.ci}{[0.793, 0.831]}
\@namedef{VJ@A2k.ts_transfer.snli_ve.aurc_maxp}{0.071}
\@namedef{VJ@A2k.ts_transfer.snli_ve.aurc_maxp.ci}{[0.059, 0.085]}
\@namedef{VJ@A2k.ts_transfer.snli_ve.brier}{0.276}
\@namedef{VJ@A2k.ts_transfer.snli_ve.brier.ci}{[0.254, 0.298]}
\@namedef{VJ@A2k.ts_transfer.snli_ve.cov@0.05}{0.369}
\@namedef{VJ@A2k.ts_transfer.snli_ve.cov@0.05.ci}{[0.350, 0.390]}
\@namedef{VJ@A2k.ts_transfer.snli_ve.cov@0.05.pct}{36.9\%}
\@namedef{VJ@A2k.ts_transfer.snli_ve.cov@0.1}{0.646}
\@namedef{VJ@A2k.ts_transfer.snli_ve.cov@0.1.ci}{[0.624, 0.668]}
\@namedef{VJ@A2k.ts_transfer.snli_ve.cov@0.1.pct}{64.6\%}
\@namedef{VJ@A2k.ts_transfer.snli_ve.ece15}{0.054}
\@namedef{VJ@A2k.ts_transfer.snli_ve.ece15.ci}{[0.047, 0.072]}
\@namedef{VJ@A2k.ts_transfer.snli_ve.nll}{0.500}
\@namedef{VJ@A2k.ts_transfer.snli_ve.nll.ci}{[0.468, 0.533]}
\@namedef{VJ@A2k.ts_transfer.snli_ve.risk@0.05}{0.043}
\@namedef{VJ@A2k.ts_transfer.snli_ve.risk@0.05.ci}{[0.029, 0.059]}
\@namedef{VJ@A2k.ts_transfer.snli_ve.risk@0.05.pct}{4.3\%}
\@namedef{VJ@A2k.ts_transfer.snli_ve.risk@0.1}{0.087}
\@namedef{VJ@A2k.ts_transfer.snli_ve.risk@0.1.ci}{[0.070, 0.106]}
\@namedef{VJ@A2k.ts_transfer.snli_ve.risk@0.1.pct}{8.7\%}
\@namedef{VJ@A2k.ts_transfer.tallyqa_l.accuracy}{0.848}
\@namedef{VJ@A2k.ts_transfer.tallyqa_l.accuracy.ci}{[0.835, 0.859]}
\@namedef{VJ@A2k.ts_transfer.tallyqa_l.aurc_maxp}{0.032}
\@namedef{VJ@A2k.ts_transfer.tallyqa_l.aurc_maxp.ci}{[0.027, 0.037]}
\@namedef{VJ@A2k.ts_transfer.tallyqa_l.brier}{0.214}
\@namedef{VJ@A2k.ts_transfer.tallyqa_l.brier.ci}{[0.201, 0.230]}
\@namedef{VJ@A2k.ts_transfer.tallyqa_l.cov@0.05}{0.780}
\@namedef{VJ@A2k.ts_transfer.tallyqa_l.cov@0.05.ci}{[0.764, 0.794]}
\@namedef{VJ@A2k.ts_transfer.tallyqa_l.cov@0.05.pct}{78.0\%}
\@namedef{VJ@A2k.ts_transfer.tallyqa_l.cov@0.1}{0.902}
\@namedef{VJ@A2k.ts_transfer.tallyqa_l.cov@0.1.ci}{[0.893, 0.912]}
\@namedef{VJ@A2k.ts_transfer.tallyqa_l.cov@0.1.pct}{90.2\%}
\@namedef{VJ@A2k.ts_transfer.tallyqa_l.ece15}{0.046}
\@namedef{VJ@A2k.ts_transfer.tallyqa_l.ece15.ci}{[0.046, 0.058]}
\@namedef{VJ@A2k.ts_transfer.tallyqa_l.nll}{0.440}
\@namedef{VJ@A2k.ts_transfer.tallyqa_l.nll.ci}{[0.414, 0.467]}
\@namedef{VJ@A2k.ts_transfer.tallyqa_l.risk@0.05}{0.059}
\@namedef{VJ@A2k.ts_transfer.tallyqa_l.risk@0.05.ci}{[0.051, 0.068]}
\@namedef{VJ@A2k.ts_transfer.tallyqa_l.risk@0.05.pct}{5.9\%}
\@namedef{VJ@A2k.ts_transfer.tallyqa_l.risk@0.1}{0.106}
\@namedef{VJ@A2k.ts_transfer.tallyqa_l.risk@0.1.ci}{[0.096, 0.117]}
\@namedef{VJ@A2k.ts_transfer.tallyqa_l.risk@0.1.pct}{10.6\%}
\@namedef{VJ@A2k.ts_transfer.textvqa_k8.accuracy}{0.974}
\@namedef{VJ@A2k.ts_transfer.textvqa_k8.accuracy.ci}{[0.967, 0.981]}
\@namedef{VJ@A2k.ts_transfer.textvqa_k8.aurc_maxp}{0.001}
\@namedef{VJ@A2k.ts_transfer.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@A2k.ts_transfer.textvqa_k8.brier}{0.039}
\@namedef{VJ@A2k.ts_transfer.textvqa_k8.brier.ci}{[0.029, 0.049]}
\@namedef{VJ@A2k.ts_transfer.textvqa_k8.cov@0.05}{0.999}
\@namedef{VJ@A2k.ts_transfer.textvqa_k8.cov@0.05.ci}{[0.998, 1.000]}
\@namedef{VJ@A2k.ts_transfer.textvqa_k8.cov@0.05.pct}{99.9\%}
\@namedef{VJ@A2k.ts_transfer.textvqa_k8.cov@0.1}{0.999}
\@namedef{VJ@A2k.ts_transfer.textvqa_k8.cov@0.1.ci}{[0.998, 1.000]}
\@namedef{VJ@A2k.ts_transfer.textvqa_k8.cov@0.1.pct}{99.9\%}
\@namedef{VJ@A2k.ts_transfer.textvqa_k8.ece15}{0.021}
\@namedef{VJ@A2k.ts_transfer.textvqa_k8.ece15.ci}{[0.022, 0.027]}
\@namedef{VJ@A2k.ts_transfer.textvqa_k8.nll}{0.103}
\@namedef{VJ@A2k.ts_transfer.textvqa_k8.nll.ci}{[0.081, 0.125]}
\@namedef{VJ@A2k.ts_transfer.textvqa_k8.risk@0.05}{0.025}
\@namedef{VJ@A2k.ts_transfer.textvqa_k8.risk@0.05.ci}{[0.019, 0.032]}
\@namedef{VJ@A2k.ts_transfer.textvqa_k8.risk@0.05.pct}{2.5\%}
\@namedef{VJ@A2k.ts_transfer.textvqa_k8.risk@0.1}{0.025}
\@namedef{VJ@A2k.ts_transfer.textvqa_k8.risk@0.1.ci}{[0.019, 0.032]}
\@namedef{VJ@A2k.ts_transfer.textvqa_k8.risk@0.1.pct}{2.5\%}
\@namedef{VJ@D_brier.raw.gqa_val.accuracy}{0.913}
\@namedef{VJ@D_brier.raw.gqa_val.accuracy.ci}{[0.906, 0.921]}
\@namedef{VJ@D_brier.raw.gqa_val.aurc_maxp}{0.015}
\@namedef{VJ@D_brier.raw.gqa_val.aurc_maxp.ci}{[0.013, 0.017]}
\@namedef{VJ@D_brier.raw.gqa_val.brier}{0.145}
\@namedef{VJ@D_brier.raw.gqa_val.brier.ci}{[0.132, 0.157]}
\@namedef{VJ@D_brier.raw.gqa_val.cov@0.05}{0.895}
\@namedef{VJ@D_brier.raw.gqa_val.cov@0.05.ci}{[0.887, 0.902]}
\@namedef{VJ@D_brier.raw.gqa_val.cov@0.05.pct}{89.5\%}
\@namedef{VJ@D_brier.raw.gqa_val.cov@0.1}{1.000}
\@namedef{VJ@D_brier.raw.gqa_val.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@D_brier.raw.gqa_val.cov@0.1.pct}{100.0\%}
\@namedef{VJ@D_brier.raw.gqa_val.ece15}{0.060}
\@namedef{VJ@D_brier.raw.gqa_val.ece15.ci}{[0.054, 0.067]}
\@namedef{VJ@D_brier.raw.gqa_val.nll}{0.303}
\@namedef{VJ@D_brier.raw.gqa_val.nll.ci}{[0.274, 0.331]}
\@namedef{VJ@D_brier.raw.gqa_val.risk@0.05}{0.048}
\@namedef{VJ@D_brier.raw.gqa_val.risk@0.05.ci}{[0.042, 0.054]}
\@namedef{VJ@D_brier.raw.gqa_val.risk@0.05.pct}{4.8\%}
\@namedef{VJ@D_brier.raw.gqa_val.risk@0.1}{0.086}
\@namedef{VJ@D_brier.raw.gqa_val.risk@0.1.ci}{[0.079, 0.094]}
\@namedef{VJ@D_brier.raw.gqa_val.risk@0.1.pct}{8.6\%}
\@namedef{VJ@D_brier.raw.macro.accuracy}{0.884}
\@namedef{VJ@D_brier.raw.macro.accuracy.ci}{[0.877, 0.890]}
\@namedef{VJ@D_brier.raw.macro.aurc_maxp}{0.031}
\@namedef{VJ@D_brier.raw.macro.aurc_maxp.ci}{[0.027, 0.034]}
\@namedef{VJ@D_brier.raw.macro.brier}{0.180}
\@namedef{VJ@D_brier.raw.macro.brier.ci}{[0.170, 0.189]}
\@namedef{VJ@D_brier.raw.macro.ece15}{0.059}
\@namedef{VJ@D_brier.raw.macro.ece15.ci}{[0.055, 0.066]}
\@namedef{VJ@D_brier.raw.macro.nll}{0.357}
\@namedef{VJ@D_brier.raw.macro.nll.ci}{[0.336, 0.377]}
\@namedef{VJ@D_brier.raw.snli_ve.accuracy}{0.803}
\@namedef{VJ@D_brier.raw.snli_ve.accuracy.ci}{[0.783, 0.823]}
\@namedef{VJ@D_brier.raw.snli_ve.aurc_maxp}{0.074}
\@namedef{VJ@D_brier.raw.snli_ve.aurc_maxp.ci}{[0.061, 0.088]}
\@namedef{VJ@D_brier.raw.snli_ve.brier}{0.303}
\@namedef{VJ@D_brier.raw.snli_ve.brier.ci}{[0.273, 0.333]}
\@namedef{VJ@D_brier.raw.snli_ve.cov@0.05}{0.296}
\@namedef{VJ@D_brier.raw.snli_ve.cov@0.05.ci}{[0.276, 0.318]}
\@namedef{VJ@D_brier.raw.snli_ve.cov@0.05.pct}{29.6\%}
\@namedef{VJ@D_brier.raw.snli_ve.cov@0.1}{0.608}
\@namedef{VJ@D_brier.raw.snli_ve.cov@0.1.ci}{[0.585, 0.631]}
\@namedef{VJ@D_brier.raw.snli_ve.cov@0.1.pct}{60.8\%}
\@namedef{VJ@D_brier.raw.snli_ve.ece15}{0.089}
\@namedef{VJ@D_brier.raw.snli_ve.ece15.ci}{[0.075, 0.109]}
\@namedef{VJ@D_brier.raw.snli_ve.nll}{0.552}
\@namedef{VJ@D_brier.raw.snli_ve.nll.ci}{[0.497, 0.608]}
\@namedef{VJ@D_brier.raw.snli_ve.risk@0.05}{0.034}
\@namedef{VJ@D_brier.raw.snli_ve.risk@0.05.ci}{[0.020, 0.050]}
\@namedef{VJ@D_brier.raw.snli_ve.risk@0.05.pct}{3.4\%}
\@namedef{VJ@D_brier.raw.snli_ve.risk@0.1}{0.079}
\@namedef{VJ@D_brier.raw.snli_ve.risk@0.1.ci}{[0.063, 0.097]}
\@namedef{VJ@D_brier.raw.snli_ve.risk@0.1.pct}{7.9\%}
\@namedef{VJ@D_brier.raw.tallyqa_l.accuracy}{0.844}
\@namedef{VJ@D_brier.raw.tallyqa_l.accuracy.ci}{[0.831, 0.856]}
\@namedef{VJ@D_brier.raw.tallyqa_l.aurc_maxp}{0.033}
\@namedef{VJ@D_brier.raw.tallyqa_l.aurc_maxp.ci}{[0.028, 0.039]}
\@namedef{VJ@D_brier.raw.tallyqa_l.brier}{0.231}
\@namedef{VJ@D_brier.raw.tallyqa_l.brier.ci}{[0.213, 0.249]}
\@namedef{VJ@D_brier.raw.tallyqa_l.cov@0.05}{0.762}
\@namedef{VJ@D_brier.raw.tallyqa_l.cov@0.05.ci}{[0.747, 0.777]}
\@namedef{VJ@D_brier.raw.tallyqa_l.cov@0.05.pct}{76.2\%}
\@namedef{VJ@D_brier.raw.tallyqa_l.cov@0.1}{0.896}
\@namedef{VJ@D_brier.raw.tallyqa_l.cov@0.1.ci}{[0.886, 0.905]}
\@namedef{VJ@D_brier.raw.tallyqa_l.cov@0.1.pct}{89.6\%}
\@namedef{VJ@D_brier.raw.tallyqa_l.ece15}{0.074}
\@namedef{VJ@D_brier.raw.tallyqa_l.ece15.ci}{[0.065, 0.085]}
\@namedef{VJ@D_brier.raw.tallyqa_l.nll}{0.468}
\@namedef{VJ@D_brier.raw.tallyqa_l.nll.ci}{[0.431, 0.508]}
\@namedef{VJ@D_brier.raw.tallyqa_l.risk@0.05}{0.052}
\@namedef{VJ@D_brier.raw.tallyqa_l.risk@0.05.ci}{[0.045, 0.060]}
\@namedef{VJ@D_brier.raw.tallyqa_l.risk@0.05.pct}{5.2\%}
\@namedef{VJ@D_brier.raw.tallyqa_l.risk@0.1}{0.105}
\@namedef{VJ@D_brier.raw.tallyqa_l.risk@0.1.ci}{[0.094, 0.116]}
\@namedef{VJ@D_brier.raw.tallyqa_l.risk@0.1.pct}{10.5\%}
\@namedef{VJ@D_brier.raw.textvqa_k8.accuracy}{0.974}
\@namedef{VJ@D_brier.raw.textvqa_k8.accuracy.ci}{[0.966, 0.981]}
\@namedef{VJ@D_brier.raw.textvqa_k8.aurc_maxp}{0.001}
\@namedef{VJ@D_brier.raw.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@D_brier.raw.textvqa_k8.brier}{0.040}
\@namedef{VJ@D_brier.raw.textvqa_k8.brier.ci}{[0.030, 0.052]}
\@namedef{VJ@D_brier.raw.textvqa_k8.cov@0.05}{1.000}
\@namedef{VJ@D_brier.raw.textvqa_k8.cov@0.05.ci}{[0.999, 1.000]}
\@namedef{VJ@D_brier.raw.textvqa_k8.cov@0.05.pct}{100.0\%}
\@namedef{VJ@D_brier.raw.textvqa_k8.cov@0.1}{1.000}
\@namedef{VJ@D_brier.raw.textvqa_k8.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@D_brier.raw.textvqa_k8.cov@0.1.pct}{100.0\%}
\@namedef{VJ@D_brier.raw.textvqa_k8.ece15}{0.013}
\@namedef{VJ@D_brier.raw.textvqa_k8.ece15.ci}{[0.009, 0.019]}
\@namedef{VJ@D_brier.raw.textvqa_k8.nll}{0.104}
\@namedef{VJ@D_brier.raw.textvqa_k8.nll.ci}{[0.072, 0.136]}
\@namedef{VJ@D_brier.raw.textvqa_k8.risk@0.05}{0.026}
\@namedef{VJ@D_brier.raw.textvqa_k8.risk@0.05.ci}{[0.019, 0.033]}
\@namedef{VJ@D_brier.raw.textvqa_k8.risk@0.05.pct}{2.6\%}
\@namedef{VJ@D_brier.raw.textvqa_k8.risk@0.1}{0.026}
\@namedef{VJ@D_brier.raw.textvqa_k8.risk@0.1.ci}{[0.019, 0.033]}
\@namedef{VJ@D_brier.raw.textvqa_k8.risk@0.1.pct}{2.6\%}
\@namedef{VJ@D_brier.ts_local.gqa_val.accuracy}{0.913}
\@namedef{VJ@D_brier.ts_local.gqa_val.accuracy.ci}{[0.906, 0.921]}
\@namedef{VJ@D_brier.ts_local.gqa_val.aurc_maxp}{0.015}
\@namedef{VJ@D_brier.ts_local.gqa_val.aurc_maxp.ci}{[0.013, 0.017]}
\@namedef{VJ@D_brier.ts_local.gqa_val.brier}{0.129}
\@namedef{VJ@D_brier.ts_local.gqa_val.brier.ci}{[0.119, 0.139]}
\@namedef{VJ@D_brier.ts_local.gqa_val.cov@0.05}{0.892}
\@namedef{VJ@D_brier.ts_local.gqa_val.cov@0.05.ci}{[0.883, 0.900]}
\@namedef{VJ@D_brier.ts_local.gqa_val.cov@0.05.pct}{89.2\%}
\@namedef{VJ@D_brier.ts_local.gqa_val.cov@0.1}{1.000}
\@namedef{VJ@D_brier.ts_local.gqa_val.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@D_brier.ts_local.gqa_val.cov@0.1.pct}{100.0\%}
\@namedef{VJ@D_brier.ts_local.gqa_val.ece15}{0.024}
\@namedef{VJ@D_brier.ts_local.gqa_val.ece15.ci}{[0.020, 0.030]}
\@namedef{VJ@D_brier.ts_local.gqa_val.nll}{0.231}
\@namedef{VJ@D_brier.ts_local.gqa_val.nll.ci}{[0.214, 0.247]}
\@namedef{VJ@D_brier.ts_local.gqa_val.risk@0.05}{0.047}
\@namedef{VJ@D_brier.ts_local.gqa_val.risk@0.05.ci}{[0.042, 0.053]}
\@namedef{VJ@D_brier.ts_local.gqa_val.risk@0.05.pct}{4.7\%}
\@namedef{VJ@D_brier.ts_local.gqa_val.risk@0.1}{0.086}
\@namedef{VJ@D_brier.ts_local.gqa_val.risk@0.1.ci}{[0.079, 0.094]}
\@namedef{VJ@D_brier.ts_local.gqa_val.risk@0.1.pct}{8.6\%}
\@namedef{VJ@D_brier.ts_local.macro.accuracy}{0.884}
\@namedef{VJ@D_brier.ts_local.macro.accuracy.ci}{[0.877, 0.890]}
\@namedef{VJ@D_brier.ts_local.macro.aurc_maxp}{0.030}
\@namedef{VJ@D_brier.ts_local.macro.aurc_maxp.ci}{[0.027, 0.034]}
\@namedef{VJ@D_brier.ts_local.macro.brier}{0.167}
\@namedef{VJ@D_brier.ts_local.macro.brier.ci}{[0.159, 0.176]}
\@namedef{VJ@D_brier.ts_local.macro.ece15}{0.029}
\@namedef{VJ@D_brier.ts_local.macro.ece15.ci}{[0.028, 0.035]}
\@namedef{VJ@D_brier.ts_local.macro.nll}{0.315}
\@namedef{VJ@D_brier.ts_local.macro.nll.ci}{[0.301, 0.329]}
\@namedef{VJ@D_brier.ts_local.snli_ve.accuracy}{0.803}
\@namedef{VJ@D_brier.ts_local.snli_ve.accuracy.ci}{[0.783, 0.823]}
\@namedef{VJ@D_brier.ts_local.snli_ve.aurc_maxp}{0.073}
\@namedef{VJ@D_brier.ts_local.snli_ve.aurc_maxp.ci}{[0.060, 0.087]}
\@namedef{VJ@D_brier.ts_local.snli_ve.brier}{0.285}
\@namedef{VJ@D_brier.ts_local.snli_ve.brier.ci}{[0.261, 0.309]}
\@namedef{VJ@D_brier.ts_local.snli_ve.cov@0.05}{0.324}
\@namedef{VJ@D_brier.ts_local.snli_ve.cov@0.05.ci}{[0.303, 0.347]}
\@namedef{VJ@D_brier.ts_local.snli_ve.cov@0.05.pct}{32.4\%}
\@namedef{VJ@D_brier.ts_local.snli_ve.cov@0.1}{0.614}
\@namedef{VJ@D_brier.ts_local.snli_ve.cov@0.1.ci}{[0.592, 0.638]}
\@namedef{VJ@D_brier.ts_local.snli_ve.cov@0.1.pct}{61.4\%}
\@namedef{VJ@D_brier.ts_local.snli_ve.ece15}{0.041}
\@namedef{VJ@D_brier.ts_local.snli_ve.ece15.ci}{[0.037, 0.059]}
\@namedef{VJ@D_brier.ts_local.snli_ve.nll}{0.507}
\@namedef{VJ@D_brier.ts_local.snli_ve.nll.ci}{[0.470, 0.544]}
\@namedef{VJ@D_brier.ts_local.snli_ve.risk@0.05}{0.035}
\@namedef{VJ@D_brier.ts_local.snli_ve.risk@0.05.ci}{[0.021, 0.052]}
\@namedef{VJ@D_brier.ts_local.snli_ve.risk@0.05.pct}{3.5\%}
\@namedef{VJ@D_brier.ts_local.snli_ve.risk@0.1}{0.080}
\@namedef{VJ@D_brier.ts_local.snli_ve.risk@0.1.ci}{[0.064, 0.098]}
\@namedef{VJ@D_brier.ts_local.snli_ve.risk@0.1.pct}{8.0\%}
\@namedef{VJ@D_brier.ts_local.tallyqa_l.accuracy}{0.844}
\@namedef{VJ@D_brier.ts_local.tallyqa_l.accuracy.ci}{[0.831, 0.856]}
\@namedef{VJ@D_brier.ts_local.tallyqa_l.aurc_maxp}{0.033}
\@namedef{VJ@D_brier.ts_local.tallyqa_l.aurc_maxp.ci}{[0.028, 0.039]}
\@namedef{VJ@D_brier.ts_local.tallyqa_l.brier}{0.217}
\@namedef{VJ@D_brier.ts_local.tallyqa_l.brier.ci}{[0.201, 0.234]}
\@namedef{VJ@D_brier.ts_local.tallyqa_l.cov@0.05}{0.761}
\@namedef{VJ@D_brier.ts_local.tallyqa_l.cov@0.05.ci}{[0.745, 0.776]}
\@namedef{VJ@D_brier.ts_local.tallyqa_l.cov@0.05.pct}{76.1\%}
\@namedef{VJ@D_brier.ts_local.tallyqa_l.cov@0.1}{0.897}
\@namedef{VJ@D_brier.ts_local.tallyqa_l.cov@0.1.ci}{[0.887, 0.906]}
\@namedef{VJ@D_brier.ts_local.tallyqa_l.cov@0.1.pct}{89.7\%}
\@namedef{VJ@D_brier.ts_local.tallyqa_l.ece15}{0.040}
\@namedef{VJ@D_brier.ts_local.tallyqa_l.ece15.ci}{[0.033, 0.050]}
\@namedef{VJ@D_brier.ts_local.tallyqa_l.nll}{0.427}
\@namedef{VJ@D_brier.ts_local.tallyqa_l.nll.ci}{[0.397, 0.458]}
\@namedef{VJ@D_brier.ts_local.tallyqa_l.risk@0.05}{0.052}
\@namedef{VJ@D_brier.ts_local.tallyqa_l.risk@0.05.ci}{[0.045, 0.060]}
\@namedef{VJ@D_brier.ts_local.tallyqa_l.risk@0.05.pct}{5.2\%}
\@namedef{VJ@D_brier.ts_local.tallyqa_l.risk@0.1}{0.104}
\@namedef{VJ@D_brier.ts_local.tallyqa_l.risk@0.1.ci}{[0.094, 0.115]}
\@namedef{VJ@D_brier.ts_local.tallyqa_l.risk@0.1.pct}{10.4\%}
\@namedef{VJ@D_brier.ts_local.textvqa_k8.accuracy}{0.974}
\@namedef{VJ@D_brier.ts_local.textvqa_k8.accuracy.ci}{[0.966, 0.981]}
\@namedef{VJ@D_brier.ts_local.textvqa_k8.aurc_maxp}{0.001}
\@namedef{VJ@D_brier.ts_local.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@D_brier.ts_local.textvqa_k8.brier}{0.039}
\@namedef{VJ@D_brier.ts_local.textvqa_k8.brier.ci}{[0.029, 0.049]}
\@namedef{VJ@D_brier.ts_local.textvqa_k8.cov@0.05}{1.000}
\@namedef{VJ@D_brier.ts_local.textvqa_k8.cov@0.05.ci}{[0.999, 1.000]}
\@namedef{VJ@D_brier.ts_local.textvqa_k8.cov@0.05.pct}{100.0\%}
\@namedef{VJ@D_brier.ts_local.textvqa_k8.cov@0.1}{1.000}
\@namedef{VJ@D_brier.ts_local.textvqa_k8.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@D_brier.ts_local.textvqa_k8.cov@0.1.pct}{100.0\%}
\@namedef{VJ@D_brier.ts_local.textvqa_k8.ece15}{0.011}
\@namedef{VJ@D_brier.ts_local.textvqa_k8.ece15.ci}{[0.009, 0.017]}
\@namedef{VJ@D_brier.ts_local.textvqa_k8.nll}{0.094}
\@namedef{VJ@D_brier.ts_local.textvqa_k8.nll.ci}{[0.069, 0.119]}
\@namedef{VJ@D_brier.ts_local.textvqa_k8.risk@0.05}{0.026}
\@namedef{VJ@D_brier.ts_local.textvqa_k8.risk@0.05.ci}{[0.019, 0.033]}
\@namedef{VJ@D_brier.ts_local.textvqa_k8.risk@0.05.pct}{2.6\%}
\@namedef{VJ@D_brier.ts_local.textvqa_k8.risk@0.1}{0.026}
\@namedef{VJ@D_brier.ts_local.textvqa_k8.risk@0.1.ci}{[0.019, 0.033]}
\@namedef{VJ@D_brier.ts_local.textvqa_k8.risk@0.1.pct}{2.6\%}
\@namedef{VJ@D_brier.ts_transfer.gqa_val.accuracy}{0.913}
\@namedef{VJ@D_brier.ts_transfer.gqa_val.accuracy.ci}{[0.906, 0.921]}
\@namedef{VJ@D_brier.ts_transfer.gqa_val.aurc_maxp}{0.015}
\@namedef{VJ@D_brier.ts_transfer.gqa_val.aurc_maxp.ci}{[0.013, 0.017]}
\@namedef{VJ@D_brier.ts_transfer.gqa_val.brier}{0.130}
\@namedef{VJ@D_brier.ts_transfer.gqa_val.brier.ci}{[0.119, 0.140]}
\@namedef{VJ@D_brier.ts_transfer.gqa_val.cov@0.05}{0.893}
\@namedef{VJ@D_brier.ts_transfer.gqa_val.cov@0.05.ci}{[0.885, 0.901]}
\@namedef{VJ@D_brier.ts_transfer.gqa_val.cov@0.05.pct}{89.3\%}
\@namedef{VJ@D_brier.ts_transfer.gqa_val.cov@0.1}{1.000}
\@namedef{VJ@D_brier.ts_transfer.gqa_val.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@D_brier.ts_transfer.gqa_val.cov@0.1.pct}{100.0\%}
\@namedef{VJ@D_brier.ts_transfer.gqa_val.ece15}{0.022}
\@namedef{VJ@D_brier.ts_transfer.gqa_val.ece15.ci}{[0.019, 0.028]}
\@namedef{VJ@D_brier.ts_transfer.gqa_val.nll}{0.231}
\@namedef{VJ@D_brier.ts_transfer.gqa_val.nll.ci}{[0.213, 0.247]}
\@namedef{VJ@D_brier.ts_transfer.gqa_val.risk@0.05}{0.048}
\@namedef{VJ@D_brier.ts_transfer.gqa_val.risk@0.05.ci}{[0.042, 0.053]}
\@namedef{VJ@D_brier.ts_transfer.gqa_val.risk@0.05.pct}{4.8\%}
\@namedef{VJ@D_brier.ts_transfer.gqa_val.risk@0.1}{0.086}
\@namedef{VJ@D_brier.ts_transfer.gqa_val.risk@0.1.ci}{[0.079, 0.094]}
\@namedef{VJ@D_brier.ts_transfer.gqa_val.risk@0.1.pct}{8.6\%}
\@namedef{VJ@D_brier.ts_transfer.macro.accuracy}{0.884}
\@namedef{VJ@D_brier.ts_transfer.macro.accuracy.ci}{[0.877, 0.890]}
\@namedef{VJ@D_brier.ts_transfer.macro.aurc_maxp}{0.030}
\@namedef{VJ@D_brier.ts_transfer.macro.aurc_maxp.ci}{[0.027, 0.034]}
\@namedef{VJ@D_brier.ts_transfer.macro.brier}{0.168}
\@namedef{VJ@D_brier.ts_transfer.macro.brier.ci}{[0.161, 0.176]}
\@namedef{VJ@D_brier.ts_transfer.macro.ece15}{0.042}
\@namedef{VJ@D_brier.ts_transfer.macro.ece15.ci}{[0.041, 0.049]}
\@namedef{VJ@D_brier.ts_transfer.macro.nll}{0.328}
\@namedef{VJ@D_brier.ts_transfer.macro.nll.ci}{[0.316, 0.341]}
\@namedef{VJ@D_brier.ts_transfer.snli_ve.accuracy}{0.803}
\@namedef{VJ@D_brier.ts_transfer.snli_ve.accuracy.ci}{[0.783, 0.823]}
\@namedef{VJ@D_brier.ts_transfer.snli_ve.aurc_maxp}{0.073}
\@namedef{VJ@D_brier.ts_transfer.snli_ve.aurc_maxp.ci}{[0.060, 0.087]}
\@namedef{VJ@D_brier.ts_transfer.snli_ve.brier}{0.287}
\@namedef{VJ@D_brier.ts_transfer.snli_ve.brier.ci}{[0.265, 0.309]}
\@namedef{VJ@D_brier.ts_transfer.snli_ve.cov@0.05}{0.308}
\@namedef{VJ@D_brier.ts_transfer.snli_ve.cov@0.05.ci}{[0.287, 0.331]}
\@namedef{VJ@D_brier.ts_transfer.snli_ve.cov@0.05.pct}{30.8\%}
\@namedef{VJ@D_brier.ts_transfer.snli_ve.cov@0.1}{0.610}
\@namedef{VJ@D_brier.ts_transfer.snli_ve.cov@0.1.ci}{[0.587, 0.633]}
\@namedef{VJ@D_brier.ts_transfer.snli_ve.cov@0.1.pct}{61.0\%}
\@namedef{VJ@D_brier.ts_transfer.snli_ve.ece15}{0.058}
\@namedef{VJ@D_brier.ts_transfer.snli_ve.ece15.ci}{[0.052, 0.075]}
\@namedef{VJ@D_brier.ts_transfer.snli_ve.nll}{0.518}
\@namedef{VJ@D_brier.ts_transfer.snli_ve.nll.ci}{[0.485, 0.551]}
\@namedef{VJ@D_brier.ts_transfer.snli_ve.risk@0.05}{0.035}
\@namedef{VJ@D_brier.ts_transfer.snli_ve.risk@0.05.ci}{[0.021, 0.053]}
\@namedef{VJ@D_brier.ts_transfer.snli_ve.risk@0.05.pct}{3.5\%}
\@namedef{VJ@D_brier.ts_transfer.snli_ve.risk@0.1}{0.080}
\@namedef{VJ@D_brier.ts_transfer.snli_ve.risk@0.1.ci}{[0.064, 0.098]}
\@namedef{VJ@D_brier.ts_transfer.snli_ve.risk@0.1.pct}{8.0\%}
\@namedef{VJ@D_brier.ts_transfer.tallyqa_l.accuracy}{0.844}
\@namedef{VJ@D_brier.ts_transfer.tallyqa_l.accuracy.ci}{[0.831, 0.856]}
\@namedef{VJ@D_brier.ts_transfer.tallyqa_l.aurc_maxp}{0.033}
\@namedef{VJ@D_brier.ts_transfer.tallyqa_l.aurc_maxp.ci}{[0.028, 0.039]}
\@namedef{VJ@D_brier.ts_transfer.tallyqa_l.brier}{0.217}
\@namedef{VJ@D_brier.ts_transfer.tallyqa_l.brier.ci}{[0.203, 0.233]}
\@namedef{VJ@D_brier.ts_transfer.tallyqa_l.cov@0.05}{0.757}
\@namedef{VJ@D_brier.ts_transfer.tallyqa_l.cov@0.05.ci}{[0.741, 0.771]}
\@namedef{VJ@D_brier.ts_transfer.tallyqa_l.cov@0.05.pct}{75.7\%}
\@namedef{VJ@D_brier.ts_transfer.tallyqa_l.cov@0.1}{0.899}
\@namedef{VJ@D_brier.ts_transfer.tallyqa_l.cov@0.1.ci}{[0.890, 0.909]}
\@namedef{VJ@D_brier.ts_transfer.tallyqa_l.cov@0.1.pct}{89.9\%}
\@namedef{VJ@D_brier.ts_transfer.tallyqa_l.ece15}{0.057}
\@namedef{VJ@D_brier.ts_transfer.tallyqa_l.ece15.ci}{[0.055, 0.067]}
\@namedef{VJ@D_brier.ts_transfer.tallyqa_l.nll}{0.455}
\@namedef{VJ@D_brier.ts_transfer.tallyqa_l.nll.ci}{[0.429, 0.481]}
\@namedef{VJ@D_brier.ts_transfer.tallyqa_l.risk@0.05}{0.051}
\@namedef{VJ@D_brier.ts_transfer.tallyqa_l.risk@0.05.ci}{[0.043, 0.059]}
\@namedef{VJ@D_brier.ts_transfer.tallyqa_l.risk@0.05.pct}{5.1\%}
\@namedef{VJ@D_brier.ts_transfer.tallyqa_l.risk@0.1}{0.105}
\@namedef{VJ@D_brier.ts_transfer.tallyqa_l.risk@0.1.ci}{[0.095, 0.116]}
\@namedef{VJ@D_brier.ts_transfer.tallyqa_l.risk@0.1.pct}{10.5\%}
\@namedef{VJ@D_brier.ts_transfer.textvqa_k8.accuracy}{0.974}
\@namedef{VJ@D_brier.ts_transfer.textvqa_k8.accuracy.ci}{[0.966, 0.981]}
\@namedef{VJ@D_brier.ts_transfer.textvqa_k8.aurc_maxp}{0.001}
\@namedef{VJ@D_brier.ts_transfer.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@D_brier.ts_transfer.textvqa_k8.brier}{0.039}
\@namedef{VJ@D_brier.ts_transfer.textvqa_k8.brier.ci}{[0.030, 0.049]}
\@namedef{VJ@D_brier.ts_transfer.textvqa_k8.cov@0.05}{1.000}
\@namedef{VJ@D_brier.ts_transfer.textvqa_k8.cov@0.05.ci}{[0.999, 1.000]}
\@namedef{VJ@D_brier.ts_transfer.textvqa_k8.cov@0.05.pct}{100.0\%}
\@namedef{VJ@D_brier.ts_transfer.textvqa_k8.cov@0.1}{1.000}
\@namedef{VJ@D_brier.ts_transfer.textvqa_k8.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@D_brier.ts_transfer.textvqa_k8.cov@0.1.pct}{100.0\%}
\@namedef{VJ@D_brier.ts_transfer.textvqa_k8.ece15}{0.030}
\@namedef{VJ@D_brier.ts_transfer.textvqa_k8.ece15.ci}{[0.029, 0.036]}
\@namedef{VJ@D_brier.ts_transfer.textvqa_k8.nll}{0.110}
\@namedef{VJ@D_brier.ts_transfer.textvqa_k8.nll.ci}{[0.089, 0.132]}
\@namedef{VJ@D_brier.ts_transfer.textvqa_k8.risk@0.05}{0.026}
\@namedef{VJ@D_brier.ts_transfer.textvqa_k8.risk@0.05.ci}{[0.019, 0.033]}
\@namedef{VJ@D_brier.ts_transfer.textvqa_k8.risk@0.05.pct}{2.6\%}
\@namedef{VJ@D_brier.ts_transfer.textvqa_k8.risk@0.1}{0.026}
\@namedef{VJ@D_brier.ts_transfer.textvqa_k8.risk@0.1.ci}{[0.019, 0.033]}
\@namedef{VJ@D_brier.ts_transfer.textvqa_k8.risk@0.1.pct}{2.6\%}
\@namedef{VJ@D_ce.raw.gqa_val.accuracy}{0.913}
\@namedef{VJ@D_ce.raw.gqa_val.accuracy.ci}{[0.906, 0.920]}
\@namedef{VJ@D_ce.raw.gqa_val.aurc_maxp}{0.015}
\@namedef{VJ@D_ce.raw.gqa_val.aurc_maxp.ci}{[0.013, 0.017]}
\@namedef{VJ@D_ce.raw.gqa_val.brier}{0.154}
\@namedef{VJ@D_ce.raw.gqa_val.brier.ci}{[0.141, 0.167]}
\@namedef{VJ@D_ce.raw.gqa_val.cov@0.05}{0.894}
\@namedef{VJ@D_ce.raw.gqa_val.cov@0.05.ci}{[0.886, 0.902]}
\@namedef{VJ@D_ce.raw.gqa_val.cov@0.05.pct}{89.4\%}
\@namedef{VJ@D_ce.raw.gqa_val.cov@0.1}{1.000}
\@namedef{VJ@D_ce.raw.gqa_val.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@D_ce.raw.gqa_val.cov@0.1.pct}{100.0\%}
\@namedef{VJ@D_ce.raw.gqa_val.ece15}{0.071}
\@namedef{VJ@D_ce.raw.gqa_val.ece15.ci}{[0.065, 0.078]}
\@namedef{VJ@D_ce.raw.gqa_val.nll}{0.402}
\@namedef{VJ@D_ce.raw.gqa_val.nll.ci}{[0.362, 0.440]}
\@namedef{VJ@D_ce.raw.gqa_val.risk@0.05}{0.047}
\@namedef{VJ@D_ce.raw.gqa_val.risk@0.05.ci}{[0.042, 0.053]}
\@namedef{VJ@D_ce.raw.gqa_val.risk@0.05.pct}{4.7\%}
\@namedef{VJ@D_ce.raw.gqa_val.risk@0.1}{0.087}
\@namedef{VJ@D_ce.raw.gqa_val.risk@0.1.ci}{[0.080, 0.094]}
\@namedef{VJ@D_ce.raw.gqa_val.risk@0.1.pct}{8.7\%}
\@namedef{VJ@D_ce.raw.macro.accuracy}{0.883}
\@namedef{VJ@D_ce.raw.macro.accuracy.ci}{[0.877, 0.890]}
\@namedef{VJ@D_ce.raw.macro.aurc_maxp}{0.031}
\@namedef{VJ@D_ce.raw.macro.aurc_maxp.ci}{[0.028, 0.035]}
\@namedef{VJ@D_ce.raw.macro.brier}{0.192}
\@namedef{VJ@D_ce.raw.macro.brier.ci}{[0.181, 0.203]}
\@namedef{VJ@D_ce.raw.macro.ece15}{0.079}
\@namedef{VJ@D_ce.raw.macro.ece15.ci}{[0.075, 0.086]}
\@namedef{VJ@D_ce.raw.macro.nll}{0.439}
\@namedef{VJ@D_ce.raw.macro.nll.ci}{[0.411, 0.465]}
\@namedef{VJ@D_ce.raw.snli_ve.accuracy}{0.803}
\@namedef{VJ@D_ce.raw.snli_ve.accuracy.ci}{[0.783, 0.822]}
\@namedef{VJ@D_ce.raw.snli_ve.aurc_maxp}{0.077}
\@namedef{VJ@D_ce.raw.snli_ve.aurc_maxp.ci}{[0.064, 0.091]}
\@namedef{VJ@D_ce.raw.snli_ve.brier}{0.325}
\@namedef{VJ@D_ce.raw.snli_ve.brier.ci}{[0.292, 0.358]}
\@namedef{VJ@D_ce.raw.snli_ve.cov@0.05}{0.281}
\@namedef{VJ@D_ce.raw.snli_ve.cov@0.05.ci}{[0.261, 0.303]}
\@namedef{VJ@D_ce.raw.snli_ve.cov@0.05.pct}{28.1\%}
\@namedef{VJ@D_ce.raw.snli_ve.cov@0.1}{0.585}
\@namedef{VJ@D_ce.raw.snli_ve.cov@0.1.ci}{[0.565, 0.608]}
\@namedef{VJ@D_ce.raw.snli_ve.cov@0.1.pct}{58.5\%}
\@namedef{VJ@D_ce.raw.snli_ve.ece15}{0.131}
\@namedef{VJ@D_ce.raw.snli_ve.ece15.ci}{[0.114, 0.150]}
\@namedef{VJ@D_ce.raw.snli_ve.nll}{0.671}
\@namedef{VJ@D_ce.raw.snli_ve.nll.ci}{[0.595, 0.747]}
\@namedef{VJ@D_ce.raw.snli_ve.risk@0.05}{0.033}
\@namedef{VJ@D_ce.raw.snli_ve.risk@0.05.ci}{[0.020, 0.048]}
\@namedef{VJ@D_ce.raw.snli_ve.risk@0.05.pct}{3.3\%}
\@namedef{VJ@D_ce.raw.snli_ve.risk@0.1}{0.080}
\@namedef{VJ@D_ce.raw.snli_ve.risk@0.1.ci}{[0.065, 0.099]}
\@namedef{VJ@D_ce.raw.snli_ve.risk@0.1.pct}{8.0\%}
\@namedef{VJ@D_ce.raw.tallyqa_l.accuracy}{0.844}
\@namedef{VJ@D_ce.raw.tallyqa_l.accuracy.ci}{[0.831, 0.856]}
\@namedef{VJ@D_ce.raw.tallyqa_l.aurc_maxp}{0.034}
\@namedef{VJ@D_ce.raw.tallyqa_l.aurc_maxp.ci}{[0.029, 0.039]}
\@namedef{VJ@D_ce.raw.tallyqa_l.brier}{0.247}
\@namedef{VJ@D_ce.raw.tallyqa_l.brier.ci}{[0.227, 0.267]}
\@namedef{VJ@D_ce.raw.tallyqa_l.cov@0.05}{0.762}
\@namedef{VJ@D_ce.raw.tallyqa_l.cov@0.05.ci}{[0.746, 0.777]}
\@namedef{VJ@D_ce.raw.tallyqa_l.cov@0.05.pct}{76.2\%}
\@namedef{VJ@D_ce.raw.tallyqa_l.cov@0.1}{0.892}
\@namedef{VJ@D_ce.raw.tallyqa_l.cov@0.1.ci}{[0.882, 0.902]}
\@namedef{VJ@D_ce.raw.tallyqa_l.cov@0.1.pct}{89.2\%}
\@namedef{VJ@D_ce.raw.tallyqa_l.ece15}{0.100}
\@namedef{VJ@D_ce.raw.tallyqa_l.ece15.ci}{[0.090, 0.111]}
\@namedef{VJ@D_ce.raw.tallyqa_l.nll}{0.560}
\@namedef{VJ@D_ce.raw.tallyqa_l.nll.ci}{[0.512, 0.611]}
\@namedef{VJ@D_ce.raw.tallyqa_l.risk@0.05}{0.053}
\@namedef{VJ@D_ce.raw.tallyqa_l.risk@0.05.ci}{[0.046, 0.061]}
\@namedef{VJ@D_ce.raw.tallyqa_l.risk@0.05.pct}{5.3\%}
\@namedef{VJ@D_ce.raw.tallyqa_l.risk@0.1}{0.103}
\@namedef{VJ@D_ce.raw.tallyqa_l.risk@0.1.ci}{[0.092, 0.114]}
\@namedef{VJ@D_ce.raw.tallyqa_l.risk@0.1.pct}{10.3\%}
\@namedef{VJ@D_ce.raw.textvqa_k8.accuracy}{0.974}
\@namedef{VJ@D_ce.raw.textvqa_k8.accuracy.ci}{[0.966, 0.981]}
\@namedef{VJ@D_ce.raw.textvqa_k8.aurc_maxp}{0.001}
\@namedef{VJ@D_ce.raw.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@D_ce.raw.textvqa_k8.brier}{0.042}
\@namedef{VJ@D_ce.raw.textvqa_k8.brier.ci}{[0.031, 0.054]}
\@namedef{VJ@D_ce.raw.textvqa_k8.cov@0.05}{1.000}
\@namedef{VJ@D_ce.raw.textvqa_k8.cov@0.05.ci}{[1.000, 1.000]}
\@namedef{VJ@D_ce.raw.textvqa_k8.cov@0.05.pct}{100.0\%}
\@namedef{VJ@D_ce.raw.textvqa_k8.cov@0.1}{1.000}
\@namedef{VJ@D_ce.raw.textvqa_k8.cov@0.1.ci}{[1.000, 1.000]}
\@namedef{VJ@D_ce.raw.textvqa_k8.cov@0.1.pct}{100.0\%}
\@namedef{VJ@D_ce.raw.textvqa_k8.ece15}{0.016}
\@namedef{VJ@D_ce.raw.textvqa_k8.ece15.ci}{[0.012, 0.023]}
\@namedef{VJ@D_ce.raw.textvqa_k8.nll}{0.121}
\@namedef{VJ@D_ce.raw.textvqa_k8.nll.ci}{[0.081, 0.159]}
\@namedef{VJ@D_ce.raw.textvqa_k8.risk@0.05}{0.026}
\@namedef{VJ@D_ce.raw.textvqa_k8.risk@0.05.ci}{[0.019, 0.034]}
\@namedef{VJ@D_ce.raw.textvqa_k8.risk@0.05.pct}{2.6\%}
\@namedef{VJ@D_ce.raw.textvqa_k8.risk@0.1}{0.026}
\@namedef{VJ@D_ce.raw.textvqa_k8.risk@0.1.ci}{[0.019, 0.034]}
\@namedef{VJ@D_ce.raw.textvqa_k8.risk@0.1.pct}{2.6\%}
\@namedef{VJ@D_ce.ts_local.gqa_val.accuracy}{0.913}
\@namedef{VJ@D_ce.ts_local.gqa_val.accuracy.ci}{[0.906, 0.920]}
\@namedef{VJ@D_ce.ts_local.gqa_val.aurc_maxp}{0.016}
\@namedef{VJ@D_ce.ts_local.gqa_val.aurc_maxp.ci}{[0.013, 0.018]}
\@namedef{VJ@D_ce.ts_local.gqa_val.brier}{0.132}
\@namedef{VJ@D_ce.ts_local.gqa_val.brier.ci}{[0.121, 0.142]}
\@namedef{VJ@D_ce.ts_local.gqa_val.cov@0.05}{0.891}
\@namedef{VJ@D_ce.ts_local.gqa_val.cov@0.05.ci}{[0.883, 0.899]}
\@namedef{VJ@D_ce.ts_local.gqa_val.cov@0.05.pct}{89.1\%}
\@namedef{VJ@D_ce.ts_local.gqa_val.cov@0.1}{0.999}
\@namedef{VJ@D_ce.ts_local.gqa_val.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@D_ce.ts_local.gqa_val.cov@0.1.pct}{99.9\%}
\@namedef{VJ@D_ce.ts_local.gqa_val.ece15}{0.025}
\@namedef{VJ@D_ce.ts_local.gqa_val.ece15.ci}{[0.021, 0.030]}
\@namedef{VJ@D_ce.ts_local.gqa_val.nll}{0.239}
\@namedef{VJ@D_ce.ts_local.gqa_val.nll.ci}{[0.221, 0.255]}
\@namedef{VJ@D_ce.ts_local.gqa_val.risk@0.05}{0.048}
\@namedef{VJ@D_ce.ts_local.gqa_val.risk@0.05.ci}{[0.042, 0.053]}
\@namedef{VJ@D_ce.ts_local.gqa_val.risk@0.05.pct}{4.8\%}
\@namedef{VJ@D_ce.ts_local.gqa_val.risk@0.1}{0.087}
\@namedef{VJ@D_ce.ts_local.gqa_val.risk@0.1.ci}{[0.079, 0.094]}
\@namedef{VJ@D_ce.ts_local.gqa_val.risk@0.1.pct}{8.7\%}
\@namedef{VJ@D_ce.ts_local.macro.accuracy}{0.883}
\@namedef{VJ@D_ce.ts_local.macro.accuracy.ci}{[0.877, 0.890]}
\@namedef{VJ@D_ce.ts_local.macro.aurc_maxp}{0.031}
\@namedef{VJ@D_ce.ts_local.macro.aurc_maxp.ci}{[0.028, 0.035]}
\@namedef{VJ@D_ce.ts_local.macro.brier}{0.169}
\@namedef{VJ@D_ce.ts_local.macro.brier.ci}{[0.161, 0.177]}
\@namedef{VJ@D_ce.ts_local.macro.ece15}{0.031}
\@namedef{VJ@D_ce.ts_local.macro.ece15.ci}{[0.029, 0.037]}
\@namedef{VJ@D_ce.ts_local.macro.nll}{0.320}
\@namedef{VJ@D_ce.ts_local.macro.nll.ci}{[0.306, 0.334]}
\@namedef{VJ@D_ce.ts_local.snli_ve.accuracy}{0.803}
\@namedef{VJ@D_ce.ts_local.snli_ve.accuracy.ci}{[0.783, 0.822]}
\@namedef{VJ@D_ce.ts_local.snli_ve.aurc_maxp}{0.074}
\@namedef{VJ@D_ce.ts_local.snli_ve.aurc_maxp.ci}{[0.062, 0.089]}
\@namedef{VJ@D_ce.ts_local.snli_ve.brier}{0.287}
\@namedef{VJ@D_ce.ts_local.snli_ve.brier.ci}{[0.263, 0.311]}
\@namedef{VJ@D_ce.ts_local.snli_ve.cov@0.05}{0.300}
\@namedef{VJ@D_ce.ts_local.snli_ve.cov@0.05.ci}{[0.280, 0.323]}
\@namedef{VJ@D_ce.ts_local.snli_ve.cov@0.05.pct}{30.0\%}
\@namedef{VJ@D_ce.ts_local.snli_ve.cov@0.1}{0.614}
\@namedef{VJ@D_ce.ts_local.snli_ve.cov@0.1.ci}{[0.592, 0.637]}
\@namedef{VJ@D_ce.ts_local.snli_ve.cov@0.1.pct}{61.4\%}
\@namedef{VJ@D_ce.ts_local.snli_ve.ece15}{0.043}
\@namedef{VJ@D_ce.ts_local.snli_ve.ece15.ci}{[0.036, 0.060]}
\@namedef{VJ@D_ce.ts_local.snli_ve.nll}{0.511}
\@namedef{VJ@D_ce.ts_local.snli_ve.nll.ci}{[0.474, 0.549]}
\@namedef{VJ@D_ce.ts_local.snli_ve.risk@0.05}{0.037}
\@namedef{VJ@D_ce.ts_local.snli_ve.risk@0.05.ci}{[0.022, 0.054]}
\@namedef{VJ@D_ce.ts_local.snli_ve.risk@0.05.pct}{3.7\%}
\@namedef{VJ@D_ce.ts_local.snli_ve.risk@0.1}{0.082}
\@namedef{VJ@D_ce.ts_local.snli_ve.risk@0.1.ci}{[0.066, 0.100]}
\@namedef{VJ@D_ce.ts_local.snli_ve.risk@0.1.pct}{8.2\%}
\@namedef{VJ@D_ce.ts_local.tallyqa_l.accuracy}{0.844}
\@namedef{VJ@D_ce.ts_local.tallyqa_l.accuracy.ci}{[0.831, 0.856]}
\@namedef{VJ@D_ce.ts_local.tallyqa_l.aurc_maxp}{0.034}
\@namedef{VJ@D_ce.ts_local.tallyqa_l.aurc_maxp.ci}{[0.029, 0.039]}
\@namedef{VJ@D_ce.ts_local.tallyqa_l.brier}{0.219}
\@namedef{VJ@D_ce.ts_local.tallyqa_l.brier.ci}{[0.203, 0.236]}
\@namedef{VJ@D_ce.ts_local.tallyqa_l.cov@0.05}{0.760}
\@namedef{VJ@D_ce.ts_local.tallyqa_l.cov@0.05.ci}{[0.744, 0.774]}
\@namedef{VJ@D_ce.ts_local.tallyqa_l.cov@0.05.pct}{76.0\%}
\@namedef{VJ@D_ce.ts_local.tallyqa_l.cov@0.1}{0.897}
\@namedef{VJ@D_ce.ts_local.tallyqa_l.cov@0.1.ci}{[0.887, 0.906]}
\@namedef{VJ@D_ce.ts_local.tallyqa_l.cov@0.1.pct}{89.7\%}
\@namedef{VJ@D_ce.ts_local.tallyqa_l.ece15}{0.045}
\@namedef{VJ@D_ce.ts_local.tallyqa_l.ece15.ci}{[0.037, 0.054]}
\@namedef{VJ@D_ce.ts_local.tallyqa_l.nll}{0.434}
\@namedef{VJ@D_ce.ts_local.tallyqa_l.nll.ci}{[0.403, 0.465]}
\@namedef{VJ@D_ce.ts_local.tallyqa_l.risk@0.05}{0.052}
\@namedef{VJ@D_ce.ts_local.tallyqa_l.risk@0.05.ci}{[0.044, 0.060]}
\@namedef{VJ@D_ce.ts_local.tallyqa_l.risk@0.05.pct}{5.2\%}
\@namedef{VJ@D_ce.ts_local.tallyqa_l.risk@0.1}{0.104}
\@namedef{VJ@D_ce.ts_local.tallyqa_l.risk@0.1.ci}{[0.094, 0.115]}
\@namedef{VJ@D_ce.ts_local.tallyqa_l.risk@0.1.pct}{10.4\%}
\@namedef{VJ@D_ce.ts_local.textvqa_k8.accuracy}{0.974}
\@namedef{VJ@D_ce.ts_local.textvqa_k8.accuracy.ci}{[0.966, 0.981]}
\@namedef{VJ@D_ce.ts_local.textvqa_k8.aurc_maxp}{0.001}
\@namedef{VJ@D_ce.ts_local.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@D_ce.ts_local.textvqa_k8.brier}{0.039}
\@namedef{VJ@D_ce.ts_local.textvqa_k8.brier.ci}{[0.029, 0.050]}
\@namedef{VJ@D_ce.ts_local.textvqa_k8.cov@0.05}{1.000}
\@namedef{VJ@D_ce.ts_local.textvqa_k8.cov@0.05.ci}{[1.000, 1.000]}
\@namedef{VJ@D_ce.ts_local.textvqa_k8.cov@0.05.pct}{100.0\%}
\@namedef{VJ@D_ce.ts_local.textvqa_k8.cov@0.1}{1.000}
\@namedef{VJ@D_ce.ts_local.textvqa_k8.cov@0.1.ci}{[1.000, 1.000]}
\@namedef{VJ@D_ce.ts_local.textvqa_k8.cov@0.1.pct}{100.0\%}
\@namedef{VJ@D_ce.ts_local.textvqa_k8.ece15}{0.011}
\@namedef{VJ@D_ce.ts_local.textvqa_k8.ece15.ci}{[0.010, 0.017]}
\@namedef{VJ@D_ce.ts_local.textvqa_k8.nll}{0.096}
\@namedef{VJ@D_ce.ts_local.textvqa_k8.nll.ci}{[0.071, 0.122]}
\@namedef{VJ@D_ce.ts_local.textvqa_k8.risk@0.05}{0.026}
\@namedef{VJ@D_ce.ts_local.textvqa_k8.risk@0.05.ci}{[0.019, 0.034]}
\@namedef{VJ@D_ce.ts_local.textvqa_k8.risk@0.05.pct}{2.6\%}
\@namedef{VJ@D_ce.ts_local.textvqa_k8.risk@0.1}{0.026}
\@namedef{VJ@D_ce.ts_local.textvqa_k8.risk@0.1.ci}{[0.019, 0.034]}
\@namedef{VJ@D_ce.ts_local.textvqa_k8.risk@0.1.pct}{2.6\%}
\@namedef{VJ@D_ce.ts_transfer.gqa_val.accuracy}{0.913}
\@namedef{VJ@D_ce.ts_transfer.gqa_val.accuracy.ci}{[0.906, 0.920]}
\@namedef{VJ@D_ce.ts_transfer.gqa_val.aurc_maxp}{0.016}
\@namedef{VJ@D_ce.ts_transfer.gqa_val.aurc_maxp.ci}{[0.013, 0.018]}
\@namedef{VJ@D_ce.ts_transfer.gqa_val.brier}{0.132}
\@namedef{VJ@D_ce.ts_transfer.gqa_val.brier.ci}{[0.121, 0.143]}
\@namedef{VJ@D_ce.ts_transfer.gqa_val.cov@0.05}{0.890}
\@namedef{VJ@D_ce.ts_transfer.gqa_val.cov@0.05.ci}{[0.882, 0.898]}
\@namedef{VJ@D_ce.ts_transfer.gqa_val.cov@0.05.pct}{89.0\%}
\@namedef{VJ@D_ce.ts_transfer.gqa_val.cov@0.1}{0.999}
\@namedef{VJ@D_ce.ts_transfer.gqa_val.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@D_ce.ts_transfer.gqa_val.cov@0.1.pct}{99.9\%}
\@namedef{VJ@D_ce.ts_transfer.gqa_val.ece15}{0.024}
\@namedef{VJ@D_ce.ts_transfer.gqa_val.ece15.ci}{[0.020, 0.029]}
\@namedef{VJ@D_ce.ts_transfer.gqa_val.nll}{0.239}
\@namedef{VJ@D_ce.ts_transfer.gqa_val.nll.ci}{[0.221, 0.256]}
\@namedef{VJ@D_ce.ts_transfer.gqa_val.risk@0.05}{0.048}
\@namedef{VJ@D_ce.ts_transfer.gqa_val.risk@0.05.ci}{[0.042, 0.053]}
\@namedef{VJ@D_ce.ts_transfer.gqa_val.risk@0.05.pct}{4.8\%}
\@namedef{VJ@D_ce.ts_transfer.gqa_val.risk@0.1}{0.087}
\@namedef{VJ@D_ce.ts_transfer.gqa_val.risk@0.1.ci}{[0.079, 0.094]}
\@namedef{VJ@D_ce.ts_transfer.gqa_val.risk@0.1.pct}{8.7\%}
\@namedef{VJ@D_ce.ts_transfer.macro.accuracy}{0.883}
\@namedef{VJ@D_ce.ts_transfer.macro.accuracy.ci}{[0.877, 0.890]}
\@namedef{VJ@D_ce.ts_transfer.macro.aurc_maxp}{0.031}
\@namedef{VJ@D_ce.ts_transfer.macro.aurc_maxp.ci}{[0.028, 0.035]}
\@namedef{VJ@D_ce.ts_transfer.macro.brier}{0.171}
\@namedef{VJ@D_ce.ts_transfer.macro.brier.ci}{[0.163, 0.178]}
\@namedef{VJ@D_ce.ts_transfer.macro.ece15}{0.049}
\@namedef{VJ@D_ce.ts_transfer.macro.ece15.ci}{[0.049, 0.056]}
\@namedef{VJ@D_ce.ts_transfer.macro.nll}{0.339}
\@namedef{VJ@D_ce.ts_transfer.macro.nll.ci}{[0.326, 0.351]}
\@namedef{VJ@D_ce.ts_transfer.snli_ve.accuracy}{0.803}
\@namedef{VJ@D_ce.ts_transfer.snli_ve.accuracy.ci}{[0.783, 0.822]}
\@namedef{VJ@D_ce.ts_transfer.snli_ve.aurc_maxp}{0.074}
\@namedef{VJ@D_ce.ts_transfer.snli_ve.aurc_maxp.ci}{[0.061, 0.089]}
\@namedef{VJ@D_ce.ts_transfer.snli_ve.brier}{0.289}
\@namedef{VJ@D_ce.ts_transfer.snli_ve.brier.ci}{[0.266, 0.312]}
\@namedef{VJ@D_ce.ts_transfer.snli_ve.cov@0.05}{0.299}
\@namedef{VJ@D_ce.ts_transfer.snli_ve.cov@0.05.ci}{[0.278, 0.321]}
\@namedef{VJ@D_ce.ts_transfer.snli_ve.cov@0.05.pct}{29.9\%}
\@namedef{VJ@D_ce.ts_transfer.snli_ve.cov@0.1}{0.614}
\@namedef{VJ@D_ce.ts_transfer.snli_ve.cov@0.1.ci}{[0.592, 0.638]}
\@namedef{VJ@D_ce.ts_transfer.snli_ve.cov@0.1.pct}{61.4\%}
\@namedef{VJ@D_ce.ts_transfer.snli_ve.ece15}{0.057}
\@namedef{VJ@D_ce.ts_transfer.snli_ve.ece15.ci}{[0.051, 0.074]}
\@namedef{VJ@D_ce.ts_transfer.snli_ve.nll}{0.519}
\@namedef{VJ@D_ce.ts_transfer.snli_ve.nll.ci}{[0.484, 0.553]}
\@namedef{VJ@D_ce.ts_transfer.snli_ve.risk@0.05}{0.038}
\@namedef{VJ@D_ce.ts_transfer.snli_ve.risk@0.05.ci}{[0.022, 0.055]}
\@namedef{VJ@D_ce.ts_transfer.snli_ve.risk@0.05.pct}{3.8\%}
\@namedef{VJ@D_ce.ts_transfer.snli_ve.risk@0.1}{0.082}
\@namedef{VJ@D_ce.ts_transfer.snli_ve.risk@0.1.ci}{[0.066, 0.100]}
\@namedef{VJ@D_ce.ts_transfer.snli_ve.risk@0.1.pct}{8.2\%}
\@namedef{VJ@D_ce.ts_transfer.tallyqa_l.accuracy}{0.844}
\@namedef{VJ@D_ce.ts_transfer.tallyqa_l.accuracy.ci}{[0.831, 0.856]}
\@namedef{VJ@D_ce.ts_transfer.tallyqa_l.aurc_maxp}{0.034}
\@namedef{VJ@D_ce.ts_transfer.tallyqa_l.aurc_maxp.ci}{[0.029, 0.039]}
\@namedef{VJ@D_ce.ts_transfer.tallyqa_l.brier}{0.220}
\@namedef{VJ@D_ce.ts_transfer.tallyqa_l.brier.ci}{[0.206, 0.235]}
\@namedef{VJ@D_ce.ts_transfer.tallyqa_l.cov@0.05}{0.759}
\@namedef{VJ@D_ce.ts_transfer.tallyqa_l.cov@0.05.ci}{[0.743, 0.773]}
\@namedef{VJ@D_ce.ts_transfer.tallyqa_l.cov@0.05.pct}{75.9\%}
\@namedef{VJ@D_ce.ts_transfer.tallyqa_l.cov@0.1}{0.896}
\@namedef{VJ@D_ce.ts_transfer.tallyqa_l.cov@0.1.ci}{[0.886, 0.905]}
\@namedef{VJ@D_ce.ts_transfer.tallyqa_l.cov@0.1.pct}{89.6\%}
\@namedef{VJ@D_ce.ts_transfer.tallyqa_l.ece15}{0.069}
\@namedef{VJ@D_ce.ts_transfer.tallyqa_l.ece15.ci}{[0.065, 0.078]}
\@namedef{VJ@D_ce.ts_transfer.tallyqa_l.nll}{0.470}
\@namedef{VJ@D_ce.ts_transfer.tallyqa_l.nll.ci}{[0.445, 0.496]}
\@namedef{VJ@D_ce.ts_transfer.tallyqa_l.risk@0.05}{0.052}
\@namedef{VJ@D_ce.ts_transfer.tallyqa_l.risk@0.05.ci}{[0.044, 0.060]}
\@namedef{VJ@D_ce.ts_transfer.tallyqa_l.risk@0.05.pct}{5.2\%}
\@namedef{VJ@D_ce.ts_transfer.tallyqa_l.risk@0.1}{0.104}
\@namedef{VJ@D_ce.ts_transfer.tallyqa_l.risk@0.1.ci}{[0.094, 0.115]}
\@namedef{VJ@D_ce.ts_transfer.tallyqa_l.risk@0.1.pct}{10.4\%}
\@namedef{VJ@D_ce.ts_transfer.textvqa_k8.accuracy}{0.974}
\@namedef{VJ@D_ce.ts_transfer.textvqa_k8.accuracy.ci}{[0.966, 0.981]}
\@namedef{VJ@D_ce.ts_transfer.textvqa_k8.aurc_maxp}{0.001}
\@namedef{VJ@D_ce.ts_transfer.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@D_ce.ts_transfer.textvqa_k8.brier}{0.041}
\@namedef{VJ@D_ce.ts_transfer.textvqa_k8.brier.ci}{[0.033, 0.051]}
\@namedef{VJ@D_ce.ts_transfer.textvqa_k8.cov@0.05}{1.000}
\@namedef{VJ@D_ce.ts_transfer.textvqa_k8.cov@0.05.ci}{[0.999, 1.000]}
\@namedef{VJ@D_ce.ts_transfer.textvqa_k8.cov@0.05.pct}{100.0\%}
\@namedef{VJ@D_ce.ts_transfer.textvqa_k8.cov@0.1}{1.000}
\@namedef{VJ@D_ce.ts_transfer.textvqa_k8.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@D_ce.ts_transfer.textvqa_k8.cov@0.1.pct}{100.0\%}
\@namedef{VJ@D_ce.ts_transfer.textvqa_k8.ece15}{0.048}
\@namedef{VJ@D_ce.ts_transfer.textvqa_k8.ece15.ci}{[0.047, 0.054]}
\@namedef{VJ@D_ce.ts_transfer.textvqa_k8.nll}{0.129}
\@namedef{VJ@D_ce.ts_transfer.textvqa_k8.nll.ci}{[0.109, 0.150]}
\@namedef{VJ@D_ce.ts_transfer.textvqa_k8.risk@0.05}{0.026}
\@namedef{VJ@D_ce.ts_transfer.textvqa_k8.risk@0.05.ci}{[0.019, 0.033]}
\@namedef{VJ@D_ce.ts_transfer.textvqa_k8.risk@0.05.pct}{2.6\%}
\@namedef{VJ@D_ce.ts_transfer.textvqa_k8.risk@0.1}{0.026}
\@namedef{VJ@D_ce.ts_transfer.textvqa_k8.risk@0.1.ci}{[0.019, 0.033]}
\@namedef{VJ@D_ce.ts_transfer.textvqa_k8.risk@0.1.pct}{2.6\%}
\@namedef{VJ@D_ceperm.raw.gqa_val.accuracy}{0.913}
\@namedef{VJ@D_ceperm.raw.gqa_val.accuracy.ci}{[0.906, 0.920]}
\@namedef{VJ@D_ceperm.raw.gqa_val.aurc_maxp}{0.015}
\@namedef{VJ@D_ceperm.raw.gqa_val.aurc_maxp.ci}{[0.012, 0.017]}
\@namedef{VJ@D_ceperm.raw.gqa_val.brier}{0.153}
\@namedef{VJ@D_ceperm.raw.gqa_val.brier.ci}{[0.140, 0.166]}
\@namedef{VJ@D_ceperm.raw.gqa_val.cov@0.05}{0.888}
\@namedef{VJ@D_ceperm.raw.gqa_val.cov@0.05.ci}{[0.880, 0.896]}
\@namedef{VJ@D_ceperm.raw.gqa_val.cov@0.05.pct}{88.8\%}
\@namedef{VJ@D_ceperm.raw.gqa_val.cov@0.1}{1.000}
\@namedef{VJ@D_ceperm.raw.gqa_val.cov@0.1.ci}{[1.000, 1.000]}
\@namedef{VJ@D_ceperm.raw.gqa_val.cov@0.1.pct}{100.0\%}
\@namedef{VJ@D_ceperm.raw.gqa_val.ece15}{0.070}
\@namedef{VJ@D_ceperm.raw.gqa_val.ece15.ci}{[0.064, 0.077]}
\@namedef{VJ@D_ceperm.raw.gqa_val.nll}{0.389}
\@namedef{VJ@D_ceperm.raw.gqa_val.nll.ci}{[0.352, 0.426]}
\@namedef{VJ@D_ceperm.raw.gqa_val.risk@0.05}{0.047}
\@namedef{VJ@D_ceperm.raw.gqa_val.risk@0.05.ci}{[0.041, 0.052]}
\@namedef{VJ@D_ceperm.raw.gqa_val.risk@0.05.pct}{4.7\%}
\@namedef{VJ@D_ceperm.raw.gqa_val.risk@0.1}{0.087}
\@namedef{VJ@D_ceperm.raw.gqa_val.risk@0.1.ci}{[0.080, 0.094]}
\@namedef{VJ@D_ceperm.raw.gqa_val.risk@0.1.pct}{8.7\%}
\@namedef{VJ@D_ceperm.raw.macro.accuracy}{0.885}
\@namedef{VJ@D_ceperm.raw.macro.accuracy.ci}{[0.878, 0.891]}
\@namedef{VJ@D_ceperm.raw.macro.aurc_maxp}{0.032}
\@namedef{VJ@D_ceperm.raw.macro.aurc_maxp.ci}{[0.028, 0.035]}
\@namedef{VJ@D_ceperm.raw.macro.brier}{0.189}
\@namedef{VJ@D_ceperm.raw.macro.brier.ci}{[0.179, 0.200]}
\@namedef{VJ@D_ceperm.raw.macro.ece15}{0.076}
\@namedef{VJ@D_ceperm.raw.macro.ece15.ci}{[0.072, 0.083]}
\@namedef{VJ@D_ceperm.raw.macro.nll}{0.423}
\@namedef{VJ@D_ceperm.raw.macro.nll.ci}{[0.396, 0.448]}
\@namedef{VJ@D_ceperm.raw.snli_ve.accuracy}{0.807}
\@namedef{VJ@D_ceperm.raw.snli_ve.accuracy.ci}{[0.786, 0.826]}
\@namedef{VJ@D_ceperm.raw.snli_ve.aurc_maxp}{0.077}
\@namedef{VJ@D_ceperm.raw.snli_ve.aurc_maxp.ci}{[0.064, 0.092]}
\@namedef{VJ@D_ceperm.raw.snli_ve.brier}{0.320}
\@namedef{VJ@D_ceperm.raw.snli_ve.brier.ci}{[0.289, 0.353]}
\@namedef{VJ@D_ceperm.raw.snli_ve.cov@0.05}{0.300}
\@namedef{VJ@D_ceperm.raw.snli_ve.cov@0.05.ci}{[0.280, 0.321]}
\@namedef{VJ@D_ceperm.raw.snli_ve.cov@0.05.pct}{30.0\%}
\@namedef{VJ@D_ceperm.raw.snli_ve.cov@0.1}{0.563}
\@namedef{VJ@D_ceperm.raw.snli_ve.cov@0.1.ci}{[0.542, 0.586]}
\@namedef{VJ@D_ceperm.raw.snli_ve.cov@0.1.pct}{56.3\%}
\@namedef{VJ@D_ceperm.raw.snli_ve.ece15}{0.126}
\@namedef{VJ@D_ceperm.raw.snli_ve.ece15.ci}{[0.109, 0.146]}
\@namedef{VJ@D_ceperm.raw.snli_ve.nll}{0.652}
\@namedef{VJ@D_ceperm.raw.snli_ve.nll.ci}{[0.580, 0.728]}
\@namedef{VJ@D_ceperm.raw.snli_ve.risk@0.05}{0.037}
\@namedef{VJ@D_ceperm.raw.snli_ve.risk@0.05.ci}{[0.023, 0.053]}
\@namedef{VJ@D_ceperm.raw.snli_ve.risk@0.05.pct}{3.7\%}
\@namedef{VJ@D_ceperm.raw.snli_ve.risk@0.1}{0.079}
\@namedef{VJ@D_ceperm.raw.snli_ve.risk@0.1.ci}{[0.062, 0.098]}
\@namedef{VJ@D_ceperm.raw.snli_ve.risk@0.1.pct}{7.9\%}
\@namedef{VJ@D_ceperm.raw.tallyqa_l.accuracy}{0.847}
\@namedef{VJ@D_ceperm.raw.tallyqa_l.accuracy.ci}{[0.834, 0.859]}
\@namedef{VJ@D_ceperm.raw.tallyqa_l.aurc_maxp}{0.034}
\@namedef{VJ@D_ceperm.raw.tallyqa_l.aurc_maxp.ci}{[0.029, 0.040]}
\@namedef{VJ@D_ceperm.raw.tallyqa_l.brier}{0.242}
\@namedef{VJ@D_ceperm.raw.tallyqa_l.brier.ci}{[0.223, 0.262]}
\@namedef{VJ@D_ceperm.raw.tallyqa_l.cov@0.05}{0.758}
\@namedef{VJ@D_ceperm.raw.tallyqa_l.cov@0.05.ci}{[0.742, 0.773]}
\@namedef{VJ@D_ceperm.raw.tallyqa_l.cov@0.05.pct}{75.8\%}
\@namedef{VJ@D_ceperm.raw.tallyqa_l.cov@0.1}{0.895}
\@namedef{VJ@D_ceperm.raw.tallyqa_l.cov@0.1.ci}{[0.885, 0.904]}
\@namedef{VJ@D_ceperm.raw.tallyqa_l.cov@0.1.pct}{89.5\%}
\@namedef{VJ@D_ceperm.raw.tallyqa_l.ece15}{0.093}
\@namedef{VJ@D_ceperm.raw.tallyqa_l.ece15.ci}{[0.084, 0.104]}
\@namedef{VJ@D_ceperm.raw.tallyqa_l.nll}{0.535}
\@namedef{VJ@D_ceperm.raw.tallyqa_l.nll.ci}{[0.488, 0.583]}
\@namedef{VJ@D_ceperm.raw.tallyqa_l.risk@0.05}{0.051}
\@namedef{VJ@D_ceperm.raw.tallyqa_l.risk@0.05.ci}{[0.044, 0.059]}
\@namedef{VJ@D_ceperm.raw.tallyqa_l.risk@0.05.pct}{5.1\%}
\@namedef{VJ@D_ceperm.raw.tallyqa_l.risk@0.1}{0.104}
\@namedef{VJ@D_ceperm.raw.tallyqa_l.risk@0.1.ci}{[0.094, 0.115]}
\@namedef{VJ@D_ceperm.raw.tallyqa_l.risk@0.1.pct}{10.4\%}
\@namedef{VJ@D_ceperm.raw.textvqa_k8.accuracy}{0.974}
\@namedef{VJ@D_ceperm.raw.textvqa_k8.accuracy.ci}{[0.966, 0.981]}
\@namedef{VJ@D_ceperm.raw.textvqa_k8.aurc_maxp}{0.001}
\@namedef{VJ@D_ceperm.raw.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@D_ceperm.raw.textvqa_k8.brier}{0.041}
\@namedef{VJ@D_ceperm.raw.textvqa_k8.brier.ci}{[0.030, 0.053]}
\@namedef{VJ@D_ceperm.raw.textvqa_k8.cov@0.05}{1.000}
\@namedef{VJ@D_ceperm.raw.textvqa_k8.cov@0.05.ci}{[1.000, 1.000]}
\@namedef{VJ@D_ceperm.raw.textvqa_k8.cov@0.05.pct}{100.0\%}
\@namedef{VJ@D_ceperm.raw.textvqa_k8.cov@0.1}{1.000}
\@namedef{VJ@D_ceperm.raw.textvqa_k8.cov@0.1.ci}{[1.000, 1.000]}
\@namedef{VJ@D_ceperm.raw.textvqa_k8.cov@0.1.pct}{100.0\%}
\@namedef{VJ@D_ceperm.raw.textvqa_k8.ece15}{0.016}
\@namedef{VJ@D_ceperm.raw.textvqa_k8.ece15.ci}{[0.012, 0.022]}
\@namedef{VJ@D_ceperm.raw.textvqa_k8.nll}{0.115}
\@namedef{VJ@D_ceperm.raw.textvqa_k8.nll.ci}{[0.077, 0.152]}
\@namedef{VJ@D_ceperm.raw.textvqa_k8.risk@0.05}{0.026}
\@namedef{VJ@D_ceperm.raw.textvqa_k8.risk@0.05.ci}{[0.019, 0.034]}
\@namedef{VJ@D_ceperm.raw.textvqa_k8.risk@0.05.pct}{2.6\%}
\@namedef{VJ@D_ceperm.raw.textvqa_k8.risk@0.1}{0.026}
\@namedef{VJ@D_ceperm.raw.textvqa_k8.risk@0.1.ci}{[0.019, 0.034]}
\@namedef{VJ@D_ceperm.raw.textvqa_k8.risk@0.1.pct}{2.6\%}
\@namedef{VJ@D_ceperm.ts_local.gqa_val.accuracy}{0.913}
\@namedef{VJ@D_ceperm.ts_local.gqa_val.accuracy.ci}{[0.906, 0.920]}
\@namedef{VJ@D_ceperm.ts_local.gqa_val.aurc_maxp}{0.016}
\@namedef{VJ@D_ceperm.ts_local.gqa_val.aurc_maxp.ci}{[0.013, 0.018]}
\@namedef{VJ@D_ceperm.ts_local.gqa_val.brier}{0.131}
\@namedef{VJ@D_ceperm.ts_local.gqa_val.brier.ci}{[0.120, 0.142]}
\@namedef{VJ@D_ceperm.ts_local.gqa_val.cov@0.05}{0.885}
\@namedef{VJ@D_ceperm.ts_local.gqa_val.cov@0.05.ci}{[0.877, 0.893]}
\@namedef{VJ@D_ceperm.ts_local.gqa_val.cov@0.05.pct}{88.5\%}
\@namedef{VJ@D_ceperm.ts_local.gqa_val.cov@0.1}{0.999}
\@namedef{VJ@D_ceperm.ts_local.gqa_val.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@D_ceperm.ts_local.gqa_val.cov@0.1.pct}{99.9\%}
\@namedef{VJ@D_ceperm.ts_local.gqa_val.ece15}{0.024}
\@namedef{VJ@D_ceperm.ts_local.gqa_val.ece15.ci}{[0.020, 0.030]}
\@namedef{VJ@D_ceperm.ts_local.gqa_val.nll}{0.237}
\@namedef{VJ@D_ceperm.ts_local.gqa_val.nll.ci}{[0.220, 0.254]}
\@namedef{VJ@D_ceperm.ts_local.gqa_val.risk@0.05}{0.046}
\@namedef{VJ@D_ceperm.ts_local.gqa_val.risk@0.05.ci}{[0.041, 0.052]}
\@namedef{VJ@D_ceperm.ts_local.gqa_val.risk@0.05.pct}{4.6\%}
\@namedef{VJ@D_ceperm.ts_local.gqa_val.risk@0.1}{0.087}
\@namedef{VJ@D_ceperm.ts_local.gqa_val.risk@0.1.ci}{[0.079, 0.094]}
\@namedef{VJ@D_ceperm.ts_local.gqa_val.risk@0.1.pct}{8.7\%}
\@namedef{VJ@D_ceperm.ts_local.macro.accuracy}{0.885}
\@namedef{VJ@D_ceperm.ts_local.macro.accuracy.ci}{[0.878, 0.891]}
\@namedef{VJ@D_ceperm.ts_local.macro.aurc_maxp}{0.031}
\@namedef{VJ@D_ceperm.ts_local.macro.aurc_maxp.ci}{[0.028, 0.035]}
\@namedef{VJ@D_ceperm.ts_local.macro.brier}{0.168}
\@namedef{VJ@D_ceperm.ts_local.macro.brier.ci}{[0.160, 0.176]}
\@namedef{VJ@D_ceperm.ts_local.macro.ece15}{0.031}
\@namedef{VJ@D_ceperm.ts_local.macro.ece15.ci}{[0.029, 0.037]}
\@namedef{VJ@D_ceperm.ts_local.macro.nll}{0.317}
\@namedef{VJ@D_ceperm.ts_local.macro.nll.ci}{[0.303, 0.331]}
\@namedef{VJ@D_ceperm.ts_local.snli_ve.accuracy}{0.807}
\@namedef{VJ@D_ceperm.ts_local.snli_ve.accuracy.ci}{[0.786, 0.826]}
\@namedef{VJ@D_ceperm.ts_local.snli_ve.aurc_maxp}{0.075}
\@namedef{VJ@D_ceperm.ts_local.snli_ve.aurc_maxp.ci}{[0.062, 0.090]}
\@namedef{VJ@D_ceperm.ts_local.snli_ve.brier}{0.285}
\@namedef{VJ@D_ceperm.ts_local.snli_ve.brier.ci}{[0.261, 0.311]}
\@namedef{VJ@D_ceperm.ts_local.snli_ve.cov@0.05}{0.293}
\@namedef{VJ@D_ceperm.ts_local.snli_ve.cov@0.05.ci}{[0.272, 0.314]}
\@namedef{VJ@D_ceperm.ts_local.snli_ve.cov@0.05.pct}{29.3\%}
\@namedef{VJ@D_ceperm.ts_local.snli_ve.cov@0.1}{0.599}
\@namedef{VJ@D_ceperm.ts_local.snli_ve.cov@0.1.ci}{[0.577, 0.621]}
\@namedef{VJ@D_ceperm.ts_local.snli_ve.cov@0.1.pct}{59.9\%}
\@namedef{VJ@D_ceperm.ts_local.snli_ve.ece15}{0.045}
\@namedef{VJ@D_ceperm.ts_local.snli_ve.ece15.ci}{[0.038, 0.061]}
\@namedef{VJ@D_ceperm.ts_local.snli_ve.nll}{0.509}
\@namedef{VJ@D_ceperm.ts_local.snli_ve.nll.ci}{[0.473, 0.547]}
\@namedef{VJ@D_ceperm.ts_local.snli_ve.risk@0.05}{0.033}
\@namedef{VJ@D_ceperm.ts_local.snli_ve.risk@0.05.ci}{[0.020, 0.049]}
\@namedef{VJ@D_ceperm.ts_local.snli_ve.risk@0.05.pct}{3.3\%}
\@namedef{VJ@D_ceperm.ts_local.snli_ve.risk@0.1}{0.082}
\@namedef{VJ@D_ceperm.ts_local.snli_ve.risk@0.1.ci}{[0.065, 0.100]}
\@namedef{VJ@D_ceperm.ts_local.snli_ve.risk@0.1.pct}{8.2\%}
\@namedef{VJ@D_ceperm.ts_local.tallyqa_l.accuracy}{0.847}
\@namedef{VJ@D_ceperm.ts_local.tallyqa_l.accuracy.ci}{[0.834, 0.859]}
\@namedef{VJ@D_ceperm.ts_local.tallyqa_l.aurc_maxp}{0.034}
\@namedef{VJ@D_ceperm.ts_local.tallyqa_l.aurc_maxp.ci}{[0.029, 0.039]}
\@namedef{VJ@D_ceperm.ts_local.tallyqa_l.brier}{0.217}
\@namedef{VJ@D_ceperm.ts_local.tallyqa_l.brier.ci}{[0.201, 0.234]}
\@namedef{VJ@D_ceperm.ts_local.tallyqa_l.cov@0.05}{0.758}
\@namedef{VJ@D_ceperm.ts_local.tallyqa_l.cov@0.05.ci}{[0.742, 0.773]}
\@namedef{VJ@D_ceperm.ts_local.tallyqa_l.cov@0.05.pct}{75.8\%}
\@namedef{VJ@D_ceperm.ts_local.tallyqa_l.cov@0.1}{0.897}
\@namedef{VJ@D_ceperm.ts_local.tallyqa_l.cov@0.1.ci}{[0.887, 0.906]}
\@namedef{VJ@D_ceperm.ts_local.tallyqa_l.cov@0.1.pct}{89.7\%}
\@namedef{VJ@D_ceperm.ts_local.tallyqa_l.ece15}{0.043}
\@namedef{VJ@D_ceperm.ts_local.tallyqa_l.ece15.ci}{[0.037, 0.053]}
\@namedef{VJ@D_ceperm.ts_local.tallyqa_l.nll}{0.429}
\@namedef{VJ@D_ceperm.ts_local.tallyqa_l.nll.ci}{[0.399, 0.460]}
\@namedef{VJ@D_ceperm.ts_local.tallyqa_l.risk@0.05}{0.051}
\@namedef{VJ@D_ceperm.ts_local.tallyqa_l.risk@0.05.ci}{[0.043, 0.059]}
\@namedef{VJ@D_ceperm.ts_local.tallyqa_l.risk@0.05.pct}{5.1\%}
\@namedef{VJ@D_ceperm.ts_local.tallyqa_l.risk@0.1}{0.104}
\@namedef{VJ@D_ceperm.ts_local.tallyqa_l.risk@0.1.ci}{[0.094, 0.115]}
\@namedef{VJ@D_ceperm.ts_local.tallyqa_l.risk@0.1.pct}{10.4\%}
\@namedef{VJ@D_ceperm.ts_local.textvqa_k8.accuracy}{0.974}
\@namedef{VJ@D_ceperm.ts_local.textvqa_k8.accuracy.ci}{[0.966, 0.981]}
\@namedef{VJ@D_ceperm.ts_local.textvqa_k8.aurc_maxp}{0.001}
\@namedef{VJ@D_ceperm.ts_local.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@D_ceperm.ts_local.textvqa_k8.brier}{0.039}
\@namedef{VJ@D_ceperm.ts_local.textvqa_k8.brier.ci}{[0.029, 0.050]}
\@namedef{VJ@D_ceperm.ts_local.textvqa_k8.cov@0.05}{1.000}
\@namedef{VJ@D_ceperm.ts_local.textvqa_k8.cov@0.05.ci}{[1.000, 1.000]}
\@namedef{VJ@D_ceperm.ts_local.textvqa_k8.cov@0.05.pct}{100.0\%}
\@namedef{VJ@D_ceperm.ts_local.textvqa_k8.cov@0.1}{1.000}
\@namedef{VJ@D_ceperm.ts_local.textvqa_k8.cov@0.1.ci}{[1.000, 1.000]}
\@namedef{VJ@D_ceperm.ts_local.textvqa_k8.cov@0.1.pct}{100.0\%}
\@namedef{VJ@D_ceperm.ts_local.textvqa_k8.ece15}{0.011}
\@namedef{VJ@D_ceperm.ts_local.textvqa_k8.ece15.ci}{[0.010, 0.017]}
\@namedef{VJ@D_ceperm.ts_local.textvqa_k8.nll}{0.094}
\@namedef{VJ@D_ceperm.ts_local.textvqa_k8.nll.ci}{[0.069, 0.119]}
\@namedef{VJ@D_ceperm.ts_local.textvqa_k8.risk@0.05}{0.026}
\@namedef{VJ@D_ceperm.ts_local.textvqa_k8.risk@0.05.ci}{[0.019, 0.034]}
\@namedef{VJ@D_ceperm.ts_local.textvqa_k8.risk@0.05.pct}{2.6\%}
\@namedef{VJ@D_ceperm.ts_local.textvqa_k8.risk@0.1}{0.026}
\@namedef{VJ@D_ceperm.ts_local.textvqa_k8.risk@0.1.ci}{[0.019, 0.034]}
\@namedef{VJ@D_ceperm.ts_local.textvqa_k8.risk@0.1.pct}{2.6\%}
\@namedef{VJ@D_ceperm.ts_transfer.gqa_val.accuracy}{0.913}
\@namedef{VJ@D_ceperm.ts_transfer.gqa_val.accuracy.ci}{[0.906, 0.920]}
\@namedef{VJ@D_ceperm.ts_transfer.gqa_val.aurc_maxp}{0.016}
\@namedef{VJ@D_ceperm.ts_transfer.gqa_val.aurc_maxp.ci}{[0.013, 0.018]}
\@namedef{VJ@D_ceperm.ts_transfer.gqa_val.brier}{0.132}
\@namedef{VJ@D_ceperm.ts_transfer.gqa_val.brier.ci}{[0.121, 0.142]}
\@namedef{VJ@D_ceperm.ts_transfer.gqa_val.cov@0.05}{0.884}
\@namedef{VJ@D_ceperm.ts_transfer.gqa_val.cov@0.05.ci}{[0.876, 0.893]}
\@namedef{VJ@D_ceperm.ts_transfer.gqa_val.cov@0.05.pct}{88.4\%}
\@namedef{VJ@D_ceperm.ts_transfer.gqa_val.cov@0.1}{0.999}
\@namedef{VJ@D_ceperm.ts_transfer.gqa_val.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@D_ceperm.ts_transfer.gqa_val.cov@0.1.pct}{99.9\%}
\@namedef{VJ@D_ceperm.ts_transfer.gqa_val.ece15}{0.023}
\@namedef{VJ@D_ceperm.ts_transfer.gqa_val.ece15.ci}{[0.019, 0.029]}
\@namedef{VJ@D_ceperm.ts_transfer.gqa_val.nll}{0.238}
\@namedef{VJ@D_ceperm.ts_transfer.gqa_val.nll.ci}{[0.220, 0.254]}
\@namedef{VJ@D_ceperm.ts_transfer.gqa_val.risk@0.05}{0.046}
\@namedef{VJ@D_ceperm.ts_transfer.gqa_val.risk@0.05.ci}{[0.040, 0.051]}
\@namedef{VJ@D_ceperm.ts_transfer.gqa_val.risk@0.05.pct}{4.6\%}
\@namedef{VJ@D_ceperm.ts_transfer.gqa_val.risk@0.1}{0.087}
\@namedef{VJ@D_ceperm.ts_transfer.gqa_val.risk@0.1.ci}{[0.079, 0.094]}
\@namedef{VJ@D_ceperm.ts_transfer.gqa_val.risk@0.1.pct}{8.7\%}
\@namedef{VJ@D_ceperm.ts_transfer.macro.accuracy}{0.885}
\@namedef{VJ@D_ceperm.ts_transfer.macro.accuracy.ci}{[0.878, 0.891]}
\@namedef{VJ@D_ceperm.ts_transfer.macro.aurc_maxp}{0.031}
\@namedef{VJ@D_ceperm.ts_transfer.macro.aurc_maxp.ci}{[0.028, 0.035]}
\@namedef{VJ@D_ceperm.ts_transfer.macro.brier}{0.170}
\@namedef{VJ@D_ceperm.ts_transfer.macro.brier.ci}{[0.162, 0.178]}
\@namedef{VJ@D_ceperm.ts_transfer.macro.ece15}{0.051}
\@namedef{VJ@D_ceperm.ts_transfer.macro.ece15.ci}{[0.050, 0.058]}
\@namedef{VJ@D_ceperm.ts_transfer.macro.nll}{0.337}
\@namedef{VJ@D_ceperm.ts_transfer.macro.nll.ci}{[0.325, 0.350]}
\@namedef{VJ@D_ceperm.ts_transfer.snli_ve.accuracy}{0.807}
\@namedef{VJ@D_ceperm.ts_transfer.snli_ve.accuracy.ci}{[0.786, 0.826]}
\@namedef{VJ@D_ceperm.ts_transfer.snli_ve.aurc_maxp}{0.074}
\@namedef{VJ@D_ceperm.ts_transfer.snli_ve.aurc_maxp.ci}{[0.062, 0.089]}
\@namedef{VJ@D_ceperm.ts_transfer.snli_ve.brier}{0.288}
\@namedef{VJ@D_ceperm.ts_transfer.snli_ve.brier.ci}{[0.266, 0.312]}
\@namedef{VJ@D_ceperm.ts_transfer.snli_ve.cov@0.05}{0.296}
\@namedef{VJ@D_ceperm.ts_transfer.snli_ve.cov@0.05.ci}{[0.275, 0.318]}
\@namedef{VJ@D_ceperm.ts_transfer.snli_ve.cov@0.05.pct}{29.6\%}
\@namedef{VJ@D_ceperm.ts_transfer.snli_ve.cov@0.1}{0.598}
\@namedef{VJ@D_ceperm.ts_transfer.snli_ve.cov@0.1.ci}{[0.576, 0.621]}
\@namedef{VJ@D_ceperm.ts_transfer.snli_ve.cov@0.1.pct}{59.8\%}
\@namedef{VJ@D_ceperm.ts_transfer.snli_ve.ece15}{0.066}
\@namedef{VJ@D_ceperm.ts_transfer.snli_ve.ece15.ci}{[0.058, 0.082]}
\@namedef{VJ@D_ceperm.ts_transfer.snli_ve.nll}{0.519}
\@namedef{VJ@D_ceperm.ts_transfer.snli_ve.nll.ci}{[0.486, 0.554]}
\@namedef{VJ@D_ceperm.ts_transfer.snli_ve.risk@0.05}{0.033}
\@namedef{VJ@D_ceperm.ts_transfer.snli_ve.risk@0.05.ci}{[0.020, 0.049]}
\@namedef{VJ@D_ceperm.ts_transfer.snli_ve.risk@0.05.pct}{3.3\%}
\@namedef{VJ@D_ceperm.ts_transfer.snli_ve.risk@0.1}{0.080}
\@namedef{VJ@D_ceperm.ts_transfer.snli_ve.risk@0.1.ci}{[0.064, 0.099]}
\@namedef{VJ@D_ceperm.ts_transfer.snli_ve.risk@0.1.pct}{8.0\%}
\@namedef{VJ@D_ceperm.ts_transfer.tallyqa_l.accuracy}{0.847}
\@namedef{VJ@D_ceperm.ts_transfer.tallyqa_l.accuracy.ci}{[0.834, 0.859]}
\@namedef{VJ@D_ceperm.ts_transfer.tallyqa_l.aurc_maxp}{0.034}
\@namedef{VJ@D_ceperm.ts_transfer.tallyqa_l.aurc_maxp.ci}{[0.029, 0.040]}
\@namedef{VJ@D_ceperm.ts_transfer.tallyqa_l.brier}{0.219}
\@namedef{VJ@D_ceperm.ts_transfer.tallyqa_l.brier.ci}{[0.205, 0.234]}
\@namedef{VJ@D_ceperm.ts_transfer.tallyqa_l.cov@0.05}{0.763}
\@namedef{VJ@D_ceperm.ts_transfer.tallyqa_l.cov@0.05.ci}{[0.746, 0.777]}
\@namedef{VJ@D_ceperm.ts_transfer.tallyqa_l.cov@0.05.pct}{76.3\%}
\@namedef{VJ@D_ceperm.ts_transfer.tallyqa_l.cov@0.1}{0.899}
\@namedef{VJ@D_ceperm.ts_transfer.tallyqa_l.cov@0.1.ci}{[0.889, 0.908]}
\@namedef{VJ@D_ceperm.ts_transfer.tallyqa_l.cov@0.1.pct}{89.9\%}
\@namedef{VJ@D_ceperm.ts_transfer.tallyqa_l.ece15}{0.070}
\@namedef{VJ@D_ceperm.ts_transfer.tallyqa_l.ece15.ci}{[0.067, 0.079]}
\@namedef{VJ@D_ceperm.ts_transfer.tallyqa_l.nll}{0.468}
\@namedef{VJ@D_ceperm.ts_transfer.tallyqa_l.nll.ci}{[0.443, 0.494]}
\@namedef{VJ@D_ceperm.ts_transfer.tallyqa_l.risk@0.05}{0.052}
\@namedef{VJ@D_ceperm.ts_transfer.tallyqa_l.risk@0.05.ci}{[0.044, 0.060]}
\@namedef{VJ@D_ceperm.ts_transfer.tallyqa_l.risk@0.05.pct}{5.2\%}
\@namedef{VJ@D_ceperm.ts_transfer.tallyqa_l.risk@0.1}{0.105}
\@namedef{VJ@D_ceperm.ts_transfer.tallyqa_l.risk@0.1.ci}{[0.095, 0.115]}
\@namedef{VJ@D_ceperm.ts_transfer.tallyqa_l.risk@0.1.pct}{10.5\%}
\@namedef{VJ@D_ceperm.ts_transfer.textvqa_k8.accuracy}{0.974}
\@namedef{VJ@D_ceperm.ts_transfer.textvqa_k8.accuracy.ci}{[0.966, 0.981]}
\@namedef{VJ@D_ceperm.ts_transfer.textvqa_k8.aurc_maxp}{0.001}
\@namedef{VJ@D_ceperm.ts_transfer.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@D_ceperm.ts_transfer.textvqa_k8.brier}{0.041}
\@namedef{VJ@D_ceperm.ts_transfer.textvqa_k8.brier.ci}{[0.032, 0.050]}
\@namedef{VJ@D_ceperm.ts_transfer.textvqa_k8.cov@0.05}{1.000}
\@namedef{VJ@D_ceperm.ts_transfer.textvqa_k8.cov@0.05.ci}{[1.000, 1.000]}
\@namedef{VJ@D_ceperm.ts_transfer.textvqa_k8.cov@0.05.pct}{100.0\%}
\@namedef{VJ@D_ceperm.ts_transfer.textvqa_k8.cov@0.1}{1.000}
\@namedef{VJ@D_ceperm.ts_transfer.textvqa_k8.cov@0.1.ci}{[1.000, 1.000]}
\@namedef{VJ@D_ceperm.ts_transfer.textvqa_k8.cov@0.1.pct}{100.0\%}
\@namedef{VJ@D_ceperm.ts_transfer.textvqa_k8.ece15}{0.046}
\@namedef{VJ@D_ceperm.ts_transfer.textvqa_k8.ece15.ci}{[0.045, 0.052]}
\@namedef{VJ@D_ceperm.ts_transfer.textvqa_k8.nll}{0.125}
\@namedef{VJ@D_ceperm.ts_transfer.textvqa_k8.nll.ci}{[0.105, 0.145]}
\@namedef{VJ@D_ceperm.ts_transfer.textvqa_k8.risk@0.05}{0.026}
\@namedef{VJ@D_ceperm.ts_transfer.textvqa_k8.risk@0.05.ci}{[0.019, 0.034]}
\@namedef{VJ@D_ceperm.ts_transfer.textvqa_k8.risk@0.05.pct}{2.6\%}
\@namedef{VJ@D_ceperm.ts_transfer.textvqa_k8.risk@0.1}{0.026}
\@namedef{VJ@D_ceperm.ts_transfer.textvqa_k8.risk@0.1.ci}{[0.019, 0.034]}
\@namedef{VJ@D_ceperm.ts_transfer.textvqa_k8.risk@0.1.pct}{2.6\%}
\@namedef{VJ@D_full.raw.gqa_val.accuracy}{0.913}
\@namedef{VJ@D_full.raw.gqa_val.accuracy.ci}{[0.906, 0.920]}
\@namedef{VJ@D_full.raw.gqa_val.aurc_maxp}{0.015}
\@namedef{VJ@D_full.raw.gqa_val.aurc_maxp.ci}{[0.013, 0.017]}
\@namedef{VJ@D_full.raw.gqa_val.brier}{0.154}
\@namedef{VJ@D_full.raw.gqa_val.brier.ci}{[0.141, 0.167]}
\@namedef{VJ@D_full.raw.gqa_val.cov@0.05}{0.894}
\@namedef{VJ@D_full.raw.gqa_val.cov@0.05.ci}{[0.887, 0.902]}
\@namedef{VJ@D_full.raw.gqa_val.cov@0.05.pct}{89.4\%}
\@namedef{VJ@D_full.raw.gqa_val.cov@0.1}{1.000}
\@namedef{VJ@D_full.raw.gqa_val.cov@0.1.ci}{[1.000, 1.000]}
\@namedef{VJ@D_full.raw.gqa_val.cov@0.1.pct}{100.0\%}
\@namedef{VJ@D_full.raw.gqa_val.ece15}{0.071}
\@namedef{VJ@D_full.raw.gqa_val.ece15.ci}{[0.065, 0.078]}
\@namedef{VJ@D_full.raw.gqa_val.nll}{0.405}
\@namedef{VJ@D_full.raw.gqa_val.nll.ci}{[0.365, 0.443]}
\@namedef{VJ@D_full.raw.gqa_val.risk@0.05}{0.047}
\@namedef{VJ@D_full.raw.gqa_val.risk@0.05.ci}{[0.042, 0.053]}
\@namedef{VJ@D_full.raw.gqa_val.risk@0.05.pct}{4.7\%}
\@namedef{VJ@D_full.raw.gqa_val.risk@0.1}{0.087}
\@namedef{VJ@D_full.raw.gqa_val.risk@0.1.ci}{[0.080, 0.094]}
\@namedef{VJ@D_full.raw.gqa_val.risk@0.1.pct}{8.7\%}
\@namedef{VJ@D_full.raw.macro.accuracy}{0.883}
\@namedef{VJ@D_full.raw.macro.accuracy.ci}{[0.877, 0.890]}
\@namedef{VJ@D_full.raw.macro.aurc_maxp}{0.032}
\@namedef{VJ@D_full.raw.macro.aurc_maxp.ci}{[0.028, 0.035]}
\@namedef{VJ@D_full.raw.macro.brier}{0.192}
\@namedef{VJ@D_full.raw.macro.brier.ci}{[0.182, 0.203]}
\@namedef{VJ@D_full.raw.macro.ece15}{0.079}
\@namedef{VJ@D_full.raw.macro.ece15.ci}{[0.075, 0.086]}
\@namedef{VJ@D_full.raw.macro.nll}{0.441}
\@namedef{VJ@D_full.raw.macro.nll.ci}{[0.413, 0.468]}
\@namedef{VJ@D_full.raw.snli_ve.accuracy}{0.802}
\@namedef{VJ@D_full.raw.snli_ve.accuracy.ci}{[0.782, 0.821]}
\@namedef{VJ@D_full.raw.snli_ve.aurc_maxp}{0.077}
\@namedef{VJ@D_full.raw.snli_ve.aurc_maxp.ci}{[0.064, 0.091]}
\@namedef{VJ@D_full.raw.snli_ve.brier}{0.325}
\@namedef{VJ@D_full.raw.snli_ve.brier.ci}{[0.291, 0.358]}
\@namedef{VJ@D_full.raw.snli_ve.cov@0.05}{0.285}
\@namedef{VJ@D_full.raw.snli_ve.cov@0.05.ci}{[0.265, 0.307]}
\@namedef{VJ@D_full.raw.snli_ve.cov@0.05.pct}{28.5\%}
\@namedef{VJ@D_full.raw.snli_ve.cov@0.1}{0.564}
\@namedef{VJ@D_full.raw.snli_ve.cov@0.1.ci}{[0.543, 0.586]}
\@namedef{VJ@D_full.raw.snli_ve.cov@0.1.pct}{56.4\%}
\@namedef{VJ@D_full.raw.snli_ve.ece15}{0.130}
\@namedef{VJ@D_full.raw.snli_ve.ece15.ci}{[0.113, 0.149]}
\@namedef{VJ@D_full.raw.snli_ve.nll}{0.674}
\@namedef{VJ@D_full.raw.snli_ve.nll.ci}{[0.598, 0.751]}
\@namedef{VJ@D_full.raw.snli_ve.risk@0.05}{0.038}
\@namedef{VJ@D_full.raw.snli_ve.risk@0.05.ci}{[0.022, 0.056]}
\@namedef{VJ@D_full.raw.snli_ve.risk@0.05.pct}{3.8\%}
\@namedef{VJ@D_full.raw.snli_ve.risk@0.1}{0.076}
\@namedef{VJ@D_full.raw.snli_ve.risk@0.1.ci}{[0.060, 0.094]}
\@namedef{VJ@D_full.raw.snli_ve.risk@0.1.pct}{7.6\%}
\@namedef{VJ@D_full.raw.tallyqa_l.accuracy}{0.845}
\@namedef{VJ@D_full.raw.tallyqa_l.accuracy.ci}{[0.832, 0.857]}
\@namedef{VJ@D_full.raw.tallyqa_l.aurc_maxp}{0.034}
\@namedef{VJ@D_full.raw.tallyqa_l.aurc_maxp.ci}{[0.029, 0.040]}
\@namedef{VJ@D_full.raw.tallyqa_l.brier}{0.247}
\@namedef{VJ@D_full.raw.tallyqa_l.brier.ci}{[0.228, 0.267]}
\@namedef{VJ@D_full.raw.tallyqa_l.cov@0.05}{0.762}
\@namedef{VJ@D_full.raw.tallyqa_l.cov@0.05.ci}{[0.747, 0.777]}
\@namedef{VJ@D_full.raw.tallyqa_l.cov@0.05.pct}{76.2\%}
\@namedef{VJ@D_full.raw.tallyqa_l.cov@0.1}{0.891}
\@namedef{VJ@D_full.raw.tallyqa_l.cov@0.1.ci}{[0.880, 0.900]}
\@namedef{VJ@D_full.raw.tallyqa_l.cov@0.1.pct}{89.1\%}
\@namedef{VJ@D_full.raw.tallyqa_l.ece15}{0.100}
\@namedef{VJ@D_full.raw.tallyqa_l.ece15.ci}{[0.090, 0.110]}
\@namedef{VJ@D_full.raw.tallyqa_l.nll}{0.564}
\@namedef{VJ@D_full.raw.tallyqa_l.nll.ci}{[0.515, 0.614]}
\@namedef{VJ@D_full.raw.tallyqa_l.risk@0.05}{0.053}
\@namedef{VJ@D_full.raw.tallyqa_l.risk@0.05.ci}{[0.046, 0.061]}
\@namedef{VJ@D_full.raw.tallyqa_l.risk@0.05.pct}{5.3\%}
\@namedef{VJ@D_full.raw.tallyqa_l.risk@0.1}{0.102}
\@namedef{VJ@D_full.raw.tallyqa_l.risk@0.1.ci}{[0.091, 0.112]}
\@namedef{VJ@D_full.raw.tallyqa_l.risk@0.1.pct}{10.2\%}
\@namedef{VJ@D_full.raw.textvqa_k8.accuracy}{0.974}
\@namedef{VJ@D_full.raw.textvqa_k8.accuracy.ci}{[0.966, 0.981]}
\@namedef{VJ@D_full.raw.textvqa_k8.aurc_maxp}{0.001}
\@namedef{VJ@D_full.raw.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@D_full.raw.textvqa_k8.brier}{0.042}
\@namedef{VJ@D_full.raw.textvqa_k8.brier.ci}{[0.031, 0.055]}
\@namedef{VJ@D_full.raw.textvqa_k8.cov@0.05}{1.000}
\@namedef{VJ@D_full.raw.textvqa_k8.cov@0.05.ci}{[1.000, 1.000]}
\@namedef{VJ@D_full.raw.textvqa_k8.cov@0.05.pct}{100.0\%}
\@namedef{VJ@D_full.raw.textvqa_k8.cov@0.1}{1.000}
\@namedef{VJ@D_full.raw.textvqa_k8.cov@0.1.ci}{[1.000, 1.000]}
\@namedef{VJ@D_full.raw.textvqa_k8.cov@0.1.pct}{100.0\%}
\@namedef{VJ@D_full.raw.textvqa_k8.ece15}{0.016}
\@namedef{VJ@D_full.raw.textvqa_k8.ece15.ci}{[0.012, 0.023]}
\@namedef{VJ@D_full.raw.textvqa_k8.nll}{0.122}
\@namedef{VJ@D_full.raw.textvqa_k8.nll.ci}{[0.082, 0.160]}
\@namedef{VJ@D_full.raw.textvqa_k8.risk@0.05}{0.026}
\@namedef{VJ@D_full.raw.textvqa_k8.risk@0.05.ci}{[0.019, 0.034]}
\@namedef{VJ@D_full.raw.textvqa_k8.risk@0.05.pct}{2.6\%}
\@namedef{VJ@D_full.raw.textvqa_k8.risk@0.1}{0.026}
\@namedef{VJ@D_full.raw.textvqa_k8.risk@0.1.ci}{[0.019, 0.034]}
\@namedef{VJ@D_full.raw.textvqa_k8.risk@0.1.pct}{2.6\%}
\@namedef{VJ@D_full.ts_local.gqa_val.accuracy}{0.913}
\@namedef{VJ@D_full.ts_local.gqa_val.accuracy.ci}{[0.906, 0.920]}
\@namedef{VJ@D_full.ts_local.gqa_val.aurc_maxp}{0.016}
\@namedef{VJ@D_full.ts_local.gqa_val.aurc_maxp.ci}{[0.013, 0.018]}
\@namedef{VJ@D_full.ts_local.gqa_val.brier}{0.131}
\@namedef{VJ@D_full.ts_local.gqa_val.brier.ci}{[0.121, 0.142]}
\@namedef{VJ@D_full.ts_local.gqa_val.cov@0.05}{0.891}
\@namedef{VJ@D_full.ts_local.gqa_val.cov@0.05.ci}{[0.883, 0.898]}
\@namedef{VJ@D_full.ts_local.gqa_val.cov@0.05.pct}{89.1\%}
\@namedef{VJ@D_full.ts_local.gqa_val.cov@0.1}{0.999}
\@namedef{VJ@D_full.ts_local.gqa_val.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@D_full.ts_local.gqa_val.cov@0.1.pct}{99.9\%}
\@namedef{VJ@D_full.ts_local.gqa_val.ece15}{0.025}
\@namedef{VJ@D_full.ts_local.gqa_val.ece15.ci}{[0.021, 0.031]}
\@namedef{VJ@D_full.ts_local.gqa_val.nll}{0.238}
\@namedef{VJ@D_full.ts_local.gqa_val.nll.ci}{[0.221, 0.255]}
\@namedef{VJ@D_full.ts_local.gqa_val.risk@0.05}{0.047}
\@namedef{VJ@D_full.ts_local.gqa_val.risk@0.05.ci}{[0.041, 0.053]}
\@namedef{VJ@D_full.ts_local.gqa_val.risk@0.05.pct}{4.7\%}
\@namedef{VJ@D_full.ts_local.gqa_val.risk@0.1}{0.087}
\@namedef{VJ@D_full.ts_local.gqa_val.risk@0.1.ci}{[0.079, 0.094]}
\@namedef{VJ@D_full.ts_local.gqa_val.risk@0.1.pct}{8.7\%}
\@namedef{VJ@D_full.ts_local.macro.accuracy}{0.883}
\@namedef{VJ@D_full.ts_local.macro.accuracy.ci}{[0.877, 0.890]}
\@namedef{VJ@D_full.ts_local.macro.aurc_maxp}{0.031}
\@namedef{VJ@D_full.ts_local.macro.aurc_maxp.ci}{[0.028, 0.035]}
\@namedef{VJ@D_full.ts_local.macro.brier}{0.169}
\@namedef{VJ@D_full.ts_local.macro.brier.ci}{[0.161, 0.177]}
\@namedef{VJ@D_full.ts_local.macro.ece15}{0.031}
\@namedef{VJ@D_full.ts_local.macro.ece15.ci}{[0.029, 0.037]}
\@namedef{VJ@D_full.ts_local.macro.nll}{0.320}
\@namedef{VJ@D_full.ts_local.macro.nll.ci}{[0.305, 0.334]}
\@namedef{VJ@D_full.ts_local.snli_ve.accuracy}{0.802}
\@namedef{VJ@D_full.ts_local.snli_ve.accuracy.ci}{[0.782, 0.821]}
\@namedef{VJ@D_full.ts_local.snli_ve.aurc_maxp}{0.075}
\@namedef{VJ@D_full.ts_local.snli_ve.aurc_maxp.ci}{[0.062, 0.089]}
\@namedef{VJ@D_full.ts_local.snli_ve.brier}{0.287}
\@namedef{VJ@D_full.ts_local.snli_ve.brier.ci}{[0.263, 0.311]}
\@namedef{VJ@D_full.ts_local.snli_ve.cov@0.05}{0.295}
\@namedef{VJ@D_full.ts_local.snli_ve.cov@0.05.ci}{[0.275, 0.317]}
\@namedef{VJ@D_full.ts_local.snli_ve.cov@0.05.pct}{29.5\%}
\@namedef{VJ@D_full.ts_local.snli_ve.cov@0.1}{0.573}
\@namedef{VJ@D_full.ts_local.snli_ve.cov@0.1.ci}{[0.551, 0.596]}
\@namedef{VJ@D_full.ts_local.snli_ve.cov@0.1.pct}{57.3\%}
\@namedef{VJ@D_full.ts_local.snli_ve.ece15}{0.043}
\@namedef{VJ@D_full.ts_local.snli_ve.ece15.ci}{[0.037, 0.060]}
\@namedef{VJ@D_full.ts_local.snli_ve.nll}{0.511}
\@namedef{VJ@D_full.ts_local.snli_ve.nll.ci}{[0.474, 0.548]}
\@namedef{VJ@D_full.ts_local.snli_ve.risk@0.05}{0.037}
\@namedef{VJ@D_full.ts_local.snli_ve.risk@0.05.ci}{[0.022, 0.055]}
\@namedef{VJ@D_full.ts_local.snli_ve.risk@0.05.pct}{3.7\%}
\@namedef{VJ@D_full.ts_local.snli_ve.risk@0.1}{0.072}
\@namedef{VJ@D_full.ts_local.snli_ve.risk@0.1.ci}{[0.057, 0.089]}
\@namedef{VJ@D_full.ts_local.snli_ve.risk@0.1.pct}{7.2\%}
\@namedef{VJ@D_full.ts_local.tallyqa_l.accuracy}{0.845}
\@namedef{VJ@D_full.ts_local.tallyqa_l.accuracy.ci}{[0.832, 0.857]}
\@namedef{VJ@D_full.ts_local.tallyqa_l.aurc_maxp}{0.034}
\@namedef{VJ@D_full.ts_local.tallyqa_l.aurc_maxp.ci}{[0.029, 0.039]}
\@namedef{VJ@D_full.ts_local.tallyqa_l.brier}{0.218}
\@namedef{VJ@D_full.ts_local.tallyqa_l.brier.ci}{[0.203, 0.236]}
\@namedef{VJ@D_full.ts_local.tallyqa_l.cov@0.05}{0.757}
\@namedef{VJ@D_full.ts_local.tallyqa_l.cov@0.05.ci}{[0.741, 0.772]}
\@namedef{VJ@D_full.ts_local.tallyqa_l.cov@0.05.pct}{75.7\%}
\@namedef{VJ@D_full.ts_local.tallyqa_l.cov@0.1}{0.891}
\@namedef{VJ@D_full.ts_local.tallyqa_l.cov@0.1.ci}{[0.881, 0.901]}
\@namedef{VJ@D_full.ts_local.tallyqa_l.cov@0.1.pct}{89.1\%}
\@namedef{VJ@D_full.ts_local.tallyqa_l.ece15}{0.043}
\@namedef{VJ@D_full.ts_local.tallyqa_l.ece15.ci}{[0.036, 0.053]}
\@namedef{VJ@D_full.ts_local.tallyqa_l.nll}{0.433}
\@namedef{VJ@D_full.ts_local.tallyqa_l.nll.ci}{[0.403, 0.464]}
\@namedef{VJ@D_full.ts_local.tallyqa_l.risk@0.05}{0.051}
\@namedef{VJ@D_full.ts_local.tallyqa_l.risk@0.05.ci}{[0.044, 0.058]}
\@namedef{VJ@D_full.ts_local.tallyqa_l.risk@0.05.pct}{5.1\%}
\@namedef{VJ@D_full.ts_local.tallyqa_l.risk@0.1}{0.101}
\@namedef{VJ@D_full.ts_local.tallyqa_l.risk@0.1.ci}{[0.092, 0.112]}
\@namedef{VJ@D_full.ts_local.tallyqa_l.risk@0.1.pct}{10.1\%}
\@namedef{VJ@D_full.ts_local.textvqa_k8.accuracy}{0.974}
\@namedef{VJ@D_full.ts_local.textvqa_k8.accuracy.ci}{[0.966, 0.981]}
\@namedef{VJ@D_full.ts_local.textvqa_k8.aurc_maxp}{0.001}
\@namedef{VJ@D_full.ts_local.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@D_full.ts_local.textvqa_k8.brier}{0.039}
\@namedef{VJ@D_full.ts_local.textvqa_k8.brier.ci}{[0.029, 0.050]}
\@namedef{VJ@D_full.ts_local.textvqa_k8.cov@0.05}{1.000}
\@namedef{VJ@D_full.ts_local.textvqa_k8.cov@0.05.ci}{[1.000, 1.000]}
\@namedef{VJ@D_full.ts_local.textvqa_k8.cov@0.05.pct}{100.0\%}
\@namedef{VJ@D_full.ts_local.textvqa_k8.cov@0.1}{1.000}
\@namedef{VJ@D_full.ts_local.textvqa_k8.cov@0.1.ci}{[1.000, 1.000]}
\@namedef{VJ@D_full.ts_local.textvqa_k8.cov@0.1.pct}{100.0\%}
\@namedef{VJ@D_full.ts_local.textvqa_k8.ece15}{0.012}
\@namedef{VJ@D_full.ts_local.textvqa_k8.ece15.ci}{[0.010, 0.018]}
\@namedef{VJ@D_full.ts_local.textvqa_k8.nll}{0.096}
\@namedef{VJ@D_full.ts_local.textvqa_k8.nll.ci}{[0.071, 0.122]}
\@namedef{VJ@D_full.ts_local.textvqa_k8.risk@0.05}{0.026}
\@namedef{VJ@D_full.ts_local.textvqa_k8.risk@0.05.ci}{[0.019, 0.034]}
\@namedef{VJ@D_full.ts_local.textvqa_k8.risk@0.05.pct}{2.6\%}
\@namedef{VJ@D_full.ts_local.textvqa_k8.risk@0.1}{0.026}
\@namedef{VJ@D_full.ts_local.textvqa_k8.risk@0.1.ci}{[0.019, 0.034]}
\@namedef{VJ@D_full.ts_local.textvqa_k8.risk@0.1.pct}{2.6\%}
\@namedef{VJ@D_full.ts_transfer.gqa_val.accuracy}{0.913}
\@namedef{VJ@D_full.ts_transfer.gqa_val.accuracy.ci}{[0.906, 0.920]}
\@namedef{VJ@D_full.ts_transfer.gqa_val.aurc_maxp}{0.016}
\@namedef{VJ@D_full.ts_transfer.gqa_val.aurc_maxp.ci}{[0.013, 0.018]}
\@namedef{VJ@D_full.ts_transfer.gqa_val.brier}{0.132}
\@namedef{VJ@D_full.ts_transfer.gqa_val.brier.ci}{[0.121, 0.142]}
\@namedef{VJ@D_full.ts_transfer.gqa_val.cov@0.05}{0.892}
\@namedef{VJ@D_full.ts_transfer.gqa_val.cov@0.05.ci}{[0.884, 0.900]}
\@namedef{VJ@D_full.ts_transfer.gqa_val.cov@0.05.pct}{89.2\%}
\@namedef{VJ@D_full.ts_transfer.gqa_val.cov@0.1}{0.999}
\@namedef{VJ@D_full.ts_transfer.gqa_val.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@D_full.ts_transfer.gqa_val.cov@0.1.pct}{99.9\%}
\@namedef{VJ@D_full.ts_transfer.gqa_val.ece15}{0.024}
\@namedef{VJ@D_full.ts_transfer.gqa_val.ece15.ci}{[0.020, 0.030]}
\@namedef{VJ@D_full.ts_transfer.gqa_val.nll}{0.238}
\@namedef{VJ@D_full.ts_transfer.gqa_val.nll.ci}{[0.220, 0.255]}
\@namedef{VJ@D_full.ts_transfer.gqa_val.risk@0.05}{0.047}
\@namedef{VJ@D_full.ts_transfer.gqa_val.risk@0.05.ci}{[0.042, 0.053]}
\@namedef{VJ@D_full.ts_transfer.gqa_val.risk@0.05.pct}{4.7\%}
\@namedef{VJ@D_full.ts_transfer.gqa_val.risk@0.1}{0.087}
\@namedef{VJ@D_full.ts_transfer.gqa_val.risk@0.1.ci}{[0.079, 0.094]}
\@namedef{VJ@D_full.ts_transfer.gqa_val.risk@0.1.pct}{8.7\%}
\@namedef{VJ@D_full.ts_transfer.macro.accuracy}{0.883}
\@namedef{VJ@D_full.ts_transfer.macro.accuracy.ci}{[0.877, 0.890]}
\@namedef{VJ@D_full.ts_transfer.macro.aurc_maxp}{0.031}
\@namedef{VJ@D_full.ts_transfer.macro.aurc_maxp.ci}{[0.028, 0.035]}
\@namedef{VJ@D_full.ts_transfer.macro.brier}{0.170}
\@namedef{VJ@D_full.ts_transfer.macro.brier.ci}{[0.163, 0.178]}
\@namedef{VJ@D_full.ts_transfer.macro.ece15}{0.049}
\@namedef{VJ@D_full.ts_transfer.macro.ece15.ci}{[0.049, 0.056]}
\@namedef{VJ@D_full.ts_transfer.macro.nll}{0.338}
\@namedef{VJ@D_full.ts_transfer.macro.nll.ci}{[0.325, 0.351]}
\@namedef{VJ@D_full.ts_transfer.snli_ve.accuracy}{0.802}
\@namedef{VJ@D_full.ts_transfer.snli_ve.accuracy.ci}{[0.782, 0.821]}
\@namedef{VJ@D_full.ts_transfer.snli_ve.aurc_maxp}{0.075}
\@namedef{VJ@D_full.ts_transfer.snli_ve.aurc_maxp.ci}{[0.062, 0.089]}
\@namedef{VJ@D_full.ts_transfer.snli_ve.brier}{0.289}
\@namedef{VJ@D_full.ts_transfer.snli_ve.brier.ci}{[0.266, 0.312]}
\@namedef{VJ@D_full.ts_transfer.snli_ve.cov@0.05}{0.288}
\@namedef{VJ@D_full.ts_transfer.snli_ve.cov@0.05.ci}{[0.268, 0.309]}
\@namedef{VJ@D_full.ts_transfer.snli_ve.cov@0.05.pct}{28.8\%}
\@namedef{VJ@D_full.ts_transfer.snli_ve.cov@0.1}{0.567}
\@namedef{VJ@D_full.ts_transfer.snli_ve.cov@0.1.ci}{[0.546, 0.591]}
\@namedef{VJ@D_full.ts_transfer.snli_ve.cov@0.1.pct}{56.7\%}
\@namedef{VJ@D_full.ts_transfer.snli_ve.ece15}{0.058}
\@namedef{VJ@D_full.ts_transfer.snli_ve.ece15.ci}{[0.051, 0.074]}
\@namedef{VJ@D_full.ts_transfer.snli_ve.nll}{0.519}
\@namedef{VJ@D_full.ts_transfer.snli_ve.nll.ci}{[0.484, 0.553]}
\@namedef{VJ@D_full.ts_transfer.snli_ve.risk@0.05}{0.035}
\@namedef{VJ@D_full.ts_transfer.snli_ve.risk@0.05.ci}{[0.021, 0.052]}
\@namedef{VJ@D_full.ts_transfer.snli_ve.risk@0.05.pct}{3.5\%}
\@namedef{VJ@D_full.ts_transfer.snli_ve.risk@0.1}{0.073}
\@namedef{VJ@D_full.ts_transfer.snli_ve.risk@0.1.ci}{[0.057, 0.090]}
\@namedef{VJ@D_full.ts_transfer.snli_ve.risk@0.1.pct}{7.3\%}
\@namedef{VJ@D_full.ts_transfer.tallyqa_l.accuracy}{0.845}
\@namedef{VJ@D_full.ts_transfer.tallyqa_l.accuracy.ci}{[0.832, 0.857]}
\@namedef{VJ@D_full.ts_transfer.tallyqa_l.aurc_maxp}{0.034}
\@namedef{VJ@D_full.ts_transfer.tallyqa_l.aurc_maxp.ci}{[0.029, 0.039]}
\@namedef{VJ@D_full.ts_transfer.tallyqa_l.brier}{0.220}
\@namedef{VJ@D_full.ts_transfer.tallyqa_l.brier.ci}{[0.206, 0.235]}
\@namedef{VJ@D_full.ts_transfer.tallyqa_l.cov@0.05}{0.758}
\@namedef{VJ@D_full.ts_transfer.tallyqa_l.cov@0.05.ci}{[0.742, 0.773]}
\@namedef{VJ@D_full.ts_transfer.tallyqa_l.cov@0.05.pct}{75.8\%}
\@namedef{VJ@D_full.ts_transfer.tallyqa_l.cov@0.1}{0.894}
\@namedef{VJ@D_full.ts_transfer.tallyqa_l.cov@0.1.ci}{[0.883, 0.903]}
\@namedef{VJ@D_full.ts_transfer.tallyqa_l.cov@0.1.pct}{89.4\%}
\@namedef{VJ@D_full.ts_transfer.tallyqa_l.ece15}{0.067}
\@namedef{VJ@D_full.ts_transfer.tallyqa_l.ece15.ci}{[0.064, 0.077]}
\@namedef{VJ@D_full.ts_transfer.tallyqa_l.nll}{0.469}
\@namedef{VJ@D_full.ts_transfer.tallyqa_l.nll.ci}{[0.444, 0.495]}
\@namedef{VJ@D_full.ts_transfer.tallyqa_l.risk@0.05}{0.052}
\@namedef{VJ@D_full.ts_transfer.tallyqa_l.risk@0.05.ci}{[0.045, 0.060]}
\@namedef{VJ@D_full.ts_transfer.tallyqa_l.risk@0.05.pct}{5.2\%}
\@namedef{VJ@D_full.ts_transfer.tallyqa_l.risk@0.1}{0.103}
\@namedef{VJ@D_full.ts_transfer.tallyqa_l.risk@0.1.ci}{[0.094, 0.114]}
\@namedef{VJ@D_full.ts_transfer.tallyqa_l.risk@0.1.pct}{10.3\%}
\@namedef{VJ@D_full.ts_transfer.textvqa_k8.accuracy}{0.974}
\@namedef{VJ@D_full.ts_transfer.textvqa_k8.accuracy.ci}{[0.966, 0.981]}
\@namedef{VJ@D_full.ts_transfer.textvqa_k8.aurc_maxp}{0.001}
\@namedef{VJ@D_full.ts_transfer.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@D_full.ts_transfer.textvqa_k8.brier}{0.041}
\@namedef{VJ@D_full.ts_transfer.textvqa_k8.brier.ci}{[0.032, 0.051]}
\@namedef{VJ@D_full.ts_transfer.textvqa_k8.cov@0.05}{1.000}
\@namedef{VJ@D_full.ts_transfer.textvqa_k8.cov@0.05.ci}{[1.000, 1.000]}
\@namedef{VJ@D_full.ts_transfer.textvqa_k8.cov@0.05.pct}{100.0\%}
\@namedef{VJ@D_full.ts_transfer.textvqa_k8.cov@0.1}{1.000}
\@namedef{VJ@D_full.ts_transfer.textvqa_k8.cov@0.1.ci}{[1.000, 1.000]}
\@namedef{VJ@D_full.ts_transfer.textvqa_k8.cov@0.1.pct}{100.0\%}
\@namedef{VJ@D_full.ts_transfer.textvqa_k8.ece15}{0.047}
\@namedef{VJ@D_full.ts_transfer.textvqa_k8.ece15.ci}{[0.047, 0.053]}
\@namedef{VJ@D_full.ts_transfer.textvqa_k8.nll}{0.128}
\@namedef{VJ@D_full.ts_transfer.textvqa_k8.nll.ci}{[0.108, 0.149]}
\@namedef{VJ@D_full.ts_transfer.textvqa_k8.risk@0.05}{0.026}
\@namedef{VJ@D_full.ts_transfer.textvqa_k8.risk@0.05.ci}{[0.019, 0.034]}
\@namedef{VJ@D_full.ts_transfer.textvqa_k8.risk@0.05.pct}{2.6\%}
\@namedef{VJ@D_full.ts_transfer.textvqa_k8.risk@0.1}{0.026}
\@namedef{VJ@D_full.ts_transfer.textvqa_k8.risk@0.1.ci}{[0.019, 0.034]}
\@namedef{VJ@D_full.ts_transfer.textvqa_k8.risk@0.1.pct}{2.6\%}
\@namedef{VJ@H2k.raw.gqa_val.accuracy}{0.919}
\@namedef{VJ@H2k.raw.gqa_val.accuracy.ci}{[0.913, 0.927]}
\@namedef{VJ@H2k.raw.gqa_val.aurc_maxp}{0.013}
\@namedef{VJ@H2k.raw.gqa_val.aurc_maxp.ci}{[0.011, 0.015]}
\@namedef{VJ@H2k.raw.gqa_val.brier}{0.134}
\@namedef{VJ@H2k.raw.gqa_val.brier.ci}{[0.123, 0.145]}
\@namedef{VJ@H2k.raw.gqa_val.cov@0.05}{0.889}
\@namedef{VJ@H2k.raw.gqa_val.cov@0.05.ci}{[0.880, 0.896]}
\@namedef{VJ@H2k.raw.gqa_val.cov@0.05.pct}{88.9\%}
\@namedef{VJ@H2k.raw.gqa_val.cov@0.1}{0.999}
\@namedef{VJ@H2k.raw.gqa_val.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@H2k.raw.gqa_val.cov@0.1.pct}{99.9\%}
\@namedef{VJ@H2k.raw.gqa_val.ece15}{0.053}
\@namedef{VJ@H2k.raw.gqa_val.ece15.ci}{[0.048, 0.059]}
\@namedef{VJ@H2k.raw.gqa_val.nll}{0.279}
\@namedef{VJ@H2k.raw.gqa_val.nll.ci}{[0.252, 0.306]}
\@namedef{VJ@H2k.raw.gqa_val.risk@0.05}{0.042}
\@namedef{VJ@H2k.raw.gqa_val.risk@0.05.ci}{[0.037, 0.047]}
\@namedef{VJ@H2k.raw.gqa_val.risk@0.05.pct}{4.2\%}
\@namedef{VJ@H2k.raw.gqa_val.risk@0.1}{0.080}
\@namedef{VJ@H2k.raw.gqa_val.risk@0.1.ci}{[0.073, 0.086]}
\@namedef{VJ@H2k.raw.gqa_val.risk@0.1.pct}{8.0\%}
\@namedef{VJ@H2k.raw.macro.accuracy}{0.884}
\@namedef{VJ@H2k.raw.macro.accuracy.ci}{[0.877, 0.890]}
\@namedef{VJ@H2k.raw.macro.aurc_maxp}{0.032}
\@namedef{VJ@H2k.raw.macro.aurc_maxp.ci}{[0.029, 0.036]}
\@namedef{VJ@H2k.raw.macro.brier}{0.187}
\@namedef{VJ@H2k.raw.macro.brier.ci}{[0.178, 0.198]}
\@namedef{VJ@H2k.raw.macro.ece15}{0.071}
\@namedef{VJ@H2k.raw.macro.ece15.ci}{[0.067, 0.077]}
\@namedef{VJ@H2k.raw.macro.nll}{0.408}
\@namedef{VJ@H2k.raw.macro.nll.ci}{[0.383, 0.433]}
\@namedef{VJ@H2k.raw.snli_ve.accuracy}{0.802}
\@namedef{VJ@H2k.raw.snli_ve.accuracy.ci}{[0.783, 0.820]}
\@namedef{VJ@H2k.raw.snli_ve.aurc_maxp}{0.082}
\@namedef{VJ@H2k.raw.snli_ve.aurc_maxp.ci}{[0.068, 0.097]}
\@namedef{VJ@H2k.raw.snli_ve.brier}{0.333}
\@namedef{VJ@H2k.raw.snli_ve.brier.ci}{[0.302, 0.367]}
\@namedef{VJ@H2k.raw.snli_ve.cov@0.05}{0.252}
\@namedef{VJ@H2k.raw.snli_ve.cov@0.05.ci}{[0.233, 0.270]}
\@namedef{VJ@H2k.raw.snli_ve.cov@0.05.pct}{25.2\%}
\@namedef{VJ@H2k.raw.snli_ve.cov@0.1}{0.514}
\@namedef{VJ@H2k.raw.snli_ve.cov@0.1.ci}{[0.490, 0.538]}
\@namedef{VJ@H2k.raw.snli_ve.cov@0.1.pct}{51.4\%}
\@namedef{VJ@H2k.raw.snli_ve.ece15}{0.134}
\@namedef{VJ@H2k.raw.snli_ve.ece15.ci}{[0.121, 0.154]}
\@namedef{VJ@H2k.raw.snli_ve.nll}{0.736}
\@namedef{VJ@H2k.raw.snli_ve.nll.ci}{[0.657, 0.814]}
\@namedef{VJ@H2k.raw.snli_ve.risk@0.05}{0.041}
\@namedef{VJ@H2k.raw.snli_ve.risk@0.05.ci}{[0.025, 0.058]}
\@namedef{VJ@H2k.raw.snli_ve.risk@0.05.pct}{4.1\%}
\@namedef{VJ@H2k.raw.snli_ve.risk@0.1}{0.072}
\@namedef{VJ@H2k.raw.snli_ve.risk@0.1.ci}{[0.056, 0.089]}
\@namedef{VJ@H2k.raw.snli_ve.risk@0.1.pct}{7.2\%}
\@namedef{VJ@H2k.raw.tallyqa_l.accuracy}{0.841}
\@namedef{VJ@H2k.raw.tallyqa_l.accuracy.ci}{[0.828, 0.853]}
\@namedef{VJ@H2k.raw.tallyqa_l.aurc_maxp}{0.034}
\@namedef{VJ@H2k.raw.tallyqa_l.aurc_maxp.ci}{[0.029, 0.039]}
\@namedef{VJ@H2k.raw.tallyqa_l.brier}{0.240}
\@namedef{VJ@H2k.raw.tallyqa_l.brier.ci}{[0.223, 0.259]}
\@namedef{VJ@H2k.raw.tallyqa_l.cov@0.05}{0.754}
\@namedef{VJ@H2k.raw.tallyqa_l.cov@0.05.ci}{[0.739, 0.769]}
\@namedef{VJ@H2k.raw.tallyqa_l.cov@0.05.pct}{75.4\%}
\@namedef{VJ@H2k.raw.tallyqa_l.cov@0.1}{0.883}
\@namedef{VJ@H2k.raw.tallyqa_l.cov@0.1.ci}{[0.873, 0.892]}
\@namedef{VJ@H2k.raw.tallyqa_l.cov@0.1.pct}{88.3\%}
\@namedef{VJ@H2k.raw.tallyqa_l.ece15}{0.081}
\@namedef{VJ@H2k.raw.tallyqa_l.ece15.ci}{[0.073, 0.092]}
\@namedef{VJ@H2k.raw.tallyqa_l.nll}{0.505}
\@namedef{VJ@H2k.raw.tallyqa_l.nll.ci}{[0.464, 0.549]}
\@namedef{VJ@H2k.raw.tallyqa_l.risk@0.05}{0.053}
\@namedef{VJ@H2k.raw.tallyqa_l.risk@0.05.ci}{[0.045, 0.061]}
\@namedef{VJ@H2k.raw.tallyqa_l.risk@0.05.pct}{5.3\%}
\@namedef{VJ@H2k.raw.tallyqa_l.risk@0.1}{0.104}
\@namedef{VJ@H2k.raw.tallyqa_l.risk@0.1.ci}{[0.094, 0.114]}
\@namedef{VJ@H2k.raw.tallyqa_l.risk@0.1.pct}{10.4\%}
\@namedef{VJ@H2k.raw.textvqa_k8.accuracy}{0.973}
\@namedef{VJ@H2k.raw.textvqa_k8.accuracy.ci}{[0.966, 0.980]}
\@namedef{VJ@H2k.raw.textvqa_k8.aurc_maxp}{0.001}
\@namedef{VJ@H2k.raw.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@H2k.raw.textvqa_k8.brier}{0.042}
\@namedef{VJ@H2k.raw.textvqa_k8.brier.ci}{[0.031, 0.054]}
\@namedef{VJ@H2k.raw.textvqa_k8.cov@0.05}{0.999}
\@namedef{VJ@H2k.raw.textvqa_k8.cov@0.05.ci}{[0.998, 1.000]}
\@namedef{VJ@H2k.raw.textvqa_k8.cov@0.05.pct}{99.9\%}
\@namedef{VJ@H2k.raw.textvqa_k8.cov@0.1}{0.999}
\@namedef{VJ@H2k.raw.textvqa_k8.cov@0.1.ci}{[0.998, 1.000]}
\@namedef{VJ@H2k.raw.textvqa_k8.cov@0.1.pct}{99.9\%}
\@namedef{VJ@H2k.raw.textvqa_k8.ece15}{0.014}
\@namedef{VJ@H2k.raw.textvqa_k8.ece15.ci}{[0.011, 0.020]}
\@namedef{VJ@H2k.raw.textvqa_k8.nll}{0.111}
\@namedef{VJ@H2k.raw.textvqa_k8.nll.ci}{[0.079, 0.145]}
\@namedef{VJ@H2k.raw.textvqa_k8.risk@0.05}{0.026}
\@namedef{VJ@H2k.raw.textvqa_k8.risk@0.05.ci}{[0.019, 0.033]}
\@namedef{VJ@H2k.raw.textvqa_k8.risk@0.05.pct}{2.6\%}
\@namedef{VJ@H2k.raw.textvqa_k8.risk@0.1}{0.026}
\@namedef{VJ@H2k.raw.textvqa_k8.risk@0.1.ci}{[0.019, 0.033]}
\@namedef{VJ@H2k.raw.textvqa_k8.risk@0.1.pct}{2.6\%}
\@namedef{VJ@H2k.ts_local.gqa_val.accuracy}{0.919}
\@namedef{VJ@H2k.ts_local.gqa_val.accuracy.ci}{[0.913, 0.927]}
\@namedef{VJ@H2k.ts_local.gqa_val.aurc_maxp}{0.013}
\@namedef{VJ@H2k.ts_local.gqa_val.aurc_maxp.ci}{[0.011, 0.015]}
\@namedef{VJ@H2k.ts_local.gqa_val.brier}{0.121}
\@namedef{VJ@H2k.ts_local.gqa_val.brier.ci}{[0.112, 0.131]}
\@namedef{VJ@H2k.ts_local.gqa_val.cov@0.05}{0.884}
\@namedef{VJ@H2k.ts_local.gqa_val.cov@0.05.ci}{[0.876, 0.892]}
\@namedef{VJ@H2k.ts_local.gqa_val.cov@0.05.pct}{88.4\%}
\@namedef{VJ@H2k.ts_local.gqa_val.cov@0.1}{0.999}
\@namedef{VJ@H2k.ts_local.gqa_val.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@H2k.ts_local.gqa_val.cov@0.1.pct}{99.9\%}
\@namedef{VJ@H2k.ts_local.gqa_val.ece15}{0.020}
\@namedef{VJ@H2k.ts_local.gqa_val.ece15.ci}{[0.017, 0.026]}
\@namedef{VJ@H2k.ts_local.gqa_val.nll}{0.224}
\@namedef{VJ@H2k.ts_local.gqa_val.nll.ci}{[0.208, 0.240]}
\@namedef{VJ@H2k.ts_local.gqa_val.risk@0.05}{0.041}
\@namedef{VJ@H2k.ts_local.gqa_val.risk@0.05.ci}{[0.036, 0.046]}
\@namedef{VJ@H2k.ts_local.gqa_val.risk@0.05.pct}{4.1\%}
\@namedef{VJ@H2k.ts_local.gqa_val.risk@0.1}{0.080}
\@namedef{VJ@H2k.ts_local.gqa_val.risk@0.1.ci}{[0.073, 0.087]}
\@namedef{VJ@H2k.ts_local.gqa_val.risk@0.1.pct}{8.0\%}
\@namedef{VJ@H2k.ts_local.macro.accuracy}{0.884}
\@namedef{VJ@H2k.ts_local.macro.accuracy.ci}{[0.877, 0.890]}
\@namedef{VJ@H2k.ts_local.macro.aurc_maxp}{0.032}
\@namedef{VJ@H2k.ts_local.macro.aurc_maxp.ci}{[0.029, 0.036]}
\@namedef{VJ@H2k.ts_local.macro.brier}{0.170}
\@namedef{VJ@H2k.ts_local.macro.brier.ci}{[0.162, 0.178]}
\@namedef{VJ@H2k.ts_local.macro.ece15}{0.028}
\@namedef{VJ@H2k.ts_local.macro.ece15.ci}{[0.027, 0.034]}
\@namedef{VJ@H2k.ts_local.macro.nll}{0.332}
\@namedef{VJ@H2k.ts_local.macro.nll.ci}{[0.318, 0.346]}
\@namedef{VJ@H2k.ts_local.snli_ve.accuracy}{0.802}
\@namedef{VJ@H2k.ts_local.snli_ve.accuracy.ci}{[0.783, 0.820]}
\@namedef{VJ@H2k.ts_local.snli_ve.aurc_maxp}{0.082}
\@namedef{VJ@H2k.ts_local.snli_ve.aurc_maxp.ci}{[0.068, 0.097]}
\@namedef{VJ@H2k.ts_local.snli_ve.brier}{0.297}
\@namedef{VJ@H2k.ts_local.snli_ve.brier.ci}{[0.273, 0.320]}
\@namedef{VJ@H2k.ts_local.snli_ve.cov@0.05}{0.253}
\@namedef{VJ@H2k.ts_local.snli_ve.cov@0.05.ci}{[0.234, 0.271]}
\@namedef{VJ@H2k.ts_local.snli_ve.cov@0.05.pct}{25.3\%}
\@namedef{VJ@H2k.ts_local.snli_ve.cov@0.1}{0.508}
\@namedef{VJ@H2k.ts_local.snli_ve.cov@0.1.ci}{[0.485, 0.532]}
\@namedef{VJ@H2k.ts_local.snli_ve.cov@0.1.pct}{50.8\%}
\@namedef{VJ@H2k.ts_local.snli_ve.ece15}{0.041}
\@namedef{VJ@H2k.ts_local.snli_ve.ece15.ci}{[0.037, 0.059]}
\@namedef{VJ@H2k.ts_local.snli_ve.nll}{0.551}
\@namedef{VJ@H2k.ts_local.snli_ve.nll.ci}{[0.514, 0.587]}
\@namedef{VJ@H2k.ts_local.snli_ve.risk@0.05}{0.041}
\@namedef{VJ@H2k.ts_local.snli_ve.risk@0.05.ci}{[0.025, 0.058]}
\@namedef{VJ@H2k.ts_local.snli_ve.risk@0.05.pct}{4.1\%}
\@namedef{VJ@H2k.ts_local.snli_ve.risk@0.1}{0.072}
\@namedef{VJ@H2k.ts_local.snli_ve.risk@0.1.ci}{[0.056, 0.088]}
\@namedef{VJ@H2k.ts_local.snli_ve.risk@0.1.pct}{7.2\%}
\@namedef{VJ@H2k.ts_local.tallyqa_l.accuracy}{0.841}
\@namedef{VJ@H2k.ts_local.tallyqa_l.accuracy.ci}{[0.828, 0.853]}
\@namedef{VJ@H2k.ts_local.tallyqa_l.aurc_maxp}{0.033}
\@namedef{VJ@H2k.ts_local.tallyqa_l.aurc_maxp.ci}{[0.029, 0.039]}
\@namedef{VJ@H2k.ts_local.tallyqa_l.brier}{0.223}
\@namedef{VJ@H2k.ts_local.tallyqa_l.brier.ci}{[0.207, 0.240]}
\@namedef{VJ@H2k.ts_local.tallyqa_l.cov@0.05}{0.755}
\@namedef{VJ@H2k.ts_local.tallyqa_l.cov@0.05.ci}{[0.739, 0.769]}
\@namedef{VJ@H2k.ts_local.tallyqa_l.cov@0.05.pct}{75.5\%}
\@namedef{VJ@H2k.ts_local.tallyqa_l.cov@0.1}{0.883}
\@namedef{VJ@H2k.ts_local.tallyqa_l.cov@0.1.ci}{[0.874, 0.892]}
\@namedef{VJ@H2k.ts_local.tallyqa_l.cov@0.1.pct}{88.3\%}
\@namedef{VJ@H2k.ts_local.tallyqa_l.ece15}{0.039}
\@namedef{VJ@H2k.ts_local.tallyqa_l.ece15.ci}{[0.033, 0.049]}
\@namedef{VJ@H2k.ts_local.tallyqa_l.nll}{0.454}
\@namedef{VJ@H2k.ts_local.tallyqa_l.nll.ci}{[0.423, 0.488]}
\@namedef{VJ@H2k.ts_local.tallyqa_l.risk@0.05}{0.053}
\@namedef{VJ@H2k.ts_local.tallyqa_l.risk@0.05.ci}{[0.046, 0.061]}
\@namedef{VJ@H2k.ts_local.tallyqa_l.risk@0.05.pct}{5.3\%}
\@namedef{VJ@H2k.ts_local.tallyqa_l.risk@0.1}{0.104}
\@namedef{VJ@H2k.ts_local.tallyqa_l.risk@0.1.ci}{[0.094, 0.114]}
\@namedef{VJ@H2k.ts_local.tallyqa_l.risk@0.1.pct}{10.4\%}
\@namedef{VJ@H2k.ts_local.textvqa_k8.accuracy}{0.973}
\@namedef{VJ@H2k.ts_local.textvqa_k8.accuracy.ci}{[0.966, 0.980]}
\@namedef{VJ@H2k.ts_local.textvqa_k8.aurc_maxp}{0.001}
\@namedef{VJ@H2k.ts_local.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@H2k.ts_local.textvqa_k8.brier}{0.040}
\@namedef{VJ@H2k.ts_local.textvqa_k8.brier.ci}{[0.030, 0.051]}
\@namedef{VJ@H2k.ts_local.textvqa_k8.cov@0.05}{0.999}
\@namedef{VJ@H2k.ts_local.textvqa_k8.cov@0.05.ci}{[0.998, 1.000]}
\@namedef{VJ@H2k.ts_local.textvqa_k8.cov@0.05.pct}{99.9\%}
\@namedef{VJ@H2k.ts_local.textvqa_k8.cov@0.1}{0.999}
\@namedef{VJ@H2k.ts_local.textvqa_k8.cov@0.1.ci}{[0.998, 1.000]}
\@namedef{VJ@H2k.ts_local.textvqa_k8.cov@0.1.pct}{99.9\%}
\@namedef{VJ@H2k.ts_local.textvqa_k8.ece15}{0.012}
\@namedef{VJ@H2k.ts_local.textvqa_k8.ece15.ci}{[0.010, 0.017]}
\@namedef{VJ@H2k.ts_local.textvqa_k8.nll}{0.100}
\@namedef{VJ@H2k.ts_local.textvqa_k8.nll.ci}{[0.075, 0.127]}
\@namedef{VJ@H2k.ts_local.textvqa_k8.risk@0.05}{0.026}
\@namedef{VJ@H2k.ts_local.textvqa_k8.risk@0.05.ci}{[0.019, 0.033]}
\@namedef{VJ@H2k.ts_local.textvqa_k8.risk@0.05.pct}{2.6\%}
\@namedef{VJ@H2k.ts_local.textvqa_k8.risk@0.1}{0.026}
\@namedef{VJ@H2k.ts_local.textvqa_k8.risk@0.1.ci}{[0.019, 0.033]}
\@namedef{VJ@H2k.ts_local.textvqa_k8.risk@0.1.pct}{2.6\%}
\@namedef{VJ@H2k.ts_transfer.gqa_val.accuracy}{0.919}
\@namedef{VJ@H2k.ts_transfer.gqa_val.accuracy.ci}{[0.913, 0.927]}
\@namedef{VJ@H2k.ts_transfer.gqa_val.aurc_maxp}{0.013}
\@namedef{VJ@H2k.ts_transfer.gqa_val.aurc_maxp.ci}{[0.011, 0.015]}
\@namedef{VJ@H2k.ts_transfer.gqa_val.brier}{0.121}
\@namedef{VJ@H2k.ts_transfer.gqa_val.brier.ci}{[0.112, 0.130]}
\@namedef{VJ@H2k.ts_transfer.gqa_val.cov@0.05}{0.887}
\@namedef{VJ@H2k.ts_transfer.gqa_val.cov@0.05.ci}{[0.878, 0.894]}
\@namedef{VJ@H2k.ts_transfer.gqa_val.cov@0.05.pct}{88.7\%}
\@namedef{VJ@H2k.ts_transfer.gqa_val.cov@0.1}{0.999}
\@namedef{VJ@H2k.ts_transfer.gqa_val.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@H2k.ts_transfer.gqa_val.cov@0.1.pct}{99.9\%}
\@namedef{VJ@H2k.ts_transfer.gqa_val.ece15}{0.020}
\@namedef{VJ@H2k.ts_transfer.gqa_val.ece15.ci}{[0.019, 0.027]}
\@namedef{VJ@H2k.ts_transfer.gqa_val.nll}{0.227}
\@namedef{VJ@H2k.ts_transfer.gqa_val.nll.ci}{[0.211, 0.242]}
\@namedef{VJ@H2k.ts_transfer.gqa_val.risk@0.05}{0.042}
\@namedef{VJ@H2k.ts_transfer.gqa_val.risk@0.05.ci}{[0.037, 0.047]}
\@namedef{VJ@H2k.ts_transfer.gqa_val.risk@0.05.pct}{4.2\%}
\@namedef{VJ@H2k.ts_transfer.gqa_val.risk@0.1}{0.080}
\@namedef{VJ@H2k.ts_transfer.gqa_val.risk@0.1.ci}{[0.073, 0.087]}
\@namedef{VJ@H2k.ts_transfer.gqa_val.risk@0.1.pct}{8.0\%}
\@namedef{VJ@H2k.ts_transfer.macro.accuracy}{0.884}
\@namedef{VJ@H2k.ts_transfer.macro.accuracy.ci}{[0.877, 0.890]}
\@namedef{VJ@H2k.ts_transfer.macro.aurc_maxp}{0.032}
\@namedef{VJ@H2k.ts_transfer.macro.aurc_maxp.ci}{[0.029, 0.036]}
\@namedef{VJ@H2k.ts_transfer.macro.brier}{0.171}
\@namedef{VJ@H2k.ts_transfer.macro.brier.ci}{[0.163, 0.179]}
\@namedef{VJ@H2k.ts_transfer.macro.ece15}{0.041}
\@namedef{VJ@H2k.ts_transfer.macro.ece15.ci}{[0.041, 0.048]}
\@namedef{VJ@H2k.ts_transfer.macro.nll}{0.348}
\@namedef{VJ@H2k.ts_transfer.macro.nll.ci}{[0.334, 0.362]}
\@namedef{VJ@H2k.ts_transfer.snli_ve.accuracy}{0.802}
\@namedef{VJ@H2k.ts_transfer.snli_ve.accuracy.ci}{[0.783, 0.820]}
\@namedef{VJ@H2k.ts_transfer.snli_ve.aurc_maxp}{0.082}
\@namedef{VJ@H2k.ts_transfer.snli_ve.aurc_maxp.ci}{[0.068, 0.097]}
\@namedef{VJ@H2k.ts_transfer.snli_ve.brier}{0.297}
\@namedef{VJ@H2k.ts_transfer.snli_ve.brier.ci}{[0.271, 0.322]}
\@namedef{VJ@H2k.ts_transfer.snli_ve.cov@0.05}{0.254}
\@namedef{VJ@H2k.ts_transfer.snli_ve.cov@0.05.ci}{[0.235, 0.272]}
\@namedef{VJ@H2k.ts_transfer.snli_ve.cov@0.05.pct}{25.4\%}
\@namedef{VJ@H2k.ts_transfer.snli_ve.cov@0.1}{0.509}
\@namedef{VJ@H2k.ts_transfer.snli_ve.cov@0.1.ci}{[0.486, 0.532]}
\@namedef{VJ@H2k.ts_transfer.snli_ve.cov@0.1.pct}{50.9\%}
\@namedef{VJ@H2k.ts_transfer.snli_ve.ece15}{0.039}
\@namedef{VJ@H2k.ts_transfer.snli_ve.ece15.ci}{[0.035, 0.057]}
\@namedef{VJ@H2k.ts_transfer.snli_ve.nll}{0.548}
\@namedef{VJ@H2k.ts_transfer.snli_ve.nll.ci}{[0.506, 0.589]}
\@namedef{VJ@H2k.ts_transfer.snli_ve.risk@0.05}{0.040}
\@namedef{VJ@H2k.ts_transfer.snli_ve.risk@0.05.ci}{[0.025, 0.058]}
\@namedef{VJ@H2k.ts_transfer.snli_ve.risk@0.05.pct}{4.0\%}
\@namedef{VJ@H2k.ts_transfer.snli_ve.risk@0.1}{0.072}
\@namedef{VJ@H2k.ts_transfer.snli_ve.risk@0.1.ci}{[0.056, 0.088]}
\@namedef{VJ@H2k.ts_transfer.snli_ve.risk@0.1.pct}{7.2\%}
\@namedef{VJ@H2k.ts_transfer.tallyqa_l.accuracy}{0.841}
\@namedef{VJ@H2k.ts_transfer.tallyqa_l.accuracy.ci}{[0.828, 0.853]}
\@namedef{VJ@H2k.ts_transfer.tallyqa_l.aurc_maxp}{0.033}
\@namedef{VJ@H2k.ts_transfer.tallyqa_l.aurc_maxp.ci}{[0.029, 0.039]}
\@namedef{VJ@H2k.ts_transfer.tallyqa_l.brier}{0.225}
\@namedef{VJ@H2k.ts_transfer.tallyqa_l.brier.ci}{[0.211, 0.240]}
\@namedef{VJ@H2k.ts_transfer.tallyqa_l.cov@0.05}{0.754}
\@namedef{VJ@H2k.ts_transfer.tallyqa_l.cov@0.05.ci}{[0.739, 0.769]}
\@namedef{VJ@H2k.ts_transfer.tallyqa_l.cov@0.05.pct}{75.4\%}
\@namedef{VJ@H2k.ts_transfer.tallyqa_l.cov@0.1}{0.886}
\@namedef{VJ@H2k.ts_transfer.tallyqa_l.cov@0.1.ci}{[0.876, 0.895]}
\@namedef{VJ@H2k.ts_transfer.tallyqa_l.cov@0.1.pct}{88.6\%}
\@namedef{VJ@H2k.ts_transfer.tallyqa_l.ece15}{0.065}
\@namedef{VJ@H2k.ts_transfer.tallyqa_l.ece15.ci}{[0.061, 0.075]}
\@namedef{VJ@H2k.ts_transfer.tallyqa_l.nll}{0.492}
\@namedef{VJ@H2k.ts_transfer.tallyqa_l.nll.ci}{[0.466, 0.519]}
\@namedef{VJ@H2k.ts_transfer.tallyqa_l.risk@0.05}{0.053}
\@namedef{VJ@H2k.ts_transfer.tallyqa_l.risk@0.05.ci}{[0.046, 0.061]}
\@namedef{VJ@H2k.ts_transfer.tallyqa_l.risk@0.05.pct}{5.3\%}
\@namedef{VJ@H2k.ts_transfer.tallyqa_l.risk@0.1}{0.104}
\@namedef{VJ@H2k.ts_transfer.tallyqa_l.risk@0.1.ci}{[0.094, 0.115]}
\@namedef{VJ@H2k.ts_transfer.tallyqa_l.risk@0.1.pct}{10.4\%}
\@namedef{VJ@H2k.ts_transfer.textvqa_k8.accuracy}{0.973}
\@namedef{VJ@H2k.ts_transfer.textvqa_k8.accuracy.ci}{[0.966, 0.980]}
\@namedef{VJ@H2k.ts_transfer.textvqa_k8.aurc_maxp}{0.001}
\@namedef{VJ@H2k.ts_transfer.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@H2k.ts_transfer.textvqa_k8.brier}{0.042}
\@namedef{VJ@H2k.ts_transfer.textvqa_k8.brier.ci}{[0.033, 0.051]}
\@namedef{VJ@H2k.ts_transfer.textvqa_k8.cov@0.05}{0.999}
\@namedef{VJ@H2k.ts_transfer.textvqa_k8.cov@0.05.ci}{[0.998, 1.000]}
\@namedef{VJ@H2k.ts_transfer.textvqa_k8.cov@0.05.pct}{99.9\%}
\@namedef{VJ@H2k.ts_transfer.textvqa_k8.cov@0.1}{0.999}
\@namedef{VJ@H2k.ts_transfer.textvqa_k8.cov@0.1.ci}{[0.998, 1.000]}
\@namedef{VJ@H2k.ts_transfer.textvqa_k8.cov@0.1.pct}{99.9\%}
\@namedef{VJ@H2k.ts_transfer.textvqa_k8.ece15}{0.038}
\@namedef{VJ@H2k.ts_transfer.textvqa_k8.ece15.ci}{[0.037, 0.045]}
\@namedef{VJ@H2k.ts_transfer.textvqa_k8.nll}{0.124}
\@namedef{VJ@H2k.ts_transfer.textvqa_k8.nll.ci}{[0.103, 0.147]}
\@namedef{VJ@H2k.ts_transfer.textvqa_k8.risk@0.05}{0.027}
\@namedef{VJ@H2k.ts_transfer.textvqa_k8.risk@0.05.ci}{[0.019, 0.034]}
\@namedef{VJ@H2k.ts_transfer.textvqa_k8.risk@0.05.pct}{2.7\%}
\@namedef{VJ@H2k.ts_transfer.textvqa_k8.risk@0.1}{0.027}
\@namedef{VJ@H2k.ts_transfer.textvqa_k8.risk@0.1.ci}{[0.019, 0.034]}
\@namedef{VJ@H2k.ts_transfer.textvqa_k8.risk@0.1.pct}{2.7\%}
\@namedef{VJ@M0.raw.gqa_val.accuracy}{0.880}
\@namedef{VJ@M0.raw.gqa_val.accuracy.ci}{[0.871, 0.889]}
\@namedef{VJ@M0.raw.gqa_val.aurc_maxp}{0.033}
\@namedef{VJ@M0.raw.gqa_val.aurc_maxp.ci}{[0.028, 0.038]}
\@namedef{VJ@M0.raw.gqa_val.brier}{0.204}
\@namedef{VJ@M0.raw.gqa_val.brier.ci}{[0.189, 0.219]}
\@namedef{VJ@M0.raw.gqa_val.cov@0.05}{0.745}
\@namedef{VJ@M0.raw.gqa_val.cov@0.05.ci}{[0.732, 0.758]}
\@namedef{VJ@M0.raw.gqa_val.cov@0.05.pct}{74.5\%}
\@namedef{VJ@M0.raw.gqa_val.cov@0.1}{0.930}
\@namedef{VJ@M0.raw.gqa_val.cov@0.1.ci}{[0.924, 0.937]}
\@namedef{VJ@M0.raw.gqa_val.cov@0.1.pct}{93.0\%}
\@namedef{VJ@M0.raw.gqa_val.ece15}{0.091}
\@namedef{VJ@M0.raw.gqa_val.ece15.ci}{[0.083, 0.099]}
\@namedef{VJ@M0.raw.gqa_val.errconf09}{64\%}
\@namedef{VJ@M0.raw.gqa_val.nll}{0.550}
\@namedef{VJ@M0.raw.gqa_val.nll.ci}{[0.504, 0.595]}
\@namedef{VJ@M0.raw.gqa_val.risk@0.05}{0.044}
\@namedef{VJ@M0.raw.gqa_val.risk@0.05.ci}{[0.038, 0.050]}
\@namedef{VJ@M0.raw.gqa_val.risk@0.05.pct}{4.4\%}
\@namedef{VJ@M0.raw.gqa_val.risk@0.1}{0.093}
\@namedef{VJ@M0.raw.gqa_val.risk@0.1.ci}{[0.084, 0.101]}
\@namedef{VJ@M0.raw.gqa_val.risk@0.1.pct}{9.3\%}
\@namedef{VJ@M0.raw.macro.accuracy}{0.834}
\@namedef{VJ@M0.raw.macro.accuracy.ci}{[0.825, 0.842]}
\@namedef{VJ@M0.raw.macro.aurc_maxp}{0.079}
\@namedef{VJ@M0.raw.macro.aurc_maxp.ci}{[0.072, 0.086]}
\@namedef{VJ@M0.raw.macro.brier}{0.294}
\@namedef{VJ@M0.raw.macro.brier.ci}{[0.280, 0.308]}
\@namedef{VJ@M0.raw.macro.ece15}{0.134}
\@namedef{VJ@M0.raw.macro.ece15.ci}{[0.128, 0.143]}
\@namedef{VJ@M0.raw.macro.nll}{1.009}
\@namedef{VJ@M0.raw.macro.nll.ci}{[0.953, 1.073]}
\@namedef{VJ@M0.raw.snli_ve.accuracy}{0.629}
\@namedef{VJ@M0.raw.snli_ve.accuracy.ci}{[0.600, 0.656]}
\@namedef{VJ@M0.raw.snli_ve.aurc_maxp}{0.246}
\@namedef{VJ@M0.raw.snli_ve.aurc_maxp.ci}{[0.222, 0.277]}
\@namedef{VJ@M0.raw.snli_ve.brier}{0.679}
\@namedef{VJ@M0.raw.snli_ve.brier.ci}{[0.632, 0.728]}
\@namedef{VJ@M0.raw.snli_ve.cov@0.05}{0.023}
\@namedef{VJ@M0.raw.snli_ve.cov@0.05.ci}{[0.014, 0.032]}
\@namedef{VJ@M0.raw.snli_ve.cov@0.05.pct}{2.3\%}
\@namedef{VJ@M0.raw.snli_ve.cov@0.1}{0.066}
\@namedef{VJ@M0.raw.snli_ve.cov@0.1.ci}{[0.052, 0.079]}
\@namedef{VJ@M0.raw.snli_ve.cov@0.1.pct}{6.6\%}
\@namedef{VJ@M0.raw.snli_ve.ece15}{0.320}
\@namedef{VJ@M0.raw.snli_ve.ece15.ci}{[0.296, 0.350]}
\@namedef{VJ@M0.raw.snli_ve.nll}{2.593}
\@namedef{VJ@M0.raw.snli_ve.nll.ci}{[2.385, 2.833]}
\@namedef{VJ@M0.raw.snli_ve.risk@0.05}{0.129}
\@namedef{VJ@M0.raw.snli_ve.risk@0.05.ci}{[0.029, 0.267]}
\@namedef{VJ@M0.raw.snli_ve.risk@0.05.pct}{12.9\%}
\@namedef{VJ@M0.raw.snli_ve.risk@0.1}{0.078}
\@namedef{VJ@M0.raw.snli_ve.risk@0.1.ci}{[0.030, 0.140]}
\@namedef{VJ@M0.raw.snli_ve.risk@0.1.pct}{7.8\%}
\@namedef{VJ@M0.raw.tallyqa_l.accuracy}{0.853}
\@namedef{VJ@M0.raw.tallyqa_l.accuracy.ci}{[0.840, 0.864]}
\@namedef{VJ@M0.raw.tallyqa_l.aurc_maxp}{0.035}
\@namedef{VJ@M0.raw.tallyqa_l.aurc_maxp.ci}{[0.029, 0.042]}
\@namedef{VJ@M0.raw.tallyqa_l.brier}{0.251}
\@namedef{VJ@M0.raw.tallyqa_l.brier.ci}{[0.230, 0.273]}
\@namedef{VJ@M0.raw.tallyqa_l.cov@0.05}{0.753}
\@namedef{VJ@M0.raw.tallyqa_l.cov@0.05.ci}{[0.736, 0.769]}
\@namedef{VJ@M0.raw.tallyqa_l.cov@0.05.pct}{75.3\%}
\@namedef{VJ@M0.raw.tallyqa_l.cov@0.1}{0.897}
\@namedef{VJ@M0.raw.tallyqa_l.cov@0.1.ci}{[0.886, 0.907]}
\@namedef{VJ@M0.raw.tallyqa_l.cov@0.1.pct}{89.7\%}
\@namedef{VJ@M0.raw.tallyqa_l.ece15}{0.110}
\@namedef{VJ@M0.raw.tallyqa_l.ece15.ci}{[0.099, 0.121]}
\@namedef{VJ@M0.raw.tallyqa_l.nll}{0.758}
\@namedef{VJ@M0.raw.tallyqa_l.nll.ci}{[0.688, 0.839]}
\@namedef{VJ@M0.raw.tallyqa_l.risk@0.05}{0.051}
\@namedef{VJ@M0.raw.tallyqa_l.risk@0.05.ci}{[0.043, 0.059]}
\@namedef{VJ@M0.raw.tallyqa_l.risk@0.05.pct}{5.1\%}
\@namedef{VJ@M0.raw.tallyqa_l.risk@0.1}{0.101}
\@namedef{VJ@M0.raw.tallyqa_l.risk@0.1.ci}{[0.091, 0.112]}
\@namedef{VJ@M0.raw.tallyqa_l.risk@0.1.pct}{10.1\%}
\@namedef{VJ@M0.raw.textvqa_k8.accuracy}{0.974}
\@namedef{VJ@M0.raw.textvqa_k8.accuracy.ci}{[0.966, 0.981]}
\@namedef{VJ@M0.raw.textvqa_k8.aurc_maxp}{0.001}
\@namedef{VJ@M0.raw.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@M0.raw.textvqa_k8.brier}{0.042}
\@namedef{VJ@M0.raw.textvqa_k8.brier.ci}{[0.030, 0.056]}
\@namedef{VJ@M0.raw.textvqa_k8.cov@0.05}{1.000}
\@namedef{VJ@M0.raw.textvqa_k8.cov@0.05.ci}{[1.000, 1.000]}
\@namedef{VJ@M0.raw.textvqa_k8.cov@0.05.pct}{100.0\%}
\@namedef{VJ@M0.raw.textvqa_k8.cov@0.1}{1.000}
\@namedef{VJ@M0.raw.textvqa_k8.cov@0.1.ci}{[1.000, 1.000]}
\@namedef{VJ@M0.raw.textvqa_k8.cov@0.1.pct}{100.0\%}
\@namedef{VJ@M0.raw.textvqa_k8.ece15}{0.017}
\@namedef{VJ@M0.raw.textvqa_k8.ece15.ci}{[0.012, 0.024]}
\@namedef{VJ@M0.raw.textvqa_k8.nll}{0.137}
\@namedef{VJ@M0.raw.textvqa_k8.nll.ci}{[0.093, 0.182]}
\@namedef{VJ@M0.raw.textvqa_k8.risk@0.05}{0.026}
\@namedef{VJ@M0.raw.textvqa_k8.risk@0.05.ci}{[0.019, 0.034]}
\@namedef{VJ@M0.raw.textvqa_k8.risk@0.05.pct}{2.6\%}
\@namedef{VJ@M0.raw.textvqa_k8.risk@0.1}{0.026}
\@namedef{VJ@M0.raw.textvqa_k8.risk@0.1.ci}{[0.019, 0.034]}
\@namedef{VJ@M0.raw.textvqa_k8.risk@0.1.pct}{2.6\%}
\@namedef{VJ@M0.ts_local.gqa_val.accuracy}{0.880}
\@namedef{VJ@M0.ts_local.gqa_val.accuracy.ci}{[0.871, 0.889]}
\@namedef{VJ@M0.ts_local.gqa_val.aurc_maxp}{0.037}
\@namedef{VJ@M0.ts_local.gqa_val.aurc_maxp.ci}{[0.031, 0.043]}
\@namedef{VJ@M0.ts_local.gqa_val.brier}{0.176}
\@namedef{VJ@M0.ts_local.gqa_val.brier.ci}{[0.165, 0.187]}
\@namedef{VJ@M0.ts_local.gqa_val.cov@0.05}{0.758}
\@namedef{VJ@M0.ts_local.gqa_val.cov@0.05.ci}{[0.745, 0.771]}
\@namedef{VJ@M0.ts_local.gqa_val.cov@0.05.pct}{75.8\%}
\@namedef{VJ@M0.ts_local.gqa_val.cov@0.1}{0.936}
\@namedef{VJ@M0.ts_local.gqa_val.cov@0.1.ci}{[0.929, 0.942]}
\@namedef{VJ@M0.ts_local.gqa_val.cov@0.1.pct}{93.6\%}
\@namedef{VJ@M0.ts_local.gqa_val.ece15}{0.012}
\@namedef{VJ@M0.ts_local.gqa_val.ece15.ci}{[0.009, 0.021]}
\@namedef{VJ@M0.ts_local.gqa_val.nll}{0.317}
\@namedef{VJ@M0.ts_local.gqa_val.nll.ci}{[0.299, 0.335]}
\@namedef{VJ@M0.ts_local.gqa_val.risk@0.05}{0.047}
\@namedef{VJ@M0.ts_local.gqa_val.risk@0.05.ci}{[0.041, 0.054]}
\@namedef{VJ@M0.ts_local.gqa_val.risk@0.05.pct}{4.7\%}
\@namedef{VJ@M0.ts_local.gqa_val.risk@0.1}{0.093}
\@namedef{VJ@M0.ts_local.gqa_val.risk@0.1.ci}{[0.085, 0.101]}
\@namedef{VJ@M0.ts_local.gqa_val.risk@0.1.pct}{9.3\%}
\@namedef{VJ@M0.ts_local.macro.accuracy}{0.834}
\@namedef{VJ@M0.ts_local.macro.accuracy.ci}{[0.825, 0.842]}
\@namedef{VJ@M0.ts_local.macro.aurc_maxp}{0.080}
\@namedef{VJ@M0.ts_local.macro.aurc_maxp.ci}{[0.074, 0.088]}
\@namedef{VJ@M0.ts_local.macro.brier}{0.230}
\@namedef{VJ@M0.ts_local.macro.brier.ci}{[0.222, 0.238]}
\@namedef{VJ@M0.ts_local.macro.ece15}{0.029}
\@namedef{VJ@M0.ts_local.macro.ece15.ci}{[0.025, 0.039]}
\@namedef{VJ@M0.ts_local.macro.nll}{0.416}
\@namedef{VJ@M0.ts_local.macro.nll.ci}{[0.402, 0.431]}
\@namedef{VJ@M0.ts_local.snli_ve.accuracy}{0.629}
\@namedef{VJ@M0.ts_local.snli_ve.accuracy.ci}{[0.600, 0.656]}
\@namedef{VJ@M0.ts_local.snli_ve.aurc_maxp}{0.247}
\@namedef{VJ@M0.ts_local.snli_ve.aurc_maxp.ci}{[0.222, 0.277]}
\@namedef{VJ@M0.ts_local.snli_ve.brier}{0.491}
\@namedef{VJ@M0.ts_local.snli_ve.brier.ci}{[0.469, 0.518]}
\@namedef{VJ@M0.ts_local.snli_ve.cov@0.05}{0.023}
\@namedef{VJ@M0.ts_local.snli_ve.cov@0.05.ci}{[0.015, 0.033]}
\@namedef{VJ@M0.ts_local.snli_ve.cov@0.05.pct}{2.3\%}
\@namedef{VJ@M0.ts_local.snli_ve.cov@0.1}{0.067}
\@namedef{VJ@M0.ts_local.snli_ve.cov@0.1.ci}{[0.054, 0.080]}
\@namedef{VJ@M0.ts_local.snli_ve.cov@0.1.pct}{6.7\%}
\@namedef{VJ@M0.ts_local.snli_ve.ece15}{0.071}
\@namedef{VJ@M0.ts_local.snli_ve.ece15.ci}{[0.050, 0.099]}
\@namedef{VJ@M0.ts_local.snli_ve.nll}{0.821}
\@namedef{VJ@M0.ts_local.snli_ve.nll.ci}{[0.789, 0.859]}
\@namedef{VJ@M0.ts_local.snli_ve.risk@0.05}{0.125}
\@namedef{VJ@M0.ts_local.snli_ve.risk@0.05.ci}{[0.029, 0.259]}
\@namedef{VJ@M0.ts_local.snli_ve.risk@0.05.pct}{12.5\%}
\@namedef{VJ@M0.ts_local.snli_ve.risk@0.1}{0.076}
\@namedef{VJ@M0.ts_local.snli_ve.risk@0.1.ci}{[0.029, 0.138]}
\@namedef{VJ@M0.ts_local.snli_ve.risk@0.1.pct}{7.6\%}
\@namedef{VJ@M0.ts_local.tallyqa_l.accuracy}{0.853}
\@namedef{VJ@M0.ts_local.tallyqa_l.accuracy.ci}{[0.840, 0.864]}
\@namedef{VJ@M0.ts_local.tallyqa_l.aurc_maxp}{0.036}
\@namedef{VJ@M0.ts_local.tallyqa_l.aurc_maxp.ci}{[0.030, 0.043]}
\@namedef{VJ@M0.ts_local.tallyqa_l.brier}{0.212}
\@namedef{VJ@M0.ts_local.tallyqa_l.brier.ci}{[0.196, 0.229]}
\@namedef{VJ@M0.ts_local.tallyqa_l.cov@0.05}{0.748}
\@namedef{VJ@M0.ts_local.tallyqa_l.cov@0.05.ci}{[0.730, 0.765]}
\@namedef{VJ@M0.ts_local.tallyqa_l.cov@0.05.pct}{74.8\%}
\@namedef{VJ@M0.ts_local.tallyqa_l.cov@0.1}{0.898}
\@namedef{VJ@M0.ts_local.tallyqa_l.cov@0.1.ci}{[0.888, 0.909]}
\@namedef{VJ@M0.ts_local.tallyqa_l.cov@0.1.pct}{89.8\%}
\@namedef{VJ@M0.ts_local.tallyqa_l.ece15}{0.026}
\@namedef{VJ@M0.ts_local.tallyqa_l.ece15.ci}{[0.020, 0.037]}
\@namedef{VJ@M0.ts_local.tallyqa_l.nll}{0.429}
\@namedef{VJ@M0.ts_local.tallyqa_l.nll.ci}{[0.398, 0.463]}
\@namedef{VJ@M0.ts_local.tallyqa_l.risk@0.05}{0.047}
\@namedef{VJ@M0.ts_local.tallyqa_l.risk@0.05.ci}{[0.039, 0.055]}
\@namedef{VJ@M0.ts_local.tallyqa_l.risk@0.05.pct}{4.7\%}
\@namedef{VJ@M0.ts_local.tallyqa_l.risk@0.1}{0.099}
\@namedef{VJ@M0.ts_local.tallyqa_l.risk@0.1.ci}{[0.089, 0.111]}
\@namedef{VJ@M0.ts_local.tallyqa_l.risk@0.1.pct}{9.9\%}
\@namedef{VJ@M0.ts_local.textvqa_k8.accuracy}{0.974}
\@namedef{VJ@M0.ts_local.textvqa_k8.accuracy.ci}{[0.966, 0.981]}
\@namedef{VJ@M0.ts_local.textvqa_k8.aurc_maxp}{0.001}
\@namedef{VJ@M0.ts_local.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@M0.ts_local.textvqa_k8.brier}{0.039}
\@namedef{VJ@M0.ts_local.textvqa_k8.brier.ci}{[0.028, 0.050]}
\@namedef{VJ@M0.ts_local.textvqa_k8.cov@0.05}{1.000}
\@namedef{VJ@M0.ts_local.textvqa_k8.cov@0.05.ci}{[1.000, 1.000]}
\@namedef{VJ@M0.ts_local.textvqa_k8.cov@0.05.pct}{100.0\%}
\@namedef{VJ@M0.ts_local.textvqa_k8.cov@0.1}{1.000}
\@namedef{VJ@M0.ts_local.textvqa_k8.cov@0.1.ci}{[1.000, 1.000]}
\@namedef{VJ@M0.ts_local.textvqa_k8.cov@0.1.pct}{100.0\%}
\@namedef{VJ@M0.ts_local.textvqa_k8.ece15}{0.008}
\@namedef{VJ@M0.ts_local.textvqa_k8.ece15.ci}{[0.007, 0.016]}
\@namedef{VJ@M0.ts_local.textvqa_k8.nll}{0.097}
\@namedef{VJ@M0.ts_local.textvqa_k8.nll.ci}{[0.071, 0.124]}
\@namedef{VJ@M0.ts_local.textvqa_k8.risk@0.05}{0.026}
\@namedef{VJ@M0.ts_local.textvqa_k8.risk@0.05.ci}{[0.019, 0.034]}
\@namedef{VJ@M0.ts_local.textvqa_k8.risk@0.05.pct}{2.6\%}
\@namedef{VJ@M0.ts_local.textvqa_k8.risk@0.1}{0.026}
\@namedef{VJ@M0.ts_local.textvqa_k8.risk@0.1.ci}{[0.019, 0.034]}
\@namedef{VJ@M0.ts_local.textvqa_k8.risk@0.1.pct}{2.6\%}
\@namedef{VJ@M0.ts_transfer.gqa_val.accuracy}{0.880}
\@namedef{VJ@M0.ts_transfer.gqa_val.accuracy.ci}{[0.871, 0.889]}
\@namedef{VJ@M0.ts_transfer.gqa_val.aurc_maxp}{0.039}
\@namedef{VJ@M0.ts_transfer.gqa_val.aurc_maxp.ci}{[0.033, 0.045]}
\@namedef{VJ@M0.ts_transfer.gqa_val.brier}{0.178}
\@namedef{VJ@M0.ts_transfer.gqa_val.brier.ci}{[0.168, 0.188]}
\@namedef{VJ@M0.ts_transfer.gqa_val.cov@0.05}{0.743}
\@namedef{VJ@M0.ts_transfer.gqa_val.cov@0.05.ci}{[0.730, 0.757]}
\@namedef{VJ@M0.ts_transfer.gqa_val.cov@0.05.pct}{74.3\%}
\@namedef{VJ@M0.ts_transfer.gqa_val.cov@0.1}{0.937}
\@namedef{VJ@M0.ts_transfer.gqa_val.cov@0.1.ci}{[0.930, 0.943]}
\@namedef{VJ@M0.ts_transfer.gqa_val.cov@0.1.pct}{93.7\%}
\@namedef{VJ@M0.ts_transfer.gqa_val.ece15}{0.038}
\@namedef{VJ@M0.ts_transfer.gqa_val.ece15.ci}{[0.034, 0.047]}
\@namedef{VJ@M0.ts_transfer.gqa_val.nll}{0.333}
\@namedef{VJ@M0.ts_transfer.gqa_val.nll.ci}{[0.318, 0.349]}
\@namedef{VJ@M0.ts_transfer.gqa_val.risk@0.05}{0.048}
\@namedef{VJ@M0.ts_transfer.gqa_val.risk@0.05.ci}{[0.041, 0.055]}
\@namedef{VJ@M0.ts_transfer.gqa_val.risk@0.05.pct}{4.8\%}
\@namedef{VJ@M0.ts_transfer.gqa_val.risk@0.1}{0.096}
\@namedef{VJ@M0.ts_transfer.gqa_val.risk@0.1.ci}{[0.088, 0.104]}
\@namedef{VJ@M0.ts_transfer.gqa_val.risk@0.1.pct}{9.6\%}
\@namedef{VJ@M0.ts_transfer.macro.accuracy}{0.834}
\@namedef{VJ@M0.ts_transfer.macro.accuracy.ci}{[0.825, 0.842]}
\@namedef{VJ@M0.ts_transfer.macro.aurc_maxp}{0.081}
\@namedef{VJ@M0.ts_transfer.macro.aurc_maxp.ci}{[0.074, 0.089]}
\@namedef{VJ@M0.ts_transfer.macro.brier}{0.248}
\@namedef{VJ@M0.ts_transfer.macro.brier.ci}{[0.239, 0.259]}
\@namedef{VJ@M0.ts_transfer.macro.ece15}{0.097}
\@namedef{VJ@M0.ts_transfer.macro.ece15.ci}{[0.093, 0.106]}
\@namedef{VJ@M0.ts_transfer.macro.nll}{0.487}
\@namedef{VJ@M0.ts_transfer.macro.nll.ci}{[0.469, 0.506]}
\@namedef{VJ@M0.ts_transfer.snli_ve.accuracy}{0.629}
\@namedef{VJ@M0.ts_transfer.snli_ve.accuracy.ci}{[0.600, 0.656]}
\@namedef{VJ@M0.ts_transfer.snli_ve.aurc_maxp}{0.247}
\@namedef{VJ@M0.ts_transfer.snli_ve.aurc_maxp.ci}{[0.222, 0.277]}
\@namedef{VJ@M0.ts_transfer.snli_ve.brier}{0.549}
\@namedef{VJ@M0.ts_transfer.snli_ve.brier.ci}{[0.515, 0.586]}
\@namedef{VJ@M0.ts_transfer.snli_ve.cov@0.05}{0.023}
\@namedef{VJ@M0.ts_transfer.snli_ve.cov@0.05.ci}{[0.015, 0.033]}
\@namedef{VJ@M0.ts_transfer.snli_ve.cov@0.05.pct}{2.3\%}
\@namedef{VJ@M0.ts_transfer.snli_ve.cov@0.1}{0.069}
\@namedef{VJ@M0.ts_transfer.snli_ve.cov@0.1.ci}{[0.055, 0.081]}
\@namedef{VJ@M0.ts_transfer.snli_ve.cov@0.1.pct}{6.9\%}
\@namedef{VJ@M0.ts_transfer.snli_ve.ece15}{0.183}
\@namedef{VJ@M0.ts_transfer.snli_ve.ece15.ci}{[0.163, 0.211]}
\@namedef{VJ@M0.ts_transfer.snli_ve.nll}{0.961}
\@namedef{VJ@M0.ts_transfer.snli_ve.nll.ci}{[0.903, 1.031]}
\@namedef{VJ@M0.ts_transfer.snli_ve.risk@0.05}{0.125}
\@namedef{VJ@M0.ts_transfer.snli_ve.risk@0.05.ci}{[0.029, 0.259]}
\@namedef{VJ@M0.ts_transfer.snli_ve.risk@0.05.pct}{12.5\%}
\@namedef{VJ@M0.ts_transfer.snli_ve.risk@0.1}{0.074}
\@namedef{VJ@M0.ts_transfer.snli_ve.risk@0.1.ci}{[0.029, 0.135]}
\@namedef{VJ@M0.ts_transfer.snli_ve.risk@0.1.pct}{7.4\%}
\@namedef{VJ@M0.ts_transfer.tallyqa_l.accuracy}{0.853}
\@namedef{VJ@M0.ts_transfer.tallyqa_l.accuracy.ci}{[0.840, 0.864]}
\@namedef{VJ@M0.ts_transfer.tallyqa_l.aurc_maxp}{0.037}
\@namedef{VJ@M0.ts_transfer.tallyqa_l.aurc_maxp.ci}{[0.030, 0.043]}
\@namedef{VJ@M0.ts_transfer.tallyqa_l.brier}{0.213}
\@namedef{VJ@M0.ts_transfer.tallyqa_l.brier.ci}{[0.199, 0.229]}
\@namedef{VJ@M0.ts_transfer.tallyqa_l.cov@0.05}{0.739}
\@namedef{VJ@M0.ts_transfer.tallyqa_l.cov@0.05.ci}{[0.721, 0.755]}
\@namedef{VJ@M0.ts_transfer.tallyqa_l.cov@0.05.pct}{73.9\%}
\@namedef{VJ@M0.ts_transfer.tallyqa_l.cov@0.1}{0.896}
\@namedef{VJ@M0.ts_transfer.tallyqa_l.cov@0.1.ci}{[0.885, 0.907]}
\@namedef{VJ@M0.ts_transfer.tallyqa_l.cov@0.1.pct}{89.6\%}
\@namedef{VJ@M0.ts_transfer.tallyqa_l.ece15}{0.055}
\@namedef{VJ@M0.ts_transfer.tallyqa_l.ece15.ci}{[0.051, 0.067]}
\@namedef{VJ@M0.ts_transfer.tallyqa_l.nll}{0.457}
\@namedef{VJ@M0.ts_transfer.tallyqa_l.nll.ci}{[0.432, 0.485]}
\@namedef{VJ@M0.ts_transfer.tallyqa_l.risk@0.05}{0.043}
\@namedef{VJ@M0.ts_transfer.tallyqa_l.risk@0.05.ci}{[0.036, 0.052]}
\@namedef{VJ@M0.ts_transfer.tallyqa_l.risk@0.05.pct}{4.3\%}
\@namedef{VJ@M0.ts_transfer.tallyqa_l.risk@0.1}{0.098}
\@namedef{VJ@M0.ts_transfer.tallyqa_l.risk@0.1.ci}{[0.088, 0.110]}
\@namedef{VJ@M0.ts_transfer.tallyqa_l.risk@0.1.pct}{9.8\%}
\@namedef{VJ@M0.ts_transfer.textvqa_k8.accuracy}{0.974}
\@namedef{VJ@M0.ts_transfer.textvqa_k8.accuracy.ci}{[0.966, 0.981]}
\@namedef{VJ@M0.ts_transfer.textvqa_k8.aurc_maxp}{0.001}
\@namedef{VJ@M0.ts_transfer.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@M0.ts_transfer.textvqa_k8.brier}{0.054}
\@namedef{VJ@M0.ts_transfer.textvqa_k8.brier.ci}{[0.046, 0.063]}
\@namedef{VJ@M0.ts_transfer.textvqa_k8.cov@0.05}{1.000}
\@namedef{VJ@M0.ts_transfer.textvqa_k8.cov@0.05.ci}{[1.000, 1.000]}
\@namedef{VJ@M0.ts_transfer.textvqa_k8.cov@0.05.pct}{100.0\%}
\@namedef{VJ@M0.ts_transfer.textvqa_k8.cov@0.1}{1.000}
\@namedef{VJ@M0.ts_transfer.textvqa_k8.cov@0.1.ci}{[1.000, 1.000]}
\@namedef{VJ@M0.ts_transfer.textvqa_k8.cov@0.1.pct}{100.0\%}
\@namedef{VJ@M0.ts_transfer.textvqa_k8.ece15}{0.111}
\@namedef{VJ@M0.ts_transfer.textvqa_k8.ece15.ci}{[0.107, 0.118]}
\@namedef{VJ@M0.ts_transfer.textvqa_k8.nll}{0.195}
\@namedef{VJ@M0.ts_transfer.textvqa_k8.nll.ci}{[0.177, 0.214]}
\@namedef{VJ@M0.ts_transfer.textvqa_k8.risk@0.05}{0.026}
\@namedef{VJ@M0.ts_transfer.textvqa_k8.risk@0.05.ci}{[0.019, 0.034]}
\@namedef{VJ@M0.ts_transfer.textvqa_k8.risk@0.05.pct}{2.6\%}
\@namedef{VJ@M0.ts_transfer.textvqa_k8.risk@0.1}{0.026}
\@namedef{VJ@M0.ts_transfer.textvqa_k8.risk@0.1.ci}{[0.019, 0.034]}
\@namedef{VJ@M0.ts_transfer.textvqa_k8.risk@0.1.pct}{2.6\%}
\@namedef{VJ@M0_8b.raw.gqa_val.accuracy}{0.885}
\@namedef{VJ@M0_8b.raw.gqa_val.accuracy.ci}{[0.876, 0.894]}
\@namedef{VJ@M0_8b.raw.gqa_val.aurc_maxp}{0.026}
\@namedef{VJ@M0_8b.raw.gqa_val.aurc_maxp.ci}{[0.023, 0.029]}
\@namedef{VJ@M0_8b.raw.gqa_val.brier}{0.190}
\@namedef{VJ@M0_8b.raw.gqa_val.brier.ci}{[0.175, 0.205]}
\@namedef{VJ@M0_8b.raw.gqa_val.cov@0.05}{0.782}
\@namedef{VJ@M0_8b.raw.gqa_val.cov@0.05.ci}{[0.770, 0.795]}
\@namedef{VJ@M0_8b.raw.gqa_val.cov@0.05.pct}{78.2\%}
\@namedef{VJ@M0_8b.raw.gqa_val.cov@0.1}{0.942}
\@namedef{VJ@M0_8b.raw.gqa_val.cov@0.1.ci}{[0.936, 0.949]}
\@namedef{VJ@M0_8b.raw.gqa_val.cov@0.1.pct}{94.2\%}
\@namedef{VJ@M0_8b.raw.gqa_val.ece15}{0.079}
\@namedef{VJ@M0_8b.raw.gqa_val.ece15.ci}{[0.071, 0.087]}
\@namedef{VJ@M0_8b.raw.gqa_val.nll}{0.469}
\@namedef{VJ@M0_8b.raw.gqa_val.nll.ci}{[0.427, 0.510]}
\@namedef{VJ@M0_8b.raw.gqa_val.risk@0.05}{0.045}
\@namedef{VJ@M0_8b.raw.gqa_val.risk@0.05.ci}{[0.039, 0.051]}
\@namedef{VJ@M0_8b.raw.gqa_val.risk@0.05.pct}{4.5\%}
\@namedef{VJ@M0_8b.raw.gqa_val.risk@0.1}{0.090}
\@namedef{VJ@M0_8b.raw.gqa_val.risk@0.1.ci}{[0.082, 0.099]}
\@namedef{VJ@M0_8b.raw.gqa_val.risk@0.1.pct}{9.0\%}
\@namedef{VJ@M0_8b.raw.macro.accuracy}{0.853}
\@namedef{VJ@M0_8b.raw.macro.accuracy.ci}{[0.846, 0.860]}
\@namedef{VJ@M0_8b.raw.macro.aurc_maxp}{0.062}
\@namedef{VJ@M0_8b.raw.macro.aurc_maxp.ci}{[0.056, 0.069]}
\@namedef{VJ@M0_8b.raw.macro.brier}{0.243}
\@namedef{VJ@M0_8b.raw.macro.brier.ci}{[0.230, 0.255]}
\@namedef{VJ@M0_8b.raw.macro.ece15}{0.101}
\@namedef{VJ@M0_8b.raw.macro.ece15.ci}{[0.095, 0.108]}
\@namedef{VJ@M0_8b.raw.macro.nll}{0.634}
\@namedef{VJ@M0_8b.raw.macro.nll.ci}{[0.596, 0.673]}
\@namedef{VJ@M0_8b.raw.snli_ve.accuracy}{0.695}
\@namedef{VJ@M0_8b.raw.snli_ve.accuracy.ci}{[0.671, 0.718]}
\@namedef{VJ@M0_8b.raw.snli_ve.aurc_maxp}{0.191}
\@namedef{VJ@M0_8b.raw.snli_ve.aurc_maxp.ci}{[0.167, 0.217]}
\@namedef{VJ@M0_8b.raw.snli_ve.brier}{0.522}
\@namedef{VJ@M0_8b.raw.snli_ve.brier.ci}{[0.483, 0.562]}
\@namedef{VJ@M0_8b.raw.snli_ve.cov@0.05}{0.015}
\@namedef{VJ@M0_8b.raw.snli_ve.cov@0.05.ci}{[0.009, 0.022]}
\@namedef{VJ@M0_8b.raw.snli_ve.cov@0.05.pct}{1.5\%}
\@namedef{VJ@M0_8b.raw.snli_ve.cov@0.1}{0.061}
\@namedef{VJ@M0_8b.raw.snli_ve.cov@0.1.ci}{[0.047, 0.073]}
\@namedef{VJ@M0_8b.raw.snli_ve.cov@0.1.pct}{6.1\%}
\@namedef{VJ@M0_8b.raw.snli_ve.ece15}{0.226}
\@namedef{VJ@M0_8b.raw.snli_ve.ece15.ci}{[0.208, 0.252]}
\@namedef{VJ@M0_8b.raw.snli_ve.nll}{1.416}
\@namedef{VJ@M0_8b.raw.snli_ve.nll.ci}{[1.292, 1.551]}
\@namedef{VJ@M0_8b.raw.snli_ve.risk@0.05}{0.048}
\@namedef{VJ@M0_8b.raw.snli_ve.risk@0.05.ci}{[0.000, 0.167]}
\@namedef{VJ@M0_8b.raw.snli_ve.risk@0.05.pct}{4.8\%}
\@namedef{VJ@M0_8b.raw.snli_ve.risk@0.1}{0.036}
\@namedef{VJ@M0_8b.raw.snli_ve.risk@0.1.ci}{[0.000, 0.079]}
\@namedef{VJ@M0_8b.raw.snli_ve.risk@0.1.pct}{3.6\%}
\@namedef{VJ@M0_8b.raw.tallyqa_l.accuracy}{0.853}
\@namedef{VJ@M0_8b.raw.tallyqa_l.accuracy.ci}{[0.840, 0.865]}
\@namedef{VJ@M0_8b.raw.tallyqa_l.aurc_maxp}{0.031}
\@namedef{VJ@M0_8b.raw.tallyqa_l.aurc_maxp.ci}{[0.026, 0.036]}
\@namedef{VJ@M0_8b.raw.tallyqa_l.brier}{0.227}
\@namedef{VJ@M0_8b.raw.tallyqa_l.brier.ci}{[0.209, 0.246]}
\@namedef{VJ@M0_8b.raw.tallyqa_l.cov@0.05}{0.755}
\@namedef{VJ@M0_8b.raw.tallyqa_l.cov@0.05.ci}{[0.737, 0.770]}
\@namedef{VJ@M0_8b.raw.tallyqa_l.cov@0.05.pct}{75.5\%}
\@namedef{VJ@M0_8b.raw.tallyqa_l.cov@0.1}{0.887}
\@namedef{VJ@M0_8b.raw.tallyqa_l.cov@0.1.ci}{[0.875, 0.898]}
\@namedef{VJ@M0_8b.raw.tallyqa_l.cov@0.1.pct}{88.7\%}
\@namedef{VJ@M0_8b.raw.tallyqa_l.ece15}{0.087}
\@namedef{VJ@M0_8b.raw.tallyqa_l.ece15.ci}{[0.077, 0.097]}
\@namedef{VJ@M0_8b.raw.tallyqa_l.nll}{0.566}
\@namedef{VJ@M0_8b.raw.tallyqa_l.nll.ci}{[0.511, 0.625]}
\@namedef{VJ@M0_8b.raw.tallyqa_l.risk@0.05}{0.044}
\@namedef{VJ@M0_8b.raw.tallyqa_l.risk@0.05.ci}{[0.036, 0.052]}
\@namedef{VJ@M0_8b.raw.tallyqa_l.risk@0.05.pct}{4.4\%}
\@namedef{VJ@M0_8b.raw.tallyqa_l.risk@0.1}{0.091}
\@namedef{VJ@M0_8b.raw.tallyqa_l.risk@0.1.ci}{[0.082, 0.102]}
\@namedef{VJ@M0_8b.raw.tallyqa_l.risk@0.1.pct}{9.1\%}
\@namedef{VJ@M0_8b.raw.textvqa_k8.accuracy}{0.979}
\@namedef{VJ@M0_8b.raw.textvqa_k8.accuracy.ci}{[0.973, 0.986]}
\@namedef{VJ@M0_8b.raw.textvqa_k8.aurc_maxp}{0.000}
\@namedef{VJ@M0_8b.raw.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@M0_8b.raw.textvqa_k8.brier}{0.031}
\@namedef{VJ@M0_8b.raw.textvqa_k8.brier.ci}{[0.022, 0.040]}
\@namedef{VJ@M0_8b.raw.textvqa_k8.cov@0.05}{1.000}
\@namedef{VJ@M0_8b.raw.textvqa_k8.cov@0.05.ci}{[1.000, 1.000]}
\@namedef{VJ@M0_8b.raw.textvqa_k8.cov@0.05.pct}{100.0\%}
\@namedef{VJ@M0_8b.raw.textvqa_k8.cov@0.1}{1.000}
\@namedef{VJ@M0_8b.raw.textvqa_k8.cov@0.1.ci}{[1.000, 1.000]}
\@namedef{VJ@M0_8b.raw.textvqa_k8.cov@0.1.pct}{100.0\%}
\@namedef{VJ@M0_8b.raw.textvqa_k8.ece15}{0.012}
\@namedef{VJ@M0_8b.raw.textvqa_k8.ece15.ci}{[0.009, 0.018]}
\@namedef{VJ@M0_8b.raw.textvqa_k8.nll}{0.084}
\@namedef{VJ@M0_8b.raw.textvqa_k8.nll.ci}{[0.055, 0.111]}
\@namedef{VJ@M0_8b.raw.textvqa_k8.risk@0.05}{0.021}
\@namedef{VJ@M0_8b.raw.textvqa_k8.risk@0.05.ci}{[0.014, 0.027]}
\@namedef{VJ@M0_8b.raw.textvqa_k8.risk@0.05.pct}{2.1\%}
\@namedef{VJ@M0_8b.raw.textvqa_k8.risk@0.1}{0.021}
\@namedef{VJ@M0_8b.raw.textvqa_k8.risk@0.1.ci}{[0.014, 0.027]}
\@namedef{VJ@M0_8b.raw.textvqa_k8.risk@0.1.pct}{2.1\%}
\@namedef{VJ@M0_8b.ts_local.gqa_val.accuracy}{0.885}
\@namedef{VJ@M0_8b.ts_local.gqa_val.accuracy.ci}{[0.876, 0.894]}
\@namedef{VJ@M0_8b.ts_local.gqa_val.aurc_maxp}{0.028}
\@namedef{VJ@M0_8b.ts_local.gqa_val.aurc_maxp.ci}{[0.024, 0.032]}
\@namedef{VJ@M0_8b.ts_local.gqa_val.brier}{0.167}
\@namedef{VJ@M0_8b.ts_local.gqa_val.brier.ci}{[0.156, 0.179]}
\@namedef{VJ@M0_8b.ts_local.gqa_val.cov@0.05}{0.784}
\@namedef{VJ@M0_8b.ts_local.gqa_val.cov@0.05.ci}{[0.771, 0.796]}
\@namedef{VJ@M0_8b.ts_local.gqa_val.cov@0.05.pct}{78.4\%}
\@namedef{VJ@M0_8b.ts_local.gqa_val.cov@0.1}{0.943}
\@namedef{VJ@M0_8b.ts_local.gqa_val.cov@0.1.ci}{[0.937, 0.950]}
\@namedef{VJ@M0_8b.ts_local.gqa_val.cov@0.1.pct}{94.3\%}
\@namedef{VJ@M0_8b.ts_local.gqa_val.ece15}{0.012}
\@namedef{VJ@M0_8b.ts_local.gqa_val.ece15.ci}{[0.010, 0.022]}
\@namedef{VJ@M0_8b.ts_local.gqa_val.nll}{0.299}
\@namedef{VJ@M0_8b.ts_local.gqa_val.nll.ci}{[0.280, 0.317]}
\@namedef{VJ@M0_8b.ts_local.gqa_val.risk@0.05}{0.046}
\@namedef{VJ@M0_8b.ts_local.gqa_val.risk@0.05.ci}{[0.039, 0.052]}
\@namedef{VJ@M0_8b.ts_local.gqa_val.risk@0.05.pct}{4.6\%}
\@namedef{VJ@M0_8b.ts_local.gqa_val.risk@0.1}{0.091}
\@namedef{VJ@M0_8b.ts_local.gqa_val.risk@0.1.ci}{[0.083, 0.099]}
\@namedef{VJ@M0_8b.ts_local.gqa_val.risk@0.1.pct}{9.1\%}
\@namedef{VJ@M0_8b.ts_local.macro.accuracy}{0.853}
\@namedef{VJ@M0_8b.ts_local.macro.accuracy.ci}{[0.846, 0.860]}
\@namedef{VJ@M0_8b.ts_local.macro.aurc_maxp}{0.062}
\@namedef{VJ@M0_8b.ts_local.macro.aurc_maxp.ci}{[0.056, 0.069]}
\@namedef{VJ@M0_8b.ts_local.macro.brier}{0.208}
\@namedef{VJ@M0_8b.ts_local.macro.brier.ci}{[0.199, 0.216]}
\@namedef{VJ@M0_8b.ts_local.macro.ece15}{0.022}
\@namedef{VJ@M0_8b.ts_local.macro.ece15.ci}{[0.021, 0.032]}
\@namedef{VJ@M0_8b.ts_local.macro.nll}{0.376}
\@namedef{VJ@M0_8b.ts_local.macro.nll.ci}{[0.362, 0.391]}
\@namedef{VJ@M0_8b.ts_local.snli_ve.accuracy}{0.695}
\@namedef{VJ@M0_8b.ts_local.snli_ve.accuracy.ci}{[0.671, 0.718]}
\@namedef{VJ@M0_8b.ts_local.snli_ve.aurc_maxp}{0.190}
\@namedef{VJ@M0_8b.ts_local.snli_ve.aurc_maxp.ci}{[0.166, 0.216]}
\@namedef{VJ@M0_8b.ts_local.snli_ve.brier}{0.432}
\@namedef{VJ@M0_8b.ts_local.snli_ve.brier.ci}{[0.408, 0.457]}
\@namedef{VJ@M0_8b.ts_local.snli_ve.cov@0.05}{0.015}
\@namedef{VJ@M0_8b.ts_local.snli_ve.cov@0.05.ci}{[0.009, 0.022]}
\@namedef{VJ@M0_8b.ts_local.snli_ve.cov@0.05.pct}{1.5\%}
\@namedef{VJ@M0_8b.ts_local.snli_ve.cov@0.1}{0.060}
\@namedef{VJ@M0_8b.ts_local.snli_ve.cov@0.1.ci}{[0.047, 0.072]}
\@namedef{VJ@M0_8b.ts_local.snli_ve.cov@0.1.pct}{6.0\%}
\@namedef{VJ@M0_8b.ts_local.snli_ve.ece15}{0.051}
\@namedef{VJ@M0_8b.ts_local.snli_ve.ece15.ci}{[0.038, 0.079]}
\@namedef{VJ@M0_8b.ts_local.snli_ve.nll}{0.738}
\@namedef{VJ@M0_8b.ts_local.snli_ve.nll.ci}{[0.703, 0.777]}
\@namedef{VJ@M0_8b.ts_local.snli_ve.risk@0.05}{0.048}
\@namedef{VJ@M0_8b.ts_local.snli_ve.risk@0.05.ci}{[0.000, 0.167]}
\@namedef{VJ@M0_8b.ts_local.snli_ve.risk@0.05.pct}{4.8\%}
\@namedef{VJ@M0_8b.ts_local.snli_ve.risk@0.1}{0.049}
\@namedef{VJ@M0_8b.ts_local.snli_ve.risk@0.1.ci}{[0.011, 0.100]}
\@namedef{VJ@M0_8b.ts_local.snli_ve.risk@0.1.pct}{4.9\%}
\@namedef{VJ@M0_8b.ts_local.tallyqa_l.accuracy}{0.853}
\@namedef{VJ@M0_8b.ts_local.tallyqa_l.accuracy.ci}{[0.840, 0.865]}
\@namedef{VJ@M0_8b.ts_local.tallyqa_l.aurc_maxp}{0.031}
\@namedef{VJ@M0_8b.ts_local.tallyqa_l.aurc_maxp.ci}{[0.026, 0.037]}
\@namedef{VJ@M0_8b.ts_local.tallyqa_l.brier}{0.202}
\@namedef{VJ@M0_8b.ts_local.tallyqa_l.brier.ci}{[0.187, 0.217]}
\@namedef{VJ@M0_8b.ts_local.tallyqa_l.cov@0.05}{0.758}
\@namedef{VJ@M0_8b.ts_local.tallyqa_l.cov@0.05.ci}{[0.740, 0.773]}
\@namedef{VJ@M0_8b.ts_local.tallyqa_l.cov@0.05.pct}{75.8\%}
\@namedef{VJ@M0_8b.ts_local.tallyqa_l.cov@0.1}{0.884}
\@namedef{VJ@M0_8b.ts_local.tallyqa_l.cov@0.1.ci}{[0.872, 0.895]}
\@namedef{VJ@M0_8b.ts_local.tallyqa_l.cov@0.1.pct}{88.4\%}
\@namedef{VJ@M0_8b.ts_local.tallyqa_l.ece15}{0.018}
\@namedef{VJ@M0_8b.ts_local.tallyqa_l.ece15.ci}{[0.014, 0.031]}
\@namedef{VJ@M0_8b.ts_local.tallyqa_l.nll}{0.399}
\@namedef{VJ@M0_8b.ts_local.tallyqa_l.nll.ci}{[0.370, 0.429]}
\@namedef{VJ@M0_8b.ts_local.tallyqa_l.risk@0.05}{0.043}
\@namedef{VJ@M0_8b.ts_local.tallyqa_l.risk@0.05.ci}{[0.035, 0.052]}
\@namedef{VJ@M0_8b.ts_local.tallyqa_l.risk@0.05.pct}{4.3\%}
\@namedef{VJ@M0_8b.ts_local.tallyqa_l.risk@0.1}{0.090}
\@namedef{VJ@M0_8b.ts_local.tallyqa_l.risk@0.1.ci}{[0.080, 0.100]}
\@namedef{VJ@M0_8b.ts_local.tallyqa_l.risk@0.1.pct}{9.0\%}
\@namedef{VJ@M0_8b.ts_local.textvqa_k8.accuracy}{0.979}
\@namedef{VJ@M0_8b.ts_local.textvqa_k8.accuracy.ci}{[0.973, 0.986]}
\@namedef{VJ@M0_8b.ts_local.textvqa_k8.aurc_maxp}{0.000}
\@namedef{VJ@M0_8b.ts_local.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@M0_8b.ts_local.textvqa_k8.brier}{0.029}
\@namedef{VJ@M0_8b.ts_local.textvqa_k8.brier.ci}{[0.021, 0.037]}
\@namedef{VJ@M0_8b.ts_local.textvqa_k8.cov@0.05}{1.000}
\@namedef{VJ@M0_8b.ts_local.textvqa_k8.cov@0.05.ci}{[1.000, 1.000]}
\@namedef{VJ@M0_8b.ts_local.textvqa_k8.cov@0.05.pct}{100.0\%}
\@namedef{VJ@M0_8b.ts_local.textvqa_k8.cov@0.1}{1.000}
\@namedef{VJ@M0_8b.ts_local.textvqa_k8.cov@0.1.ci}{[1.000, 1.000]}
\@namedef{VJ@M0_8b.ts_local.textvqa_k8.cov@0.1.pct}{100.0\%}
\@namedef{VJ@M0_8b.ts_local.textvqa_k8.ece15}{0.008}
\@namedef{VJ@M0_8b.ts_local.textvqa_k8.ece15.ci}{[0.007, 0.014]}
\@namedef{VJ@M0_8b.ts_local.textvqa_k8.nll}{0.069}
\@namedef{VJ@M0_8b.ts_local.textvqa_k8.nll.ci}{[0.049, 0.088]}
\@namedef{VJ@M0_8b.ts_local.textvqa_k8.risk@0.05}{0.021}
\@namedef{VJ@M0_8b.ts_local.textvqa_k8.risk@0.05.ci}{[0.014, 0.027]}
\@namedef{VJ@M0_8b.ts_local.textvqa_k8.risk@0.05.pct}{2.1\%}
\@namedef{VJ@M0_8b.ts_local.textvqa_k8.risk@0.1}{0.021}
\@namedef{VJ@M0_8b.ts_local.textvqa_k8.risk@0.1.ci}{[0.014, 0.027]}
\@namedef{VJ@M0_8b.ts_local.textvqa_k8.risk@0.1.pct}{2.1\%}
\@namedef{VJ@M0_8b.ts_transfer.gqa_val.accuracy}{0.885}
\@namedef{VJ@M0_8b.ts_transfer.gqa_val.accuracy.ci}{[0.876, 0.894]}
\@namedef{VJ@M0_8b.ts_transfer.gqa_val.aurc_maxp}{0.029}
\@namedef{VJ@M0_8b.ts_transfer.gqa_val.aurc_maxp.ci}{[0.025, 0.033]}
\@namedef{VJ@M0_8b.ts_transfer.gqa_val.brier}{0.167}
\@namedef{VJ@M0_8b.ts_transfer.gqa_val.brier.ci}{[0.156, 0.178]}
\@namedef{VJ@M0_8b.ts_transfer.gqa_val.cov@0.05}{0.780}
\@namedef{VJ@M0_8b.ts_transfer.gqa_val.cov@0.05.ci}{[0.767, 0.793]}
\@namedef{VJ@M0_8b.ts_transfer.gqa_val.cov@0.05.pct}{78.0\%}
\@namedef{VJ@M0_8b.ts_transfer.gqa_val.cov@0.1}{0.940}
\@namedef{VJ@M0_8b.ts_transfer.gqa_val.cov@0.1.ci}{[0.934, 0.947]}
\@namedef{VJ@M0_8b.ts_transfer.gqa_val.cov@0.1.pct}{94.0\%}
\@namedef{VJ@M0_8b.ts_transfer.gqa_val.ece15}{0.013}
\@namedef{VJ@M0_8b.ts_transfer.gqa_val.ece15.ci}{[0.011, 0.023]}
\@namedef{VJ@M0_8b.ts_transfer.gqa_val.nll}{0.302}
\@namedef{VJ@M0_8b.ts_transfer.gqa_val.nll.ci}{[0.285, 0.320]}
\@namedef{VJ@M0_8b.ts_transfer.gqa_val.risk@0.05}{0.046}
\@namedef{VJ@M0_8b.ts_transfer.gqa_val.risk@0.05.ci}{[0.039, 0.052]}
\@namedef{VJ@M0_8b.ts_transfer.gqa_val.risk@0.05.pct}{4.6\%}
\@namedef{VJ@M0_8b.ts_transfer.gqa_val.risk@0.1}{0.090}
\@namedef{VJ@M0_8b.ts_transfer.gqa_val.risk@0.1.ci}{[0.083, 0.099]}
\@namedef{VJ@M0_8b.ts_transfer.gqa_val.risk@0.1.pct}{9.0\%}
\@namedef{VJ@M0_8b.ts_transfer.macro.accuracy}{0.853}
\@namedef{VJ@M0_8b.ts_transfer.macro.accuracy.ci}{[0.846, 0.860]}
\@namedef{VJ@M0_8b.ts_transfer.macro.aurc_maxp}{0.063}
\@namedef{VJ@M0_8b.ts_transfer.macro.aurc_maxp.ci}{[0.056, 0.069]}
\@namedef{VJ@M0_8b.ts_transfer.macro.brier}{0.212}
\@namedef{VJ@M0_8b.ts_transfer.macro.brier.ci}{[0.203, 0.221]}
\@namedef{VJ@M0_8b.ts_transfer.macro.ece15}{0.052}
\@namedef{VJ@M0_8b.ts_transfer.macro.ece15.ci}{[0.048, 0.061]}
\@namedef{VJ@M0_8b.ts_transfer.macro.nll}{0.401}
\@namedef{VJ@M0_8b.ts_transfer.macro.nll.ci}{[0.385, 0.417]}
\@namedef{VJ@M0_8b.ts_transfer.snli_ve.accuracy}{0.695}
\@namedef{VJ@M0_8b.ts_transfer.snli_ve.accuracy.ci}{[0.671, 0.718]}
\@namedef{VJ@M0_8b.ts_transfer.snli_ve.aurc_maxp}{0.190}
\@namedef{VJ@M0_8b.ts_transfer.snli_ve.aurc_maxp.ci}{[0.166, 0.216]}
\@namedef{VJ@M0_8b.ts_transfer.snli_ve.brier}{0.443}
\@namedef{VJ@M0_8b.ts_transfer.snli_ve.brier.ci}{[0.415, 0.472]}
\@namedef{VJ@M0_8b.ts_transfer.snli_ve.cov@0.05}{0.016}
\@namedef{VJ@M0_8b.ts_transfer.snli_ve.cov@0.05.ci}{[0.009, 0.023]}
\@namedef{VJ@M0_8b.ts_transfer.snli_ve.cov@0.05.pct}{1.6\%}
\@namedef{VJ@M0_8b.ts_transfer.snli_ve.cov@0.1}{0.061}
\@namedef{VJ@M0_8b.ts_transfer.snli_ve.cov@0.1.ci}{[0.048, 0.074]}
\@namedef{VJ@M0_8b.ts_transfer.snli_ve.cov@0.1.pct}{6.1\%}
\@namedef{VJ@M0_8b.ts_transfer.snli_ve.ece15}{0.093}
\@namedef{VJ@M0_8b.ts_transfer.snli_ve.ece15.ci}{[0.076, 0.118]}
\@namedef{VJ@M0_8b.ts_transfer.snli_ve.nll}{0.762}
\@namedef{VJ@M0_8b.ts_transfer.snli_ve.nll.ci}{[0.717, 0.809]}
\@namedef{VJ@M0_8b.ts_transfer.snli_ve.risk@0.05}{0.045}
\@namedef{VJ@M0_8b.ts_transfer.snli_ve.risk@0.05.ci}{[0.000, 0.167]}
\@namedef{VJ@M0_8b.ts_transfer.snli_ve.risk@0.05.pct}{4.5\%}
\@namedef{VJ@M0_8b.ts_transfer.snli_ve.risk@0.1}{0.048}
\@namedef{VJ@M0_8b.ts_transfer.snli_ve.risk@0.1.ci}{[0.011, 0.098]}
\@namedef{VJ@M0_8b.ts_transfer.snli_ve.risk@0.1.pct}{4.8\%}
\@namedef{VJ@M0_8b.ts_transfer.tallyqa_l.accuracy}{0.853}
\@namedef{VJ@M0_8b.ts_transfer.tallyqa_l.accuracy.ci}{[0.840, 0.865]}
\@namedef{VJ@M0_8b.ts_transfer.tallyqa_l.aurc_maxp}{0.031}
\@namedef{VJ@M0_8b.ts_transfer.tallyqa_l.aurc_maxp.ci}{[0.026, 0.037]}
\@namedef{VJ@M0_8b.ts_transfer.tallyqa_l.brier}{0.203}
\@namedef{VJ@M0_8b.ts_transfer.tallyqa_l.brier.ci}{[0.189, 0.218]}
\@namedef{VJ@M0_8b.ts_transfer.tallyqa_l.cov@0.05}{0.764}
\@namedef{VJ@M0_8b.ts_transfer.tallyqa_l.cov@0.05.ci}{[0.746, 0.779]}
\@namedef{VJ@M0_8b.ts_transfer.tallyqa_l.cov@0.05.pct}{76.4\%}
\@namedef{VJ@M0_8b.ts_transfer.tallyqa_l.cov@0.1}{0.885}
\@namedef{VJ@M0_8b.ts_transfer.tallyqa_l.cov@0.1.ci}{[0.872, 0.896]}
\@namedef{VJ@M0_8b.ts_transfer.tallyqa_l.cov@0.1.pct}{88.5\%}
\@namedef{VJ@M0_8b.ts_transfer.tallyqa_l.ece15}{0.039}
\@namedef{VJ@M0_8b.ts_transfer.tallyqa_l.ece15.ci}{[0.034, 0.050]}
\@namedef{VJ@M0_8b.ts_transfer.tallyqa_l.nll}{0.416}
\@namedef{VJ@M0_8b.ts_transfer.tallyqa_l.nll.ci}{[0.391, 0.443]}
\@namedef{VJ@M0_8b.ts_transfer.tallyqa_l.risk@0.05}{0.045}
\@namedef{VJ@M0_8b.ts_transfer.tallyqa_l.risk@0.05.ci}{[0.037, 0.054]}
\@namedef{VJ@M0_8b.ts_transfer.tallyqa_l.risk@0.05.pct}{4.5\%}
\@namedef{VJ@M0_8b.ts_transfer.tallyqa_l.risk@0.1}{0.089}
\@namedef{VJ@M0_8b.ts_transfer.tallyqa_l.risk@0.1.ci}{[0.079, 0.100]}
\@namedef{VJ@M0_8b.ts_transfer.tallyqa_l.risk@0.1.pct}{8.9\%}
\@namedef{VJ@M0_8b.ts_transfer.textvqa_k8.accuracy}{0.979}
\@namedef{VJ@M0_8b.ts_transfer.textvqa_k8.accuracy.ci}{[0.973, 0.986]}
\@namedef{VJ@M0_8b.ts_transfer.textvqa_k8.aurc_maxp}{0.001}
\@namedef{VJ@M0_8b.ts_transfer.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@M0_8b.ts_transfer.textvqa_k8.brier}{0.036}
\@namedef{VJ@M0_8b.ts_transfer.textvqa_k8.brier.ci}{[0.028, 0.043]}
\@namedef{VJ@M0_8b.ts_transfer.textvqa_k8.cov@0.05}{1.000}
\@namedef{VJ@M0_8b.ts_transfer.textvqa_k8.cov@0.05.ci}{[1.000, 1.000]}
\@namedef{VJ@M0_8b.ts_transfer.textvqa_k8.cov@0.05.pct}{100.0\%}
\@namedef{VJ@M0_8b.ts_transfer.textvqa_k8.cov@0.1}{1.000}
\@namedef{VJ@M0_8b.ts_transfer.textvqa_k8.cov@0.1.ci}{[1.000, 1.000]}
\@namedef{VJ@M0_8b.ts_transfer.textvqa_k8.cov@0.1.pct}{100.0\%}
\@namedef{VJ@M0_8b.ts_transfer.textvqa_k8.ece15}{0.062}
\@namedef{VJ@M0_8b.ts_transfer.textvqa_k8.ece15.ci}{[0.058, 0.068]}
\@namedef{VJ@M0_8b.ts_transfer.textvqa_k8.nll}{0.122}
\@namedef{VJ@M0_8b.ts_transfer.textvqa_k8.nll.ci}{[0.107, 0.138]}
\@namedef{VJ@M0_8b.ts_transfer.textvqa_k8.risk@0.05}{0.021}
\@namedef{VJ@M0_8b.ts_transfer.textvqa_k8.risk@0.05.ci}{[0.014, 0.027]}
\@namedef{VJ@M0_8b.ts_transfer.textvqa_k8.risk@0.05.pct}{2.1\%}
\@namedef{VJ@M0_8b.ts_transfer.textvqa_k8.risk@0.1}{0.021}
\@namedef{VJ@M0_8b.ts_transfer.textvqa_k8.risk@0.1.ci}{[0.014, 0.027]}
\@namedef{VJ@M0_8b.ts_transfer.textvqa_k8.risk@0.1.pct}{2.1\%}
\@namedef{VJ@M1.raw.gqa_val.accuracy}{0.916}
\@namedef{VJ@M1.raw.gqa_val.accuracy.ci}{[0.910, 0.923]}
\@namedef{VJ@M1.raw.gqa_val.aurc_maxp}{0.014}
\@namedef{VJ@M1.raw.gqa_val.aurc_maxp.ci}{[0.012, 0.016]}
\@namedef{VJ@M1.raw.gqa_val.brier}{0.135}
\@namedef{VJ@M1.raw.gqa_val.brier.ci}{[0.123, 0.146]}
\@namedef{VJ@M1.raw.gqa_val.cov@0.05}{0.890}
\@namedef{VJ@M1.raw.gqa_val.cov@0.05.ci}{[0.881, 0.897]}
\@namedef{VJ@M1.raw.gqa_val.cov@0.05.pct}{89.0\%}
\@namedef{VJ@M1.raw.gqa_val.cov@0.1}{0.999}
\@namedef{VJ@M1.raw.gqa_val.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@M1.raw.gqa_val.cov@0.1.pct}{99.9\%}
\@namedef{VJ@M1.raw.gqa_val.ece15}{0.049}
\@namedef{VJ@M1.raw.gqa_val.ece15.ci}{[0.044, 0.056]}
\@namedef{VJ@M1.raw.gqa_val.errconf09}{53\%}
\@namedef{VJ@M1.raw.gqa_val.nll}{0.264}
\@namedef{VJ@M1.raw.gqa_val.nll.ci}{[0.238, 0.288]}
\@namedef{VJ@M1.raw.gqa_val.risk@0.05}{0.045}
\@namedef{VJ@M1.raw.gqa_val.risk@0.05.ci}{[0.040, 0.051]}
\@namedef{VJ@M1.raw.gqa_val.risk@0.05.pct}{4.5\%}
\@namedef{VJ@M1.raw.gqa_val.risk@0.1}{0.083}
\@namedef{VJ@M1.raw.gqa_val.risk@0.1.ci}{[0.076, 0.090]}
\@namedef{VJ@M1.raw.gqa_val.risk@0.1.pct}{8.3\%}
\@namedef{VJ@M1.raw.macro.accuracy}{0.885}
\@namedef{VJ@M1.raw.macro.accuracy.ci}{[0.879, 0.892]}
\@namedef{VJ@M1.raw.macro.aurc_maxp}{0.030}
\@namedef{VJ@M1.raw.macro.aurc_maxp.ci}{[0.027, 0.034]}
\@namedef{VJ@M1.raw.macro.brier}{0.172}
\@namedef{VJ@M1.raw.macro.brier.ci}{[0.163, 0.182]}
\@namedef{VJ@M1.raw.macro.ece15}{0.047}
\@namedef{VJ@M1.raw.macro.ece15.ci}{[0.043, 0.054]}
\@namedef{VJ@M1.raw.macro.nll}{0.331}
\@namedef{VJ@M1.raw.macro.nll.ci}{[0.312, 0.349]}
\@namedef{VJ@M1.raw.snli_ve.accuracy}{0.808}
\@namedef{VJ@M1.raw.snli_ve.accuracy.ci}{[0.789, 0.827]}
\@namedef{VJ@M1.raw.snli_ve.aurc_maxp}{0.072}
\@namedef{VJ@M1.raw.snli_ve.aurc_maxp.ci}{[0.059, 0.086]}
\@namedef{VJ@M1.raw.snli_ve.brier}{0.289}
\@namedef{VJ@M1.raw.snli_ve.brier.ci}{[0.261, 0.318]}
\@namedef{VJ@M1.raw.snli_ve.cov@0.05}{0.327}
\@namedef{VJ@M1.raw.snli_ve.cov@0.05.ci}{[0.305, 0.349]}
\@namedef{VJ@M1.raw.snli_ve.cov@0.05.pct}{32.7\%}
\@namedef{VJ@M1.raw.snli_ve.cov@0.1}{0.621}
\@namedef{VJ@M1.raw.snli_ve.cov@0.1.ci}{[0.599, 0.644]}
\@namedef{VJ@M1.raw.snli_ve.cov@0.1.pct}{62.1\%}
\@namedef{VJ@M1.raw.snli_ve.ece15}{0.067}
\@namedef{VJ@M1.raw.snli_ve.ece15.ci}{[0.055, 0.088]}
\@namedef{VJ@M1.raw.snli_ve.nll}{0.516}
\@namedef{VJ@M1.raw.snli_ve.nll.ci}{[0.468, 0.566]}
\@namedef{VJ@M1.raw.snli_ve.risk@0.05}{0.038}
\@namedef{VJ@M1.raw.snli_ve.risk@0.05.ci}{[0.025, 0.055]}
\@namedef{VJ@M1.raw.snli_ve.risk@0.05.pct}{3.8\%}
\@namedef{VJ@M1.raw.snli_ve.risk@0.1}{0.079}
\@namedef{VJ@M1.raw.snli_ve.risk@0.1.ci}{[0.063, 0.098]}
\@namedef{VJ@M1.raw.snli_ve.risk@0.1.pct}{7.9\%}
\@namedef{VJ@M1.raw.tallyqa_l.accuracy}{0.841}
\@namedef{VJ@M1.raw.tallyqa_l.accuracy.ci}{[0.828, 0.854]}
\@namedef{VJ@M1.raw.tallyqa_l.aurc_maxp}{0.034}
\@namedef{VJ@M1.raw.tallyqa_l.aurc_maxp.ci}{[0.029, 0.040]}
\@namedef{VJ@M1.raw.tallyqa_l.brier}{0.228}
\@namedef{VJ@M1.raw.tallyqa_l.brier.ci}{[0.211, 0.246]}
\@namedef{VJ@M1.raw.tallyqa_l.cov@0.05}{0.763}
\@namedef{VJ@M1.raw.tallyqa_l.cov@0.05.ci}{[0.747, 0.778]}
\@namedef{VJ@M1.raw.tallyqa_l.cov@0.05.pct}{76.3\%}
\@namedef{VJ@M1.raw.tallyqa_l.cov@0.1}{0.884}
\@namedef{VJ@M1.raw.tallyqa_l.cov@0.1.ci}{[0.874, 0.893]}
\@namedef{VJ@M1.raw.tallyqa_l.cov@0.1.pct}{88.4\%}
\@namedef{VJ@M1.raw.tallyqa_l.ece15}{0.061}
\@namedef{VJ@M1.raw.tallyqa_l.ece15.ci}{[0.052, 0.071]}
\@namedef{VJ@M1.raw.tallyqa_l.nll}{0.445}
\@namedef{VJ@M1.raw.tallyqa_l.nll.ci}{[0.410, 0.481]}
\@namedef{VJ@M1.raw.tallyqa_l.risk@0.05}{0.054}
\@namedef{VJ@M1.raw.tallyqa_l.risk@0.05.ci}{[0.047, 0.063]}
\@namedef{VJ@M1.raw.tallyqa_l.risk@0.05.pct}{5.4\%}
\@namedef{VJ@M1.raw.tallyqa_l.risk@0.1}{0.103}
\@namedef{VJ@M1.raw.tallyqa_l.risk@0.1.ci}{[0.092, 0.113]}
\@namedef{VJ@M1.raw.tallyqa_l.risk@0.1.pct}{10.3\%}
\@namedef{VJ@M1.raw.textvqa_k8.accuracy}{0.975}
\@namedef{VJ@M1.raw.textvqa_k8.accuracy.ci}{[0.968, 0.982]}
\@namedef{VJ@M1.raw.textvqa_k8.aurc_maxp}{0.001}
\@namedef{VJ@M1.raw.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@M1.raw.textvqa_k8.brier}{0.039}
\@namedef{VJ@M1.raw.textvqa_k8.brier.ci}{[0.028, 0.049]}
\@namedef{VJ@M1.raw.textvqa_k8.cov@0.05}{1.000}
\@namedef{VJ@M1.raw.textvqa_k8.cov@0.05.ci}{[0.999, 1.000]}
\@namedef{VJ@M1.raw.textvqa_k8.cov@0.05.pct}{100.0\%}
\@namedef{VJ@M1.raw.textvqa_k8.cov@0.1}{1.000}
\@namedef{VJ@M1.raw.textvqa_k8.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@M1.raw.textvqa_k8.cov@0.1.pct}{100.0\%}
\@namedef{VJ@M1.raw.textvqa_k8.ece15}{0.011}
\@namedef{VJ@M1.raw.textvqa_k8.ece15.ci}{[0.009, 0.018]}
\@namedef{VJ@M1.raw.textvqa_k8.nll}{0.100}
\@namedef{VJ@M1.raw.textvqa_k8.nll.ci}{[0.069, 0.129]}
\@namedef{VJ@M1.raw.textvqa_k8.risk@0.05}{0.025}
\@namedef{VJ@M1.raw.textvqa_k8.risk@0.05.ci}{[0.017, 0.031]}
\@namedef{VJ@M1.raw.textvqa_k8.risk@0.05.pct}{2.5\%}
\@namedef{VJ@M1.raw.textvqa_k8.risk@0.1}{0.025}
\@namedef{VJ@M1.raw.textvqa_k8.risk@0.1.ci}{[0.017, 0.031]}
\@namedef{VJ@M1.raw.textvqa_k8.risk@0.1.pct}{2.5\%}
\@namedef{VJ@M1.ts_local.gqa_val.accuracy}{0.916}
\@namedef{VJ@M1.ts_local.gqa_val.accuracy.ci}{[0.910, 0.923]}
\@namedef{VJ@M1.ts_local.gqa_val.aurc_maxp}{0.014}
\@namedef{VJ@M1.ts_local.gqa_val.aurc_maxp.ci}{[0.012, 0.016]}
\@namedef{VJ@M1.ts_local.gqa_val.brier}{0.124}
\@namedef{VJ@M1.ts_local.gqa_val.brier.ci}{[0.114, 0.133]}
\@namedef{VJ@M1.ts_local.gqa_val.cov@0.05}{0.888}
\@namedef{VJ@M1.ts_local.gqa_val.cov@0.05.ci}{[0.879, 0.896]}
\@namedef{VJ@M1.ts_local.gqa_val.cov@0.05.pct}{88.8\%}
\@namedef{VJ@M1.ts_local.gqa_val.cov@0.1}{0.999}
\@namedef{VJ@M1.ts_local.gqa_val.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@M1.ts_local.gqa_val.cov@0.1.pct}{99.9\%}
\@namedef{VJ@M1.ts_local.gqa_val.ece15}{0.017}
\@namedef{VJ@M1.ts_local.gqa_val.ece15.ci}{[0.015, 0.023]}
\@namedef{VJ@M1.ts_local.gqa_val.nll}{0.221}
\@namedef{VJ@M1.ts_local.gqa_val.nll.ci}{[0.205, 0.236]}
\@namedef{VJ@M1.ts_local.gqa_val.risk@0.05}{0.044}
\@namedef{VJ@M1.ts_local.gqa_val.risk@0.05.ci}{[0.039, 0.050]}
\@namedef{VJ@M1.ts_local.gqa_val.risk@0.05.pct}{4.4\%}
\@namedef{VJ@M1.ts_local.gqa_val.risk@0.1}{0.083}
\@namedef{VJ@M1.ts_local.gqa_val.risk@0.1.ci}{[0.076, 0.090]}
\@namedef{VJ@M1.ts_local.gqa_val.risk@0.1.pct}{8.3\%}
\@namedef{VJ@M1.ts_local.macro.accuracy}{0.885}
\@namedef{VJ@M1.ts_local.macro.accuracy.ci}{[0.879, 0.892]}
\@namedef{VJ@M1.ts_local.macro.aurc_maxp}{0.030}
\@namedef{VJ@M1.ts_local.macro.aurc_maxp.ci}{[0.026, 0.034]}
\@namedef{VJ@M1.ts_local.macro.brier}{0.165}
\@namedef{VJ@M1.ts_local.macro.brier.ci}{[0.156, 0.173]}
\@namedef{VJ@M1.ts_local.macro.ece15}{0.025}
\@namedef{VJ@M1.ts_local.macro.ece15.ci}{[0.025, 0.032]}
\@namedef{VJ@M1.ts_local.macro.nll}{0.309}
\@namedef{VJ@M1.ts_local.macro.nll.ci}{[0.294, 0.323]}
\@namedef{VJ@M1.ts_local.snli_ve.accuracy}{0.808}
\@namedef{VJ@M1.ts_local.snli_ve.accuracy.ci}{[0.789, 0.827]}
\@namedef{VJ@M1.ts_local.snli_ve.aurc_maxp}{0.071}
\@namedef{VJ@M1.ts_local.snli_ve.aurc_maxp.ci}{[0.059, 0.085]}
\@namedef{VJ@M1.ts_local.snli_ve.brier}{0.279}
\@namedef{VJ@M1.ts_local.snli_ve.brier.ci}{[0.255, 0.303]}
\@namedef{VJ@M1.ts_local.snli_ve.cov@0.05}{0.346}
\@namedef{VJ@M1.ts_local.snli_ve.cov@0.05.ci}{[0.324, 0.369]}
\@namedef{VJ@M1.ts_local.snli_ve.cov@0.05.pct}{34.6\%}
\@namedef{VJ@M1.ts_local.snli_ve.cov@0.1}{0.626}
\@namedef{VJ@M1.ts_local.snli_ve.cov@0.1.ci}{[0.604, 0.650]}
\@namedef{VJ@M1.ts_local.snli_ve.cov@0.1.pct}{62.6\%}
\@namedef{VJ@M1.ts_local.snli_ve.ece15}{0.038}
\@namedef{VJ@M1.ts_local.snli_ve.ece15.ci}{[0.032, 0.056]}
\@namedef{VJ@M1.ts_local.snli_ve.nll}{0.496}
\@namedef{VJ@M1.ts_local.snli_ve.nll.ci}{[0.460, 0.532]}
\@namedef{VJ@M1.ts_local.snli_ve.risk@0.05}{0.038}
\@namedef{VJ@M1.ts_local.snli_ve.risk@0.05.ci}{[0.025, 0.054]}
\@namedef{VJ@M1.ts_local.snli_ve.risk@0.05.pct}{3.8\%}
\@namedef{VJ@M1.ts_local.snli_ve.risk@0.1}{0.079}
\@namedef{VJ@M1.ts_local.snli_ve.risk@0.1.ci}{[0.063, 0.096]}
\@namedef{VJ@M1.ts_local.snli_ve.risk@0.1.pct}{7.9\%}
\@namedef{VJ@M1.ts_local.tallyqa_l.accuracy}{0.841}
\@namedef{VJ@M1.ts_local.tallyqa_l.accuracy.ci}{[0.828, 0.854]}
\@namedef{VJ@M1.ts_local.tallyqa_l.aurc_maxp}{0.034}
\@namedef{VJ@M1.ts_local.tallyqa_l.aurc_maxp.ci}{[0.029, 0.040]}
\@namedef{VJ@M1.ts_local.tallyqa_l.brier}{0.219}
\@namedef{VJ@M1.ts_local.tallyqa_l.brier.ci}{[0.203, 0.236]}
\@namedef{VJ@M1.ts_local.tallyqa_l.cov@0.05}{0.764}
\@namedef{VJ@M1.ts_local.tallyqa_l.cov@0.05.ci}{[0.748, 0.779]}
\@namedef{VJ@M1.ts_local.tallyqa_l.cov@0.05.pct}{76.4\%}
\@namedef{VJ@M1.ts_local.tallyqa_l.cov@0.1}{0.887}
\@namedef{VJ@M1.ts_local.tallyqa_l.cov@0.1.ci}{[0.877, 0.897]}
\@namedef{VJ@M1.ts_local.tallyqa_l.cov@0.1.pct}{88.7\%}
\@namedef{VJ@M1.ts_local.tallyqa_l.ece15}{0.038}
\@namedef{VJ@M1.ts_local.tallyqa_l.ece15.ci}{[0.032, 0.048]}
\@namedef{VJ@M1.ts_local.tallyqa_l.nll}{0.426}
\@namedef{VJ@M1.ts_local.tallyqa_l.nll.ci}{[0.397, 0.457]}
\@namedef{VJ@M1.ts_local.tallyqa_l.risk@0.05}{0.053}
\@namedef{VJ@M1.ts_local.tallyqa_l.risk@0.05.ci}{[0.046, 0.061]}
\@namedef{VJ@M1.ts_local.tallyqa_l.risk@0.05.pct}{5.3\%}
\@namedef{VJ@M1.ts_local.tallyqa_l.risk@0.1}{0.103}
\@namedef{VJ@M1.ts_local.tallyqa_l.risk@0.1.ci}{[0.093, 0.114]}
\@namedef{VJ@M1.ts_local.tallyqa_l.risk@0.1.pct}{10.3\%}
\@namedef{VJ@M1.ts_local.textvqa_k8.accuracy}{0.975}
\@namedef{VJ@M1.ts_local.textvqa_k8.accuracy.ci}{[0.968, 0.982]}
\@namedef{VJ@M1.ts_local.textvqa_k8.aurc_maxp}{0.001}
\@namedef{VJ@M1.ts_local.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@M1.ts_local.textvqa_k8.brier}{0.038}
\@namedef{VJ@M1.ts_local.textvqa_k8.brier.ci}{[0.028, 0.048]}
\@namedef{VJ@M1.ts_local.textvqa_k8.cov@0.05}{1.000}
\@namedef{VJ@M1.ts_local.textvqa_k8.cov@0.05.ci}{[0.999, 1.000]}
\@namedef{VJ@M1.ts_local.textvqa_k8.cov@0.05.pct}{100.0\%}
\@namedef{VJ@M1.ts_local.textvqa_k8.cov@0.1}{1.000}
\@namedef{VJ@M1.ts_local.textvqa_k8.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@M1.ts_local.textvqa_k8.cov@0.1.pct}{100.0\%}
\@namedef{VJ@M1.ts_local.textvqa_k8.ece15}{0.008}
\@namedef{VJ@M1.ts_local.textvqa_k8.ece15.ci}{[0.008, 0.015]}
\@namedef{VJ@M1.ts_local.textvqa_k8.nll}{0.093}
\@namedef{VJ@M1.ts_local.textvqa_k8.nll.ci}{[0.067, 0.118]}
\@namedef{VJ@M1.ts_local.textvqa_k8.risk@0.05}{0.025}
\@namedef{VJ@M1.ts_local.textvqa_k8.risk@0.05.ci}{[0.017, 0.031]}
\@namedef{VJ@M1.ts_local.textvqa_k8.risk@0.05.pct}{2.5\%}
\@namedef{VJ@M1.ts_local.textvqa_k8.risk@0.1}{0.025}
\@namedef{VJ@M1.ts_local.textvqa_k8.risk@0.1.ci}{[0.017, 0.031]}
\@namedef{VJ@M1.ts_local.textvqa_k8.risk@0.1.pct}{2.5\%}
\@namedef{VJ@M1.ts_transfer.gqa_val.accuracy}{0.916}
\@namedef{VJ@M1.ts_transfer.gqa_val.accuracy.ci}{[0.910, 0.923]}
\@namedef{VJ@M1.ts_transfer.gqa_val.aurc_maxp}{0.014}
\@namedef{VJ@M1.ts_transfer.gqa_val.aurc_maxp.ci}{[0.012, 0.016]}
\@namedef{VJ@M1.ts_transfer.gqa_val.brier}{0.124}
\@namedef{VJ@M1.ts_transfer.gqa_val.brier.ci}{[0.114, 0.134]}
\@namedef{VJ@M1.ts_transfer.gqa_val.cov@0.05}{0.889}
\@namedef{VJ@M1.ts_transfer.gqa_val.cov@0.05.ci}{[0.880, 0.897]}
\@namedef{VJ@M1.ts_transfer.gqa_val.cov@0.05.pct}{88.9\%}
\@namedef{VJ@M1.ts_transfer.gqa_val.cov@0.1}{0.999}
\@namedef{VJ@M1.ts_transfer.gqa_val.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@M1.ts_transfer.gqa_val.cov@0.1.pct}{99.9\%}
\@namedef{VJ@M1.ts_transfer.gqa_val.ece15}{0.017}
\@namedef{VJ@M1.ts_transfer.gqa_val.ece15.ci}{[0.015, 0.023]}
\@namedef{VJ@M1.ts_transfer.gqa_val.nll}{0.221}
\@namedef{VJ@M1.ts_transfer.gqa_val.nll.ci}{[0.204, 0.236]}
\@namedef{VJ@M1.ts_transfer.gqa_val.risk@0.05}{0.045}
\@namedef{VJ@M1.ts_transfer.gqa_val.risk@0.05.ci}{[0.039, 0.050]}
\@namedef{VJ@M1.ts_transfer.gqa_val.risk@0.05.pct}{4.5\%}
\@namedef{VJ@M1.ts_transfer.gqa_val.risk@0.1}{0.083}
\@namedef{VJ@M1.ts_transfer.gqa_val.risk@0.1.ci}{[0.076, 0.090]}
\@namedef{VJ@M1.ts_transfer.gqa_val.risk@0.1.pct}{8.3\%}
\@namedef{VJ@M1.ts_transfer.macro.accuracy}{0.885}
\@namedef{VJ@M1.ts_transfer.macro.accuracy.ci}{[0.879, 0.892]}
\@namedef{VJ@M1.ts_transfer.macro.aurc_maxp}{0.030}
\@namedef{VJ@M1.ts_transfer.macro.aurc_maxp.ci}{[0.026, 0.033]}
\@namedef{VJ@M1.ts_transfer.macro.brier}{0.166}
\@namedef{VJ@M1.ts_transfer.macro.brier.ci}{[0.158, 0.173]}
\@namedef{VJ@M1.ts_transfer.macro.ece15}{0.037}
\@namedef{VJ@M1.ts_transfer.macro.ece15.ci}{[0.036, 0.044]}
\@namedef{VJ@M1.ts_transfer.macro.nll}{0.319}
\@namedef{VJ@M1.ts_transfer.macro.nll.ci}{[0.306, 0.332]}
\@namedef{VJ@M1.ts_transfer.snli_ve.accuracy}{0.808}
\@namedef{VJ@M1.ts_transfer.snli_ve.accuracy.ci}{[0.789, 0.827]}
\@namedef{VJ@M1.ts_transfer.snli_ve.aurc_maxp}{0.071}
\@namedef{VJ@M1.ts_transfer.snli_ve.aurc_maxp.ci}{[0.058, 0.085]}
\@namedef{VJ@M1.ts_transfer.snli_ve.brier}{0.282}
\@namedef{VJ@M1.ts_transfer.snli_ve.brier.ci}{[0.260, 0.304]}
\@namedef{VJ@M1.ts_transfer.snli_ve.cov@0.05}{0.347}
\@namedef{VJ@M1.ts_transfer.snli_ve.cov@0.05.ci}{[0.325, 0.370]}
\@namedef{VJ@M1.ts_transfer.snli_ve.cov@0.05.pct}{34.7\%}
\@namedef{VJ@M1.ts_transfer.snli_ve.cov@0.1}{0.623}
\@namedef{VJ@M1.ts_transfer.snli_ve.cov@0.1.ci}{[0.600, 0.646]}
\@namedef{VJ@M1.ts_transfer.snli_ve.cov@0.1.pct}{62.3\%}
\@namedef{VJ@M1.ts_transfer.snli_ve.ece15}{0.055}
\@namedef{VJ@M1.ts_transfer.snli_ve.ece15.ci}{[0.047, 0.071]}
\@namedef{VJ@M1.ts_transfer.snli_ve.nll}{0.507}
\@namedef{VJ@M1.ts_transfer.snli_ve.nll.ci}{[0.475, 0.539]}
\@namedef{VJ@M1.ts_transfer.snli_ve.risk@0.05}{0.039}
\@namedef{VJ@M1.ts_transfer.snli_ve.risk@0.05.ci}{[0.025, 0.056]}
\@namedef{VJ@M1.ts_transfer.snli_ve.risk@0.05.pct}{3.9\%}
\@namedef{VJ@M1.ts_transfer.snli_ve.risk@0.1}{0.077}
\@namedef{VJ@M1.ts_transfer.snli_ve.risk@0.1.ci}{[0.062, 0.095]}
\@namedef{VJ@M1.ts_transfer.snli_ve.risk@0.1.pct}{7.7\%}
\@namedef{VJ@M1.ts_transfer.tallyqa_l.accuracy}{0.841}
\@namedef{VJ@M1.ts_transfer.tallyqa_l.accuracy.ci}{[0.828, 0.854]}
\@namedef{VJ@M1.ts_transfer.tallyqa_l.aurc_maxp}{0.034}
\@namedef{VJ@M1.ts_transfer.tallyqa_l.aurc_maxp.ci}{[0.029, 0.040]}
\@namedef{VJ@M1.ts_transfer.tallyqa_l.brier}{0.219}
\@namedef{VJ@M1.ts_transfer.tallyqa_l.brier.ci}{[0.205, 0.234]}
\@namedef{VJ@M1.ts_transfer.tallyqa_l.cov@0.05}{0.765}
\@namedef{VJ@M1.ts_transfer.tallyqa_l.cov@0.05.ci}{[0.749, 0.780]}
\@namedef{VJ@M1.ts_transfer.tallyqa_l.cov@0.05.pct}{76.5\%}
\@namedef{VJ@M1.ts_transfer.tallyqa_l.cov@0.1}{0.884}
\@namedef{VJ@M1.ts_transfer.tallyqa_l.cov@0.1.ci}{[0.873, 0.894]}
\@namedef{VJ@M1.ts_transfer.tallyqa_l.cov@0.1.pct}{88.4\%}
\@namedef{VJ@M1.ts_transfer.tallyqa_l.ece15}{0.054}
\@namedef{VJ@M1.ts_transfer.tallyqa_l.ece15.ci}{[0.051, 0.064]}
\@namedef{VJ@M1.ts_transfer.tallyqa_l.nll}{0.450}
\@namedef{VJ@M1.ts_transfer.tallyqa_l.nll.ci}{[0.424, 0.476]}
\@namedef{VJ@M1.ts_transfer.tallyqa_l.risk@0.05}{0.053}
\@namedef{VJ@M1.ts_transfer.tallyqa_l.risk@0.05.ci}{[0.046, 0.061]}
\@namedef{VJ@M1.ts_transfer.tallyqa_l.risk@0.05.pct}{5.3\%}
\@namedef{VJ@M1.ts_transfer.tallyqa_l.risk@0.1}{0.102}
\@namedef{VJ@M1.ts_transfer.tallyqa_l.risk@0.1.ci}{[0.092, 0.112]}
\@namedef{VJ@M1.ts_transfer.tallyqa_l.risk@0.1.pct}{10.2\%}
\@namedef{VJ@M1.ts_transfer.textvqa_k8.accuracy}{0.975}
\@namedef{VJ@M1.ts_transfer.textvqa_k8.accuracy.ci}{[0.968, 0.982]}
\@namedef{VJ@M1.ts_transfer.textvqa_k8.aurc_maxp}{0.001}
\@namedef{VJ@M1.ts_transfer.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@M1.ts_transfer.textvqa_k8.brier}{0.038}
\@namedef{VJ@M1.ts_transfer.textvqa_k8.brier.ci}{[0.028, 0.048]}
\@namedef{VJ@M1.ts_transfer.textvqa_k8.cov@0.05}{1.000}
\@namedef{VJ@M1.ts_transfer.textvqa_k8.cov@0.05.ci}{[0.999, 1.000]}
\@namedef{VJ@M1.ts_transfer.textvqa_k8.cov@0.05.pct}{100.0\%}
\@namedef{VJ@M1.ts_transfer.textvqa_k8.cov@0.1}{1.000}
\@namedef{VJ@M1.ts_transfer.textvqa_k8.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@M1.ts_transfer.textvqa_k8.cov@0.1.pct}{100.0\%}
\@namedef{VJ@M1.ts_transfer.textvqa_k8.ece15}{0.021}
\@namedef{VJ@M1.ts_transfer.textvqa_k8.ece15.ci}{[0.020, 0.027]}
\@namedef{VJ@M1.ts_transfer.textvqa_k8.nll}{0.100}
\@namedef{VJ@M1.ts_transfer.textvqa_k8.nll.ci}{[0.079, 0.122]}
\@namedef{VJ@M1.ts_transfer.textvqa_k8.risk@0.05}{0.025}
\@namedef{VJ@M1.ts_transfer.textvqa_k8.risk@0.05.ci}{[0.017, 0.031]}
\@namedef{VJ@M1.ts_transfer.textvqa_k8.risk@0.05.pct}{2.5\%}
\@namedef{VJ@M1.ts_transfer.textvqa_k8.risk@0.1}{0.025}
\@namedef{VJ@M1.ts_transfer.textvqa_k8.risk@0.1.ci}{[0.017, 0.031]}
\@namedef{VJ@M1.ts_transfer.textvqa_k8.risk@0.1.pct}{2.5\%}
\@namedef{VJ@M1_8b.raw.gqa_val.accuracy}{0.919}
\@namedef{VJ@M1_8b.raw.gqa_val.accuracy.ci}{[0.912, 0.926]}
\@namedef{VJ@M1_8b.raw.gqa_val.aurc_maxp}{0.012}
\@namedef{VJ@M1_8b.raw.gqa_val.aurc_maxp.ci}{[0.010, 0.014]}
\@namedef{VJ@M1_8b.raw.gqa_val.brier}{0.128}
\@namedef{VJ@M1_8b.raw.gqa_val.brier.ci}{[0.116, 0.139]}
\@namedef{VJ@M1_8b.raw.gqa_val.cov@0.05}{0.891}
\@namedef{VJ@M1_8b.raw.gqa_val.cov@0.05.ci}{[0.882, 0.898]}
\@namedef{VJ@M1_8b.raw.gqa_val.cov@0.05.pct}{89.1\%}
\@namedef{VJ@M1_8b.raw.gqa_val.cov@0.1}{0.999}
\@namedef{VJ@M1_8b.raw.gqa_val.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@M1_8b.raw.gqa_val.cov@0.1.pct}{99.9\%}
\@namedef{VJ@M1_8b.raw.gqa_val.ece15}{0.045}
\@namedef{VJ@M1_8b.raw.gqa_val.ece15.ci}{[0.039, 0.051]}
\@namedef{VJ@M1_8b.raw.gqa_val.nll}{0.236}
\@namedef{VJ@M1_8b.raw.gqa_val.nll.ci}{[0.214, 0.257]}
\@namedef{VJ@M1_8b.raw.gqa_val.risk@0.05}{0.041}
\@namedef{VJ@M1_8b.raw.gqa_val.risk@0.05.ci}{[0.035, 0.046]}
\@namedef{VJ@M1_8b.raw.gqa_val.risk@0.05.pct}{4.1\%}
\@namedef{VJ@M1_8b.raw.gqa_val.risk@0.1}{0.081}
\@namedef{VJ@M1_8b.raw.gqa_val.risk@0.1.ci}{[0.074, 0.088]}
\@namedef{VJ@M1_8b.raw.gqa_val.risk@0.1.pct}{8.1\%}
\@namedef{VJ@M1_8b.raw.macro.accuracy}{0.893}
\@namedef{VJ@M1_8b.raw.macro.accuracy.ci}{[0.886, 0.898]}
\@namedef{VJ@M1_8b.raw.macro.aurc_maxp}{0.027}
\@namedef{VJ@M1_8b.raw.macro.aurc_maxp.ci}{[0.024, 0.031]}
\@namedef{VJ@M1_8b.raw.macro.brier}{0.158}
\@namedef{VJ@M1_8b.raw.macro.brier.ci}{[0.150, 0.167]}
\@namedef{VJ@M1_8b.raw.macro.ece15}{0.037}
\@namedef{VJ@M1_8b.raw.macro.ece15.ci}{[0.034, 0.044]}
\@namedef{VJ@M1_8b.raw.macro.nll}{0.298}
\@namedef{VJ@M1_8b.raw.macro.nll.ci}{[0.281, 0.314]}
\@namedef{VJ@M1_8b.raw.snli_ve.accuracy}{0.818}
\@namedef{VJ@M1_8b.raw.snli_ve.accuracy.ci}{[0.798, 0.837]}
\@namedef{VJ@M1_8b.raw.snli_ve.aurc_maxp}{0.067}
\@namedef{VJ@M1_8b.raw.snli_ve.aurc_maxp.ci}{[0.055, 0.080]}
\@namedef{VJ@M1_8b.raw.snli_ve.brier}{0.269}
\@namedef{VJ@M1_8b.raw.snli_ve.brier.ci}{[0.243, 0.295]}
\@namedef{VJ@M1_8b.raw.snli_ve.cov@0.05}{0.349}
\@namedef{VJ@M1_8b.raw.snli_ve.cov@0.05.ci}{[0.328, 0.370]}
\@namedef{VJ@M1_8b.raw.snli_ve.cov@0.05.pct}{34.9\%}
\@namedef{VJ@M1_8b.raw.snli_ve.cov@0.1}{0.630}
\@namedef{VJ@M1_8b.raw.snli_ve.cov@0.1.ci}{[0.608, 0.652]}
\@namedef{VJ@M1_8b.raw.snli_ve.cov@0.1.pct}{63.0\%}
\@namedef{VJ@M1_8b.raw.snli_ve.ece15}{0.051}
\@namedef{VJ@M1_8b.raw.snli_ve.ece15.ci}{[0.040, 0.070]}
\@namedef{VJ@M1_8b.raw.snli_ve.nll}{0.480}
\@namedef{VJ@M1_8b.raw.snli_ve.nll.ci}{[0.435, 0.527]}
\@namedef{VJ@M1_8b.raw.snli_ve.risk@0.05}{0.043}
\@namedef{VJ@M1_8b.raw.snli_ve.risk@0.05.ci}{[0.028, 0.059]}
\@namedef{VJ@M1_8b.raw.snli_ve.risk@0.05.pct}{4.3\%}
\@namedef{VJ@M1_8b.raw.snli_ve.risk@0.1}{0.077}
\@namedef{VJ@M1_8b.raw.snli_ve.risk@0.1.ci}{[0.061, 0.094]}
\@namedef{VJ@M1_8b.raw.snli_ve.risk@0.1.pct}{7.7\%}
\@namedef{VJ@M1_8b.raw.tallyqa_l.accuracy}{0.855}
\@namedef{VJ@M1_8b.raw.tallyqa_l.accuracy.ci}{[0.843, 0.867]}
\@namedef{VJ@M1_8b.raw.tallyqa_l.aurc_maxp}{0.029}
\@namedef{VJ@M1_8b.raw.tallyqa_l.aurc_maxp.ci}{[0.025, 0.033]}
\@namedef{VJ@M1_8b.raw.tallyqa_l.brier}{0.206}
\@namedef{VJ@M1_8b.raw.tallyqa_l.brier.ci}{[0.190, 0.222]}
\@namedef{VJ@M1_8b.raw.tallyqa_l.cov@0.05}{0.792}
\@namedef{VJ@M1_8b.raw.tallyqa_l.cov@0.05.ci}{[0.776, 0.805]}
\@namedef{VJ@M1_8b.raw.tallyqa_l.cov@0.05.pct}{79.2\%}
\@namedef{VJ@M1_8b.raw.tallyqa_l.cov@0.1}{0.922}
\@namedef{VJ@M1_8b.raw.tallyqa_l.cov@0.1.ci}{[0.914, 0.930]}
\@namedef{VJ@M1_8b.raw.tallyqa_l.cov@0.1.pct}{92.2\%}
\@namedef{VJ@M1_8b.raw.tallyqa_l.ece15}{0.044}
\@namedef{VJ@M1_8b.raw.tallyqa_l.ece15.ci}{[0.036, 0.054]}
\@namedef{VJ@M1_8b.raw.tallyqa_l.nll}{0.398}
\@namedef{VJ@M1_8b.raw.tallyqa_l.nll.ci}{[0.367, 0.431]}
\@namedef{VJ@M1_8b.raw.tallyqa_l.risk@0.05}{0.056}
\@namedef{VJ@M1_8b.raw.tallyqa_l.risk@0.05.ci}{[0.049, 0.065]}
\@namedef{VJ@M1_8b.raw.tallyqa_l.risk@0.05.pct}{5.6\%}
\@namedef{VJ@M1_8b.raw.tallyqa_l.risk@0.1}{0.107}
\@namedef{VJ@M1_8b.raw.tallyqa_l.risk@0.1.ci}{[0.096, 0.117]}
\@namedef{VJ@M1_8b.raw.tallyqa_l.risk@0.1.pct}{10.7\%}
\@namedef{VJ@M1_8b.raw.textvqa_k8.accuracy}{0.979}
\@namedef{VJ@M1_8b.raw.textvqa_k8.accuracy.ci}{[0.972, 0.985]}
\@namedef{VJ@M1_8b.raw.textvqa_k8.aurc_maxp}{0.000}
\@namedef{VJ@M1_8b.raw.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@M1_8b.raw.textvqa_k8.brier}{0.032}
\@namedef{VJ@M1_8b.raw.textvqa_k8.brier.ci}{[0.022, 0.041]}
\@namedef{VJ@M1_8b.raw.textvqa_k8.cov@0.05}{0.999}
\@namedef{VJ@M1_8b.raw.textvqa_k8.cov@0.05.ci}{[0.999, 1.000]}
\@namedef{VJ@M1_8b.raw.textvqa_k8.cov@0.05.pct}{99.9\%}
\@namedef{VJ@M1_8b.raw.textvqa_k8.cov@0.1}{0.999}
\@namedef{VJ@M1_8b.raw.textvqa_k8.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@M1_8b.raw.textvqa_k8.cov@0.1.pct}{99.9\%}
\@namedef{VJ@M1_8b.raw.textvqa_k8.ece15}{0.010}
\@namedef{VJ@M1_8b.raw.textvqa_k8.ece15.ci}{[0.008, 0.016]}
\@namedef{VJ@M1_8b.raw.textvqa_k8.nll}{0.078}
\@namedef{VJ@M1_8b.raw.textvqa_k8.nll.ci}{[0.053, 0.102]}
\@namedef{VJ@M1_8b.raw.textvqa_k8.risk@0.05}{0.021}
\@namedef{VJ@M1_8b.raw.textvqa_k8.risk@0.05.ci}{[0.015, 0.027]}
\@namedef{VJ@M1_8b.raw.textvqa_k8.risk@0.05.pct}{2.1\%}
\@namedef{VJ@M1_8b.raw.textvqa_k8.risk@0.1}{0.021}
\@namedef{VJ@M1_8b.raw.textvqa_k8.risk@0.1.ci}{[0.015, 0.027]}
\@namedef{VJ@M1_8b.raw.textvqa_k8.risk@0.1.pct}{2.1\%}
\@namedef{VJ@M1_8b.ts_local.gqa_val.accuracy}{0.919}
\@namedef{VJ@M1_8b.ts_local.gqa_val.accuracy.ci}{[0.912, 0.926]}
\@namedef{VJ@M1_8b.ts_local.gqa_val.aurc_maxp}{0.012}
\@namedef{VJ@M1_8b.ts_local.gqa_val.aurc_maxp.ci}{[0.010, 0.014]}
\@namedef{VJ@M1_8b.ts_local.gqa_val.brier}{0.118}
\@namedef{VJ@M1_8b.ts_local.gqa_val.brier.ci}{[0.109, 0.128]}
\@namedef{VJ@M1_8b.ts_local.gqa_val.cov@0.05}{0.890}
\@namedef{VJ@M1_8b.ts_local.gqa_val.cov@0.05.ci}{[0.881, 0.898]}
\@namedef{VJ@M1_8b.ts_local.gqa_val.cov@0.05.pct}{89.0\%}
\@namedef{VJ@M1_8b.ts_local.gqa_val.cov@0.1}{0.999}
\@namedef{VJ@M1_8b.ts_local.gqa_val.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@M1_8b.ts_local.gqa_val.cov@0.1.pct}{99.9\%}
\@namedef{VJ@M1_8b.ts_local.gqa_val.ece15}{0.022}
\@namedef{VJ@M1_8b.ts_local.gqa_val.ece15.ci}{[0.019, 0.028]}
\@namedef{VJ@M1_8b.ts_local.gqa_val.nll}{0.208}
\@namedef{VJ@M1_8b.ts_local.gqa_val.nll.ci}{[0.194, 0.223]}
\@namedef{VJ@M1_8b.ts_local.gqa_val.risk@0.05}{0.041}
\@namedef{VJ@M1_8b.ts_local.gqa_val.risk@0.05.ci}{[0.036, 0.046]}
\@namedef{VJ@M1_8b.ts_local.gqa_val.risk@0.05.pct}{4.1\%}
\@namedef{VJ@M1_8b.ts_local.gqa_val.risk@0.1}{0.081}
\@namedef{VJ@M1_8b.ts_local.gqa_val.risk@0.1.ci}{[0.074, 0.088]}
\@namedef{VJ@M1_8b.ts_local.gqa_val.risk@0.1.pct}{8.1\%}
\@namedef{VJ@M1_8b.ts_local.macro.accuracy}{0.893}
\@namedef{VJ@M1_8b.ts_local.macro.accuracy.ci}{[0.886, 0.898]}
\@namedef{VJ@M1_8b.ts_local.macro.aurc_maxp}{0.027}
\@namedef{VJ@M1_8b.ts_local.macro.aurc_maxp.ci}{[0.024, 0.031]}
\@namedef{VJ@M1_8b.ts_local.macro.brier}{0.154}
\@namedef{VJ@M1_8b.ts_local.macro.brier.ci}{[0.146, 0.161]}
\@namedef{VJ@M1_8b.ts_local.macro.ece15}{0.021}
\@namedef{VJ@M1_8b.ts_local.macro.ece15.ci}{[0.022, 0.029]}
\@namedef{VJ@M1_8b.ts_local.macro.nll}{0.285}
\@namedef{VJ@M1_8b.ts_local.macro.nll.ci}{[0.271, 0.297]}
\@namedef{VJ@M1_8b.ts_local.snli_ve.accuracy}{0.818}
\@namedef{VJ@M1_8b.ts_local.snli_ve.accuracy.ci}{[0.798, 0.837]}
\@namedef{VJ@M1_8b.ts_local.snli_ve.aurc_maxp}{0.067}
\@namedef{VJ@M1_8b.ts_local.snli_ve.aurc_maxp.ci}{[0.055, 0.080]}
\@namedef{VJ@M1_8b.ts_local.snli_ve.brier}{0.264}
\@namedef{VJ@M1_8b.ts_local.snli_ve.brier.ci}{[0.242, 0.288]}
\@namedef{VJ@M1_8b.ts_local.snli_ve.cov@0.05}{0.351}
\@namedef{VJ@M1_8b.ts_local.snli_ve.cov@0.05.ci}{[0.329, 0.371]}
\@namedef{VJ@M1_8b.ts_local.snli_ve.cov@0.05.pct}{35.1\%}
\@namedef{VJ@M1_8b.ts_local.snli_ve.cov@0.1}{0.631}
\@namedef{VJ@M1_8b.ts_local.snli_ve.cov@0.1.ci}{[0.609, 0.652]}
\@namedef{VJ@M1_8b.ts_local.snli_ve.cov@0.1.pct}{63.1\%}
\@namedef{VJ@M1_8b.ts_local.snli_ve.ece15}{0.034}
\@namedef{VJ@M1_8b.ts_local.snli_ve.ece15.ci}{[0.032, 0.052]}
\@namedef{VJ@M1_8b.ts_local.snli_ve.nll}{0.471}
\@namedef{VJ@M1_8b.ts_local.snli_ve.nll.ci}{[0.435, 0.506]}
\@namedef{VJ@M1_8b.ts_local.snli_ve.risk@0.05}{0.041}
\@namedef{VJ@M1_8b.ts_local.snli_ve.risk@0.05.ci}{[0.027, 0.057]}
\@namedef{VJ@M1_8b.ts_local.snli_ve.risk@0.05.pct}{4.1\%}
\@namedef{VJ@M1_8b.ts_local.snli_ve.risk@0.1}{0.079}
\@namedef{VJ@M1_8b.ts_local.snli_ve.risk@0.1.ci}{[0.063, 0.095]}
\@namedef{VJ@M1_8b.ts_local.snli_ve.risk@0.1.pct}{7.9\%}
\@namedef{VJ@M1_8b.ts_local.tallyqa_l.accuracy}{0.855}
\@namedef{VJ@M1_8b.ts_local.tallyqa_l.accuracy.ci}{[0.843, 0.867]}
\@namedef{VJ@M1_8b.ts_local.tallyqa_l.aurc_maxp}{0.028}
\@namedef{VJ@M1_8b.ts_local.tallyqa_l.aurc_maxp.ci}{[0.024, 0.033]}
\@namedef{VJ@M1_8b.ts_local.tallyqa_l.brier}{0.201}
\@namedef{VJ@M1_8b.ts_local.tallyqa_l.brier.ci}{[0.186, 0.216]}
\@namedef{VJ@M1_8b.ts_local.tallyqa_l.cov@0.05}{0.790}
\@namedef{VJ@M1_8b.ts_local.tallyqa_l.cov@0.05.ci}{[0.775, 0.803]}
\@namedef{VJ@M1_8b.ts_local.tallyqa_l.cov@0.05.pct}{79.0\%}
\@namedef{VJ@M1_8b.ts_local.tallyqa_l.cov@0.1}{0.922}
\@namedef{VJ@M1_8b.ts_local.tallyqa_l.cov@0.1.ci}{[0.914, 0.930]}
\@namedef{VJ@M1_8b.ts_local.tallyqa_l.cov@0.1.pct}{92.2\%}
\@namedef{VJ@M1_8b.ts_local.tallyqa_l.ece15}{0.024}
\@namedef{VJ@M1_8b.ts_local.tallyqa_l.ece15.ci}{[0.020, 0.034]}
\@namedef{VJ@M1_8b.ts_local.tallyqa_l.nll}{0.387}
\@namedef{VJ@M1_8b.ts_local.tallyqa_l.nll.ci}{[0.358, 0.415]}
\@namedef{VJ@M1_8b.ts_local.tallyqa_l.risk@0.05}{0.055}
\@namedef{VJ@M1_8b.ts_local.tallyqa_l.risk@0.05.ci}{[0.048, 0.064]}
\@namedef{VJ@M1_8b.ts_local.tallyqa_l.risk@0.05.pct}{5.5\%}
\@namedef{VJ@M1_8b.ts_local.tallyqa_l.risk@0.1}{0.106}
\@namedef{VJ@M1_8b.ts_local.tallyqa_l.risk@0.1.ci}{[0.096, 0.117]}
\@namedef{VJ@M1_8b.ts_local.tallyqa_l.risk@0.1.pct}{10.6\%}
\@namedef{VJ@M1_8b.ts_local.textvqa_k8.accuracy}{0.979}
\@namedef{VJ@M1_8b.ts_local.textvqa_k8.accuracy.ci}{[0.972, 0.985]}
\@namedef{VJ@M1_8b.ts_local.textvqa_k8.aurc_maxp}{0.000}
\@namedef{VJ@M1_8b.ts_local.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@M1_8b.ts_local.textvqa_k8.brier}{0.031}
\@namedef{VJ@M1_8b.ts_local.textvqa_k8.brier.ci}{[0.022, 0.040]}
\@namedef{VJ@M1_8b.ts_local.textvqa_k8.cov@0.05}{0.999}
\@namedef{VJ@M1_8b.ts_local.textvqa_k8.cov@0.05.ci}{[0.999, 1.000]}
\@namedef{VJ@M1_8b.ts_local.textvqa_k8.cov@0.05.pct}{99.9\%}
\@namedef{VJ@M1_8b.ts_local.textvqa_k8.cov@0.1}{0.999}
\@namedef{VJ@M1_8b.ts_local.textvqa_k8.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@M1_8b.ts_local.textvqa_k8.cov@0.1.pct}{99.9\%}
\@namedef{VJ@M1_8b.ts_local.textvqa_k8.ece15}{0.006}
\@namedef{VJ@M1_8b.ts_local.textvqa_k8.ece15.ci}{[0.006, 0.012]}
\@namedef{VJ@M1_8b.ts_local.textvqa_k8.nll}{0.073}
\@namedef{VJ@M1_8b.ts_local.textvqa_k8.nll.ci}{[0.051, 0.094]}
\@namedef{VJ@M1_8b.ts_local.textvqa_k8.risk@0.05}{0.021}
\@namedef{VJ@M1_8b.ts_local.textvqa_k8.risk@0.05.ci}{[0.015, 0.027]}
\@namedef{VJ@M1_8b.ts_local.textvqa_k8.risk@0.05.pct}{2.1\%}
\@namedef{VJ@M1_8b.ts_local.textvqa_k8.risk@0.1}{0.021}
\@namedef{VJ@M1_8b.ts_local.textvqa_k8.risk@0.1.ci}{[0.015, 0.027]}
\@namedef{VJ@M1_8b.ts_local.textvqa_k8.risk@0.1.pct}{2.1\%}
\@namedef{VJ@M1_8b.ts_transfer.gqa_val.accuracy}{0.919}
\@namedef{VJ@M1_8b.ts_transfer.gqa_val.accuracy.ci}{[0.912, 0.926]}
\@namedef{VJ@M1_8b.ts_transfer.gqa_val.aurc_maxp}{0.012}
\@namedef{VJ@M1_8b.ts_transfer.gqa_val.aurc_maxp.ci}{[0.010, 0.014]}
\@namedef{VJ@M1_8b.ts_transfer.gqa_val.brier}{0.119}
\@namedef{VJ@M1_8b.ts_transfer.gqa_val.brier.ci}{[0.109, 0.128]}
\@namedef{VJ@M1_8b.ts_transfer.gqa_val.cov@0.05}{0.892}
\@namedef{VJ@M1_8b.ts_transfer.gqa_val.cov@0.05.ci}{[0.883, 0.900]}
\@namedef{VJ@M1_8b.ts_transfer.gqa_val.cov@0.05.pct}{89.2\%}
\@namedef{VJ@M1_8b.ts_transfer.gqa_val.cov@0.1}{0.999}
\@namedef{VJ@M1_8b.ts_transfer.gqa_val.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@M1_8b.ts_transfer.gqa_val.cov@0.1.pct}{99.9\%}
\@namedef{VJ@M1_8b.ts_transfer.gqa_val.ece15}{0.022}
\@namedef{VJ@M1_8b.ts_transfer.gqa_val.ece15.ci}{[0.018, 0.027]}
\@namedef{VJ@M1_8b.ts_transfer.gqa_val.nll}{0.207}
\@namedef{VJ@M1_8b.ts_transfer.gqa_val.nll.ci}{[0.193, 0.223]}
\@namedef{VJ@M1_8b.ts_transfer.gqa_val.risk@0.05}{0.041}
\@namedef{VJ@M1_8b.ts_transfer.gqa_val.risk@0.05.ci}{[0.036, 0.047]}
\@namedef{VJ@M1_8b.ts_transfer.gqa_val.risk@0.05.pct}{4.1\%}
\@namedef{VJ@M1_8b.ts_transfer.gqa_val.risk@0.1}{0.081}
\@namedef{VJ@M1_8b.ts_transfer.gqa_val.risk@0.1.ci}{[0.074, 0.088]}
\@namedef{VJ@M1_8b.ts_transfer.gqa_val.risk@0.1.pct}{8.1\%}
\@namedef{VJ@M1_8b.ts_transfer.macro.accuracy}{0.893}
\@namedef{VJ@M1_8b.ts_transfer.macro.accuracy.ci}{[0.886, 0.898]}
\@namedef{VJ@M1_8b.ts_transfer.macro.aurc_maxp}{0.027}
\@namedef{VJ@M1_8b.ts_transfer.macro.aurc_maxp.ci}{[0.024, 0.031]}
\@namedef{VJ@M1_8b.ts_transfer.macro.brier}{0.154}
\@namedef{VJ@M1_8b.ts_transfer.macro.brier.ci}{[0.147, 0.162]}
\@namedef{VJ@M1_8b.ts_transfer.macro.ece15}{0.033}
\@namedef{VJ@M1_8b.ts_transfer.macro.ece15.ci}{[0.033, 0.040]}
\@namedef{VJ@M1_8b.ts_transfer.macro.nll}{0.293}
\@namedef{VJ@M1_8b.ts_transfer.macro.nll.ci}{[0.281, 0.304]}
\@namedef{VJ@M1_8b.ts_transfer.snli_ve.accuracy}{0.818}
\@namedef{VJ@M1_8b.ts_transfer.snli_ve.accuracy.ci}{[0.798, 0.837]}
\@namedef{VJ@M1_8b.ts_transfer.snli_ve.aurc_maxp}{0.067}
\@namedef{VJ@M1_8b.ts_transfer.snli_ve.aurc_maxp.ci}{[0.055, 0.080]}
\@namedef{VJ@M1_8b.ts_transfer.snli_ve.brier}{0.268}
\@namedef{VJ@M1_8b.ts_transfer.snli_ve.brier.ci}{[0.246, 0.289]}
\@namedef{VJ@M1_8b.ts_transfer.snli_ve.cov@0.05}{0.375}
\@namedef{VJ@M1_8b.ts_transfer.snli_ve.cov@0.05.ci}{[0.353, 0.396]}
\@namedef{VJ@M1_8b.ts_transfer.snli_ve.cov@0.05.pct}{37.5\%}
\@namedef{VJ@M1_8b.ts_transfer.snli_ve.cov@0.1}{0.630}
\@namedef{VJ@M1_8b.ts_transfer.snli_ve.cov@0.1.ci}{[0.608, 0.651]}
\@namedef{VJ@M1_8b.ts_transfer.snli_ve.cov@0.1.pct}{63.0\%}
\@namedef{VJ@M1_8b.ts_transfer.snli_ve.ece15}{0.055}
\@namedef{VJ@M1_8b.ts_transfer.snli_ve.ece15.ci}{[0.048, 0.074]}
\@namedef{VJ@M1_8b.ts_transfer.snli_ve.nll}{0.482}
\@namedef{VJ@M1_8b.ts_transfer.snli_ve.nll.ci}{[0.450, 0.513]}
\@namedef{VJ@M1_8b.ts_transfer.snli_ve.risk@0.05}{0.042}
\@namedef{VJ@M1_8b.ts_transfer.snli_ve.risk@0.05.ci}{[0.029, 0.058]}
\@namedef{VJ@M1_8b.ts_transfer.snli_ve.risk@0.05.pct}{4.2\%}
\@namedef{VJ@M1_8b.ts_transfer.snli_ve.risk@0.1}{0.077}
\@namedef{VJ@M1_8b.ts_transfer.snli_ve.risk@0.1.ci}{[0.061, 0.093]}
\@namedef{VJ@M1_8b.ts_transfer.snli_ve.risk@0.1.pct}{7.7\%}
\@namedef{VJ@M1_8b.ts_transfer.tallyqa_l.accuracy}{0.855}
\@namedef{VJ@M1_8b.ts_transfer.tallyqa_l.accuracy.ci}{[0.843, 0.867]}
\@namedef{VJ@M1_8b.ts_transfer.tallyqa_l.aurc_maxp}{0.028}
\@namedef{VJ@M1_8b.ts_transfer.tallyqa_l.aurc_maxp.ci}{[0.024, 0.033]}
\@namedef{VJ@M1_8b.ts_transfer.tallyqa_l.brier}{0.201}
\@namedef{VJ@M1_8b.ts_transfer.tallyqa_l.brier.ci}{[0.187, 0.214]}
\@namedef{VJ@M1_8b.ts_transfer.tallyqa_l.cov@0.05}{0.788}
\@namedef{VJ@M1_8b.ts_transfer.tallyqa_l.cov@0.05.ci}{[0.772, 0.801]}
\@namedef{VJ@M1_8b.ts_transfer.tallyqa_l.cov@0.05.pct}{78.8\%}
\@namedef{VJ@M1_8b.ts_transfer.tallyqa_l.cov@0.1}{0.915}
\@namedef{VJ@M1_8b.ts_transfer.tallyqa_l.cov@0.1.ci}{[0.906, 0.923]}
\@namedef{VJ@M1_8b.ts_transfer.tallyqa_l.cov@0.1.pct}{91.5\%}
\@namedef{VJ@M1_8b.ts_transfer.tallyqa_l.ece15}{0.039}
\@namedef{VJ@M1_8b.ts_transfer.tallyqa_l.ece15.ci}{[0.037, 0.050]}
\@namedef{VJ@M1_8b.ts_transfer.tallyqa_l.nll}{0.404}
\@namedef{VJ@M1_8b.ts_transfer.tallyqa_l.nll.ci}{[0.380, 0.429]}
\@namedef{VJ@M1_8b.ts_transfer.tallyqa_l.risk@0.05}{0.054}
\@namedef{VJ@M1_8b.ts_transfer.tallyqa_l.risk@0.05.ci}{[0.047, 0.063]}
\@namedef{VJ@M1_8b.ts_transfer.tallyqa_l.risk@0.05.pct}{5.4\%}
\@namedef{VJ@M1_8b.ts_transfer.tallyqa_l.risk@0.1}{0.103}
\@namedef{VJ@M1_8b.ts_transfer.tallyqa_l.risk@0.1.ci}{[0.093, 0.113]}
\@namedef{VJ@M1_8b.ts_transfer.tallyqa_l.risk@0.1.pct}{10.3\%}
\@namedef{VJ@M1_8b.ts_transfer.textvqa_k8.accuracy}{0.979}
\@namedef{VJ@M1_8b.ts_transfer.textvqa_k8.accuracy.ci}{[0.972, 0.985]}
\@namedef{VJ@M1_8b.ts_transfer.textvqa_k8.aurc_maxp}{0.000}
\@namedef{VJ@M1_8b.ts_transfer.textvqa_k8.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@M1_8b.ts_transfer.textvqa_k8.brier}{0.031}
\@namedef{VJ@M1_8b.ts_transfer.textvqa_k8.brier.ci}{[0.022, 0.039]}
\@namedef{VJ@M1_8b.ts_transfer.textvqa_k8.cov@0.05}{0.999}
\@namedef{VJ@M1_8b.ts_transfer.textvqa_k8.cov@0.05.ci}{[0.999, 1.000]}
\@namedef{VJ@M1_8b.ts_transfer.textvqa_k8.cov@0.05.pct}{99.9\%}
\@namedef{VJ@M1_8b.ts_transfer.textvqa_k8.cov@0.1}{0.999}
\@namedef{VJ@M1_8b.ts_transfer.textvqa_k8.cov@0.1.ci}{[0.999, 1.000]}
\@namedef{VJ@M1_8b.ts_transfer.textvqa_k8.cov@0.1.pct}{99.9\%}
\@namedef{VJ@M1_8b.ts_transfer.textvqa_k8.ece15}{0.016}
\@namedef{VJ@M1_8b.ts_transfer.textvqa_k8.ece15.ci}{[0.016, 0.021]}
\@namedef{VJ@M1_8b.ts_transfer.textvqa_k8.nll}{0.078}
\@namedef{VJ@M1_8b.ts_transfer.textvqa_k8.nll.ci}{[0.059, 0.096]}
\@namedef{VJ@M1_8b.ts_transfer.textvqa_k8.risk@0.05}{0.021}
\@namedef{VJ@M1_8b.ts_transfer.textvqa_k8.risk@0.05.ci}{[0.015, 0.027]}
\@namedef{VJ@M1_8b.ts_transfer.textvqa_k8.risk@0.05.pct}{2.1\%}
\@namedef{VJ@M1_8b.ts_transfer.textvqa_k8.risk@0.1}{0.021}
\@namedef{VJ@M1_8b.ts_transfer.textvqa_k8.risk@0.1.ci}{[0.015, 0.027]}
\@namedef{VJ@M1_8b.ts_transfer.textvqa_k8.risk@0.1.pct}{2.1\%}
\@namedef{VJ@T.B1_k.gqa_val}{2.81}
\@namedef{VJ@T.B1_k.snli_ve}{6.47}
\@namedef{VJ@T.B1_k.tallyqa_l}{2.67}
\@namedef{VJ@T.B1_k.textvqa_k8}{1.82}
\@namedef{VJ@T.M0.range}{1.8--6.5}
\@namedef{VJ@T.M1.range}{1.2--1.8}
\@namedef{VJ@T.a2_s0.gqa_val}{1.70}
\@namedef{VJ@T.a2_s0.snli_ve}{1.36}
\@namedef{VJ@T.a2_s0.tallyqa_l}{1.32}
\@namedef{VJ@T.a2_s0.textvqa_k8}{1.32}
\@namedef{VJ@T.a2_s1.gqa_val}{1.77}
\@namedef{VJ@T.a2_s1.snli_ve}{1.43}
\@namedef{VJ@T.a2_s1.tallyqa_l}{1.24}
\@namedef{VJ@T.a2_s1.textvqa_k8}{1.26}
\@namedef{VJ@T.a2_s2.gqa_val}{1.71}
\@namedef{VJ@T.a2_s2.snli_ve}{1.45}
\@namedef{VJ@T.a2_s2.tallyqa_l}{1.25}
\@namedef{VJ@T.a2_s2.textvqa_k8}{1.31}
\@namedef{VJ@api.API_jev.auroc}{0.870}
\@namedef{VJ@api.API_jev.cost}{0.00}
\@namedef{VJ@api.API_jev.failed}{1.9\%}
\@namedef{VJ@api.API_jev.gqa_val.auroc}{0.873}
\@namedef{VJ@api.API_jev.gqa_val.cov@0.05}{0.779}
\@namedef{VJ@api.API_jev.gqa_val.cov@0.1}{0.952}
\@namedef{VJ@api.API_jev.gqa_val.risk@0.05}{0.041}
\@namedef{VJ@api.API_jev.gqa_val.risk@0.05.ci}{[0.035, 0.047]}
\@namedef{VJ@api.API_jev.gqa_val.risk@0.1}{0.090}
\@namedef{VJ@api.API_jev.gqa_val.risk@0.1.ci}{[0.082, 0.098]}
\@namedef{VJ@api.API_jev.perm.gqa_val.consistent}{96.8\%}
\@namedef{VJ@api.API_jev.perm.gqa_val.flip@0.05}{5.5\%}
\@namedef{VJ@api.API_jev.perm.gqa_val.tv}{0.020}
\@namedef{VJ@api.API_jev.perm.snli_ve.consistent}{91.9\%}
\@namedef{VJ@api.API_jev.perm.snli_ve.flip@0.05}{11.0\%}
\@namedef{VJ@api.API_jev.perm.snli_ve.tv}{0.040}
\@namedef{VJ@api.API_jev.perm.tallyqa.consistent}{55.4\%}
\@namedef{VJ@api.API_jev.perm.tallyqa.flip@0.05}{8.9\%}
\@namedef{VJ@api.API_jev.perm.tallyqa.tv}{0.107}
\@namedef{VJ@api.API_jev.perm.textvqa_k8.consistent}{98.8\%}
\@namedef{VJ@api.API_jev.perm.textvqa_k8.flip@0.05}{0.2\%}
\@namedef{VJ@api.API_jev.perm.textvqa_k8.tv}{0.007}
\@namedef{VJ@api.API_jev.repeat.gqa_val.changed}{0.8\%}
\@namedef{VJ@api.API_jev.repeat.gqa_val.identical}{60.7\%}
\@namedef{VJ@api.API_jev.repeat.gqa_val.same}{99.2\%}
\@namedef{VJ@api.API_jev.repeat.snli_ve.changed}{2.7\%}
\@namedef{VJ@api.API_jev.repeat.snli_ve.identical}{30.7\%}
\@namedef{VJ@api.API_jev.repeat.snli_ve.same}{97.3\%}
\@namedef{VJ@api.API_jev.repeat.tallyqa.changed}{10.3\%}
\@namedef{VJ@api.API_jev.repeat.tallyqa.identical}{11.6\%}
\@namedef{VJ@api.API_jev.repeat.tallyqa.same}{89.7\%}
\@namedef{VJ@api.API_jev.requests}{19,091}
\@namedef{VJ@api.API_jev.round.gqa_val.one}{38\%}
\@namedef{VJ@api.API_jev.round.snli_ve.one}{12\%}
\@namedef{VJ@api.API_jev.round.tallyqa_l.one}{23\%}
\@namedef{VJ@api.API_jev.round.textvqa_k8.one}{84\%}
\@namedef{VJ@api.API_jev.short.accuracy}{0.506}
\@namedef{VJ@api.API_jev.snli_ve.auroc}{0.728}
\@namedef{VJ@api.API_jev.snli_ve.cov@0.05}{0.194}
\@namedef{VJ@api.API_jev.snli_ve.cov@0.1}{0.219}
\@namedef{VJ@api.API_jev.snli_ve.risk@0.05}{0.060}
\@namedef{VJ@api.API_jev.snli_ve.risk@0.05.ci}{[0.033, 0.090]}
\@namedef{VJ@api.API_jev.snli_ve.risk@0.1}{0.073}
\@namedef{VJ@api.API_jev.snli_ve.risk@0.1.ci}{[0.045, 0.102]}
\@namedef{VJ@api.API_jev.tallyqa_l.auroc}{0.912}
\@namedef{VJ@api.API_jev.tallyqa_l.cov@0.05}{0.808}
\@namedef{VJ@api.API_jev.tallyqa_l.cov@0.1}{0.919}
\@namedef{VJ@api.API_jev.tallyqa_l.risk@0.05}{0.054}
\@namedef{VJ@api.API_jev.tallyqa_l.risk@0.05.ci}{[0.046, 0.064]}
\@namedef{VJ@api.API_jev.tallyqa_l.risk@0.1}{0.102}
\@namedef{VJ@api.API_jev.tallyqa_l.risk@0.1.ci}{[0.091, 0.113]}
\@namedef{VJ@api.API_jev.textvqa_k8.auroc}{0.968}
\@namedef{VJ@api.API_jev.textvqa_k8.cov@0.05}{0.998}
\@namedef{VJ@api.API_jev.textvqa_k8.cov@0.1}{0.998}
\@namedef{VJ@api.API_jev.textvqa_k8.risk@0.05}{0.017}
\@namedef{VJ@api.API_jev.textvqa_k8.risk@0.05.ci}{[0.011, 0.023]}
\@namedef{VJ@api.API_jev.textvqa_k8.risk@0.1}{0.017}
\@namedef{VJ@api.API_jev.textvqa_k8.risk@0.1.ci}{[0.011, 0.023]}
\@namedef{VJ@api.API_luna.auroc}{0.833}
\@namedef{VJ@api.API_luna.cost}{1.34}
\@namedef{VJ@api.API_luna.failed}{0.3\%}
\@namedef{VJ@api.API_luna.gqa_val.auroc}{0.793}
\@namedef{VJ@api.API_luna.gqa_val.cov@0.05}{0.247}
\@namedef{VJ@api.API_luna.gqa_val.cov@0.1}{0.815}
\@namedef{VJ@api.API_luna.gqa_val.risk@0.05}{0.053}
\@namedef{VJ@api.API_luna.gqa_val.risk@0.05.ci}{[0.041, 0.065]}
\@namedef{VJ@api.API_luna.gqa_val.risk@0.1}{0.103}
\@namedef{VJ@api.API_luna.gqa_val.risk@0.1.ci}{[0.094, 0.112]}
\@namedef{VJ@api.API_luna.perm.gqa_val.consistent}{90.7\%}
\@namedef{VJ@api.API_luna.perm.gqa_val.flip@0.05}{5.0\%}
\@namedef{VJ@api.API_luna.perm.gqa_val.tv}{0.066}
\@namedef{VJ@api.API_luna.perm.snli_ve.consistent}{82.7\%}
\@namedef{VJ@api.API_luna.perm.snli_ve.flip@0.05}{17.5\%}
\@namedef{VJ@api.API_luna.perm.snli_ve.tv}{0.080}
\@namedef{VJ@api.API_luna.perm.tallyqa.consistent}{100.0\%}
\@namedef{VJ@api.API_luna.perm.tallyqa.flip@0.05}{0.0\%}
\@namedef{VJ@api.API_luna.perm.tallyqa.tv}{0.000}
\@namedef{VJ@api.API_luna.perm.textvqa_k8.consistent}{96.2\%}
\@namedef{VJ@api.API_luna.perm.textvqa_k8.flip@0.05}{0.0\%}
\@namedef{VJ@api.API_luna.perm.textvqa_k8.tv}{0.024}
\@namedef{VJ@api.API_luna.repeat.gqa_val.changed}{0.0\%}
\@namedef{VJ@api.API_luna.repeat.gqa_val.identical}{100.0\%}
\@namedef{VJ@api.API_luna.repeat.gqa_val.same}{100.0\%}
\@namedef{VJ@api.API_luna.repeat.snli_ve.changed}{0.0\%}
\@namedef{VJ@api.API_luna.repeat.snli_ve.identical}{100.0\%}
\@namedef{VJ@api.API_luna.repeat.snli_ve.same}{100.0\%}
\@namedef{VJ@api.API_luna.repeat.tallyqa.changed}{0.0\%}
\@namedef{VJ@api.API_luna.repeat.tallyqa.identical}{100.0\%}
\@namedef{VJ@api.API_luna.repeat.tallyqa.same}{100.0\%}
\@namedef{VJ@api.API_luna.requests}{19,016}
\@namedef{VJ@api.API_luna.round.gqa_val.one}{42\%}
\@namedef{VJ@api.API_luna.round.snli_ve.one}{28\%}
\@namedef{VJ@api.API_luna.round.tallyqa_l.one}{29\%}
\@namedef{VJ@api.API_luna.round.textvqa_k8.one}{76\%}
\@namedef{VJ@api.API_luna.short.accuracy}{0.420}
\@namedef{VJ@api.API_luna.snli_ve.auroc}{0.709}
\@namedef{VJ@api.API_luna.snli_ve.cov@0.05}{0.278}
\@namedef{VJ@api.API_luna.snli_ve.cov@0.1}{0.278}
\@namedef{VJ@api.API_luna.snli_ve.risk@0.05}{0.089}
\@namedef{VJ@api.API_luna.snli_ve.risk@0.05.ci}{[0.064, 0.120]}
\@namedef{VJ@api.API_luna.snli_ve.risk@0.1}{0.089}
\@namedef{VJ@api.API_luna.snli_ve.risk@0.1.ci}{[0.064, 0.120]}
\@namedef{VJ@api.API_luna.tallyqa_l.auroc}{0.864}
\@namedef{VJ@api.API_luna.tallyqa_l.cov@0.05}{0.697}
\@namedef{VJ@api.API_luna.tallyqa_l.cov@0.1}{0.848}
\@namedef{VJ@api.API_luna.tallyqa_l.risk@0.05}{0.060}
\@namedef{VJ@api.API_luna.tallyqa_l.risk@0.05.ci}{[0.050, 0.070]}
\@namedef{VJ@api.API_luna.tallyqa_l.risk@0.1}{0.112}
\@namedef{VJ@api.API_luna.tallyqa_l.risk@0.1.ci}{[0.101, 0.124]}
\@namedef{VJ@api.API_luna.textvqa_k8.auroc}{0.965}
\@namedef{VJ@api.API_luna.textvqa_k8.cov@0.05}{1.000}
\@namedef{VJ@api.API_luna.textvqa_k8.cov@0.1}{1.000}
\@namedef{VJ@api.API_luna.textvqa_k8.risk@0.05}{0.045}
\@namedef{VJ@api.API_luna.textvqa_k8.risk@0.05.ci}{[0.034, 0.054]}
\@namedef{VJ@api.API_luna.textvqa_k8.risk@0.1}{0.045}
\@namedef{VJ@api.API_luna.textvqa_k8.risk@0.1.ci}{[0.034, 0.054]}
\@namedef{VJ@api.M0.accuracy.pct}{83.4\%}
\@namedef{VJ@api.M0.auroc}{0.834}
\@namedef{VJ@api.M0.gqa_val.auroc}{0.833}
\@namedef{VJ@api.M0.gqa_val.cov@0.05}{0.758}
\@namedef{VJ@api.M0.gqa_val.cov@0.1}{0.936}
\@namedef{VJ@api.M0.gqa_val.risk@0.05}{0.047}
\@namedef{VJ@api.M0.gqa_val.risk@0.05.ci}{[0.041, 0.054]}
\@namedef{VJ@api.M0.gqa_val.risk@0.1}{0.093}
\@namedef{VJ@api.M0.gqa_val.risk@0.1.ci}{[0.085, 0.101]}
\@namedef{VJ@api.M0.perm.gqa_val.consistent}{93.3\%}
\@namedef{VJ@api.M0.perm.gqa_val.flip@0.05}{14.0\%}
\@namedef{VJ@api.M0.perm.gqa_val.tv}{0.065}
\@namedef{VJ@api.M0.perm.snli_ve.consistent}{74.8\%}
\@namedef{VJ@api.M0.perm.snli_ve.flip@0.05}{2.6\%}
\@namedef{VJ@api.M0.perm.snli_ve.tv}{0.108}
\@namedef{VJ@api.M0.perm.tallyqa.consistent}{32.5\%}
\@namedef{VJ@api.M0.perm.tallyqa.flip@0.05}{8.6\%}
\@namedef{VJ@api.M0.perm.tallyqa.tv}{0.174}
\@namedef{VJ@api.M0.perm.textvqa_k8.consistent}{96.9\%}
\@namedef{VJ@api.M0.perm.textvqa_k8.flip@0.05}{0.0\%}
\@namedef{VJ@api.M0.perm.textvqa_k8.tv}{0.022}
\@namedef{VJ@api.M0.snli_ve.auroc}{0.646}
\@namedef{VJ@api.M0.snli_ve.cov@0.05}{0.023}
\@namedef{VJ@api.M0.snli_ve.cov@0.1}{0.067}
\@namedef{VJ@api.M0.snli_ve.risk@0.05}{0.125}
\@namedef{VJ@api.M0.snli_ve.risk@0.05.ci}{[0.029, 0.259]}
\@namedef{VJ@api.M0.snli_ve.risk@0.1}{0.076}
\@namedef{VJ@api.M0.snli_ve.risk@0.1.ci}{[0.029, 0.138]}
\@namedef{VJ@api.M0.tallyqa_l.auroc}{0.871}
\@namedef{VJ@api.M0.tallyqa_l.cov@0.05}{0.748}
\@namedef{VJ@api.M0.tallyqa_l.cov@0.1}{0.898}
\@namedef{VJ@api.M0.tallyqa_l.risk@0.05}{0.047}
\@namedef{VJ@api.M0.tallyqa_l.risk@0.05.ci}{[0.039, 0.055]}
\@namedef{VJ@api.M0.tallyqa_l.risk@0.1}{0.099}
\@namedef{VJ@api.M0.tallyqa_l.risk@0.1.ci}{[0.089, 0.111]}
\@namedef{VJ@api.M0.textvqa_k8.auroc}{0.985}
\@namedef{VJ@api.M0.textvqa_k8.cov@0.05}{1.000}
\@namedef{VJ@api.M0.textvqa_k8.cov@0.1}{1.000}
\@namedef{VJ@api.M0.textvqa_k8.risk@0.05}{0.026}
\@namedef{VJ@api.M0.textvqa_k8.risk@0.05.ci}{[0.019, 0.034]}
\@namedef{VJ@api.M0.textvqa_k8.risk@0.1}{0.026}
\@namedef{VJ@api.M0.textvqa_k8.risk@0.1.ci}{[0.019, 0.034]}
\@namedef{VJ@api.M1.accuracy.pct}{88.5\%}
\@namedef{VJ@api.M1.auroc}{0.890}
\@namedef{VJ@api.M1.gqa_val.auroc}{0.892}
\@namedef{VJ@api.M1.gqa_val.cov@0.05}{0.888}
\@namedef{VJ@api.M1.gqa_val.cov@0.1}{0.999}
\@namedef{VJ@api.M1.gqa_val.risk@0.05}{0.044}
\@namedef{VJ@api.M1.gqa_val.risk@0.05.ci}{[0.039, 0.050]}
\@namedef{VJ@api.M1.gqa_val.risk@0.1}{0.083}
\@namedef{VJ@api.M1.gqa_val.risk@0.1.ci}{[0.076, 0.090]}
\@namedef{VJ@api.M1.perm.gqa_val.consistent}{97.5\%}
\@namedef{VJ@api.M1.perm.gqa_val.flip@0.05}{4.8\%}
\@namedef{VJ@api.M1.perm.gqa_val.tv}{0.022}
\@namedef{VJ@api.M1.perm.snli_ve.consistent}{92.6\%}
\@namedef{VJ@api.M1.perm.snli_ve.flip@0.05}{17.0\%}
\@namedef{VJ@api.M1.perm.snli_ve.tv}{0.062}
\@namedef{VJ@api.M1.perm.tallyqa.consistent}{46.4\%}
\@namedef{VJ@api.M1.perm.tallyqa.flip@0.05}{7.8\%}
\@namedef{VJ@api.M1.perm.tallyqa.tv}{0.138}
\@namedef{VJ@api.M1.perm.textvqa_k8.consistent}{97.2\%}
\@namedef{VJ@api.M1.perm.textvqa_k8.flip@0.05}{0.1\%}
\@namedef{VJ@api.M1.perm.textvqa_k8.tv}{0.016}
\@namedef{VJ@api.M1.short.accuracy}{0.345}
\@namedef{VJ@api.M1.snli_ve.auroc}{0.792}
\@namedef{VJ@api.M1.snli_ve.cov@0.05}{0.346}
\@namedef{VJ@api.M1.snli_ve.cov@0.1}{0.626}
\@namedef{VJ@api.M1.snli_ve.risk@0.05}{0.038}
\@namedef{VJ@api.M1.snli_ve.risk@0.05.ci}{[0.025, 0.054]}
\@namedef{VJ@api.M1.snli_ve.risk@0.1}{0.079}
\@namedef{VJ@api.M1.snli_ve.risk@0.1.ci}{[0.063, 0.096]}
\@namedef{VJ@api.M1.tallyqa_l.auroc}{0.892}
\@namedef{VJ@api.M1.tallyqa_l.cov@0.05}{0.764}
\@namedef{VJ@api.M1.tallyqa_l.cov@0.1}{0.887}
\@namedef{VJ@api.M1.tallyqa_l.risk@0.05}{0.053}
\@namedef{VJ@api.M1.tallyqa_l.risk@0.05.ci}{[0.046, 0.061]}
\@namedef{VJ@api.M1.tallyqa_l.risk@0.1}{0.103}
\@namedef{VJ@api.M1.tallyqa_l.risk@0.1.ci}{[0.093, 0.114]}
\@namedef{VJ@api.M1.textvqa_k8.auroc}{0.984}
\@namedef{VJ@api.M1.textvqa_k8.cov@0.05}{1.000}
\@namedef{VJ@api.M1.textvqa_k8.cov@0.1}{1.000}
\@namedef{VJ@api.M1.textvqa_k8.risk@0.05}{0.025}
\@namedef{VJ@api.M1.textvqa_k8.risk@0.05.ci}{[0.017, 0.031]}
\@namedef{VJ@api.M1.textvqa_k8.risk@0.1}{0.025}
\@namedef{VJ@api.M1.textvqa_k8.risk@0.1.ci}{[0.017, 0.031]}
\@namedef{VJ@api.d.jev_m1.macro.accuracy}{$-$0.028}
\@namedef{VJ@api.d.jev_m1.macro.accuracy.ci}{[$-$0.035, $-$0.020]}
\@namedef{VJ@api.d.luna_m1.macro.accuracy}{$-$0.051}
\@namedef{VJ@api.d.luna_m1.macro.accuracy.ci}{[$-$0.058, $-$0.043]}
\@namedef{VJ@api.gain_vs_jev.pp}{2.77}
\@namedef{VJ@api.gain_vs_luna.pp}{5.06}
\@namedef{VJ@d.Dbrier-Dce.gqa_val.accuracy}{+0.000}
\@namedef{VJ@d.Dbrier-Dce.gqa_val.accuracy.ci}{[$-$0.001, 0.002]}
\@namedef{VJ@d.Dbrier-Dce.gqa_val.aurc_maxp}{$-$0.001}
\@namedef{VJ@d.Dbrier-Dce.gqa_val.aurc_maxp.ci}{[$-$0.001, $-$0.000]}
\@namedef{VJ@d.Dbrier-Dce.gqa_val.brier}{$-$0.002}
\@namedef{VJ@d.Dbrier-Dce.gqa_val.brier.ci}{[$-$0.003, $-$0.002]}
\@namedef{VJ@d.Dbrier-Dce.gqa_val.ece15}{$-$0.001}
\@namedef{VJ@d.Dbrier-Dce.gqa_val.ece15.ci}{[$-$0.004, 0.002]}
\@namedef{VJ@d.Dbrier-Dce.gqa_val.nll}{$-$0.008}
\@namedef{VJ@d.Dbrier-Dce.gqa_val.nll.ci}{[$-$0.009, $-$0.006]}
\@namedef{VJ@d.Dbrier-Dce.macro.accuracy}{+0.000}
\@namedef{VJ@d.Dbrier-Dce.macro.accuracy.ci}{[$-$0.001, 0.001]}
\@namedef{VJ@d.Dbrier-Dce.macro.aurc_maxp}{$-$0.001}
\@namedef{VJ@d.Dbrier-Dce.macro.aurc_maxp.ci}{[$-$0.001, $-$0.000]}
\@namedef{VJ@d.Dbrier-Dce.macro.brier}{$-$0.002}
\@namedef{VJ@d.Dbrier-Dce.macro.brier.ci}{[$-$0.002, $-$0.001]}
\@namedef{VJ@d.Dbrier-Dce.macro.ece15}{$-$0.002}
\@namedef{VJ@d.Dbrier-Dce.macro.ece15.ci}{[$-$0.004, 0.001]}
\@namedef{VJ@d.Dbrier-Dce.macro.nll}{$-$0.005}
\@namedef{VJ@d.Dbrier-Dce.macro.nll.ci}{[$-$0.006, $-$0.004]}
\@namedef{VJ@d.Dbrier-Dce.snli_ve.accuracy}{+0.000}
\@namedef{VJ@d.Dbrier-Dce.snli_ve.accuracy.ci}{[$-$0.003, 0.004]}
\@namedef{VJ@d.Dbrier-Dce.snli_ve.aurc_maxp}{$-$0.002}
\@namedef{VJ@d.Dbrier-Dce.snli_ve.aurc_maxp.ci}{[$-$0.003, $-$0.000]}
\@namedef{VJ@d.Dbrier-Dce.snli_ve.brier}{$-$0.002}
\@namedef{VJ@d.Dbrier-Dce.snli_ve.brier.ci}{[$-$0.003, $-$0.000]}
\@namedef{VJ@d.Dbrier-Dce.snli_ve.ece15}{$-$0.002}
\@namedef{VJ@d.Dbrier-Dce.snli_ve.ece15.ci}{[$-$0.008, 0.009]}
\@namedef{VJ@d.Dbrier-Dce.snli_ve.nll}{$-$0.004}
\@namedef{VJ@d.Dbrier-Dce.snli_ve.nll.ci}{[$-$0.006, $-$0.002]}
\@namedef{VJ@d.Dbrier-Dce.tallyqa_l.accuracy}{+0.000}
\@namedef{VJ@d.Dbrier-Dce.tallyqa_l.accuracy.ci}{[$-$0.002, 0.002]}
\@namedef{VJ@d.Dbrier-Dce.tallyqa_l.aurc_maxp}{$-$0.000}
\@namedef{VJ@d.Dbrier-Dce.tallyqa_l.aurc_maxp.ci}{[$-$0.001, 0.000]}
\@namedef{VJ@d.Dbrier-Dce.tallyqa_l.brier}{$-$0.002}
\@namedef{VJ@d.Dbrier-Dce.tallyqa_l.brier.ci}{[$-$0.003, $-$0.001]}
\@namedef{VJ@d.Dbrier-Dce.tallyqa_l.ece15}{$-$0.005}
\@namedef{VJ@d.Dbrier-Dce.tallyqa_l.ece15.ci}{[$-$0.007, $-$0.002]}
\@namedef{VJ@d.Dbrier-Dce.tallyqa_l.nll}{$-$0.007}
\@namedef{VJ@d.Dbrier-Dce.tallyqa_l.nll.ci}{[$-$0.008, $-$0.005]}
\@namedef{VJ@d.Dbrier-Dce.textvqa_k8.accuracy}{+0.000}
\@namedef{VJ@d.Dbrier-Dce.textvqa_k8.accuracy.ci}{[$-$0.000, 0.001]}
\@namedef{VJ@d.Dbrier-Dce.textvqa_k8.aurc_maxp}{$-$0.000}
\@namedef{VJ@d.Dbrier-Dce.textvqa_k8.aurc_maxp.ci}{[$-$0.000, 0.000]}
\@namedef{VJ@d.Dbrier-Dce.textvqa_k8.brier}{$-$0.001}
\@namedef{VJ@d.Dbrier-Dce.textvqa_k8.brier.ci}{[$-$0.001, $-$0.000]}
\@namedef{VJ@d.Dbrier-Dce.textvqa_k8.ece15}{+0.000}
\@namedef{VJ@d.Dbrier-Dce.textvqa_k8.ece15.ci}{[$-$0.002, 0.002]}
\@namedef{VJ@d.Dbrier-Dce.textvqa_k8.nll}{$-$0.002}
\@namedef{VJ@d.Dbrier-Dce.textvqa_k8.nll.ci}{[$-$0.003, $-$0.001]}
\@namedef{VJ@d.Dbrier-Dfull.gqa_val.accuracy}{+0.000}
\@namedef{VJ@d.Dbrier-Dfull.gqa_val.accuracy.ci}{[$-$0.001, 0.001]}
\@namedef{VJ@d.Dbrier-Dfull.gqa_val.aurc_maxp}{$-$0.001}
\@namedef{VJ@d.Dbrier-Dfull.gqa_val.aurc_maxp.ci}{[$-$0.001, $-$0.000]}
\@namedef{VJ@d.Dbrier-Dfull.gqa_val.brier}{$-$0.002}
\@namedef{VJ@d.Dbrier-Dfull.gqa_val.brier.ci}{[$-$0.003, $-$0.002]}
\@namedef{VJ@d.Dbrier-Dfull.gqa_val.ece15}{$-$0.001}
\@namedef{VJ@d.Dbrier-Dfull.gqa_val.ece15.ci}{[$-$0.004, 0.002]}
\@namedef{VJ@d.Dbrier-Dfull.gqa_val.nll}{$-$0.007}
\@namedef{VJ@d.Dbrier-Dfull.gqa_val.nll.ci}{[$-$0.009, $-$0.006]}
\@namedef{VJ@d.Dbrier-Dfull.macro.accuracy}{+0.000}
\@namedef{VJ@d.Dbrier-Dfull.macro.accuracy.ci}{[$-$0.001, 0.001]}
\@namedef{VJ@d.Dbrier-Dfull.macro.aurc_maxp}{$-$0.001}
\@namedef{VJ@d.Dbrier-Dfull.macro.aurc_maxp.ci}{[$-$0.001, $-$0.000]}
\@namedef{VJ@d.Dbrier-Dfull.macro.brier}{$-$0.002}
\@namedef{VJ@d.Dbrier-Dfull.macro.brier.ci}{[$-$0.002, $-$0.001]}
\@namedef{VJ@d.Dbrier-Dfull.macro.ece15}{$-$0.002}
\@namedef{VJ@d.Dbrier-Dfull.macro.ece15.ci}{[$-$0.004, 0.001]}
\@namedef{VJ@d.Dbrier-Dfull.macro.nll}{$-$0.005}
\@namedef{VJ@d.Dbrier-Dfull.macro.nll.ci}{[$-$0.006, $-$0.004]}
\@namedef{VJ@d.Dbrier-Dfull.snli_ve.accuracy}{+0.001}
\@namedef{VJ@d.Dbrier-Dfull.snli_ve.accuracy.ci}{[$-$0.002, 0.004]}
\@namedef{VJ@d.Dbrier-Dfull.snli_ve.aurc_maxp}{$-$0.002}
\@namedef{VJ@d.Dbrier-Dfull.snli_ve.aurc_maxp.ci}{[$-$0.004, $-$0.001]}
\@namedef{VJ@d.Dbrier-Dfull.snli_ve.brier}{$-$0.002}
\@namedef{VJ@d.Dbrier-Dfull.snli_ve.brier.ci}{[$-$0.003, $-$0.000]}
\@namedef{VJ@d.Dbrier-Dfull.snli_ve.ece15}{$-$0.003}
\@namedef{VJ@d.Dbrier-Dfull.snli_ve.ece15.ci}{[$-$0.009, 0.009]}
\@namedef{VJ@d.Dbrier-Dfull.snli_ve.nll}{$-$0.004}
\@namedef{VJ@d.Dbrier-Dfull.snli_ve.nll.ci}{[$-$0.006, $-$0.002]}
\@namedef{VJ@d.Dbrier-Dfull.tallyqa_l.accuracy}{$-$0.001}
\@namedef{VJ@d.Dbrier-Dfull.tallyqa_l.accuracy.ci}{[$-$0.002, 0.001]}
\@namedef{VJ@d.Dbrier-Dfull.tallyqa_l.aurc_maxp}{$-$0.000}
\@namedef{VJ@d.Dbrier-Dfull.tallyqa_l.aurc_maxp.ci}{[$-$0.001, $-$0.000]}
\@namedef{VJ@d.Dbrier-Dfull.tallyqa_l.brier}{$-$0.002}
\@namedef{VJ@d.Dbrier-Dfull.tallyqa_l.brier.ci}{[$-$0.002, $-$0.001]}
\@namedef{VJ@d.Dbrier-Dfull.tallyqa_l.ece15}{$-$0.003}
\@namedef{VJ@d.Dbrier-Dfull.tallyqa_l.ece15.ci}{[$-$0.006, $-$0.001]}
\@namedef{VJ@d.Dbrier-Dfull.tallyqa_l.nll}{$-$0.006}
\@namedef{VJ@d.Dbrier-Dfull.tallyqa_l.nll.ci}{[$-$0.007, $-$0.004]}
\@namedef{VJ@d.Dbrier-Dfull.textvqa_k8.accuracy}{+0.000}
\@namedef{VJ@d.Dbrier-Dfull.textvqa_k8.accuracy.ci}{[$-$0.000, 0.001]}
\@namedef{VJ@d.Dbrier-Dfull.textvqa_k8.aurc_maxp}{$-$0.000}
\@namedef{VJ@d.Dbrier-Dfull.textvqa_k8.aurc_maxp.ci}{[$-$0.000, $-$0.000]}
\@namedef{VJ@d.Dbrier-Dfull.textvqa_k8.brier}{$-$0.001}
\@namedef{VJ@d.Dbrier-Dfull.textvqa_k8.brier.ci}{[$-$0.001, $-$0.000]}
\@namedef{VJ@d.Dbrier-Dfull.textvqa_k8.ece15}{$-$0.001}
\@namedef{VJ@d.Dbrier-Dfull.textvqa_k8.ece15.ci}{[$-$0.003, 0.001]}
\@namedef{VJ@d.Dbrier-Dfull.textvqa_k8.nll}{$-$0.002}
\@namedef{VJ@d.Dbrier-Dfull.textvqa_k8.nll.ci}{[$-$0.003, $-$0.001]}
\@namedef{VJ@d.Dce-Dfull.gqa_val.accuracy}{$-$0.000}
\@namedef{VJ@d.Dce-Dfull.gqa_val.accuracy.ci}{[$-$0.001, 0.000]}
\@namedef{VJ@d.Dce-Dfull.gqa_val.aurc_maxp}{+0.000}
\@namedef{VJ@d.Dce-Dfull.gqa_val.aurc_maxp.ci}{[$-$0.000, 0.000]}
\@namedef{VJ@d.Dce-Dfull.gqa_val.brier}{+0.000}
\@namedef{VJ@d.Dce-Dfull.gqa_val.brier.ci}{[$-$0.000, 0.000]}
\@namedef{VJ@d.Dce-Dfull.gqa_val.ece15}{$-$0.000}
\@namedef{VJ@d.Dce-Dfull.gqa_val.ece15.ci}{[$-$0.002, 0.001]}
\@namedef{VJ@d.Dce-Dfull.gqa_val.nll}{+0.001}
\@namedef{VJ@d.Dce-Dfull.gqa_val.nll.ci}{[0.000, 0.001]}
\@namedef{VJ@d.Dce-Dfull.macro.accuracy}{+0.000}
\@namedef{VJ@d.Dce-Dfull.macro.accuracy.ci}{[$-$0.001, 0.001]}
\@namedef{VJ@d.Dce-Dfull.macro.aurc_maxp}{$-$0.000}
\@namedef{VJ@d.Dce-Dfull.macro.aurc_maxp.ci}{[$-$0.000, 0.000]}
\@namedef{VJ@d.Dce-Dfull.macro.brier}{+0.000}
\@namedef{VJ@d.Dce-Dfull.macro.brier.ci}{[$-$0.000, 0.000]}
\@namedef{VJ@d.Dce-Dfull.macro.ece15}{$-$0.000}
\@namedef{VJ@d.Dce-Dfull.macro.ece15.ci}{[$-$0.002, 0.001]}
\@namedef{VJ@d.Dce-Dfull.macro.nll}{+0.000}
\@namedef{VJ@d.Dce-Dfull.macro.nll.ci}{[0.000, 0.001]}
\@namedef{VJ@d.Dce-Dfull.snli_ve.accuracy}{+0.001}
\@namedef{VJ@d.Dce-Dfull.snli_ve.accuracy.ci}{[$-$0.001, 0.003]}
\@namedef{VJ@d.Dce-Dfull.snli_ve.aurc_maxp}{$-$0.000}
\@namedef{VJ@d.Dce-Dfull.snli_ve.aurc_maxp.ci}{[$-$0.001, 0.000]}
\@namedef{VJ@d.Dce-Dfull.snli_ve.brier}{+0.000}
\@namedef{VJ@d.Dce-Dfull.snli_ve.brier.ci}{[$-$0.000, 0.001]}
\@namedef{VJ@d.Dce-Dfull.snli_ve.ece15}{$-$0.001}
\@namedef{VJ@d.Dce-Dfull.snli_ve.ece15.ci}{[$-$0.005, 0.005]}
\@namedef{VJ@d.Dce-Dfull.snli_ve.nll}{+0.000}
\@namedef{VJ@d.Dce-Dfull.snli_ve.nll.ci}{[$-$0.001, 0.001]}
\@namedef{VJ@d.Dce-Dfull.tallyqa_l.accuracy}{$-$0.001}
\@namedef{VJ@d.Dce-Dfull.tallyqa_l.accuracy.ci}{[$-$0.002, 0.001]}
\@namedef{VJ@d.Dce-Dfull.tallyqa_l.aurc_maxp}{$-$0.000}
\@namedef{VJ@d.Dce-Dfull.tallyqa_l.aurc_maxp.ci}{[$-$0.000, 0.000]}
\@namedef{VJ@d.Dce-Dfull.tallyqa_l.brier}{+0.000}
\@namedef{VJ@d.Dce-Dfull.tallyqa_l.brier.ci}{[$-$0.000, 0.001]}
\@namedef{VJ@d.Dce-Dfull.tallyqa_l.ece15}{+0.001}
\@namedef{VJ@d.Dce-Dfull.tallyqa_l.ece15.ci}{[$-$0.001, 0.003]}
\@namedef{VJ@d.Dce-Dfull.tallyqa_l.nll}{+0.001}
\@namedef{VJ@d.Dce-Dfull.tallyqa_l.nll.ci}{[0.000, 0.001]}
\@namedef{VJ@d.Dce-Dfull.textvqa_k8.accuracy}{+0.000}
\@namedef{VJ@d.Dce-Dfull.textvqa_k8.accuracy.ci}{[0.000, 0.001]}
\@namedef{VJ@d.Dce-Dfull.textvqa_k8.aurc_maxp}{$-$0.000}
\@namedef{VJ@d.Dce-Dfull.textvqa_k8.aurc_maxp.ci}{[$-$0.000, 0.000]}
\@namedef{VJ@d.Dce-Dfull.textvqa_k8.brier}{$-$0.000}
\@namedef{VJ@d.Dce-Dfull.textvqa_k8.brier.ci}{[$-$0.000, 0.000]}
\@namedef{VJ@d.Dce-Dfull.textvqa_k8.ece15}{$-$0.001}
\@namedef{VJ@d.Dce-Dfull.textvqa_k8.ece15.ci}{[$-$0.003, 0.001]}
\@namedef{VJ@d.Dce-Dfull.textvqa_k8.nll}{+0.000}
\@namedef{VJ@d.Dce-Dfull.textvqa_k8.nll.ci}{[$-$0.000, 0.000]}
\@namedef{VJ@d.Dceperm-Dce.gqa_val.accuracy}{+0.000}
\@namedef{VJ@d.Dceperm-Dce.gqa_val.accuracy.ci}{[$-$0.001, 0.002]}
\@namedef{VJ@d.Dceperm-Dce.gqa_val.aurc_maxp}{+0.000}
\@namedef{VJ@d.Dceperm-Dce.gqa_val.aurc_maxp.ci}{[$-$0.000, 0.000]}
\@namedef{VJ@d.Dceperm-Dce.gqa_val.brier}{$-$0.000}
\@namedef{VJ@d.Dceperm-Dce.gqa_val.brier.ci}{[$-$0.001, 0.000]}
\@namedef{VJ@d.Dceperm-Dce.gqa_val.ece15}{$-$0.001}
\@namedef{VJ@d.Dceperm-Dce.gqa_val.ece15.ci}{[$-$0.003, 0.002]}
\@namedef{VJ@d.Dceperm-Dce.gqa_val.nll}{$-$0.001}
\@namedef{VJ@d.Dceperm-Dce.gqa_val.nll.ci}{[$-$0.002, $-$0.000]}
\@namedef{VJ@d.Dceperm-Dce.macro.accuracy}{+0.002}
\@namedef{VJ@d.Dceperm-Dce.macro.accuracy.ci}{[0.000, 0.003]}
\@namedef{VJ@d.Dceperm-Dce.macro.aurc_maxp}{+0.000}
\@namedef{VJ@d.Dceperm-Dce.macro.aurc_maxp.ci}{[$-$0.000, 0.001]}
\@namedef{VJ@d.Dceperm-Dce.macro.brier}{$-$0.001}
\@namedef{VJ@d.Dceperm-Dce.macro.brier.ci}{[$-$0.002, $-$0.000]}
\@namedef{VJ@d.Dceperm-Dce.macro.ece15}{$-$0.000}
\@namedef{VJ@d.Dceperm-Dce.macro.ece15.ci}{[$-$0.002, 0.003]}
\@namedef{VJ@d.Dceperm-Dce.macro.nll}{$-$0.003}
\@namedef{VJ@d.Dceperm-Dce.macro.nll.ci}{[$-$0.004, $-$0.001]}
\@namedef{VJ@d.Dceperm-Dce.snli_ve.accuracy}{+0.004}
\@namedef{VJ@d.Dceperm-Dce.snli_ve.accuracy.ci}{[$-$0.002, 0.010]}
\@namedef{VJ@d.Dceperm-Dce.snli_ve.aurc_maxp}{+0.000}
\@namedef{VJ@d.Dceperm-Dce.snli_ve.aurc_maxp.ci}{[$-$0.001, 0.002]}
\@namedef{VJ@d.Dceperm-Dce.snli_ve.brier}{$-$0.002}
\@namedef{VJ@d.Dceperm-Dce.snli_ve.brier.ci}{[$-$0.005, 0.002]}
\@namedef{VJ@d.Dceperm-Dce.snli_ve.ece15}{+0.002}
\@namedef{VJ@d.Dceperm-Dce.snli_ve.ece15.ci}{[$-$0.008, 0.011]}
\@namedef{VJ@d.Dceperm-Dce.snli_ve.nll}{$-$0.002}
\@namedef{VJ@d.Dceperm-Dce.snli_ve.nll.ci}{[$-$0.007, 0.003]}
\@namedef{VJ@d.Dceperm-Dce.tallyqa_l.accuracy}{+0.002}
\@namedef{VJ@d.Dceperm-Dce.tallyqa_l.accuracy.ci}{[0.000, 0.005]}
\@namedef{VJ@d.Dceperm-Dce.tallyqa_l.aurc_maxp}{$-$0.000}
\@namedef{VJ@d.Dceperm-Dce.tallyqa_l.aurc_maxp.ci}{[$-$0.001, 0.001]}
\@namedef{VJ@d.Dceperm-Dce.tallyqa_l.brier}{$-$0.002}
\@namedef{VJ@d.Dceperm-Dce.tallyqa_l.brier.ci}{[$-$0.003, $-$0.001]}
\@namedef{VJ@d.Dceperm-Dce.tallyqa_l.ece15}{$-$0.002}
\@namedef{VJ@d.Dceperm-Dce.tallyqa_l.ece15.ci}{[$-$0.004, 0.003]}
\@namedef{VJ@d.Dceperm-Dce.tallyqa_l.nll}{$-$0.005}
\@namedef{VJ@d.Dceperm-Dce.tallyqa_l.nll.ci}{[$-$0.007, $-$0.003]}
\@namedef{VJ@d.Dceperm-Dce.textvqa_k8.accuracy}{+0.000}
\@namedef{VJ@d.Dceperm-Dce.textvqa_k8.accuracy.ci}{[$-$0.001, 0.001]}
\@namedef{VJ@d.Dceperm-Dce.textvqa_k8.aurc_maxp}{$-$0.000}
\@namedef{VJ@d.Dceperm-Dce.textvqa_k8.aurc_maxp.ci}{[$-$0.000, 0.000]}
\@namedef{VJ@d.Dceperm-Dce.textvqa_k8.brier}{$-$0.001}
\@namedef{VJ@d.Dceperm-Dce.textvqa_k8.brier.ci}{[$-$0.001, 0.000]}
\@namedef{VJ@d.Dceperm-Dce.textvqa_k8.ece15}{+0.000}
\@namedef{VJ@d.Dceperm-Dce.textvqa_k8.ece15.ci}{[$-$0.002, 0.003]}
\@namedef{VJ@d.Dceperm-Dce.textvqa_k8.nll}{$-$0.002}
\@namedef{VJ@d.Dceperm-Dce.textvqa_k8.nll.ci}{[$-$0.004, $-$0.001]}
\@namedef{VJ@d.Dceperm-Dfull.gqa_val.accuracy}{+0.000}
\@namedef{VJ@d.Dceperm-Dfull.gqa_val.accuracy.ci}{[$-$0.001, 0.001]}
\@namedef{VJ@d.Dceperm-Dfull.gqa_val.aurc_maxp}{+0.000}
\@namedef{VJ@d.Dceperm-Dfull.gqa_val.aurc_maxp.ci}{[$-$0.000, 0.000]}
\@namedef{VJ@d.Dceperm-Dfull.gqa_val.brier}{$-$0.000}
\@namedef{VJ@d.Dceperm-Dfull.gqa_val.brier.ci}{[$-$0.001, 0.000]}
\@namedef{VJ@d.Dceperm-Dfull.gqa_val.ece15}{$-$0.001}
\@namedef{VJ@d.Dceperm-Dfull.gqa_val.ece15.ci}{[$-$0.003, 0.002]}
\@namedef{VJ@d.Dceperm-Dfull.gqa_val.nll}{$-$0.001}
\@namedef{VJ@d.Dceperm-Dfull.gqa_val.nll.ci}{[$-$0.002, 0.001]}
\@namedef{VJ@d.Dceperm-Dfull.macro.accuracy}{+0.002}
\@namedef{VJ@d.Dceperm-Dfull.macro.accuracy.ci}{[$-$0.000, 0.003]}
\@namedef{VJ@d.Dceperm-Dfull.macro.aurc_maxp}{+0.000}
\@namedef{VJ@d.Dceperm-Dfull.macro.aurc_maxp.ci}{[$-$0.000, 0.000]}
\@namedef{VJ@d.Dceperm-Dfull.macro.brier}{$-$0.001}
\@namedef{VJ@d.Dceperm-Dfull.macro.brier.ci}{[$-$0.002, $-$0.000]}
\@namedef{VJ@d.Dceperm-Dfull.macro.ece15}{$-$0.000}
\@namedef{VJ@d.Dceperm-Dfull.macro.ece15.ci}{[$-$0.003, 0.003]}
\@namedef{VJ@d.Dceperm-Dfull.macro.nll}{$-$0.002}
\@namedef{VJ@d.Dceperm-Dfull.macro.nll.ci}{[$-$0.004, $-$0.001]}
\@namedef{VJ@d.Dceperm-Dfull.snli_ve.accuracy}{+0.004}
\@namedef{VJ@d.Dceperm-Dfull.snli_ve.accuracy.ci}{[$-$0.001, 0.011]}
\@namedef{VJ@d.Dceperm-Dfull.snli_ve.aurc_maxp}{+0.000}
\@namedef{VJ@d.Dceperm-Dfull.snli_ve.aurc_maxp.ci}{[$-$0.002, 0.002]}
\@namedef{VJ@d.Dceperm-Dfull.snli_ve.brier}{$-$0.002}
\@namedef{VJ@d.Dceperm-Dfull.snli_ve.brier.ci}{[$-$0.005, 0.002]}
\@namedef{VJ@d.Dceperm-Dfull.snli_ve.ece15}{+0.001}
\@namedef{VJ@d.Dceperm-Dfull.snli_ve.ece15.ci}{[$-$0.008, 0.011]}
\@namedef{VJ@d.Dceperm-Dfull.snli_ve.nll}{$-$0.002}
\@namedef{VJ@d.Dceperm-Dfull.snli_ve.nll.ci}{[$-$0.007, 0.003]}
\@namedef{VJ@d.Dceperm-Dfull.tallyqa_l.accuracy}{+0.002}
\@namedef{VJ@d.Dceperm-Dfull.tallyqa_l.accuracy.ci}{[$-$0.000, 0.004]}
\@namedef{VJ@d.Dceperm-Dfull.tallyqa_l.aurc_maxp}{$-$0.000}
\@namedef{VJ@d.Dceperm-Dfull.tallyqa_l.aurc_maxp.ci}{[$-$0.001, 0.001]}
\@namedef{VJ@d.Dceperm-Dfull.tallyqa_l.brier}{$-$0.002}
\@namedef{VJ@d.Dceperm-Dfull.tallyqa_l.brier.ci}{[$-$0.002, $-$0.001]}
\@namedef{VJ@d.Dceperm-Dfull.tallyqa_l.ece15}{$-$0.000}
\@namedef{VJ@d.Dceperm-Dfull.tallyqa_l.ece15.ci}{[$-$0.003, 0.004]}
\@namedef{VJ@d.Dceperm-Dfull.tallyqa_l.nll}{$-$0.004}
\@namedef{VJ@d.Dceperm-Dfull.tallyqa_l.nll.ci}{[$-$0.006, $-$0.003]}
\@namedef{VJ@d.Dceperm-Dfull.textvqa_k8.accuracy}{+0.000}
\@namedef{VJ@d.Dceperm-Dfull.textvqa_k8.accuracy.ci}{[$-$0.001, 0.002]}
\@namedef{VJ@d.Dceperm-Dfull.textvqa_k8.aurc_maxp}{$-$0.000}
\@namedef{VJ@d.Dceperm-Dfull.textvqa_k8.aurc_maxp.ci}{[$-$0.000, $-$0.000]}
\@namedef{VJ@d.Dceperm-Dfull.textvqa_k8.brier}{$-$0.001}
\@namedef{VJ@d.Dceperm-Dfull.textvqa_k8.brier.ci}{[$-$0.001, $-$0.000]}
\@namedef{VJ@d.Dceperm-Dfull.textvqa_k8.ece15}{$-$0.001}
\@namedef{VJ@d.Dceperm-Dfull.textvqa_k8.ece15.ci}{[$-$0.003, 0.002]}
\@namedef{VJ@d.Dceperm-Dfull.textvqa_k8.nll}{$-$0.002}
\@namedef{VJ@d.Dceperm-Dfull.textvqa_k8.nll.ci}{[$-$0.004, $-$0.001]}
\@namedef{VJ@d.Dfull-M3.gqa_val.accuracy}{$-$0.003}
\@namedef{VJ@d.Dfull-M3.gqa_val.accuracy.ci}{[$-$0.006, $-$0.001]}
\@namedef{VJ@d.Dfull-M3.gqa_val.aurc_maxp}{+0.002}
\@namedef{VJ@d.Dfull-M3.gqa_val.aurc_maxp.ci}{[0.001, 0.002]}
\@namedef{VJ@d.Dfull-M3.gqa_val.brier}{+0.007}
\@namedef{VJ@d.Dfull-M3.gqa_val.brier.ci}{[0.005, 0.010]}
\@namedef{VJ@d.Dfull-M3.gqa_val.ece15}{+0.008}
\@namedef{VJ@d.Dfull-M3.gqa_val.ece15.ci}{[0.003, 0.010]}
\@namedef{VJ@d.Dfull-M3.gqa_val.nll}{+0.017}
\@namedef{VJ@d.Dfull-M3.gqa_val.nll.ci}{[0.013, 0.021]}
\@namedef{VJ@d.Dfull-M3.macro.accuracy}{$-$0.002}
\@namedef{VJ@d.Dfull-M3.macro.accuracy.ci}{[$-$0.004, 0.000]}
\@namedef{VJ@d.Dfull-M3.macro.aurc_maxp}{+0.001}
\@namedef{VJ@d.Dfull-M3.macro.aurc_maxp.ci}{[0.001, 0.002]}
\@namedef{VJ@d.Dfull-M3.macro.brier}{+0.004}
\@namedef{VJ@d.Dfull-M3.macro.brier.ci}{[0.002, 0.006]}
\@namedef{VJ@d.Dfull-M3.macro.ece15}{+0.006}
\@namedef{VJ@d.Dfull-M3.macro.ece15.ci}{[0.001, 0.008]}
\@namedef{VJ@d.Dfull-M3.macro.nll}{+0.011}
\@namedef{VJ@d.Dfull-M3.macro.nll.ci}{[0.008, 0.013]}
\@namedef{VJ@d.Dfull-M3.snli_ve.accuracy}{$-$0.006}
\@namedef{VJ@d.Dfull-M3.snli_ve.accuracy.ci}{[$-$0.014, 0.002]}
\@namedef{VJ@d.Dfull-M3.snli_ve.aurc_maxp}{+0.004}
\@namedef{VJ@d.Dfull-M3.snli_ve.aurc_maxp.ci}{[0.001, 0.006]}
\@namedef{VJ@d.Dfull-M3.snli_ve.brier}{+0.008}
\@namedef{VJ@d.Dfull-M3.snli_ve.brier.ci}{[0.002, 0.013]}
\@namedef{VJ@d.Dfull-M3.snli_ve.ece15}{+0.005}
\@namedef{VJ@d.Dfull-M3.snli_ve.ece15.ci}{[$-$0.006, 0.015]}
\@namedef{VJ@d.Dfull-M3.snli_ve.nll}{+0.016}
\@namedef{VJ@d.Dfull-M3.snli_ve.nll.ci}{[0.008, 0.023]}
\@namedef{VJ@d.Dfull-M3.tallyqa_l.accuracy}{+0.004}
\@namedef{VJ@d.Dfull-M3.tallyqa_l.accuracy.ci}{[0.000, 0.007]}
\@namedef{VJ@d.Dfull-M3.tallyqa_l.aurc_maxp}{+0.000}
\@namedef{VJ@d.Dfull-M3.tallyqa_l.aurc_maxp.ci}{[$-$0.001, 0.001]}
\@namedef{VJ@d.Dfull-M3.tallyqa_l.brier}{$-$0.000}
\@namedef{VJ@d.Dfull-M3.tallyqa_l.brier.ci}{[$-$0.002, 0.002]}
\@namedef{VJ@d.Dfull-M3.tallyqa_l.ece15}{+0.006}
\@namedef{VJ@d.Dfull-M3.tallyqa_l.ece15.ci}{[0.000, 0.008]}
\@namedef{VJ@d.Dfull-M3.tallyqa_l.nll}{+0.007}
\@namedef{VJ@d.Dfull-M3.tallyqa_l.nll.ci}{[0.003, 0.012]}
\@namedef{VJ@d.Dfull-M3.textvqa_k8.accuracy}{$-$0.002}
\@namedef{VJ@d.Dfull-M3.textvqa_k8.accuracy.ci}{[$-$0.003, 0.000]}
\@namedef{VJ@d.Dfull-M3.textvqa_k8.aurc_maxp}{+0.000}
\@namedef{VJ@d.Dfull-M3.textvqa_k8.aurc_maxp.ci}{[0.000, 0.000]}
\@namedef{VJ@d.Dfull-M3.textvqa_k8.brier}{+0.002}
\@namedef{VJ@d.Dfull-M3.textvqa_k8.brier.ci}{[0.000, 0.003]}
\@namedef{VJ@d.Dfull-M3.textvqa_k8.ece15}{+0.004}
\@namedef{VJ@d.Dfull-M3.textvqa_k8.ece15.ci}{[$-$0.000, 0.005]}
\@namedef{VJ@d.Dfull-M3.textvqa_k8.nll}{+0.003}
\@namedef{VJ@d.Dfull-M3.textvqa_k8.nll.ci}{[0.000, 0.007]}
\@namedef{VJ@d.H2k-A2k.raw.gqa_val.accuracy}{$-$0.002}
\@namedef{VJ@d.H2k-A2k.raw.gqa_val.accuracy.ci}{[$-$0.004, 0.001]}
\@namedef{VJ@d.H2k-A2k.raw.gqa_val.aurc_maxp}{+0.001}
\@namedef{VJ@d.H2k-A2k.raw.gqa_val.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@d.H2k-A2k.raw.gqa_val.brier}{+0.007}
\@namedef{VJ@d.H2k-A2k.raw.gqa_val.brier.ci}{[0.004, 0.010]}
\@namedef{VJ@d.H2k-A2k.raw.gqa_val.ece15}{+0.008}
\@namedef{VJ@d.H2k-A2k.raw.gqa_val.ece15.ci}{[0.006, 0.011]}
\@namedef{VJ@d.H2k-A2k.raw.gqa_val.nll}{+0.037}
\@namedef{VJ@d.H2k-A2k.raw.gqa_val.nll.ci}{[0.030, 0.044]}
\@namedef{VJ@d.H2k-A2k.raw.macro.accuracy}{$-$0.005}
\@namedef{VJ@d.H2k-A2k.raw.macro.accuracy.ci}{[$-$0.007, $-$0.002]}
\@namedef{VJ@d.H2k-A2k.raw.macro.aurc_maxp}{+0.003}
\@namedef{VJ@d.H2k-A2k.raw.macro.aurc_maxp.ci}{[0.002, 0.005]}
\@namedef{VJ@d.H2k-A2k.raw.macro.brier}{+0.020}
\@namedef{VJ@d.H2k-A2k.raw.macro.brier.ci}{[0.016, 0.024]}
\@namedef{VJ@d.H2k-A2k.raw.macro.ece15}{+0.027}
\@namedef{VJ@d.H2k-A2k.raw.macro.ece15.ci}{[0.024, 0.030]}
\@namedef{VJ@d.H2k-A2k.raw.macro.nll}{+0.085}
\@namedef{VJ@d.H2k-A2k.raw.macro.nll.ci}{[0.074, 0.098]}
\@namedef{VJ@d.H2k-A2k.raw.snli_ve.accuracy}{$-$0.009}
\@namedef{VJ@d.H2k-A2k.raw.snli_ve.accuracy.ci}{[$-$0.019, 0.000]}
\@namedef{VJ@d.H2k-A2k.raw.snli_ve.aurc_maxp}{+0.010}
\@namedef{VJ@d.H2k-A2k.raw.snli_ve.aurc_maxp.ci}{[0.004, 0.017]}
\@namedef{VJ@d.H2k-A2k.raw.snli_ve.brier}{+0.052}
\@namedef{VJ@d.H2k-A2k.raw.snli_ve.brier.ci}{[0.038, 0.067]}
\@namedef{VJ@d.H2k-A2k.raw.snli_ve.ece15}{+0.071}
\@namedef{VJ@d.H2k-A2k.raw.snli_ve.ece15.ci}{[0.061, 0.081]}
\@namedef{VJ@d.H2k-A2k.raw.snli_ve.nll}{+0.230}
\@namedef{VJ@d.H2k-A2k.raw.snli_ve.nll.ci}{[0.187, 0.273]}
\@namedef{VJ@d.H2k-A2k.raw.tallyqa_l.accuracy}{$-$0.007}
\@namedef{VJ@d.H2k-A2k.raw.tallyqa_l.accuracy.ci}{[$-$0.010, $-$0.003]}
\@namedef{VJ@d.H2k-A2k.raw.tallyqa_l.aurc_maxp}{+0.001}
\@namedef{VJ@d.H2k-A2k.raw.tallyqa_l.aurc_maxp.ci}{[0.000, 0.002]}
\@namedef{VJ@d.H2k-A2k.raw.tallyqa_l.brier}{+0.018}
\@namedef{VJ@d.H2k-A2k.raw.tallyqa_l.brier.ci}{[0.015, 0.022]}
\@namedef{VJ@d.H2k-A2k.raw.tallyqa_l.ece15}{+0.028}
\@namedef{VJ@d.H2k-A2k.raw.tallyqa_l.ece15.ci}{[0.024, 0.031]}
\@namedef{VJ@d.H2k-A2k.raw.tallyqa_l.nll}{+0.067}
\@namedef{VJ@d.H2k-A2k.raw.tallyqa_l.nll.ci}{[0.057, 0.077]}
\@namedef{VJ@d.H2k-A2k.raw.textvqa_k8.accuracy}{$-$0.001}
\@namedef{VJ@d.H2k-A2k.raw.textvqa_k8.accuracy.ci}{[$-$0.003, 0.001]}
\@namedef{VJ@d.H2k-A2k.raw.textvqa_k8.aurc_maxp}{+0.000}
\@namedef{VJ@d.H2k-A2k.raw.textvqa_k8.aurc_maxp.ci}{[$-$0.000, 0.000]}
\@namedef{VJ@d.H2k-A2k.raw.textvqa_k8.brier}{+0.002}
\@namedef{VJ@d.H2k-A2k.raw.textvqa_k8.brier.ci}{[0.001, 0.004]}
\@namedef{VJ@d.H2k-A2k.raw.textvqa_k8.ece15}{+0.003}
\@namedef{VJ@d.H2k-A2k.raw.textvqa_k8.ece15.ci}{[0.000, 0.005]}
\@namedef{VJ@d.H2k-A2k.raw.textvqa_k8.nll}{+0.008}
\@namedef{VJ@d.H2k-A2k.raw.textvqa_k8.nll.ci}{[0.002, 0.015]}
\@namedef{VJ@d.H2k-A2k.ts.gqa_val.accuracy}{$-$0.002}
\@namedef{VJ@d.H2k-A2k.ts.gqa_val.accuracy.ci}{[$-$0.004, 0.001]}
\@namedef{VJ@d.H2k-A2k.ts.gqa_val.aurc_maxp}{+0.001}
\@namedef{VJ@d.H2k-A2k.ts.gqa_val.aurc_maxp.ci}{[0.000, 0.001]}
\@namedef{VJ@d.H2k-A2k.ts.gqa_val.brier}{+0.004}
\@namedef{VJ@d.H2k-A2k.ts.gqa_val.brier.ci}{[0.002, 0.006]}
\@namedef{VJ@d.H2k-A2k.ts.gqa_val.ece15}{+0.001}
\@namedef{VJ@d.H2k-A2k.ts.gqa_val.ece15.ci}{[$-$0.003, 0.003]}
\@namedef{VJ@d.H2k-A2k.ts.gqa_val.nll}{+0.015}
\@namedef{VJ@d.H2k-A2k.ts.gqa_val.nll.ci}{[0.011, 0.018]}
\@namedef{VJ@d.H2k-A2k.ts.macro.accuracy}{$-$0.005}
\@namedef{VJ@d.H2k-A2k.ts.macro.accuracy.ci}{[$-$0.007, $-$0.002]}
\@namedef{VJ@d.H2k-A2k.ts.macro.aurc_maxp}{+0.003}
\@namedef{VJ@d.H2k-A2k.ts.macro.aurc_maxp.ci}{[0.002, 0.005]}
\@namedef{VJ@d.H2k-A2k.ts.macro.brier}{+0.009}
\@namedef{VJ@d.H2k-A2k.ts.macro.brier.ci}{[0.007, 0.012]}
\@namedef{VJ@d.H2k-A2k.ts.macro.ece15}{+0.003}
\@namedef{VJ@d.H2k-A2k.ts.macro.ece15.ci}{[$-$0.001, 0.006]}
\@namedef{VJ@d.H2k-A2k.ts.macro.nll}{+0.029}
\@namedef{VJ@d.H2k-A2k.ts.macro.nll.ci}{[0.024, 0.033]}
\@namedef{VJ@d.H2k-A2k.ts.snli_ve.accuracy}{$-$0.009}
\@namedef{VJ@d.H2k-A2k.ts.snli_ve.accuracy.ci}{[$-$0.019, 0.000]}
\@namedef{VJ@d.H2k-A2k.ts.snli_ve.aurc_maxp}{+0.011}
\@namedef{VJ@d.H2k-A2k.ts.snli_ve.aurc_maxp.ci}{[0.005, 0.017]}
\@namedef{VJ@d.H2k-A2k.ts.snli_ve.brier}{+0.023}
\@namedef{VJ@d.H2k-A2k.ts.snli_ve.brier.ci}{[0.014, 0.033]}
\@namedef{VJ@d.H2k-A2k.ts.snli_ve.ece15}{+0.005}
\@namedef{VJ@d.H2k-A2k.ts.snli_ve.ece15.ci}{[$-$0.008, 0.018]}
\@namedef{VJ@d.H2k-A2k.ts.snli_ve.nll}{+0.061}
\@namedef{VJ@d.H2k-A2k.ts.snli_ve.nll.ci}{[0.044, 0.078]}
\@namedef{VJ@d.H2k-A2k.ts.tallyqa_l.accuracy}{$-$0.007}
\@namedef{VJ@d.H2k-A2k.ts.tallyqa_l.accuracy.ci}{[$-$0.010, $-$0.003]}
\@namedef{VJ@d.H2k-A2k.ts.tallyqa_l.aurc_maxp}{+0.001}
\@namedef{VJ@d.H2k-A2k.ts.tallyqa_l.aurc_maxp.ci}{[0.000, 0.002]}
\@namedef{VJ@d.H2k-A2k.ts.tallyqa_l.brier}{+0.009}
\@namedef{VJ@d.H2k-A2k.ts.tallyqa_l.brier.ci}{[0.006, 0.011]}
\@namedef{VJ@d.H2k-A2k.ts.tallyqa_l.ece15}{+0.003}
\@namedef{VJ@d.H2k-A2k.ts.tallyqa_l.ece15.ci}{[$-$0.001, 0.008]}
\@namedef{VJ@d.H2k-A2k.ts.tallyqa_l.nll}{+0.034}
\@namedef{VJ@d.H2k-A2k.ts.tallyqa_l.nll.ci}{[0.029, 0.040]}
\@namedef{VJ@d.H2k-A2k.ts.textvqa_k8.accuracy}{$-$0.001}
\@namedef{VJ@d.H2k-A2k.ts.textvqa_k8.accuracy.ci}{[$-$0.003, 0.001]}
\@namedef{VJ@d.H2k-A2k.ts.textvqa_k8.aurc_maxp}{+0.000}
\@namedef{VJ@d.H2k-A2k.ts.textvqa_k8.aurc_maxp.ci}{[$-$0.000, 0.000]}
\@namedef{VJ@d.H2k-A2k.ts.textvqa_k8.brier}{+0.001}
\@namedef{VJ@d.H2k-A2k.ts.textvqa_k8.brier.ci}{[0.000, 0.003]}
\@namedef{VJ@d.H2k-A2k.ts.textvqa_k8.ece15}{+0.004}
\@namedef{VJ@d.H2k-A2k.ts.textvqa_k8.ece15.ci}{[$-$0.001, 0.006]}
\@namedef{VJ@d.H2k-A2k.ts.textvqa_k8.nll}{+0.004}
\@namedef{VJ@d.H2k-A2k.ts.textvqa_k8.nll.ci}{[$-$0.000, 0.009]}
\@namedef{VJ@d.M1-M0.gqa_val.accuracy}{+0.037}
\@namedef{VJ@d.M1-M0.gqa_val.accuracy.ci}{[0.030, 0.044]}
\@namedef{VJ@d.M1-M0.gqa_val.aurc_maxp}{$-$0.019}
\@namedef{VJ@d.M1-M0.gqa_val.aurc_maxp.ci}{[$-$0.024, $-$0.015]}
\@namedef{VJ@d.M1-M0.gqa_val.brier}{$-$0.070}
\@namedef{VJ@d.M1-M0.gqa_val.brier.ci}{[$-$0.081, $-$0.058]}
\@namedef{VJ@d.M1-M0.gqa_val.ece15}{$-$0.042}
\@namedef{VJ@d.M1-M0.gqa_val.ece15.ci}{[$-$0.048, $-$0.034]}
\@namedef{VJ@d.M1-M0.gqa_val.nll}{$-$0.286}
\@namedef{VJ@d.M1-M0.gqa_val.nll.ci}{[$-$0.322, $-$0.252]}
\@namedef{VJ@d.M1-M0.macro.accuracy}{+0.051}
\@namedef{VJ@d.M1-M0.macro.accuracy.ci}{[0.044, 0.059]}
\@namedef{VJ@d.M1-M0.macro.aurc_maxp}{$-$0.049}
\@namedef{VJ@d.M1-M0.macro.aurc_maxp.ci}{[$-$0.056, $-$0.042]}
\@namedef{VJ@d.M1-M0.macro.brier}{$-$0.122}
\@namedef{VJ@d.M1-M0.macro.brier.ci}{[$-$0.134, $-$0.109]}
\@namedef{VJ@d.M1-M0.macro.ece15}{$-$0.088}
\@namedef{VJ@d.M1-M0.macro.ece15.ci}{[$-$0.094, $-$0.080]}
\@namedef{VJ@d.M1-M0.macro.nll}{$-$0.678}
\@namedef{VJ@d.M1-M0.macro.nll.ci}{[$-$0.737, $-$0.626]}
\@namedef{VJ@d.M1-M0.snli_ve.accuracy}{+0.180}
\@namedef{VJ@d.M1-M0.snli_ve.accuracy.ci}{[0.152, 0.207]}
\@namedef{VJ@d.M1-M0.snli_ve.aurc_maxp}{$-$0.175}
\@namedef{VJ@d.M1-M0.snli_ve.aurc_maxp.ci}{[$-$0.202, $-$0.149]}
\@namedef{VJ@d.M1-M0.snli_ve.brier}{$-$0.390}
\@namedef{VJ@d.M1-M0.snli_ve.brier.ci}{[$-$0.437, $-$0.344]}
\@namedef{VJ@d.M1-M0.snli_ve.ece15}{$-$0.254}
\@namedef{VJ@d.M1-M0.snli_ve.ece15.ci}{[$-$0.279, $-$0.226]}
\@namedef{VJ@d.M1-M0.snli_ve.nll}{$-$2.077}
\@namedef{VJ@d.M1-M0.snli_ve.nll.ci}{[$-$2.299, $-$1.883]}
\@namedef{VJ@d.M1-M0.tallyqa_l.accuracy}{$-$0.011}
\@namedef{VJ@d.M1-M0.tallyqa_l.accuracy.ci}{[$-$0.019, $-$0.004]}
\@namedef{VJ@d.M1-M0.tallyqa_l.aurc_maxp}{$-$0.001}
\@namedef{VJ@d.M1-M0.tallyqa_l.aurc_maxp.ci}{[$-$0.006, 0.002]}
\@namedef{VJ@d.M1-M0.tallyqa_l.brier}{$-$0.023}
\@namedef{VJ@d.M1-M0.tallyqa_l.brier.ci}{[$-$0.035, $-$0.012]}
\@namedef{VJ@d.M1-M0.tallyqa_l.ece15}{$-$0.049}
\@namedef{VJ@d.M1-M0.tallyqa_l.ece15.ci}{[$-$0.057, $-$0.041]}
\@namedef{VJ@d.M1-M0.tallyqa_l.nll}{$-$0.313}
\@namedef{VJ@d.M1-M0.tallyqa_l.nll.ci}{[$-$0.366, $-$0.266]}
\@namedef{VJ@d.M1-M0.textvqa_k8.accuracy}{+0.001}
\@namedef{VJ@d.M1-M0.textvqa_k8.accuracy.ci}{[$-$0.002, 0.004]}
\@namedef{VJ@d.M1-M0.textvqa_k8.aurc_maxp}{$-$0.000}
\@namedef{VJ@d.M1-M0.textvqa_k8.aurc_maxp.ci}{[$-$0.000, 0.000]}
\@namedef{VJ@d.M1-M0.textvqa_k8.brier}{$-$0.004}
\@namedef{VJ@d.M1-M0.textvqa_k8.brier.ci}{[$-$0.008, 0.001]}
\@namedef{VJ@d.M1-M0.textvqa_k8.ece15}{$-$0.006}
\@namedef{VJ@d.M1-M0.textvqa_k8.ece15.ci}{[$-$0.009, $-$0.001]}
\@namedef{VJ@d.M1-M0.textvqa_k8.nll}{$-$0.037}
\@namedef{VJ@d.M1-M0.textvqa_k8.nll.ci}{[$-$0.057, $-$0.019]}
\@namedef{VJ@d.M2-M0.gqa_val.accuracy}{+0.000}
\@namedef{VJ@d.M2-M0.gqa_val.accuracy.ci}{[0.000, 0.000]}
\@namedef{VJ@d.M2-M0.gqa_val.aurc_maxp}{+0.004}
\@namedef{VJ@d.M2-M0.gqa_val.aurc_maxp.ci}{[0.003, 0.005]}
\@namedef{VJ@d.M2-M0.gqa_val.brier}{$-$0.029}
\@namedef{VJ@d.M2-M0.gqa_val.brier.ci}{[$-$0.033, $-$0.024]}
\@namedef{VJ@d.M2-M0.gqa_val.ece15}{$-$0.079}
\@namedef{VJ@d.M2-M0.gqa_val.ece15.ci}{[$-$0.083, $-$0.068]}
\@namedef{VJ@d.M2-M0.gqa_val.nll}{$-$0.233}
\@namedef{VJ@d.M2-M0.gqa_val.nll.ci}{[$-$0.262, $-$0.204]}
\@namedef{VJ@d.M2-M0.macro.accuracy}{+0.000}
\@namedef{VJ@d.M2-M0.macro.accuracy.ci}{[0.000, 0.000]}
\@namedef{VJ@d.M2-M0.macro.aurc_maxp}{+0.001}
\@namedef{VJ@d.M2-M0.macro.aurc_maxp.ci}{[0.001, 0.002]}
\@namedef{VJ@d.M2-M0.macro.brier}{$-$0.064}
\@namedef{VJ@d.M2-M0.macro.brier.ci}{[$-$0.072, $-$0.057]}
\@namedef{VJ@d.M2-M0.macro.ece15}{$-$0.105}
\@namedef{VJ@d.M2-M0.macro.ece15.ci}{[$-$0.111, $-$0.096]}
\@namedef{VJ@d.M2-M0.macro.nll}{$-$0.593}
\@namedef{VJ@d.M2-M0.macro.nll.ci}{[$-$0.645, $-$0.546]}
\@namedef{VJ@d.M2-M0.snli_ve.accuracy}{+0.000}
\@namedef{VJ@d.M2-M0.snli_ve.accuracy.ci}{[0.000, 0.000]}
\@namedef{VJ@d.M2-M0.snli_ve.aurc_maxp}{+0.001}
\@namedef{VJ@d.M2-M0.snli_ve.aurc_maxp.ci}{[$-$0.001, 0.002]}
\@namedef{VJ@d.M2-M0.snli_ve.brier}{$-$0.188}
\@namedef{VJ@d.M2-M0.snli_ve.brier.ci}{[$-$0.216, $-$0.161]}
\@namedef{VJ@d.M2-M0.snli_ve.ece15}{$-$0.249}
\@namedef{VJ@d.M2-M0.snli_ve.ece15.ci}{[$-$0.273, $-$0.224]}
\@namedef{VJ@d.M2-M0.snli_ve.nll}{$-$1.772}
\@namedef{VJ@d.M2-M0.snli_ve.nll.ci}{[$-$1.976, $-$1.591]}
\@namedef{VJ@d.M2-M0.tallyqa_l.accuracy}{+0.000}
\@namedef{VJ@d.M2-M0.tallyqa_l.accuracy.ci}{[0.000, 0.000]}
\@namedef{VJ@d.M2-M0.tallyqa_l.aurc_maxp}{+0.001}
\@namedef{VJ@d.M2-M0.tallyqa_l.aurc_maxp.ci}{[0.000, 0.002]}
\@namedef{VJ@d.M2-M0.tallyqa_l.brier}{$-$0.039}
\@namedef{VJ@d.M2-M0.tallyqa_l.brier.ci}{[$-$0.045, $-$0.033]}
\@namedef{VJ@d.M2-M0.tallyqa_l.ece15}{$-$0.084}
\@namedef{VJ@d.M2-M0.tallyqa_l.ece15.ci}{[$-$0.091, $-$0.071]}
\@namedef{VJ@d.M2-M0.tallyqa_l.nll}{$-$0.329}
\@namedef{VJ@d.M2-M0.tallyqa_l.nll.ci}{[$-$0.376, $-$0.287]}
\@namedef{VJ@d.M2-M0.textvqa_k8.accuracy}{+0.000}
\@namedef{VJ@d.M2-M0.textvqa_k8.accuracy.ci}{[0.000, 0.000]}
\@namedef{VJ@d.M2-M0.textvqa_k8.aurc_maxp}{+0.000}
\@namedef{VJ@d.M2-M0.textvqa_k8.aurc_maxp.ci}{[$-$0.000, 0.000]}
\@namedef{VJ@d.M2-M0.textvqa_k8.brier}{$-$0.003}
\@namedef{VJ@d.M2-M0.textvqa_k8.brier.ci}{[$-$0.005, $-$0.001]}
\@namedef{VJ@d.M2-M0.textvqa_k8.ece15}{$-$0.009}
\@namedef{VJ@d.M2-M0.textvqa_k8.ece15.ci}{[$-$0.012, $-$0.000]}
\@namedef{VJ@d.M2-M0.textvqa_k8.nll}{$-$0.040}
\@namedef{VJ@d.M2-M0.textvqa_k8.nll.ci}{[$-$0.059, $-$0.022]}
\@namedef{VJ@d.M3-M1.gqa_val.accuracy}{+0.000}
\@namedef{VJ@d.M3-M1.gqa_val.accuracy.ci}{[0.000, 0.000]}
\@namedef{VJ@d.M3-M1.gqa_val.aurc_maxp}{$-$0.000}
\@namedef{VJ@d.M3-M1.gqa_val.aurc_maxp.ci}{[$-$0.000, 0.000]}
\@namedef{VJ@d.M3-M1.gqa_val.brier}{$-$0.011}
\@namedef{VJ@d.M3-M1.gqa_val.brier.ci}{[$-$0.013, $-$0.009]}
\@namedef{VJ@d.M3-M1.gqa_val.ece15}{$-$0.032}
\@namedef{VJ@d.M3-M1.gqa_val.ece15.ci}{[$-$0.036, $-$0.025]}
\@namedef{VJ@d.M3-M1.gqa_val.nll}{$-$0.043}
\@namedef{VJ@d.M3-M1.gqa_val.nll.ci}{[$-$0.052, $-$0.033]}
\@namedef{VJ@d.M3-M1.macro.accuracy}{+0.000}
\@namedef{VJ@d.M3-M1.macro.accuracy.ci}{[0.000, 0.000]}
\@namedef{VJ@d.M3-M1.macro.aurc_maxp}{$-$0.000}
\@namedef{VJ@d.M3-M1.macro.aurc_maxp.ci}{[$-$0.000, $-$0.000]}
\@namedef{VJ@d.M3-M1.macro.brier}{$-$0.008}
\@namedef{VJ@d.M3-M1.macro.brier.ci}{[$-$0.009, $-$0.006]}
\@namedef{VJ@d.M3-M1.macro.ece15}{$-$0.022}
\@namedef{VJ@d.M3-M1.macro.ece15.ci}{[$-$0.026, $-$0.014]}
\@namedef{VJ@d.M3-M1.macro.nll}{$-$0.022}
\@namedef{VJ@d.M3-M1.macro.nll.ci}{[$-$0.027, $-$0.017]}
\@namedef{VJ@d.M3-M1.snli_ve.accuracy}{+0.000}
\@namedef{VJ@d.M3-M1.snli_ve.accuracy.ci}{[0.000, 0.000]}
\@namedef{VJ@d.M3-M1.snli_ve.aurc_maxp}{$-$0.001}
\@namedef{VJ@d.M3-M1.snli_ve.aurc_maxp.ci}{[$-$0.001, $-$0.000]}
\@namedef{VJ@d.M3-M1.snli_ve.brier}{$-$0.010}
\@namedef{VJ@d.M3-M1.snli_ve.brier.ci}{[$-$0.015, $-$0.005]}
\@namedef{VJ@d.M3-M1.snli_ve.ece15}{$-$0.028}
\@namedef{VJ@d.M3-M1.snli_ve.ece15.ci}{[$-$0.047, $-$0.007]}
\@namedef{VJ@d.M3-M1.snli_ve.nll}{$-$0.020}
\@namedef{VJ@d.M3-M1.snli_ve.nll.ci}{[$-$0.034, $-$0.007]}
\@namedef{VJ@d.M3-M1.tallyqa_l.accuracy}{+0.000}
\@namedef{VJ@d.M3-M1.tallyqa_l.accuracy.ci}{[0.000, 0.000]}
\@namedef{VJ@d.M3-M1.tallyqa_l.aurc_maxp}{$-$0.000}
\@namedef{VJ@d.M3-M1.tallyqa_l.aurc_maxp.ci}{[$-$0.000, 0.000]}
\@namedef{VJ@d.M3-M1.tallyqa_l.brier}{$-$0.009}
\@namedef{VJ@d.M3-M1.tallyqa_l.brier.ci}{[$-$0.011, $-$0.007]}
\@namedef{VJ@d.M3-M1.tallyqa_l.ece15}{$-$0.023}
\@namedef{VJ@d.M3-M1.tallyqa_l.ece15.ci}{[$-$0.028, $-$0.016]}
\@namedef{VJ@d.M3-M1.tallyqa_l.nll}{$-$0.019}
\@namedef{VJ@d.M3-M1.tallyqa_l.nll.ci}{[$-$0.026, $-$0.013]}
\@namedef{VJ@d.M3-M1.textvqa_k8.accuracy}{+0.000}
\@namedef{VJ@d.M3-M1.textvqa_k8.accuracy.ci}{[0.000, 0.000]}
\@namedef{VJ@d.M3-M1.textvqa_k8.aurc_maxp}{$-$0.000}
\@namedef{VJ@d.M3-M1.textvqa_k8.aurc_maxp.ci}{[$-$0.000, $-$0.000]}
\@namedef{VJ@d.M3-M1.textvqa_k8.brier}{$-$0.001}
\@namedef{VJ@d.M3-M1.textvqa_k8.brier.ci}{[$-$0.002, 0.000]}
\@namedef{VJ@d.M3-M1.textvqa_k8.ece15}{$-$0.003}
\@namedef{VJ@d.M3-M1.textvqa_k8.ece15.ci}{[$-$0.006, 0.003]}
\@namedef{VJ@d.M3-M1.textvqa_k8.nll}{$-$0.007}
\@namedef{VJ@d.M3-M1.textvqa_k8.nll.ci}{[$-$0.013, $-$0.001]}
\@namedef{VJ@d.M3-M2.gqa_val.accuracy}{+0.037}
\@namedef{VJ@d.M3-M2.gqa_val.accuracy.ci}{[0.030, 0.044]}
\@namedef{VJ@d.M3-M2.gqa_val.aurc_maxp}{$-$0.023}
\@namedef{VJ@d.M3-M2.gqa_val.aurc_maxp.ci}{[$-$0.028, $-$0.018]}
\@namedef{VJ@d.M3-M2.gqa_val.brier}{$-$0.052}
\@namedef{VJ@d.M3-M2.gqa_val.brier.ci}{[$-$0.059, $-$0.044]}
\@namedef{VJ@d.M3-M2.gqa_val.ece15}{+0.005}
\@namedef{VJ@d.M3-M2.gqa_val.ece15.ci}{[$-$0.002, 0.011]}
\@namedef{VJ@d.M3-M2.gqa_val.nll}{$-$0.096}
\@namedef{VJ@d.M3-M2.gqa_val.nll.ci}{[$-$0.108, $-$0.083]}
\@namedef{VJ@d.M3-M2.macro.accuracy}{+0.051}
\@namedef{VJ@d.M3-M2.macro.accuracy.ci}{[0.044, 0.059]}
\@namedef{VJ@d.M3-M2.macro.aurc_maxp}{$-$0.050}
\@namedef{VJ@d.M3-M2.macro.aurc_maxp.ci}{[$-$0.057, $-$0.044]}
\@namedef{VJ@d.M3-M2.macro.brier}{$-$0.065}
\@namedef{VJ@d.M3-M2.macro.brier.ci}{[$-$0.071, $-$0.057]}
\@namedef{VJ@d.M3-M2.macro.ece15}{$-$0.004}
\@namedef{VJ@d.M3-M2.macro.ece15.ci}{[$-$0.011, 0.004]}
\@namedef{VJ@d.M3-M2.macro.nll}{$-$0.107}
\@namedef{VJ@d.M3-M2.macro.nll.ci}{[$-$0.117, $-$0.096]}
\@namedef{VJ@d.M3-M2.snli_ve.accuracy}{+0.180}
\@namedef{VJ@d.M3-M2.snli_ve.accuracy.ci}{[0.152, 0.207]}
\@namedef{VJ@d.M3-M2.snli_ve.aurc_maxp}{$-$0.176}
\@namedef{VJ@d.M3-M2.snli_ve.aurc_maxp.ci}{[$-$0.203, $-$0.150]}
\@namedef{VJ@d.M3-M2.snli_ve.brier}{$-$0.212}
\@namedef{VJ@d.M3-M2.snli_ve.brier.ci}{[$-$0.238, $-$0.186]}
\@namedef{VJ@d.M3-M2.snli_ve.ece15}{$-$0.033}
\@namedef{VJ@d.M3-M2.snli_ve.ece15.ci}{[$-$0.058, $-$0.004]}
\@namedef{VJ@d.M3-M2.snli_ve.nll}{$-$0.325}
\@namedef{VJ@d.M3-M2.snli_ve.nll.ci}{[$-$0.363, $-$0.287]}
\@namedef{VJ@d.M3-M2.tallyqa_l.accuracy}{$-$0.011}
\@namedef{VJ@d.M3-M2.tallyqa_l.accuracy.ci}{[$-$0.019, $-$0.004]}
\@namedef{VJ@d.M3-M2.tallyqa_l.aurc_maxp}{$-$0.002}
\@namedef{VJ@d.M3-M2.tallyqa_l.aurc_maxp.ci}{[$-$0.007, 0.002]}
\@namedef{VJ@d.M3-M2.tallyqa_l.brier}{+0.007}
\@namedef{VJ@d.M3-M2.tallyqa_l.brier.ci}{[$-$0.001, 0.014]}
\@namedef{VJ@d.M3-M2.tallyqa_l.ece15}{+0.012}
\@namedef{VJ@d.M3-M2.tallyqa_l.ece15.ci}{[0.001, 0.019]}
\@namedef{VJ@d.M3-M2.tallyqa_l.nll}{$-$0.003}
\@namedef{VJ@d.M3-M2.tallyqa_l.nll.ci}{[$-$0.018, 0.010]}
\@namedef{VJ@d.M3-M2.textvqa_k8.accuracy}{+0.001}
\@namedef{VJ@d.M3-M2.textvqa_k8.accuracy.ci}{[$-$0.002, 0.004]}
\@namedef{VJ@d.M3-M2.textvqa_k8.aurc_maxp}{$-$0.000}
\@namedef{VJ@d.M3-M2.textvqa_k8.aurc_maxp.ci}{[$-$0.000, 0.000]}
\@namedef{VJ@d.M3-M2.textvqa_k8.brier}{$-$0.001}
\@namedef{VJ@d.M3-M2.textvqa_k8.brier.ci}{[$-$0.005, 0.002]}
\@namedef{VJ@d.M3-M2.textvqa_k8.ece15}{+0.000}
\@namedef{VJ@d.M3-M2.textvqa_k8.ece15.ci}{[$-$0.004, 0.005]}
\@namedef{VJ@d.M3-M2.textvqa_k8.nll}{$-$0.004}
\@namedef{VJ@d.M3-M2.textvqa_k8.nll.ci}{[$-$0.012, 0.004]}
\@namedef{VJ@drift.a2.snli.hf_vllm.flip5}{13/632}
\@namedef{VJ@drift.flip5.maxpct}{2.1\%}
\@namedef{VJ@drift.matrix.argmax.max}{3}
\@namedef{VJ@drift.matrix.flip10.max}{0}
\@namedef{VJ@drift.matrix.flip5.max}{15}
\@namedef{VJ@drift.matrix.flip5.min}{8}
\@namedef{VJ@drift.matrix.n}{1,920}
\@namedef{VJ@ens.M0.perm_avg_ts.aurc}{0.173}
\@namedef{VJ@ens.M0.perm_avg_ts.nll}{0.665}
\@namedef{VJ@ens.M0.single_ts.aurc}{0.185}
\@namedef{VJ@ens.M0.single_ts.nll}{0.698}
\@namedef{VJ@ens.M1.perm_avg_ts.aurc}{0.130}
\@namedef{VJ@ens.M1.perm_avg_ts.nll}{0.580}
\@namedef{VJ@ens.M1.single_ts.aurc}{0.131}
\@namedef{VJ@ens.M1.single_ts.nll}{0.591}
\@namedef{VJ@ex.T}{1.36}
\@namedef{VJ@ex.gold}{not determined by the image}
\@namedef{VJ@ex.o0.dec}{accept}
\@namedef{VJ@ex.o0.top}{0.89}
\@namedef{VJ@ex.o1.dec}{review}
\@namedef{VJ@ex.o1.top}{0.78}
\@namedef{VJ@ex.statement}{Two men enjoy doing karate.}
\@namedef{VJ@ex.thr}{0.88}
\@namedef{VJ@load.S1.32.1.p50}{183}
\@namedef{VJ@load.S1.32.1.p95}{301}
\@namedef{VJ@load.S1.32.2.p50}{187}
\@namedef{VJ@load.S1.32.2.p95}{478}
\@namedef{VJ@load.S1.32.3.p50}{209}
\@namedef{VJ@load.S1.32.3.p95}{497}
\@namedef{VJ@load.S1.32.4.p50}{339}
\@namedef{VJ@load.S1.32.4.p95}{802}
\@namedef{VJ@load.S1.32.5.p50}{514}
\@namedef{VJ@load.S1.32.5.p95}{1427}
\@namedef{VJ@load.S1.32.6.p50}{2814}
\@namedef{VJ@load.S1.32.6.p95}{4143}
\@namedef{VJ@load.S1.32.7.p50}{6235}
\@namedef{VJ@load.S1.32.7.p95}{9076}
\@namedef{VJ@load.S1.32.8.p50}{6164}
\@namedef{VJ@load.S1.32.8.p95}{11974}
\@namedef{VJ@load.S1.32.max}{5.6}
\@namedef{VJ@load.S1.32.maxq}{181}
\@namedef{VJ@load.S1.8.10.p50}{233}
\@namedef{VJ@load.S1.8.10.p95}{552}
\@namedef{VJ@load.S1.8.12.p50}{823}
\@namedef{VJ@load.S1.8.12.p95}{2136}
\@namedef{VJ@load.S1.8.14.p50}{2847}
\@namedef{VJ@load.S1.8.14.p95}{5879}
\@namedef{VJ@load.S1.8.16.p50}{3193}
\@namedef{VJ@load.S1.8.16.p95}{5677}
\@namedef{VJ@load.S1.8.2.p50}{94}
\@namedef{VJ@load.S1.8.2.p95}{198}
\@namedef{VJ@load.S1.8.4.p50}{97}
\@namedef{VJ@load.S1.8.4.p95}{208}
\@namedef{VJ@load.S1.8.6.p50}{121}
\@namedef{VJ@load.S1.8.6.p95}{308}
\@namedef{VJ@load.S1.8.8.p50}{196}
\@namedef{VJ@load.S1.8.8.p95}{648}
\@namedef{VJ@load.S1.8.max}{10.9}
\@namedef{VJ@load.S1.8.maxq}{87}
\@namedef{VJ@load.S2.32.1.p50}{511}
\@namedef{VJ@load.S2.32.1.p95}{1013}
\@namedef{VJ@load.S2.32.2.p50}{4385}
\@namedef{VJ@load.S2.32.2.p95}{6990}
\@namedef{VJ@load.S2.32.3.p50}{10344}
\@namedef{VJ@load.S2.32.3.p95}{23116}
\@namedef{VJ@load.S2.32.4.p50}{22557}
\@namedef{VJ@load.S2.32.4.p95}{40403}
\@namedef{VJ@load.S2.32.5.p50}{25261}
\@namedef{VJ@load.S2.32.5.p95}{45285}
\@namedef{VJ@load.S2.32.6.p50}{27733}
\@namedef{VJ@load.S2.32.6.p95}{50905}
\@namedef{VJ@load.S2.32.7.p50}{31993}
\@namedef{VJ@load.S2.32.7.p95}{58009}
\@namedef{VJ@load.S2.32.8.p50}{32292}
\@namedef{VJ@load.S2.32.8.p95}{60712}
\@namedef{VJ@load.S2.32.max}{2.3}
\@namedef{VJ@load.S2.32.maxq}{74}
\@namedef{VJ@load.S2.8.10.p50}{1143}
\@namedef{VJ@load.S2.8.10.p95}{1785}
\@namedef{VJ@load.S2.8.12.p50}{2436}
\@namedef{VJ@load.S2.8.12.p95}{5451}
\@namedef{VJ@load.S2.8.14.p50}{4878}
\@namedef{VJ@load.S2.8.14.p95}{9297}
\@namedef{VJ@load.S2.8.16.p50}{5211}
\@namedef{VJ@load.S2.8.16.p95}{9040}
\@namedef{VJ@load.S2.8.2.p50}{162}
\@namedef{VJ@load.S2.8.2.p95}{286}
\@namedef{VJ@load.S2.8.4.p50}{186}
\@namedef{VJ@load.S2.8.4.p95}{370}
\@namedef{VJ@load.S2.8.6.p50}{224}
\@namedef{VJ@load.S2.8.6.p95}{505}
\@namedef{VJ@load.S2.8.8.p50}{459}
\@namedef{VJ@load.S2.8.8.p95}{1114}
\@namedef{VJ@load.S2.8.max}{9.1}
\@namedef{VJ@load.S2.8.maxq}{73}
\@namedef{VJ@load.S3.32.1.p50}{234}
\@namedef{VJ@load.S3.32.1.p95}{389}
\@namedef{VJ@load.S3.32.2.p50}{259}
\@namedef{VJ@load.S3.32.2.p95}{620}
\@namedef{VJ@load.S3.32.3.p50}{304}
\@namedef{VJ@load.S3.32.3.p95}{671}
\@namedef{VJ@load.S3.32.4.p50}{653}
\@namedef{VJ@load.S3.32.4.p95}{1510}
\@namedef{VJ@load.S3.32.5.p50}{1863}
\@namedef{VJ@load.S3.32.5.p95}{3035}
\@namedef{VJ@load.S3.32.6.p50}{5592}
\@namedef{VJ@load.S3.32.6.p95}{8703}
\@namedef{VJ@load.S3.32.7.p50}{8935}
\@namedef{VJ@load.S3.32.7.p95}{14036}
\@namedef{VJ@load.S3.32.8.p50}{8978}
\@namedef{VJ@load.S3.32.8.p95}{17091}
\@namedef{VJ@load.S3.32.max}{4.9}
\@namedef{VJ@load.S3.32.maxq}{157}
\@namedef{VJ@load.S3.8.10.p50}{97}
\@namedef{VJ@load.S3.8.10.p95}{181}
\@namedef{VJ@load.S3.8.12.p50}{103}
\@namedef{VJ@load.S3.8.12.p95}{211}
\@namedef{VJ@load.S3.8.14.p50}{167}
\@namedef{VJ@load.S3.8.14.p95}{349}
\@namedef{VJ@load.S3.8.16.p50}{178}
\@namedef{VJ@load.S3.8.16.p95}{463}
\@namedef{VJ@load.S3.8.2.p50}{77}
\@namedef{VJ@load.S3.8.2.p95}{118}
\@namedef{VJ@load.S3.8.4.p50}{79}
\@namedef{VJ@load.S3.8.4.p95}{127}
\@namedef{VJ@load.S3.8.6.p50}{83}
\@namedef{VJ@load.S3.8.6.p95}{140}
\@namedef{VJ@load.S3.8.8.p50}{93}
\@namedef{VJ@load.S3.8.8.p95}{171}
\@namedef{VJ@load.S3.8.max}{16.2}
\@namedef{VJ@load.S3.8.maxq}{129}
\@namedef{VJ@load.ref32}{3}
\@namedef{VJ@load.ref8}{8}
\@namedef{VJ@n.gqa_val.calib}{2,259}
\@namedef{VJ@n.gqa_val.test}{5,447}
\@namedef{VJ@n.gqa_val.testimg}{1,060}
\@namedef{VJ@n.snli_ve.calib}{632}
\@namedef{VJ@n.snli_ve.test}{1,368}
\@namedef{VJ@n.snli_ve.testimg}{583}
\@namedef{VJ@n.tallyqa_l.all}{5,180}
\@namedef{VJ@n.tallyqa_l.calib}{1,499}
\@namedef{VJ@n.tallyqa_l.dropimg}{255}
\@namedef{VJ@n.tallyqa_l.dropq}{568}
\@namedef{VJ@n.tallyqa_l.images}{2,531}
\@namedef{VJ@n.tallyqa_l.test}{3,681}
\@namedef{VJ@n.tallyqa_short.calib}{160}
\@namedef{VJ@n.tallyqa_short.test}{338}
\@namedef{VJ@n.textvqa_k8.calib}{758}
\@namedef{VJ@n.textvqa_k8.test}{1,742}
\@namedef{VJ@n.textvqa_k8.testimg}{1,430}
\@namedef{VJ@par.B1_k.apc0.dacc}{0.15}
\@namedef{VJ@par.B1_k.apc0.fliprate}{0.54\%}
\@namedef{VJ@par.B1_k.apc0.flips}{18}
\@namedef{VJ@par.B1_k.apc0.n}{3,319}
\@namedef{VJ@par.B1_k.apc0.tvp95}{0.046}
\@namedef{VJ@par.B1_k.apc1.dacc}{0.12}
\@namedef{VJ@par.B1_k.apc1.fliprate}{0.54\%}
\@namedef{VJ@par.B1_k.apc1.flips}{18}
\@namedef{VJ@par.B1_k.apc1.n}{3,319}
\@namedef{VJ@par.B1_k.apc1.tvp95}{0.052}
\@namedef{VJ@par.a2_s0.apc0.dacc}{0.12}
\@namedef{VJ@par.a2_s0.apc0.fliprate}{0.33\%}
\@namedef{VJ@par.a2_s0.apc0.flips}{11}
\@namedef{VJ@par.a2_s0.apc0.n}{3,319}
\@namedef{VJ@par.a2_s0.apc0.tvp95}{0.027}
\@namedef{VJ@par.a2_s0.apc1.dacc}{0.03}
\@namedef{VJ@par.a2_s0.apc1.fliprate}{0.45\%}
\@namedef{VJ@par.a2_s0.apc1.flips}{15}
\@namedef{VJ@par.a2_s0.apc1.n}{3,319}
\@namedef{VJ@par.a2_s0.apc1.tvp95}{0.029}
\@namedef{VJ@perm.D_brier.gqa_val.consistent}{0.974}
\@namedef{VJ@perm.D_brier.gqa_val.consistent.pct}{97\%}
\@namedef{VJ@perm.D_brier.gqa_val.first_pos}{0.374}
\@namedef{VJ@perm.D_brier.gqa_val.first_pos.pct}{37\%}
\@namedef{VJ@perm.D_brier.gqa_val.first_position_chance}{0.370}
\@namedef{VJ@perm.D_brier.gqa_val.first_position_chance.pct}{37\%}
\@namedef{VJ@perm.D_brier.gqa_val.flip@0.05}{0.051}
\@namedef{VJ@perm.D_brier.gqa_val.flip@0.05.pct}{5\%}
\@namedef{VJ@perm.D_brier.gqa_val.flip@0.1}{0.001}
\@namedef{VJ@perm.D_brier.gqa_val.flip@0.1.pct}{0\%}
\@namedef{VJ@perm.D_brier.gqa_val.tv}{0.025}
\@namedef{VJ@perm.D_brier.gqa_val.tv.pct}{3\%}
\@namedef{VJ@perm.D_brier.snli_ve.consistent}{0.918}
\@namedef{VJ@perm.D_brier.snli_ve.consistent.pct}{92\%}
\@namedef{VJ@perm.D_brier.snli_ve.first_pos}{0.307}
\@namedef{VJ@perm.D_brier.snli_ve.first_pos.pct}{31\%}
\@namedef{VJ@perm.D_brier.snli_ve.first_position_chance}{0.333}
\@namedef{VJ@perm.D_brier.snli_ve.first_position_chance.pct}{33\%}
\@namedef{VJ@perm.D_brier.snli_ve.flip@0.05}{0.168}
\@namedef{VJ@perm.D_brier.snli_ve.flip@0.05.pct}{17\%}
\@namedef{VJ@perm.D_brier.snli_ve.flip@0.1}{0.158}
\@namedef{VJ@perm.D_brier.snli_ve.flip@0.1.pct}{16\%}
\@namedef{VJ@perm.D_brier.snli_ve.tv}{0.064}
\@namedef{VJ@perm.D_brier.snli_ve.tv.pct}{6\%}
\@namedef{VJ@perm.D_brier.tallyqa.consistent}{0.472}
\@namedef{VJ@perm.D_brier.tallyqa.consistent.pct}{47\%}
\@namedef{VJ@perm.D_brier.tallyqa.first_pos}{0.238}
\@namedef{VJ@perm.D_brier.tallyqa.first_pos.pct}{24\%}
\@namedef{VJ@perm.D_brier.tallyqa.first_position_chance}{0.167}
\@namedef{VJ@perm.D_brier.tallyqa.first_position_chance.pct}{17\%}
\@namedef{VJ@perm.D_brier.tallyqa.flip@0.05}{0.093}
\@namedef{VJ@perm.D_brier.tallyqa.flip@0.05.pct}{9\%}
\@namedef{VJ@perm.D_brier.tallyqa.flip@0.1}{0.139}
\@namedef{VJ@perm.D_brier.tallyqa.flip@0.1.pct}{14\%}
\@namedef{VJ@perm.D_brier.tallyqa.tv}{0.142}
\@namedef{VJ@perm.D_brier.tallyqa.tv.pct}{14\%}
\@namedef{VJ@perm.D_brier.textvqa_k8.consistent}{0.973}
\@namedef{VJ@perm.D_brier.textvqa_k8.consistent.pct}{97\%}
\@namedef{VJ@perm.D_brier.textvqa_k8.first_pos}{0.123}
\@namedef{VJ@perm.D_brier.textvqa_k8.first_pos.pct}{12\%}
\@namedef{VJ@perm.D_brier.textvqa_k8.first_position_chance}{0.125}
\@namedef{VJ@perm.D_brier.textvqa_k8.first_position_chance.pct}{12\%}
\@namedef{VJ@perm.D_brier.textvqa_k8.flip@0.05}{0.001}
\@namedef{VJ@perm.D_brier.textvqa_k8.flip@0.05.pct}{0\%}
\@namedef{VJ@perm.D_brier.textvqa_k8.flip@0.1}{0.001}
\@namedef{VJ@perm.D_brier.textvqa_k8.flip@0.1.pct}{0\%}
\@namedef{VJ@perm.D_brier.textvqa_k8.tv}{0.017}
\@namedef{VJ@perm.D_brier.textvqa_k8.tv.pct}{2\%}
\@namedef{VJ@perm.D_ce.gqa_val.consistent}{0.974}
\@namedef{VJ@perm.D_ce.gqa_val.consistent.pct}{97\%}
\@namedef{VJ@perm.D_ce.gqa_val.first_pos}{0.374}
\@namedef{VJ@perm.D_ce.gqa_val.first_pos.pct}{37\%}
\@namedef{VJ@perm.D_ce.gqa_val.first_position_chance}{0.370}
\@namedef{VJ@perm.D_ce.gqa_val.first_position_chance.pct}{37\%}
\@namedef{VJ@perm.D_ce.gqa_val.flip@0.05}{0.055}
\@namedef{VJ@perm.D_ce.gqa_val.flip@0.05.pct}{6\%}
\@namedef{VJ@perm.D_ce.gqa_val.flip@0.1}{0.001}
\@namedef{VJ@perm.D_ce.gqa_val.flip@0.1.pct}{0\%}
\@namedef{VJ@perm.D_ce.gqa_val.tv}{0.026}
\@namedef{VJ@perm.D_ce.gqa_val.tv.pct}{3\%}
\@namedef{VJ@perm.D_ce.snli_ve.consistent}{0.920}
\@namedef{VJ@perm.D_ce.snli_ve.consistent.pct}{92\%}
\@namedef{VJ@perm.D_ce.snli_ve.first_pos}{0.306}
\@namedef{VJ@perm.D_ce.snli_ve.first_pos.pct}{31\%}
\@namedef{VJ@perm.D_ce.snli_ve.first_position_chance}{0.333}
\@namedef{VJ@perm.D_ce.snli_ve.first_position_chance.pct}{33\%}
\@namedef{VJ@perm.D_ce.snli_ve.flip@0.05}{0.172}
\@namedef{VJ@perm.D_ce.snli_ve.flip@0.05.pct}{17\%}
\@namedef{VJ@perm.D_ce.snli_ve.flip@0.1}{0.177}
\@namedef{VJ@perm.D_ce.snli_ve.flip@0.1.pct}{18\%}
\@namedef{VJ@perm.D_ce.snli_ve.tv}{0.068}
\@namedef{VJ@perm.D_ce.snli_ve.tv.pct}{7\%}
\@namedef{VJ@perm.D_ce.tallyqa.consistent}{0.476}
\@namedef{VJ@perm.D_ce.tallyqa.consistent.pct}{48\%}
\@namedef{VJ@perm.D_ce.tallyqa.first_pos}{0.225}
\@namedef{VJ@perm.D_ce.tallyqa.first_pos.pct}{22\%}
\@namedef{VJ@perm.D_ce.tallyqa.first_position_chance}{0.167}
\@namedef{VJ@perm.D_ce.tallyqa.first_position_chance.pct}{17\%}
\@namedef{VJ@perm.D_ce.tallyqa.flip@0.05}{0.091}
\@namedef{VJ@perm.D_ce.tallyqa.flip@0.05.pct}{9\%}
\@namedef{VJ@perm.D_ce.tallyqa.flip@0.1}{0.126}
\@namedef{VJ@perm.D_ce.tallyqa.flip@0.1.pct}{13\%}
\@namedef{VJ@perm.D_ce.tallyqa.tv}{0.138}
\@namedef{VJ@perm.D_ce.tallyqa.tv.pct}{14\%}
\@namedef{VJ@perm.D_ce.textvqa_k8.consistent}{0.972}
\@namedef{VJ@perm.D_ce.textvqa_k8.consistent.pct}{97\%}
\@namedef{VJ@perm.D_ce.textvqa_k8.first_pos}{0.122}
\@namedef{VJ@perm.D_ce.textvqa_k8.first_pos.pct}{12\%}
\@namedef{VJ@perm.D_ce.textvqa_k8.first_position_chance}{0.125}
\@namedef{VJ@perm.D_ce.textvqa_k8.first_position_chance.pct}{12\%}
\@namedef{VJ@perm.D_ce.textvqa_k8.flip@0.05}{0.001}
\@namedef{VJ@perm.D_ce.textvqa_k8.flip@0.05.pct}{0\%}
\@namedef{VJ@perm.D_ce.textvqa_k8.flip@0.1}{0.001}
\@namedef{VJ@perm.D_ce.textvqa_k8.flip@0.1.pct}{0\%}
\@namedef{VJ@perm.D_ce.textvqa_k8.tv}{0.018}
\@namedef{VJ@perm.D_ce.textvqa_k8.tv.pct}{2\%}
\@namedef{VJ@perm.D_ce_perm.gqa_val.consistent}{0.973}
\@namedef{VJ@perm.D_ce_perm.gqa_val.consistent.pct}{97\%}
\@namedef{VJ@perm.D_ce_perm.gqa_val.first_pos}{0.372}
\@namedef{VJ@perm.D_ce_perm.gqa_val.first_pos.pct}{37\%}
\@namedef{VJ@perm.D_ce_perm.gqa_val.first_position_chance}{0.370}
\@namedef{VJ@perm.D_ce_perm.gqa_val.first_position_chance.pct}{37\%}
\@namedef{VJ@perm.D_ce_perm.gqa_val.flip@0.05}{0.051}
\@namedef{VJ@perm.D_ce_perm.gqa_val.flip@0.05.pct}{5\%}
\@namedef{VJ@perm.D_ce_perm.gqa_val.flip@0.1}{0.001}
\@namedef{VJ@perm.D_ce_perm.gqa_val.flip@0.1.pct}{0\%}
\@namedef{VJ@perm.D_ce_perm.gqa_val.tv}{0.024}
\@namedef{VJ@perm.D_ce_perm.gqa_val.tv.pct}{2\%}
\@namedef{VJ@perm.D_ce_perm.snli_ve.consistent}{0.938}
\@namedef{VJ@perm.D_ce_perm.snli_ve.consistent.pct}{94\%}
\@namedef{VJ@perm.D_ce_perm.snli_ve.first_pos}{0.326}
\@namedef{VJ@perm.D_ce_perm.snli_ve.first_pos.pct}{33\%}
\@namedef{VJ@perm.D_ce_perm.snli_ve.first_position_chance}{0.333}
\@namedef{VJ@perm.D_ce_perm.snli_ve.first_position_chance.pct}{33\%}
\@namedef{VJ@perm.D_ce_perm.snli_ve.flip@0.05}{0.163}
\@namedef{VJ@perm.D_ce_perm.snli_ve.flip@0.05.pct}{16\%}
\@namedef{VJ@perm.D_ce_perm.snli_ve.flip@0.1}{0.156}
\@namedef{VJ@perm.D_ce_perm.snli_ve.flip@0.1.pct}{16\%}
\@namedef{VJ@perm.D_ce_perm.snli_ve.tv}{0.047}
\@namedef{VJ@perm.D_ce_perm.snli_ve.tv.pct}{5\%}
\@namedef{VJ@perm.D_ce_perm.tallyqa.consistent}{0.481}
\@namedef{VJ@perm.D_ce_perm.tallyqa.consistent.pct}{48\%}
\@namedef{VJ@perm.D_ce_perm.tallyqa.first_pos}{0.217}
\@namedef{VJ@perm.D_ce_perm.tallyqa.first_pos.pct}{22\%}
\@namedef{VJ@perm.D_ce_perm.tallyqa.first_position_chance}{0.167}
\@namedef{VJ@perm.D_ce_perm.tallyqa.first_position_chance.pct}{17\%}
\@namedef{VJ@perm.D_ce_perm.tallyqa.flip@0.05}{0.084}
\@namedef{VJ@perm.D_ce_perm.tallyqa.flip@0.05.pct}{8\%}
\@namedef{VJ@perm.D_ce_perm.tallyqa.flip@0.1}{0.142}
\@namedef{VJ@perm.D_ce_perm.tallyqa.flip@0.1.pct}{14\%}
\@namedef{VJ@perm.D_ce_perm.tallyqa.tv}{0.132}
\@namedef{VJ@perm.D_ce_perm.tallyqa.tv.pct}{13\%}
\@namedef{VJ@perm.D_ce_perm.textvqa_k8.consistent}{0.973}
\@namedef{VJ@perm.D_ce_perm.textvqa_k8.consistent.pct}{97\%}
\@namedef{VJ@perm.D_ce_perm.textvqa_k8.first_pos}{0.122}
\@namedef{VJ@perm.D_ce_perm.textvqa_k8.first_pos.pct}{12\%}
\@namedef{VJ@perm.D_ce_perm.textvqa_k8.first_position_chance}{0.125}
\@namedef{VJ@perm.D_ce_perm.textvqa_k8.first_position_chance.pct}{12\%}
\@namedef{VJ@perm.D_ce_perm.textvqa_k8.flip@0.05}{0.001}
\@namedef{VJ@perm.D_ce_perm.textvqa_k8.flip@0.05.pct}{0\%}
\@namedef{VJ@perm.D_ce_perm.textvqa_k8.flip@0.1}{0.001}
\@namedef{VJ@perm.D_ce_perm.textvqa_k8.flip@0.1.pct}{0\%}
\@namedef{VJ@perm.D_ce_perm.textvqa_k8.tv}{0.016}
\@namedef{VJ@perm.D_ce_perm.textvqa_k8.tv.pct}{2\%}
\@namedef{VJ@perm.D_full.gqa_val.consistent}{0.973}
\@namedef{VJ@perm.D_full.gqa_val.consistent.pct}{97\%}
\@namedef{VJ@perm.D_full.gqa_val.first_pos}{0.373}
\@namedef{VJ@perm.D_full.gqa_val.first_pos.pct}{37\%}
\@namedef{VJ@perm.D_full.gqa_val.first_position_chance}{0.370}
\@namedef{VJ@perm.D_full.gqa_val.first_position_chance.pct}{37\%}
\@namedef{VJ@perm.D_full.gqa_val.flip@0.05}{0.056}
\@namedef{VJ@perm.D_full.gqa_val.flip@0.05.pct}{6\%}
\@namedef{VJ@perm.D_full.gqa_val.flip@0.1}{0.001}
\@namedef{VJ@perm.D_full.gqa_val.flip@0.1.pct}{0\%}
\@namedef{VJ@perm.D_full.gqa_val.tv}{0.026}
\@namedef{VJ@perm.D_full.gqa_val.tv.pct}{3\%}
\@namedef{VJ@perm.D_full.snli_ve.consistent}{0.922}
\@namedef{VJ@perm.D_full.snli_ve.consistent.pct}{92\%}
\@namedef{VJ@perm.D_full.snli_ve.first_pos}{0.306}
\@namedef{VJ@perm.D_full.snli_ve.first_pos.pct}{31\%}
\@namedef{VJ@perm.D_full.snli_ve.first_position_chance}{0.333}
\@namedef{VJ@perm.D_full.snli_ve.first_position_chance.pct}{33\%}
\@namedef{VJ@perm.D_full.snli_ve.flip@0.05}{0.167}
\@namedef{VJ@perm.D_full.snli_ve.flip@0.05.pct}{17\%}
\@namedef{VJ@perm.D_full.snli_ve.flip@0.1}{0.179}
\@namedef{VJ@perm.D_full.snli_ve.flip@0.1.pct}{18\%}
\@namedef{VJ@perm.D_full.snli_ve.tv}{0.067}
\@namedef{VJ@perm.D_full.snli_ve.tv.pct}{7\%}
\@namedef{VJ@perm.D_full.tallyqa.consistent}{0.478}
\@namedef{VJ@perm.D_full.tallyqa.consistent.pct}{48\%}
\@namedef{VJ@perm.D_full.tallyqa.first_pos}{0.226}
\@namedef{VJ@perm.D_full.tallyqa.first_pos.pct}{23\%}
\@namedef{VJ@perm.D_full.tallyqa.first_position_chance}{0.167}
\@namedef{VJ@perm.D_full.tallyqa.first_position_chance.pct}{17\%}
\@namedef{VJ@perm.D_full.tallyqa.flip@0.05}{0.095}
\@namedef{VJ@perm.D_full.tallyqa.flip@0.05.pct}{9\%}
\@namedef{VJ@perm.D_full.tallyqa.flip@0.1}{0.122}
\@namedef{VJ@perm.D_full.tallyqa.flip@0.1.pct}{12\%}
\@namedef{VJ@perm.D_full.tallyqa.tv}{0.138}
\@namedef{VJ@perm.D_full.tallyqa.tv.pct}{14\%}
\@namedef{VJ@perm.D_full.textvqa_k8.consistent}{0.972}
\@namedef{VJ@perm.D_full.textvqa_k8.consistent.pct}{97\%}
\@namedef{VJ@perm.D_full.textvqa_k8.first_pos}{0.122}
\@namedef{VJ@perm.D_full.textvqa_k8.first_pos.pct}{12\%}
\@namedef{VJ@perm.D_full.textvqa_k8.first_position_chance}{0.125}
\@namedef{VJ@perm.D_full.textvqa_k8.first_position_chance.pct}{12\%}
\@namedef{VJ@perm.D_full.textvqa_k8.flip@0.05}{0.001}
\@namedef{VJ@perm.D_full.textvqa_k8.flip@0.05.pct}{0\%}
\@namedef{VJ@perm.D_full.textvqa_k8.flip@0.1}{0.001}
\@namedef{VJ@perm.D_full.textvqa_k8.flip@0.1.pct}{0\%}
\@namedef{VJ@perm.D_full.textvqa_k8.tv}{0.018}
\@namedef{VJ@perm.D_full.textvqa_k8.tv.pct}{2\%}
\@namedef{VJ@perm.M0.gqa_val.consistent}{0.933}
\@namedef{VJ@perm.M0.gqa_val.consistent.pct}{93\%}
\@namedef{VJ@perm.M0.gqa_val.first_pos}{0.402}
\@namedef{VJ@perm.M0.gqa_val.first_pos.pct}{40\%}
\@namedef{VJ@perm.M0.gqa_val.first_position_chance}{0.370}
\@namedef{VJ@perm.M0.gqa_val.first_position_chance.pct}{37\%}
\@namedef{VJ@perm.M0.gqa_val.flip@0.05}{0.140}
\@namedef{VJ@perm.M0.gqa_val.flip@0.05.pct}{14\%}
\@namedef{VJ@perm.M0.gqa_val.flip@0.1}{0.091}
\@namedef{VJ@perm.M0.gqa_val.flip@0.1.pct}{9\%}
\@namedef{VJ@perm.M0.gqa_val.tv}{0.065}
\@namedef{VJ@perm.M0.gqa_val.tv.pct}{7\%}
\@namedef{VJ@perm.M0.snli_ve.consistent}{0.748}
\@namedef{VJ@perm.M0.snli_ve.consistent.pct}{75\%}
\@namedef{VJ@perm.M0.snli_ve.first_pos}{0.378}
\@namedef{VJ@perm.M0.snli_ve.first_pos.pct}{38\%}
\@namedef{VJ@perm.M0.snli_ve.first_position_chance}{0.333}
\@namedef{VJ@perm.M0.snli_ve.first_position_chance.pct}{33\%}
\@namedef{VJ@perm.M0.snli_ve.flip@0.05}{0.026}
\@namedef{VJ@perm.M0.snli_ve.flip@0.05.pct}{3\%}
\@namedef{VJ@perm.M0.snli_ve.flip@0.1}{0.074}
\@namedef{VJ@perm.M0.snli_ve.flip@0.1.pct}{7\%}
\@namedef{VJ@perm.M0.snli_ve.tv}{0.108}
\@namedef{VJ@perm.M0.snli_ve.tv.pct}{11\%}
\@namedef{VJ@perm.M0.tallyqa.consistent}{0.325}
\@namedef{VJ@perm.M0.tallyqa.consistent.pct}{33\%}
\@namedef{VJ@perm.M0.tallyqa.first_pos}{0.315}
\@namedef{VJ@perm.M0.tallyqa.first_pos.pct}{31\%}
\@namedef{VJ@perm.M0.tallyqa.first_position_chance}{0.167}
\@namedef{VJ@perm.M0.tallyqa.first_position_chance.pct}{17\%}
\@namedef{VJ@perm.M0.tallyqa.flip@0.05}{0.086}
\@namedef{VJ@perm.M0.tallyqa.flip@0.05.pct}{9\%}
\@namedef{VJ@perm.M0.tallyqa.flip@0.1}{0.104}
\@namedef{VJ@perm.M0.tallyqa.flip@0.1.pct}{10\%}
\@namedef{VJ@perm.M0.tallyqa.tv}{0.174}
\@namedef{VJ@perm.M0.tallyqa.tv.pct}{17\%}
\@namedef{VJ@perm.M0.textvqa_k8.consistent}{0.969}
\@namedef{VJ@perm.M0.textvqa_k8.consistent.pct}{97\%}
\@namedef{VJ@perm.M0.textvqa_k8.first_pos}{0.125}
\@namedef{VJ@perm.M0.textvqa_k8.first_pos.pct}{13\%}
\@namedef{VJ@perm.M0.textvqa_k8.first_position_chance}{0.125}
\@namedef{VJ@perm.M0.textvqa_k8.first_position_chance.pct}{12\%}
\@namedef{VJ@perm.M0.textvqa_k8.flip@0.05}{0.000}
\@namedef{VJ@perm.M0.textvqa_k8.flip@0.05.pct}{0\%}
\@namedef{VJ@perm.M0.textvqa_k8.flip@0.1}{0.000}
\@namedef{VJ@perm.M0.textvqa_k8.flip@0.1.pct}{0\%}
\@namedef{VJ@perm.M0.textvqa_k8.tv}{0.022}
\@namedef{VJ@perm.M0.textvqa_k8.tv.pct}{2\%}
\@namedef{VJ@perm.M1.gqa_val.consistent}{0.975}
\@namedef{VJ@perm.M1.gqa_val.consistent.pct}{98\%}
\@namedef{VJ@perm.M1.gqa_val.first_pos}{0.375}
\@namedef{VJ@perm.M1.gqa_val.first_pos.pct}{37\%}
\@namedef{VJ@perm.M1.gqa_val.first_position_chance}{0.370}
\@namedef{VJ@perm.M1.gqa_val.first_position_chance.pct}{37\%}
\@namedef{VJ@perm.M1.gqa_val.flip@0.05}{0.048}
\@namedef{VJ@perm.M1.gqa_val.flip@0.05.pct}{5\%}
\@namedef{VJ@perm.M1.gqa_val.flip@0.1}{0.001}
\@namedef{VJ@perm.M1.gqa_val.flip@0.1.pct}{0\%}
\@namedef{VJ@perm.M1.gqa_val.tv}{0.022}
\@namedef{VJ@perm.M1.gqa_val.tv.pct}{2\%}
\@namedef{VJ@perm.M1.snli_ve.consistent}{0.926}
\@namedef{VJ@perm.M1.snli_ve.consistent.pct}{93\%}
\@namedef{VJ@perm.M1.snli_ve.first_pos}{0.313}
\@namedef{VJ@perm.M1.snli_ve.first_pos.pct}{31\%}
\@namedef{VJ@perm.M1.snli_ve.first_position_chance}{0.333}
\@namedef{VJ@perm.M1.snli_ve.first_position_chance.pct}{33\%}
\@namedef{VJ@perm.M1.snli_ve.flip@0.05}{0.170}
\@namedef{VJ@perm.M1.snli_ve.flip@0.05.pct}{17\%}
\@namedef{VJ@perm.M1.snli_ve.flip@0.1}{0.151}
\@namedef{VJ@perm.M1.snli_ve.flip@0.1.pct}{15\%}
\@namedef{VJ@perm.M1.snli_ve.tv}{0.062}
\@namedef{VJ@perm.M1.snli_ve.tv.pct}{6\%}
\@namedef{VJ@perm.M1.tallyqa.consistent}{0.464}
\@namedef{VJ@perm.M1.tallyqa.consistent.pct}{46\%}
\@namedef{VJ@perm.M1.tallyqa.first_pos}{0.248}
\@namedef{VJ@perm.M1.tallyqa.first_pos.pct}{25\%}
\@namedef{VJ@perm.M1.tallyqa.first_position_chance}{0.167}
\@namedef{VJ@perm.M1.tallyqa.first_position_chance.pct}{17\%}
\@namedef{VJ@perm.M1.tallyqa.flip@0.05}{0.078}
\@namedef{VJ@perm.M1.tallyqa.flip@0.05.pct}{8\%}
\@namedef{VJ@perm.M1.tallyqa.flip@0.1}{0.120}
\@namedef{VJ@perm.M1.tallyqa.flip@0.1.pct}{12\%}
\@namedef{VJ@perm.M1.tallyqa.tv}{0.138}
\@namedef{VJ@perm.M1.tallyqa.tv.pct}{14\%}
\@namedef{VJ@perm.M1.textvqa_k8.consistent}{0.972}
\@namedef{VJ@perm.M1.textvqa_k8.consistent.pct}{97\%}
\@namedef{VJ@perm.M1.textvqa_k8.first_pos}{0.123}
\@namedef{VJ@perm.M1.textvqa_k8.first_pos.pct}{12\%}
\@namedef{VJ@perm.M1.textvqa_k8.first_position_chance}{0.125}
\@namedef{VJ@perm.M1.textvqa_k8.first_position_chance.pct}{12\%}
\@namedef{VJ@perm.M1.textvqa_k8.flip@0.05}{0.001}
\@namedef{VJ@perm.M1.textvqa_k8.flip@0.05.pct}{0\%}
\@namedef{VJ@perm.M1.textvqa_k8.flip@0.1}{0.001}
\@namedef{VJ@perm.M1.textvqa_k8.flip@0.1.pct}{0\%}
\@namedef{VJ@perm.M1.textvqa_k8.tv}{0.016}
\@namedef{VJ@perm.M1.textvqa_k8.tv.pct}{2\%}
\@namedef{VJ@ratio.order_vs_exec}{8}
\@namedef{VJ@rk.D_brier.gqa_val.aurc}{0.015}
\@namedef{VJ@rk.D_brier.gqa_val.auroc}{0.890}
\@namedef{VJ@rk.D_brier.gqa_val.e_aurc}{0.011}
\@namedef{VJ@rk.D_brier.macro.aurc}{0.030}
\@namedef{VJ@rk.D_brier.macro.auroc}{0.890}
\@namedef{VJ@rk.D_brier.macro.e_aurc}{0.021}
\@namedef{VJ@rk.D_brier.snli_ve.aurc}{0.073}
\@namedef{VJ@rk.D_brier.snli_ve.auroc}{0.796}
\@namedef{VJ@rk.D_brier.snli_ve.e_aurc}{0.052}
\@namedef{VJ@rk.D_brier.tallyqa_l.aurc}{0.033}
\@namedef{VJ@rk.D_brier.tallyqa_l.auroc}{0.891}
\@namedef{VJ@rk.D_brier.tallyqa_l.e_aurc}{0.020}
\@namedef{VJ@rk.D_brier.textvqa_k8.aurc}{0.001}
\@namedef{VJ@rk.D_brier.textvqa_k8.auroc}{0.984}
\@namedef{VJ@rk.D_brier.textvqa_k8.e_aurc}{0.000}
\@namedef{VJ@rk.D_ce.gqa_val.aurc}{0.016}
\@namedef{VJ@rk.D_ce.gqa_val.auroc}{0.884}
\@namedef{VJ@rk.D_ce.gqa_val.e_aurc}{0.012}
\@namedef{VJ@rk.D_ce.macro.aurc}{0.031}
\@namedef{VJ@rk.D_ce.macro.auroc}{0.887}
\@namedef{VJ@rk.D_ce.macro.e_aurc}{0.022}
\@namedef{VJ@rk.D_ce.snli_ve.aurc}{0.074}
\@namedef{VJ@rk.D_ce.snli_ve.auroc}{0.792}
\@namedef{VJ@rk.D_ce.snli_ve.e_aurc}{0.054}
\@namedef{VJ@rk.D_ce.tallyqa_l.aurc}{0.034}
\@namedef{VJ@rk.D_ce.tallyqa_l.auroc}{0.889}
\@namedef{VJ@rk.D_ce.tallyqa_l.e_aurc}{0.021}
\@namedef{VJ@rk.D_ce.textvqa_k8.aurc}{0.001}
\@namedef{VJ@rk.D_ce.textvqa_k8.auroc}{0.984}
\@namedef{VJ@rk.D_ce.textvqa_k8.e_aurc}{0.000}
\@namedef{VJ@rk.D_ceperm.gqa_val.aurc}{0.016}
\@namedef{VJ@rk.D_ceperm.gqa_val.auroc}{0.884}
\@namedef{VJ@rk.D_ceperm.gqa_val.e_aurc}{0.012}
\@namedef{VJ@rk.D_ceperm.macro.aurc}{0.031}
\@namedef{VJ@rk.D_ceperm.macro.auroc}{0.885}
\@namedef{VJ@rk.D_ceperm.macro.e_aurc}{0.022}
\@namedef{VJ@rk.D_ceperm.snli_ve.aurc}{0.075}
\@namedef{VJ@rk.D_ceperm.snli_ve.auroc}{0.785}
\@namedef{VJ@rk.D_ceperm.snli_ve.e_aurc}{0.055}
\@namedef{VJ@rk.D_ceperm.tallyqa_l.aurc}{0.034}
\@namedef{VJ@rk.D_ceperm.tallyqa_l.auroc}{0.886}
\@namedef{VJ@rk.D_ceperm.tallyqa_l.e_aurc}{0.021}
\@namedef{VJ@rk.D_ceperm.textvqa_k8.aurc}{0.001}
\@namedef{VJ@rk.D_ceperm.textvqa_k8.auroc}{0.985}
\@namedef{VJ@rk.D_ceperm.textvqa_k8.e_aurc}{0.000}
\@namedef{VJ@rk.D_full.gqa_val.aurc}{0.016}
\@namedef{VJ@rk.D_full.gqa_val.auroc}{0.885}
\@namedef{VJ@rk.D_full.gqa_val.e_aurc}{0.012}
\@namedef{VJ@rk.D_full.macro.aurc}{0.031}
\@namedef{VJ@rk.D_full.macro.auroc}{0.887}
\@namedef{VJ@rk.D_full.macro.e_aurc}{0.022}
\@namedef{VJ@rk.D_full.snli_ve.aurc}{0.075}
\@namedef{VJ@rk.D_full.snli_ve.auroc}{0.792}
\@namedef{VJ@rk.D_full.snli_ve.e_aurc}{0.054}
\@namedef{VJ@rk.D_full.tallyqa_l.aurc}{0.034}
\@namedef{VJ@rk.D_full.tallyqa_l.auroc}{0.888}
\@namedef{VJ@rk.D_full.tallyqa_l.e_aurc}{0.021}
\@namedef{VJ@rk.D_full.textvqa_k8.aurc}{0.001}
\@namedef{VJ@rk.D_full.textvqa_k8.auroc}{0.984}
\@namedef{VJ@rk.D_full.textvqa_k8.e_aurc}{0.000}
\@namedef{VJ@rk.M0.gqa_val.aurc}{0.037}
\@namedef{VJ@rk.M0.gqa_val.auroc}{0.833}
\@namedef{VJ@rk.M0.gqa_val.e_aurc}{0.029}
\@namedef{VJ@rk.M0.macro.aurc}{0.080}
\@namedef{VJ@rk.M0.macro.auroc}{0.834}
\@namedef{VJ@rk.M0.macro.e_aurc}{0.055}
\@namedef{VJ@rk.M0.snli_ve.aurc}{0.247}
\@namedef{VJ@rk.M0.snli_ve.auroc}{0.646}
\@namedef{VJ@rk.M0.snli_ve.e_aurc}{0.168}
\@namedef{VJ@rk.M0.tallyqa_l.aurc}{0.036}
\@namedef{VJ@rk.M0.tallyqa_l.auroc}{0.871}
\@namedef{VJ@rk.M0.tallyqa_l.e_aurc}{0.025}
\@namedef{VJ@rk.M0.textvqa_k8.aurc}{0.001}
\@namedef{VJ@rk.M0.textvqa_k8.auroc}{0.985}
\@namedef{VJ@rk.M0.textvqa_k8.e_aurc}{0.000}
\@namedef{VJ@rk.M0_8b.gqa_val.aurc}{0.028}
\@namedef{VJ@rk.M0_8b.gqa_val.auroc}{0.854}
\@namedef{VJ@rk.M0_8b.gqa_val.e_aurc}{0.021}
\@namedef{VJ@rk.M0_8b.macro.aurc}{0.062}
\@namedef{VJ@rk.M0_8b.macro.auroc}{0.851}
\@namedef{VJ@rk.M0_8b.macro.e_aurc}{0.045}
\@namedef{VJ@rk.M0_8b.snli_ve.aurc}{0.190}
\@namedef{VJ@rk.M0_8b.snli_ve.auroc}{0.669}
\@namedef{VJ@rk.M0_8b.snli_ve.e_aurc}{0.138}
\@namedef{VJ@rk.M0_8b.tallyqa_l.aurc}{0.031}
\@namedef{VJ@rk.M0_8b.tallyqa_l.auroc}{0.892}
\@namedef{VJ@rk.M0_8b.tallyqa_l.e_aurc}{0.020}
\@namedef{VJ@rk.M0_8b.textvqa_k8.aurc}{0.000}
\@namedef{VJ@rk.M0_8b.textvqa_k8.auroc}{0.988}
\@namedef{VJ@rk.M0_8b.textvqa_k8.e_aurc}{0.000}
\@namedef{VJ@rk.M1.gqa_val.aurc}{0.014}
\@namedef{VJ@rk.M1.gqa_val.auroc}{0.892}
\@namedef{VJ@rk.M1.gqa_val.e_aurc}{0.010}
\@namedef{VJ@rk.M1.macro.aurc}{0.030}
\@namedef{VJ@rk.M1.macro.auroc}{0.890}
\@namedef{VJ@rk.M1.macro.e_aurc}{0.021}
\@namedef{VJ@rk.M1.snli_ve.aurc}{0.071}
\@namedef{VJ@rk.M1.snli_ve.auroc}{0.792}
\@namedef{VJ@rk.M1.snli_ve.e_aurc}{0.051}
\@namedef{VJ@rk.M1.tallyqa_l.aurc}{0.034}
\@namedef{VJ@rk.M1.tallyqa_l.auroc}{0.892}
\@namedef{VJ@rk.M1.tallyqa_l.e_aurc}{0.020}
\@namedef{VJ@rk.M1.textvqa_k8.aurc}{0.001}
\@namedef{VJ@rk.M1.textvqa_k8.auroc}{0.984}
\@namedef{VJ@rk.M1.textvqa_k8.e_aurc}{0.000}
\@namedef{VJ@rk.M1_8b.gqa_val.aurc}{0.012}
\@namedef{VJ@rk.M1_8b.gqa_val.auroc}{0.906}
\@namedef{VJ@rk.M1_8b.gqa_val.e_aurc}{0.008}
\@namedef{VJ@rk.M1_8b.macro.aurc}{0.027}
\@namedef{VJ@rk.M1_8b.macro.auroc}{0.896}
\@namedef{VJ@rk.M1_8b.macro.e_aurc}{0.019}
\@namedef{VJ@rk.M1_8b.snli_ve.aurc}{0.067}
\@namedef{VJ@rk.M1_8b.snli_ve.auroc}{0.794}
\@namedef{VJ@rk.M1_8b.snli_ve.e_aurc}{0.049}
\@namedef{VJ@rk.M1_8b.tallyqa_l.aurc}{0.028}
\@namedef{VJ@rk.M1_8b.tallyqa_l.auroc}{0.895}
\@namedef{VJ@rk.M1_8b.tallyqa_l.e_aurc}{0.017}
\@namedef{VJ@rk.M1_8b.textvqa_k8.aurc}{0.000}
\@namedef{VJ@rk.M1_8b.textvqa_k8.auroc}{0.988}
\@namedef{VJ@rk.M1_8b.textvqa_k8.e_aurc}{0.000}
\@namedef{VJ@rk.d.M1-M0.macro.aurc}{$-$0.050}
\@namedef{VJ@rk.d.M1-M0.macro.aurc.ci}{[$-$0.057, $-$0.044]}
\@namedef{VJ@rk.d.M1-M0.macro.auroc}{+0.056}
\@namedef{VJ@rk.d.M1-M0.macro.auroc.ci}{[0.047, 0.066]}
\@namedef{VJ@rk.d.M1-M0.macro.e_aurc}{$-$0.035}
\@namedef{VJ@rk.d.M1-M0.macro.e_aurc.ci}{[$-$0.040, $-$0.030]}
\@namedef{VJ@s4.B1_k.acc}{0.706}
\@namedef{VJ@s4.B1_k.aurc}{0.185}
\@namedef{VJ@s4.B1_k.ecets}{0.050}
\@namedef{VJ@s4.B1_k.nllts}{0.698}
\@namedef{VJ@s4.S4_B1_k.acc}{0.717}
\@namedef{VJ@s4.S4_B1_k.aurc}{0.173}
\@namedef{VJ@s4.S4_B1_k.ecets}{0.041}
\@namedef{VJ@s4.S4_B1_k.nllts}{0.675}
\@namedef{VJ@s4.S4_a2_s0.acc}{0.761}
\@namedef{VJ@s4.S4_a2_s0.aurc}{0.135}
\@namedef{VJ@s4.S4_a2_s0.ecets}{0.044}
\@namedef{VJ@s4.S4_a2_s0.nllts}{0.594}
\@namedef{VJ@s4.a2_s0.acc}{0.758}
\@namedef{VJ@s4.a2_s0.aurc}{0.137}
\@namedef{VJ@s4.a2_s0.ecets}{0.043}
\@namedef{VJ@s4.a2_s0.nllts}{0.597}
\@namedef{VJ@s4.d.base.acc}{+0.011}
\@namedef{VJ@s4.d.base.acc.ci}{[0.002, 0.021]}
\@namedef{VJ@short.M0.raw.tallyqa.accuracy}{0.340}
\@namedef{VJ@short.M0.ts_local.tallyqa.cov@0.05}{0.160}
\@namedef{VJ@short.M0.ts_local.tallyqa.cov@0.1}{0.175}
\@namedef{VJ@short.M0.ts_local.tallyqa.risk@0.05}{0.185}
\@namedef{VJ@short.M0.ts_local.tallyqa.risk@0.1}{0.203}
\@namedef{VJ@short.M1.raw.tallyqa.accuracy}{0.345}
\@namedef{VJ@short.M1.ts_local.tallyqa.cov@0.05}{0.155}
\@namedef{VJ@short.M1.ts_local.tallyqa.cov@0.1}{0.205}
\@namedef{VJ@short.M1.ts_local.tallyqa.risk@0.05}{0.108}
\@namedef{VJ@short.M1.ts_local.tallyqa.risk@0.1}{0.235}
\@namedef{VJ@srv.S0.cold.1.cap}{151}
\@namedef{VJ@srv.S0.cold.1.kv}{38}
\@namedef{VJ@srv.S0.cold.1.msq}{47.6}
\@namedef{VJ@srv.S0.cold.1.p50}{47}
\@namedef{VJ@srv.S0.cold.1.p95}{51}
\@namedef{VJ@srv.S0.cold.32.cap}{4}
\@namedef{VJ@srv.S0.cold.32.kv}{1218}
\@namedef{VJ@srv.S0.cold.32.msq}{20.5}
\@namedef{VJ@srv.S0.cold.32.p50}{669}
\@namedef{VJ@srv.S0.cold.32.p95}{836}
\@namedef{VJ@srv.S0.cold.8.cap}{18}
\@namedef{VJ@srv.S0.cold.8.kv}{305}
\@namedef{VJ@srv.S0.cold.8.msq}{20.8}
\@namedef{VJ@srv.S0.cold.8.p50}{168}
\@namedef{VJ@srv.S0.cold.8.p95}{212}
\@namedef{VJ@srv.S1.cold.1.cap}{80}
\@namedef{VJ@srv.S1.cold.1.kv}{70}
\@namedef{VJ@srv.S1.cold.1.msq}{82.6}
\@namedef{VJ@srv.S1.cold.1.p50}{81}
\@namedef{VJ@srv.S1.cold.1.p95}{95}
\@namedef{VJ@srv.S1.cold.32.cap}{4}
\@namedef{VJ@srv.S1.cold.32.kv}{1249}
\@namedef{VJ@srv.S1.cold.32.msq}{5.6}
\@namedef{VJ@srv.S1.cold.32.p50}{177}
\@namedef{VJ@srv.S1.cold.32.p95}{202}
\@namedef{VJ@srv.S1.cold.8.cap}{17}
\@namedef{VJ@srv.S1.cold.8.kv}{336}
\@namedef{VJ@srv.S1.cold.8.msq}{11.4}
\@namedef{VJ@srv.S1.cold.8.p50}{89}
\@namedef{VJ@srv.S1.cold.8.p95}{111}
\@namedef{VJ@srv.S1.speedup32}{3.7}
\@namedef{VJ@srv.S2.cold.1.cap}{145}
\@namedef{VJ@srv.S2.cold.1.kv}{39}
\@namedef{VJ@srv.S2.cold.1.msq}{39.2}
\@namedef{VJ@srv.S2.cold.1.p50}{39}
\@namedef{VJ@srv.S2.cold.1.p95}{46}
\@namedef{VJ@srv.S2.cold.32.cap}{4}
\@namedef{VJ@srv.S2.cold.32.kv}{1257}
\@namedef{VJ@srv.S2.cold.32.msq}{19.0}
\@namedef{VJ@srv.S2.cold.32.p50}{618}
\@namedef{VJ@srv.S2.cold.32.p95}{789}
\@namedef{VJ@srv.S2.cold.8.cap}{18}
\@namedef{VJ@srv.S2.cold.8.kv}{315}
\@namedef{VJ@srv.S2.cold.8.msq}{18.6}
\@namedef{VJ@srv.S2.cold.8.p50}{152}
\@namedef{VJ@srv.S2.cold.8.p95}{184}
\@namedef{VJ@srv.S3.cold.1.cap}{145}
\@namedef{VJ@srv.S3.cold.1.kv}{39}
\@namedef{VJ@srv.S3.cold.1.msq}{43.2}
\@namedef{VJ@srv.S3.cold.1.p50}{42}
\@namedef{VJ@srv.S3.cold.1.p95}{59}
\@namedef{VJ@srv.S3.cold.32.cap}{25}
\@namedef{VJ@srv.S3.cold.32.kv}{304}
\@namedef{VJ@srv.S3.cold.32.msq}{7.0}
\@namedef{VJ@srv.S3.cold.32.p50}{221}
\@namedef{VJ@srv.S3.cold.32.p95}{276}
\@namedef{VJ@srv.S3.cold.8.cap}{71}
\@namedef{VJ@srv.S3.cold.8.kv}{99}
\@namedef{VJ@srv.S3.cold.8.msq}{11.4}
\@namedef{VJ@srv.S3.cold.8.p50}{94}
\@namedef{VJ@srv.S3.cold.8.p95}{112}
\@namedef{VJ@srv.S3.warm.1.cap}{145}
\@namedef{VJ@srv.S3.warm.1.kv}{39}
\@namedef{VJ@srv.S3.warm.1.msq}{24.5}
\@namedef{VJ@srv.S3.warm.1.p50}{25}
\@namedef{VJ@srv.S3.warm.1.p95}{29}
\@namedef{VJ@srv.S3.warm.32.cap}{25}
\@namedef{VJ@srv.S3.warm.32.kv}{304}
\@namedef{VJ@srv.S3.warm.32.msq}{6.9}
\@namedef{VJ@srv.S3.warm.32.p50}{221}
\@namedef{VJ@srv.S3.warm.32.p95}{267}
\@namedef{VJ@srv.S3.warm.8.cap}{71}
\@namedef{VJ@srv.S3.warm.8.kv}{99}
\@namedef{VJ@srv.S3.warm.8.msq}{9.2}
\@namedef{VJ@srv.S3.warm.8.p50}{70}
\@namedef{VJ@srv.S3.warm.8.p95}{93}
\@namedef{VJ@srv.agree.S1.flips}{3}
\@namedef{VJ@srv.agree.S2.flips}{1}
\@namedef{VJ@srv.agree.S3.flips}{0}
\@namedef{VJ@srv.agree.n}{1,920}
\@namedef{VJ@srv.capratio}{6}
\@namedef{VJ@srv.kvpercent}{24.3\%}
\@namedef{VJ@srv.kvratio}{4.1}
\@namedef{VJ@tallyqa_short.M0.acc_clean}{0.361}
\@namedef{VJ@tallyqa_short.M0.acc_overlap}{0.326}
\@namedef{VJ@tallyqa_short.M1.acc_clean}{0.366}
\@namedef{VJ@tallyqa_short.M1.acc_overlap}{0.341}
\@namedef{VJ@tallyqa_short.overlap}{46}
\@namedef{VJ@tallyqa_short.overlap_pct}{9.2\%}
\makeatother

